Exploiting Shared Representations for Personalized Federated Learning

Deep neural networks have shown the ability to extract universal feature representations from data such as images and text that have been useful for a variety of learning tasks. However, the fruits of representation learning have yet to be fully-realized in federated settings. Although data in federated settings is often non-i.i.d. across clients, the success of centralized deep learning suggests that data often shares a global feature representation, while the statistical heterogeneity across clients or tasks is concentrated in the labels. Based on this intuition, we propose a novel federated learning framework and algorithm for learning a shared data representation across clients and unique local heads for each client. Our algorithm harnesses the distributed computational power across clients to perform many local-updates with respect to the low-dimensional local parameters for every update of the representation. We prove that this method obtains linear convergence to the ground-truth representation with near-optimal sample complexity in a linear setting, demonstrating that it can efficiently reduce the problem dimension for each client. This result is of interest beyond federated learning to a broad class of problems in which we aim to learn a shared low-dimensional representation among data distributions, for example in meta-learning and multi-task learning. Further, extensive experimental results show the empirical improvement of our method over alternative personalized federated learning approaches in federated environments with heterogeneous data.

==> arxiv_version/Related_Works_arxiv.tex <==
% \section{Related Works}

% \citet{} proposes an algorithm for local representation learning. The main advantage is that learning a local representation reduces the dimensionality of the global problem. However, it does not take advantage of the similarity of representations across clients.
% issues: what if you have different representations? 

% global model acting as a regularizer to prevent overfitting. But it is not really leveraging info across devices
% same head, different reps

% The paper poses two testing paradigms: 1) `Local Test' in which a (new) test sample is drawn on a particular device, and the local model for that device is used to extract the features, then the global model does the prediction, and 2) `New Test' in which a new device enters the system, and an ensemble of all of the local models is used to extract the features.

% Theoretical analysis:
% The authors assume that the existence of ground truth models that generate the local data for each device, where the ground truth model for device $m$ is given by $u_m = v + r_m \in \mathbb{R}^d$, where $v$ is global information and $r_m$ is local. The local information is drawn $\sim \mathcal{N}(0,\rho^2 I_d)$, so $\rho^2$ controls the variance in the data across devices (the larger $\rho^2$, the more the data varies across devices). To model variance across the local data, the authors assume that the local data is corrupted by gaussian noise $\epsilon \sim \mathcal{N}(0,\sigma^2)$, so the training targets on model $m$ are given by $\tilde{f}_{u_m} = f_{u_m} + \epsilon$.

\textbf{Related Work.} 
A variety of recent works have studied personalization in federated learning using, for example, local fine-tuning \citep{wang2019federated, yu2020salvaging}, meta-learning \citep{ chen2018federated,khodak2019adaptive, jiang2019improving,fallah2020personalized}, additive mixtures of local and global models \citep{hanzely2020federated, deng2020adaptive, mansour2020three}, and multi-task learning \citep{smith2017federated}. In all of these methods, each client's subproblem is still full-dimensional - there is no notion of learning a dimensionality-reduced set of local parameters. 
% which can generally be broken into regularization, multi-task learning, and fine-tuning categories. 
% As noted in \citet{deng2020adaptive}, methods to achieve personalization in federated learning generally fall into one of the following five categories. 
% Perhaps the most similar work to ours is 
% Like our work, \citet{smith2017federated} applied multi-task learning techniques to achieve personalization in the federated setting, but did not attempt to reduce the problem dimension by learning a global representation.
More recently, \citet{liang2020think} also proposed a representation learning method for federated learning, but their method attempts to learn many local representations and a single global head as opposed to a single global representation and many local heads.
% Also, their analysis considers a distinct framework in which the learning model is a mixture of local and global models, more reminiscent of formulations presented by \citet{deng2020adaptive,mansour2020three}.
% \citet{zhang2020federated} experimentally considers unsupervised federated representation learning. 
%  \citet{li2020lotteryfl} presents an algorithm for learning lottery ticket networks for each of the clients, which allow for personalization because of their sparsity. They also present a synthetic dataset with non-i.i.d. data across clients which may be useful.
Earlier, \citet{arivazhagan2019federated} presented an algorithm to learn local heads and a global network body, but their local procedure jointly updates the head and body (using the same number of updates), and they did not provide any theoretical justification for their proposed method. Meanwhile, another line of work has studied federated learning in heterogeneous settings  \citep{karimireddy2020scaffold, wang2020tackling, pathak2020fedsplit, haddadpour2020federated, reddi2020adaptive,reisizadeh2020straggler,mitra2021achieving}, and the optimization-based insights from these works may be used to supplement our formulation and algorithm.
% The authors also propose to learn the final neural network layer(s) locally in order to achieve personalization, while learning the network body globally. However, their proposed algorithm makes equal numbers of local updates for both the personalized layers and the body, meaning they do not take advantage of the low-dimensionality of the personalized layers from an optimization perspective. Moreover, they do not provide any theoretical justification of their method.


%% \noindent \textbf{Notations.} We use boldface notation to denote vectors $\mathbf{v}$ and matrices $\mathbf{A}$. The notation $\mathbf{e}_i$ denotes the $i$-th canonical basis vector in $\mathbb{R}^n$. We denote the set $\{1,\dots,n\}$ by $[n]$.


==> arxiv_version/new_Problem_Formulation_arxiv.tex <==
\section{Problem Formulation}
The generic form of federated learning with $n$ clients is
\begin{equation}
    \min_{(\boldsymbol{\theta}_1,\dots,\boldsymbol{\theta}_n) \in \Theta_n} \frac{1}{n}\sum_{i=1}^n  f_i(\boldsymbol{\theta}_i) \label{obj1},
\end{equation}
where $f_i$ and $\boldsymbol{\theta}_i$ are the error function and learning model parameters for the $i$-th client, respectively, and $\Theta_n$ is the space of feasible sets of $n$ models. 
% For example, $\mathcal{Q}_n$ could be limited to sets of equivalent models, i.e., $q=q_1=...=q_n$. At the other extreme, $\mathcal{Q}_n$ could be
We consider a supervised setting in which the data for the $i$-th client is generated by a distribution $(\mathbf{x}_i,y_i) \sim \mathcal{D}_i$. The learning model $q(\cdot;\boldsymbol{\theta}_i) : \mathbb{R}^d \rightarrow \mathcal{Y}$ maps inputs $\mathbf{x}_i \in \mathbb{R}^d$ to predicted labels $q(\mathbf{x}_i;\boldsymbol{\theta}_i)  \in \mathcal{Y}$, which we would like to resemble the true labels $y_i$.
% where $\mathcal{X}$ is the input space and $\mathcal{Y}$ is the label space. 
% The loss $f_i(q_i)$ is the average prediction error of $q_i$ on samples $(\mathbf{x},y)$ from the data distribution $\mathcal{D}_i$ corresponding to the $i$-th client. \textcolor{red}{you can remove the previous sentence given the next} 
 The error $f_i$ is in the form of an expected risk over $\mathcal{D}_i$, namely
    $f_i(\mathbf{\theta}_i) \coloneqq \mathbb{E}_{(\mathbf{x}_i,y_i)\sim \mathcal{D}_i} [\ell(q(\mathbf{x}_i; \mathbf{\theta}_i),y_i)]$,
where $\ell:\mathcal{Y}\times\mathcal{Y}\rightarrow\mathbb{R}$ is a loss function that penalizes the distance of $q(\mathbf{x}_i; \boldsymbol{\theta}_i)$ from~$y_i$. 

In order to minimize $f_i$, the $i$-th client accesses a dataset of $m$ labelled samples $\{ (\mathbf{x}_i^j, y_i^j)\}_{j=1}^{m}$ from $\mathcal{D}_i$ for training. 
Federated learning addresses settings in which $m$ is typically small relative to the problem dimension while the number of clients $n$ is large. Thus, clients may not be able to obtain solutions $\boldsymbol{\theta}_i$ with small expected risk by training completely locally on {\em only} their $m$ local samples. Instead, federated learning enables the clients to cooperate
by exchanging messages with a central server in order to  learn models using the cumulative data of all the clients.  
% from the rest of the clients
% Federated learning aims to solve the empirical problem $\min_{(q_1,\dots,q_n) \in \mathcal{Q}} \frac{1}{n}\sum_{i=1}^n  \hat{f}_i(q_i),
% $
% where $\hat{f}_i(q_i)$ is the empirical loss of $q_i$ on the $i$-th client's $M_i$ training samples.  Federated learning addresses settings in which 
% This will be accomplished 

% We assume that each dataset $\mathcal{D}_i$ is a finite set of $m$ samples. 
% We will often let $\mathcal{X}= \mathbb{R}^d$ and $\mathcal{Y}= \mathbb{R}$. 
% The case of all the $\phi_i$'s being independent is at the local end of the local-global spectrum, and the case $\phi_1 = \dots = \phi_n$, i.e. a single model is learned for all clients, is at the global end. 
% Ultimately, we hope that the models $\phi_i$ perform well with respect to the true data distribution for each client, namely that the population loss 
%While solving this problem, the server can only access high-level information from the clients, such as gradients, in order to meet privacy and communication standards.

% As it relates to this paper, the primary distinction of federated learning from standard supervised learning is that the central authority cannot access the local data on each client due to privacy and communication constraints. Thus, methods to solve \eqref{obj1} must rely on only higher-level information, such as gradients, to be communicated from the clients to the server. Furthermore, 

Standard approaches to federated learning aim at learning a {\em single} shared model $\boldsymbol{\theta} =\boldsymbol{\theta}_1=\dots=\boldsymbol{\theta}_n$ that performs well on average across the clients \citep{mcmahan2017communication, li2018federated}. In this way, the clients aim to solve a special version of Problem~\eqref{obj1}, which is to minimize $(1/n) \sum_i f_i(\boldsymbol{\theta})$ over the choice of the shared model $q$.  However, this approach
%this approach does not address the
% The first is learning each $q_
% i$ using only the $m_i$ local samples pertaining to client $i$, which is typically unwise because $m_i$ is often too small to learn a model that generalizes well without further information supplied by other clients. At the other extreme, training a single global model $q = q_1 = \dots = q_n$ does not account for the 
may yield a solution that performs poorly in heterogeneous settings where the data distributions $\mathcal{D}_i$ vary across the clients. Indeed, in the presence of data heterogeneity, the error functions $f_i$ will have different forms and their minimizers are not the same. Hence, learning a shared model $\boldsymbol{\theta}$ may not provide good solution to  Problem~\eqref{obj1}. This necessitates the search for more personalized solutions $\{\boldsymbol{\theta}_i\}$ that can be learned in a federated manner using the clients' data. 
%We will further demonstrate this fundamental gap in our theoretical setting  in Section~\ref{sec:pf_example}.  

% \begin{comment}
% %\textbf{Remark.} 
% \begin{remark}
% {\bf Representation learning as an interpolation between local and global learning.} Insights from deep learning suggest that data distributed across clients or tasks may share a common representation despite having different labels \cite{bengio2013representation, lecun2015deep}. For example, images of faces may share similar distinguishing features such as nose shape and eye color, while having unique labels on each device. It follows that the server should leverage all of the data to learn a {\em global representation}, while accounting for label heterogeneity by having {each client} learn a {\em unique head} mapping from the representation space to the label space using only its local data. 
% % Thus, it makewe hypothesize that data in federated settings may only be heterogeneous in the label space, while being mostly hypothesis in the 
% \end{remark}
% \end{comment}

% One of the key insights from the success of deep learning is that data of the same type, such as images, often shares similar features 
% the 
% distributions
% $\mathcal{D}_i$ 
% In many real settings, 

% this paper we make the general and  realistic assumption that the local data distributions $\{\mathcal{D}_i\}_i$ are distinct, but share some commonalities. For example, in image classification applications, each client may have {\em different labels} of images, but all image may share {\em common features}.

% In this work we propose to learn a {\em global representation} and client-specific network heads in order to effectively balance the trade-off between local and global strategies. 

\noindent \textbf{Learning a Common Representation.} We are motivated by insights from centralized machine learning that suggest that heterogeneous data distributed across tasks may share a common representation despite having different labels \citep{bengio2013representation, lecun2015deep}; e.g., shared features across many types of images, or across word-prediction tasks.  
% Such insight from deep learning suggests that in real-world settings, while data among the clients is heterogeneous, the main features can be captured through a common representation. 
Using this common (low-dimensional) representation, the labels for each client can be simply learned using a linear classifier or a shallow neural network. 

%%%%%%%HHHHHHHHHHHH
\begin{figure}[t]
%\vskip 0.2inS
\begin{center}
\centerline{\includegraphics[width=0.56\columnwidth]{schematic.pdf}}
\vspace{-2mm}
\caption{Federated representation learning structure where clients and the server aim at learning a global representation $\phi$ together, while each client $i$ learns its unique head $h_i$ locally. }
\label{fig:fedrep2}
\end{center}
\vskip -0.1in
\end{figure}

Formally, we consider a setting consisting of a global representation $\phi(\cdot;\boldsymbol{\theta}_\phi): \mathbb{R}^d \rightarrow \mathbb{R}^k$, which is a function parameterized by $\boldsymbol{\theta}_\phi$ that maps data points to a lower space of dimension $k$, and client-specific heads $h_i(\cdot; \boldsymbol{\theta}_{h_i}) : \mathbb{R}^k \rightarrow \mathcal{Y}$, which are functions parameterized by $\boldsymbol{\theta}_{h_i}$ for $i \in [n]$ that map from the low-dimensional representation space to the label space. 
% We let $\Phi$ be the class of feasible representations and $\mathcal{H}$ be the class of feasible heads.  
The model for the $i$-th client is the composition of the client's local parameters and the representation: $q(\mathbf{x}_i;\boldsymbol{\theta}_i) = h_i(\phi(\mathbf{x}_i; \boldsymbol{\theta}_\phi); \boldsymbol{\theta}_{h_i})$, where $\boldsymbol{\theta}_i = \{\boldsymbol{\theta}_\phi, \boldsymbol{\theta}_{h_i}\}$.
% In practice, we consider deep learning settings in which $\phi$ is the global network body and each $h_i$ is a unique setting of the final one or two layers. 
Critically, $k \ll d$, meaning that the \textcolor{black}{number of parameters} that must be learned locally by each client may be small. Thus, we can assume that any client's optimal classifier for any {\em fixed representation} is \textcolor{black}{easy} to compute, which motivates the following re-written global objective:
%
% Consider that we are in a federated learning setting with $n$ clients. Instead of the classical setting in which the central authority aims to find a single global model that performs well on average across all of the clients, here we imagine a scenario in which the goal of the central authority is to find some global information helpful to solve each of the clients' problems, from which each client can locally adapt to find an optimal solution. 
% In particular, we consider a supervised setting in which data for the $i$-th client is drawn from the distribution $\mu_i$ over the joint data space $\mathcal{X} \times \mathcal{Y}$, where $\mathcal{X} = \mathbb{R}^d$ is the feature space and $\mathcal{Y} = \mathbb{R}$ is the label space. For training, we only have access to $m$ labelled samples per client. The performance of the $i$-th client's model $\phi_i$ on the their local data is given by $F_i(\phi_i) \coloneqq \mathbb{E}_{(x,y) \sim \mu_i}[f_i(\phi_i;x,y)]$, where $f_i$ is a local error function of a single data point. 
% We assume that for each client $i$, $m$ samples from $\mu_i$ are accessible for training. 
% The generic federated learning training problem is then to solve:
% \begin{align}
%     \min_{\phi_1,\dots,\phi_n} \sum_{i=1}^n F_i = \sum_{i=1}^n \sum_{j=1}^m f_i(\phi_i; x^i_j, y^i_j).
% \end{align}
% Ultimately, we hope to reduce dimensionality
% Here we propose to learn a 
\begin{align}
    \min_{\phi \in \Phi} \ \frac{1}{n} \sum_{i=1}^n  \min_{h_i \in \mathcal{H}}\ f_i(h_i, \phi),  \label{obj}
\end{align}
% where we have used the shorthand $f_i(\phi, \mathbf{w}_i) \equiv f_i(\mathbf{w}_i^\top \phi )$, and 
where we have used the shorthand $f_i(h_i,  \phi) \coloneqq f_i(q_{h_i}\circ q_\phi)$ for ease of notation.
In our proposed scheme, clients cooperate to learn the global model using all clients' data, while they use their local information to learn their personalized head. We discuss this in detail in Section~\ref{sec:alg}.




%That is, the server aims to learn the global data representation for which the corresponding optimal local heads yield the smallest net error.
%In Section \ref{sec:alg}, we will show how the server can learn this representation in a federated manner.


\subsection{Comparison with Standard Federated Learning} \label{sec:pf_example}
% We discuss an  example to 
%% Here we give a simple example 

%\sanjay{
{To formally demonstrate the advantage of our formulation over the standard (single-model) federated learning formulation in heterogeneous settings with a shared representation, we study a linear representation setting with  quadratic loss. As we will see below,  standard federated learning {\em cannot recover the underlying representation in the face of heterogeneity}, while our formulation does indeed recover it.}

%% \sanjay{change the language. this section is NOT a simple example. This section is the heart of the paper. The analysis holds only for this "simple example".}

 Consider a setting in which the functions $f_i$ are quadratic losses, the representation $q_\phi$ is a projection onto a $k$-dimensional subspace of $\mathbb{R}^d$ given by matrix $\mathbf{B} \in \mathbb{R}^{d \times k}$, and the $i$-th client's local head $q_{h_i}$ is a vector $\mathbf{w}_i \in \mathbb{R}^k$. In this setting, we model the local data of clients $\{\mathcal{D}_i\}_i$ such that
$ y_i =  {\mathbf{w}_i^\ast}^\top {\mathbf{B}^\ast}^\top\mathbf{x}_i$
for some ground-truth representation $\mathbf{B}^\ast \in \mathbb{R}^{d\times k}$ and local heads $\mathbf{w}_i^\ast \in \mathbb{R}^k$.
 This setting will be described in detail in Section~\ref{sec:linear}. One can show that the expected error over the data distribution $\mathcal{D}_i$ has the following form:
$
    f_i(\mathbf{w}_i, \mathbf{B}) \coloneqq \frac{1}{2}\|\mathbf{B} \mathbf{w}_i - \mathbf{B}^\ast \mathbf{w}^\ast_i\|_2^2
$. Consequently, Problem~\eqref{obj} becomes
\begin{align}
\min_{\mathbf{B} \in \mathbb{R}^{d \times k}, \mathbf{w}_i,\dots,\mathbf{w}_n \in\mathbb{R}^k} \frac{1}{2n}\sum_{i=1}^n\|\mathbf{B} \mathbf{w}_i - \mathbf{B}^\ast \mathbf{w}^\ast_i\|_2^2\label{us}.
\end{align}
In contrast, standard federated learning methods aim to learn a shared model $(\mathbf{B}, \mathbf{w})$ for all the clients, and solve
\begin{align}
\min_{\mathbf{B} \in \mathbb{R}^{d \times k}, \mathbf{w} \in\mathbb{R}^k}\frac{1}{2n}\sum_{i=1}^n\|\mathbf{B} \mathbf{w} - \mathbf{B}^\ast \mathbf{w}^\ast_i\|_2^2. \label{them}
\end{align}
Let $(\hat{\mathbf{B}}, \{\hat{{\mathbf{w}}_i}\}_i) 
$  denote a global minimizer of  
\eqref{us}.  We thus have
$\hat{\mathbf{B}} \hat{\mathbf{w}}_i = \mathbf{B}^\ast \mathbf{w}^\ast_i$ for all $i\in [n]$. Also, it is not hard to see that $({\mathbf{B}}^\diamond, \mathbf{w}^\diamond) 
$ is a global minimizer of \eqref{them} if and only if ${\mathbf{B}}^\diamond \mathbf{w}^\diamond = {\mathbf{B}}^\ast (\frac{1}{n}\sum_{i=1}^n \mathbf{w}^\ast_i)
$. Thus, our formulation finds an exact solution with zero global error, whereas standard federated learning has global error of 
$
 \frac{1}{2n}\sum_{i=1}^n \| \frac{1}{n} \mathbf{B}^\ast\sum_{i'=1}^n (\mathbf{w}^\ast_{i'} - \mathbf{w}^\ast_i)\|_2^2
$, which grows with the heterogeneity of the $\mathbf{w}_i^\ast$. Moreover, since solving our formulation provides $n$ matrix equations, we can fully recover the column space of $\mathbf{B}^\ast$ as long as $\mathbf{w}_i^*$'s span $\mathbb{R}^k$. In contrast, solving \eqref{them} yields only one matrix equation, so there is no hope to recover the column space of $\mathbf{B}^\ast$ for any $k>1$.



%  the server aims to learn $(\mathbf{B}, \mathbf{w})$ rather than $(\mathbf{B}, \{\mathbf{w}_i\}_{i=1}^n )$. Further assume that In this case, the optimal solution $(\bar{\mathbf{B}}, \bar{\mathbf{w}})$ is equal to the average of the clients' optimal solutions, namely 





% {\color{red}{Here is the point that you should mention that simple example to highlight the advantage of our proposed formulation compared to the classic FL formulation.}}

% Often, we will concatenate the $\mathbf{w}_i$'s in the matrix $\mathbf{W} = [\mathbf{w}_1, \dots, \mathbf{w}_n]^\top \in \mathbb{R}^{n\times k}$, and rewrite the objective \eqref{obj} as 
% \begin{align}
%     \min_{\phi \in \Phi;\mathbf{W} \in \mathbb{R}^{n\times k}} \{F(\phi, \mathbf{W}) \coloneqq \frac{1}{n} \sum_{i=1}^n f_i(\phi, \mathbf{w}_i)\}  \label{objF}
% \end{align}


%F(\phi, \mathbf{w}_1,...,\mathbf{w}_n) \coloneqq 
% where the loss function $f_i$ for the $i$-th client is the average mean-squared loss on the client's $m$ samples $\{(\mathbf{x}_i^j, y_i^j)\}_{j=1}^m$, namely
% \begin{align}
%     %f_i(\phi, \mathbf{w}_i) = \tfrac{1}{2}\mathbb{E}_{(\mathbf{x}_i, y_i) \sim \mu_i} [(y_i - \langle \mathbf{w}_i, \phi(\mathbf{x}_i)\rangle)^2]
%     f_i(\phi, \mathbf{w}_i) = \frac{1}{2}\sum_{j=1}^m (y_i^j - \langle \mathbf{w}_i, \phi(\mathbf{x}_i^j)\rangle)^2
% \end{align}


% Each client's local model is the composition of a global representation $\phi \in \Phi$, which maps $\mathcal{X} \rightarrow \mathbb{R}^k$, where $k \ll d$, and client-specific linear models $\{ \mathbf{w}_i \in \mathbb{R}^k\}_{i=1}^n$. That is, $z_i = w_i^\top \phi$


% In our framework, the central authority solves for the global representation $\phi$, while each client solves for their respective $\mathbf{w}_i$. The representation may be a linear map or a nonlinear neural network, we leave those details aside for now. The point is that learning and distributing the optimal representation to the clients allows them to solve their regression problem more easily, by reducing its dimension. 

% Learning a representation only makes sense if there exists a ground truth representation of the data, which is a reasonable assumption to make for most learning problems. Formally, we assume that the data $\{(\mathbf{x}_i^j, y_i^j)\}_{j=1}^m$ for each client is generated from some common representation $\phi^\ast \in \Phi$ and linear models $\mathbf{w}_1^\ast,...,\mathbf{w}_n^\ast \in \mathbb{R}^k$ such that
% \begin{align}
%     {y}_i^j = \langle \mathbf{w}_i^\ast, \phi^\ast(\mathbf{x}_i^j)\rangle + z_i^j, %\quad \text{where} \; \mathbf{x}_i &\sim p_i, \; z_i \sim \mathcal{N}(0,\sigma_i^2)
% \end{align}
% for each $(\mathbf{x}_i^j, y_i^j)\in \mathcal{D}_i$, where $z_i^j \sim \mathcal{N}(0,\nu^2)$. 

%The question now becomes how to learn the optimal $\phi^\ast$ and $w_1^\ast,\dots,w_n^\ast$.

% {\color{red} Do we evaluate on new data at test time? How about new clients?}




% Let the distribution $p_i$ have mean $\mathbf{0}$ and covariance $\Sigma_i$.
%We will typically assume that $p_i$ is the multi-variate normal distribution in $d$ dimensions with mean 0 and covariance $\Sigma_i$... but just need to assume subgaussian



%Here we propose a novel federated learning algorithm to solve for $\phi$ in \eqref{obj} and characterize its convergence rate in terms of the number of communication rounds between the central authority and the clients, the data and client batch sizes, and the number of local updates that each client executes to solve their local minimization problem. We show that our scheme reduces the number of samples required by the clients to solve their problems by a factor proportional to $k/d$, which no other existing federated learning algorithm can match because no other algorithm attempts to learn the representation. Not only is our algorithm the first to learn the representati
% how is federated learning different from multi-task learning context?
%Previous work has shown that solving for the optimal representation $\phi$ reduces the sample complexity to solve a new linear regression task with the same representation by a factor proportional to $k/d$ \citep{du2020fewshot,tripuraneni2020provable}. 

==> arxiv_version_Experiments_arxiv.tex <==
\section{Experiments} \label{sec:experiments}
We focus on three points in our experiments: (i) the effect of many local updates for the local head in FedRep (ii) the quality of the global representation learned by FedRep and (iii) the applicability of FedRep to a wide range of datasets. Full experimental details are provided in Appendix \ref{app:experiments}.

\subsection{Synthetic Data}


We start by experimenting with an instance of the multi-linear regression problem analyzed in Section \ref{sec:linear}. Consistent 
with this formulation, we generate synthetic samples $\mathbf{x}_i^j \sim \mathcal{N}(0, \mathbf{I}_d)$ and labels $y_{i}^j \sim \mathcal{N}(\mathbf{w}_i^{\ast^\top}{\mathbf{B}}^{\ast^\top}\mathbf{x}_i^j, 10^{-3})$ (here we include an additive Gaussian noise). The ground-truth heads $\mathbf{w}_i^\ast \in \mathbb{R}^k$ for clients $i \in [n]$ and the ground-truth representation ${\mathbf{B}}^\ast \in \mathbb{R}^{d \times k}$ are generated randomly by sampling and normalizing Gaussian matrices. 
% and optimal solutions as
% \begin{align}
%     \mathbf{x}_i^j &\sim \mathcal{N}(0, \mathbf{I}_d)\; \forall i \in [n], j \in [m] \\
%     \mathbf{w}_i^\ast &\sim \mathcal{N}(0, \mathbf{I}_k)\; \forall i \in [n],
% \end{align}
% and $\mathbf{B}$ is an orthogonal basis for a $k$-dimensional subspace of $\mathbb{R}^d$.
% Here we consider the noisy case:
% \begin{align}
%     \hat{F}(\mathbf{W},\mathbf{B}) = \frac{1}{2nm} \sum_{i=1}^n \sum_{j=1}^m (\langle \mathbf{x}_{i}^j, \mathbf{B}\mathbf{w}_i\rangle - y_i^j )^2
% \end{align}
% where $y_i^j \sim \mathcal{N}(\langle \mathbf{x}_{i}^j, \mathbf{B}_\ast\mathbf{w}_i^\ast \rangle, \zeta_i )$.

% Note that in this setting, the measurements are i.i.d., but the data itself is non-i.i.d. across clients because each client has a distinct ground-truth solution.


%%%%%%%HHHHHHHHHH
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.7\columnwidth]{old_synth3.eps}}
\vspace{-2mm}
\caption{Comparison of (principal angle) distances between the ground-truth and estimated representations by FedRep and alternating gradient descent algorithms for different numbers of clients $n$. In all plots, $d=10$, $k=2$, $m=5$, and $r=0.1$.}
\label{fig:synth11}
\end{center}
\vskip -0.3in
\end{figure}


\textbf{Benefit of finding the optimal head.}  We first demonstrate that the convergence of FedRep improves with larger number of clients $n$, making it highly applicable to federated settings. Further, we give evidence showing that this improvement is augmented by the minimization step in FedRep, since methods that replace the minimization step in FedRep with 1 and 10 steps of gradient descent (GD-GD and 10GD-GD, respectively) do not scale properly with $n$. 
In Figure \ref{fig:synth11}, we plot convergence trajectories for FedRep, GD-GD, and 10GD-GD for four different values of $n$ and fixed $m, d, k$ and $r$.  As we observe in Figure \ref{fig:synth11}, by increasing the number of nodes $n$, clients converge to the true representation faster. Also, running more local updates for finding the local head accelerates the convergence speed of FedRep. In particular, FedRep which exactly finds the optimal local head at each round has the fastest rate compared to GD-GD and 10GD-GD that only run 1 and 10 local updates, respectively, to learn the head.


% We plot the principal angle distance between the estimated and optimal representation. The plots for function value is similar and is included in the Appendix.


% \begin{table}[t]
% \caption{Smallest $m$ for which $F(\mathbf{W}_{500}, \mathbf{B}_{500}) \leq 10^{-6}$. Here $d=10$, $k=2$ and $\sigma = 0.1$ for all trials. We see that the  minimum $m$ required to achieve the desired accuracy actually decreases with $n$.}
% \label{table1}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Algorithm & $n=10$  &  $n=50$ & n=100 & n=500\\
% \midrule
% AltMinGD      & &  & &  \\
% AltGD-GD    &  &  & &      \\
% % LG-Fed & 85.35$\pm$ & 68/74  \\
% % FedAvg + LG-Fed & $\pm$ &   \\
% % FedAvg   & $\pm$ &   \\
% % FedSGD   & 60.67$\pm$ & 30 \\
% % Fed-MTL     & 76.59$\pm$ &   \\
% % Local     & 92.5 $\pm$ & 88.19  \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
% \caption{Function values and representation learning errors for AltMinGD and AltGD-GD. The value of $m$ is fixed in each row and $n$ is fixed in each column. We see that the relative improvement of AltMinGD over AltGD-GD increases with $n$, highlighting the advantage of AltMinGD in large-$n$ settings.}
% \label{fig:synthetic1}
% \end{center}
% \vskip -0.2in
% \end{figure}

\textbf{Generalization to new clients.} 
Next, we evaluate the effectiveness of the representation learned by FedRep in reducing the sample complexity for a new client which has not participated in training. We compare against FedSGD, which executes distributed SGD to learn a single model $(\mathbf{B},\mathbf{w})$. We first train FedRep and FedSGD on a fixed set of $n=100$ clients as in Figure~\ref{fig:fedrep1},  where $(d,k)\!=\!(20,2)$. 
The new client has access to $m_{\text{new}}$ labeled local samples. It will use the representation $\mathbf{{B}}^*\in \mathbb{R}^{d \times k}$ learned from the training clients, and learns a personalized head using this representation and its local training samples. For both FedRep and FedSGD, we solve for the optimal head given these samples and the representation learned during training. We compare the MSE of the resulting model on the new client's test data to that of a model trained by only using the $m_{\text{new}}$ labeled samples from the new client (Local Only) in Figure \ref{fig:bar_new}. The large error for FedSGD demonstrates that it does not learn the ground-truth representation. Meanwhile, the representation learned by FedRep allows an accurate model to be found for the new client as long as $m_{\text{new}}\geq k$, which drastically improves over the complexity for Local Only ($m_{\text{new}}\!=\!\Omega(d)$).

% Next, we compare against learning a single model in , learning a single overparameterized model,  MTL and AltGD-GD.

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
% \caption{Function values and representation learning errors for AltMinGD and AltGD-GD. The value of $m$ is fixed in each row and $n$ is fixed in each column. We see that the relative improvement of AltMinGD over AltGD-GD increases with $n$, highlighting the advantage of AltMinGD in large-$n$ settings.}
% \label{fig:synthetic1}
% \end{center}
% \vskip -0.2in
% \end{figure}



%%% HHHHHHHH
\begin{figure}[t]
%\vspace{-0.1in}
\begin{center}
\centerline{\includegraphics[width=0.53\columnwidth]{bar_new.eps}}
%\vskip -0.15in
\vspace{-2mm}
\caption{MSE on new clients sharing the representation after fine-tuning using various numbers of samples from the new client.}
\label{fig:bar_new}
\end{center}
\end{figure}



\subsection{Real Data}
We next investigate whether these insights apply to nonlinear models and real datasets.

\textbf{Datasets and Models.} We use four real datasets: CIFAR10 and CIFAR100 \citep{krizhevsky2009learning}, FEMNIST \citep{caldas2018leaf,cohen2017emnist} and Sent140 \citep{caldas2018leaf}. The first three are image datasets and the last is a text dataset for which the goal is to classify the sentiment of a tweet as positive or negative. 
%  each contain 50,000 training samples and 10,000 test samples from 10 and 100 classes, respectively. 
 We control the heterogeneity of CIFAR10 and CIFAR100 by assigning different numbers $S$ of classes per client, from among 10 and 100 total classes, respectively.  Each client is assigned the same number of training samples, namely $50000/n$. For FEMNIST, we restrict the dataset to 10 handwritten letters and assign samples to clients according to a log-normal distribution as in \cite{li2019feddane}. We consider a partition of $n\!=\!150$ clients with an average of 148 samples/client. For Sent140, we use the natural assignment of tweets to their author, and use $n\!=\!183$ clients with an average of 72 samples per client. We use 5-layer CNNs for the CIFAR datasets, a 2-layer MLP for FEMNIST, and an RNN for Sent$140$ \textcolor{black}{(details provided in Appendix \ref{app:experiments})}.

\textbf{Baselines.} We compare against a variety of personalized federated learning techniques as well as methods for learning a single global model and their fine-tuned analogues. Among the personalized methods, FedPer \citep{arivazhagan2019federated} is most similar to ours, as it also learns a global representation and personalized heads, but makes simultaneous local updates for both sets of parameters, therefore makes the same number of local updates for the head and the representation on each local round. Fed-MTL \citep{smith2017federated} learns local models and a regularizer to encode relationships among the clients, PerFedAvg \citep{fallah2020personalized} leverages meta-learning  to learn a single model that performs well after adaptation on each task, and LG-FedAvg \citep{liang2020think} learns local representations and a global head. APFL \citep{deng2020adaptive} interpolates between local and global models, and L2GD \citep{hanzely2020federated} and Ditto \citep{li2020ditto} learn local models that are encouraged to be close together by global regularization. For global FL methods, we consider FedAvg \citep{mcmahan2017communication}, SCAFFOLD \citep{karimireddy2020scaffold}, and FedProx \citep{li2018federated}. To obtain fine-tuning results, we first train the global model for the full training period, then each client then fine-tunes only the head on its local training data for 10 epochs of SGD before computing the final test accuracy. 
% (5) local only training with no global communication. Method (2) is the standard federated learning technique, (3) is a well-known method for achieving personalized models, and (1) and (4) are methods with similar intuitions as ours.



% We use the same five-layer CNN as in \citep{liang2020think} for CIFAR10 and an LSTM for . On each communication round, a constant fraction $r=0.1$ of all of the clients are sampled. To implement AltMinGD, each client executes $\tau \gg 1$ local minibatch SGD steps on the final layer using a batch of size $B$. Then, the base layers are updated with one minibatch SGD step with batch size $B$ and sent to the server. 



% First, we compare the output of AltMinGD to that produced by vanilla federated averaging \cite{mcmahan2017communication} with $E = 20$ local update steps.

% The parameter $E$ denotes the number of local communication rounds for FedAvg. FedSGD is FedAvg with $E=1$, i.e. distributed SGD.


% \begin{table*}[ht]
% \caption{Average local test accuracies over the final 10 rounds out of $T=200$ total rounds, with 95\% confidence intervals.
% }
% \vskip 0.15in
% \begin{center}
% \begin{small}
% % \begin{sc}
% \begin{tabular}{lcccccccc}
% \toprule\label{bigtable1}
% Dataset & FedRep & GD-GD & FedAvg &  Fed-MTL &   LG-FedAvg  & Local \\%& Post-Adapt  \\
% \midrule
% CIFAR10, $S=2$, $n=100$ & $86.08\pm .3$ & $83.52 \pm .4$ & $44.29\pm 1.9$ & $70.44 \pm .2$  & $78.12 \pm 1.1$  & $87.28 \pm .6$ \\
% CIFAR10, $S=2$, $n=1000$ &$76.41\pm .5$ & $73.07 \pm .5$ & $41.11\pm 1.6$ & $56.90 \pm .1$ &  $68.32 \pm 1.4$  &$72.17 \pm .3$\\
% CIFAR10, $S=5$, $n=100$ & $72.19 \pm .9$  &$72.26 \pm 1.0$ & $58.14 \pm 1.5$ & $54.21\pm .3$&  $57.83 \pm 1.2$  & $67.76 \pm .5$\\ %$72.66 \pm .2$
% CIFAR10, $S=5$, $n=1000$ & $53.41 \pm .7$ & $52.27 \pm .8$ & $50.40 \pm .9$ & $34.58 \pm .5$ & $41.05 \pm 1.3$ &  $47.56 \pm .4$\\ %$48.63\pm .7$
% CIFAR100, $S=20$, $n=100$ & $38.17 \pm .8$ & $37.41 \pm .5$ & $15.74 \pm .8$ & $23.38 \pm .3$ & $31.06 \pm .5$ & $32.04 \pm .7$ \\
% CIFAR100, $S=20$, $n=500$ & $21.88 \pm .6$ & $21.92 \pm .6$ & $19.43 \pm .7$  & $10.56 \pm .3$ & $14.83 \pm .4$ & $21.06 \pm .6$ \\ %24.30 \pm .6^*
% % CIFAR100, $S=50$, $n=100$ & $23.71 \pm .7$ & $23.45 \pm .6$ & $20.25\pm .8$ & $14.72 \pm .3$ & $25.07 \pm .4$ & & $17.10\pm 1.1$ \\
% % CIFAR100, $S=50$, $n=500$ & $13.33^*$ & $11.50 \pm .3$ & $18.82\pm.4$ & $6.09 \pm .2$ & $45.56$& &  $11.66 \pm 1.4$\\
% FEMNIST, $n=150$ & $65.52 \pm .8$  & $39.21 \pm .6$ & $60.71 \pm 1.8$ & $32.34 \pm .7$  & $29.78\pm .5$  &$29.12 \pm .9$ \\
% Sent$140$, $n=183$ & $72.13 \pm .2$ &$69.57 \pm .8$ & $56.82 \pm 1.4$ & $54.82 \pm .5$ & $70.84 \pm 1.4$ & $70.22 \pm .8$\\%$70.64 \pm .9$
% % FEMNIST, $n=100$ & & &  & & & & &\\
% \bottomrule
% \end{tabular}
% % \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}

\begin{table*}[ht]
\caption{Average test accuracies on various partitions of CIFAR10, CIFAR100, Sent140 and FEMNIST with participation rate $r\!=\!0.1$.
}
\vskip -1in
% \vskip 0.15in
\begin{center}
% \begin{sc}
\footnotesize
\begin{tabular}{l|ccc|cc|c|c}
\toprule\label{bigtable1}
& \multicolumn{3}{c|}{{CIFAR10}}  &  \multicolumn{2}{c|}{{CIFAR100}}       & Sent140 & FEMNIST  \\
\midrule
(\# clients $n$, \# classes per client $S$) & $(100,2)\!$ & $\!(100,5)$ & $(1000,2)$ & $(100,5)$  & $(100,20)$ & $(183,2)$ & $(150,3)$ \\%& Post-Adapt  \\
\midrule
Local Only & $\mathbf{89.79}$ & 70.68 & 78.30 & 75.29 & 41.29 & 69.88 &  60.86 \\
\midrule
FedAvg \citep{mcmahan2017communication} &  42.65 & 51.78 & 44.31 & 23.94 & 31.97 & 52.75 & 51.64 \\ %53.75 
FedAvg+FT & 87.65 & 73.68  & 82.04 & $\mathbf{79.34}$ & 55.44  &71.92  & 72.41\\ %71.54
FedProx \citep{li2018federated} & 39.92 & 50.99 & 21.93  & 20.17 & 28.52 & 52.33 &  18.89 \\
FedProx+FT & 85.81 & 72.75 & 75.41 & 78.52 & 55.09 & 71.21 & 53.54 \\
SCAFFOLD \citep{karimireddy2020scaffold} & $37.72$ & $47.33$ & $33.79$ &  20.32 & 22.52 & $51.31$ & 17.65 \\
SCAFFOLD+FT  & $86.35$ &  $68.23$ &$78.24$ & 78.88 & 44.34 & 71.49  & 52.11  \\
\midrule 
Fed-MTL \citep{smith2017federated} & 80.46 & 58.31  & 76.53  & 71.47 & 41.25 & 71.20 & 54.11 \\
PerFedAvg \citep{fallah2020personalized} & 82.27 & 67.20 & 67.36 & 72.05 &  52.49  & 68.45 & 71.51 \\
LG-Fed \citep{liang2020think} & 84.14  & 63.02 &  77.48 & 72.44 &38.76 & 70.37 & 62.08 \\
L2GD \citep{hanzely2020federated} & 81.04 & 59.98 & 71.96 & 72.13 & 42.84 & 70.67 & 66.18  \\
APFL  \citep{deng2020adaptive} & 83.77 & 72.29 & 82.39 & 78.20 & 55.44 & 69.87 & 70.74 \\
Ditto \citep{li2020ditto} & 85.39 & 70.34 & 80.36 & 78.91 &  $\mathbf{56.34}$ & 71.04 & 68.28 \\
FedPer \citep{arivazhagan2019federated} & 87.13 & 73.84 & 81.73 & 76.00 & 55.68 & 72.12 & 76.91 \\
\midrule
FedRep (Ours) & $\mathbf{87.70}$ & $\mathbf{75.68}$ & $\mathbf{83.27}$ & 79.15 & 56.10 &  $\mathbf{72.41}$ & $\mathbf{78.56}$ \\ 
\bottomrule
\end{tabular}
% \end{sc}
\end{center}
\vskip -0.1in
\end{table*}



\textbf{Implementation.}
In each experiment we sample a ratio $r\!=\!0.1$ of all the clients on every round. We initialize all models randomly and train for $T\!=\!100$ communication rounds for the CIFAR datasets, $T\!=\!50$ for Sent140, and $T\!=\!200$ for FEMNIST. In each case, for each local updates FedRep executes ten local epochs of SGD with momentum to train the local head, followed by one epoch for the representation in the case of CIFAR10 with $n\!=\!100$ and 5 epochs in all other cases. All other methods use the same number of local epochs as FedRep does for updating the representation. Accuracies are computed by taking the average local accuracies for all users over the final 10 rounds of communication, except for the fine-tuning methods. These accuracies are computed after locally training the head of the fully-trained global model for ten epochs for each client. 


%%%%%%%%%%HHHHHHH
\begin{figure}[t]
\begin{center}
%\vspace{-2mm}
\centerline{\includegraphics[width=0.56\columnwidth]{cifar.eps}}
%\vskip -0.05in
\caption{CIFAR10 local test errors for different numbers of local epochs $E$ for  FedAvg and for the heads in FedRep.}
\label{fig:cifar}
\end{center}
\vspace{-2mm}
\end{figure}



\textbf{Benefit of more local updates.} As mentioned in Section \ref{sec:intro}, a key advantage of our formulation is that it enables clients to run many local updates without causing divergence from the global optimal solution. We demonstrate an example of this in Figure \ref{fig:cifar}. Here, there are $n\!=\!100$ clients where each has $S\!=\!2$ classes of images. For FedAvg, we observe running more local updates does not necessarily improve the performance. In contrast, FedRep's performance is monotonically non-decreasing with the number of local epochs for the heads, i.e., {\em FedRep  is never hurt by more local computation on the heads.}  %, making it especially conducive to federated settings in which we want to distribute as much of the computation as possible

\textbf{Robustness to varying levels of heterogeneity, number of clients and number of samples per client.} We show the average local test errors for all of the algorithms for a variety of settings in Table \ref{bigtable1}. Recall that for the CIFAR datasets, the number of training samples per client is equal to $50000/n$, so the columns with 100 clients have 500 training samples per client, and the column with 1000 clients has only 50 training samples per client. In all cases, FedRep is either the top-performing method or is very close to the top-performing method. Surprisingly, the fine-tuning methods perform very well, especially FedAvg+FT. The superior performance of FedAvg relative SCAFFOLD is likely because all settings involve partial client participation. 
% We also observe that fine-tuning methods perform relatively well

% ideas for another plot: 1) move version of fedrep vs gdgd with comm time from rebuttal to the main body 2) show degredation of gd-gd with more local epochs... but what to compare against? fedavg with 


% Not surprisingly, the largest gain for FedRep over FedAvg comes in heterogeneous settings with many samples/client: CIFAR10 and CIFAR100 with 2 and 20 classes/client, respectively, and $n=100$. In these settings, FedRep matches, or nearly matches, the performance of local-only training.
% Meanwhile, even in homogeneous and small-data settings conducive to global-only training, i.e. $S\!=\!5$ and $n\!=\!1000$ on CIFAR10, FedRep still outperforms all the baselines, even without any regularization added to prevent over-fitting to the head. {\em This evidence supports our intuition that FedRep effectively interpolates between local and global learning.} Furthermore, FedRep outperforms all other baselines.



%% \textcolor{red}{why doe we only talk about fedrep vs fedavg? we should say we outperform all those baselines}


%%%%%%%%%%%%%%%HHHHHHHHHHHHHH
\begin{figure}[t]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.64\columnwidth]{new_users.eps}}
\vspace{-2mm}
\caption{Test accuracy on handwritten digits from FEMNIST after fine-tuning the head of models trained on FEMNIST-letters.}
\label{fig:new_clients}
\end{center}
\vspace{-6mm}
\end{figure}

\textbf{Generalization to new clients.} 
We also evaluate the strength of the representation learned by FedRep in terms of %its ability to lead to 
adaptation for new users. To do so, we first train FedRep, FedAvg, PerFedAvg, LG-FedAvg, APFL, L2GD and FedProx
in the usual setting on the partition of FEMNIST containing images of 10 handwritten letters (FEMNIST-letters). Then, we encounter clients with data from a different partition of the FEMNIST dataset, containing images of handwritten digits. We assume we have access to a dataset of 500 samples at this new client to fine tune the head. Using these, with each of the algorithms, we fine tune the head over multiple epochs while keeping the representation fixed. 
% Over each epoch, we train the head by sweeping over these new samples, and test over a holdout validation set (again from this new partition). 
In Figure \ref{fig:new_clients}, we repeatedly sweep over the same 500 samples over multiple epochs to further refine the head, and plot the corresponding local test accuracy. As is apparent, FedRep has significantly better performance than these baselines.  


==> notes.tex <==


---------------------------

We first consider the term $\| \hat{U}_{t+1} V_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F$:
% $$\|\hat{U}_{t+1}  \hat{V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F \leq \|U_\ast \Sigma_\ast R_t^\top {V}_t - U_\ast \Sigma_\ast V_\ast^\top \|_F$$
\begin{align}
    \|\hat{U}_{t+1}  {V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F &\leq  \frac{1}{1-\delta_{2k}}\|\mathcal{A}(\hat{U}_{t+1}  {V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top) \|_F \label{krip2} \\
    &\leq \frac{1}{1-\delta_{2k}}\|\mathcal{A}(U_\ast \Sigma_\ast V_\ast^\top V_t {V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top) \|_F \label{lss} \\
    &\leq \frac{1+\delta_{2k}}{1-\delta_{2k}}\|U_\ast \Sigma_\ast V_\ast^\top V_t {V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F \label{krip3} \\
    &\leq \frac{1+\delta_{2k}}{1-\delta_{2k}} \|U_\ast\|_F \| \Sigma_\ast\|_2 \| (V_\ast^\top V_t {V}_t^\top - V_\ast^\top) \|_2 \label{cs1} \\
    &\leq \sqrt{k}\frac{1+\delta_{2k}}{1-\delta_{2k}} \| \Sigma_\ast\|_2 \| V_\ast^\top (V_t {V}_t^\top - I) \|_2 \label{rtk} \\
    % &= \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \Sigma_\ast\|_2 \| V_\ast^\top (V_t {V}_t^\top - I) \|_2 \nonumber \\
    &= \sqrt{k} \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \Sigma_\ast\|_2 \;\text{dist}(V_t, V_\ast) \label{step1}
\end{align}
where \eqref{krip2} and \eqref{krip3} follow by $2k$-RIP, \eqref{lss} follows by the fact that $\hat{U}_{t+1}$ is the least squares solution, \eqref{cs1} follows by Cauchy-Schwarz, \eqref{rtk} follows since $\|U\|_F \leq \sqrt{k} \|U\|_2$ = $\sqrt{k}$. Next we consider that for any $x:\|x\|_2=1$,
\begin{align}
    \|\hat{U}_{t+1} x x^\top {V}_t^\top \|_F &\leq  \|\hat{U}_{t+1} x x^\top\|_F\| \|V_t\|_2 \nonumber \\
    &\leq\|\hat{U}_{t+1}\|_2 \|xx^\top \|_F  \nonumber \\
    &= \|\hat{U}_{t+1}\|_2 \label{step2}.
\end{align}
We have 
\begin{align}
    \|\hat{U}_{t+1}\|_2 &\leq 
    % \| B^{-1} C S \tilde{u}^\ast \|_2 \nonumber \\
    \| U_\ast \Sigma_\ast V_\ast^\top V_t \|_2 + \|F\|_2 \nonumber \\
    &\leq \| \Sigma_\ast\|_2  + \|F\|_F  \nonumber \\
    &\leq \| \Sigma_\ast\|_2 + \frac{\sqrt{k}}{1-\delta_{2k}}\|\Sigma_\ast\|_2\|(BD-C)\|_2  \nonumber \\ 
    &\leq \|\Sigma_\ast\|_2 + \frac{k\delta_{2k}}{1-\delta_{2k}}\|\Sigma_\ast\|_2  \nonumber \\
    &= \frac{1 + (k-1)\delta_{2k}}{1-\delta_{2k}}\|\Sigma_\ast\|_2 \label{boundU}
    % &\leq \| B^{-1}\|_2 \| C \|_2 \| S \|_2 \nonumber \\
    %&\leq \sqrt{k}\frac{1+ \sqrt{k}\delta_{2k}}{1-\delta_{2k}} \|\Sigma_\ast\|_2
\end{align}
using Lemmas B.2 to bound $\|B^{-1}\|_2$ and 4.6 to bound $\|BD-C\|_2$ in JNS14, recalling that $\hat{U}_{t+1} = U_\ast \Sigma_\ast V_\ast^\top V_t - F$ where $vec(F) = B^{-1}(BD-C)S \tilde{u}^\ast$. Thus we have
\begin{align}
    \max_{x: \|x\|_2=1}\lambda_{\max}(V_t^\top S_t^\top \hat{U}_{t+1} + \hat{U}_{t+1}^\top S_t V_t) \leq 2k \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \Sigma_\ast\|_2 \;\text{dist}(V_t, V_\ast) \frac{(1+\delta_{2k})^2(1 + (k-1)\delta_{2k})}{(1-\delta_{2k})^2}\|\Sigma_\ast\|_2^2 \; \text{dist}^2(V_t, V_\ast)
\end{align}
% where
% \begin{align}
%     V_t^\top S_t^\top \hat{U}_{t+1} + \hat{U}_{t+1}^\top S_t V_t &= V_t^\top (\mathcal{A}^\ast \mathcal{A}(Q_t))^\top \hat{U}_{t+1} + \hat{U}_{t+1}^\top \mathcal{A}^\ast \mathcal{A}(Q_t) V_t \nonumber
% \end{align}


% Analyzing one of the terms,

%     \begin{align}
% V_t^\top (\mathcal{A}^\ast \mathcal{A}(Q_t))^\top \hat{U}_{t+1}
%     &= V_t^\top \sum_{i=1}^N \langle A_i, \hat{U}_{t+1}V_t^\top - U_\ast \Sigma_\ast V_\ast^\top \rangle A_i^\top \hat{U}_{t+1} \nonumber \\
%     &=  \sum_{i=1}^N \langle A_i, \hat{U}_{t+1}V_t^\top - U_\ast \Sigma_\ast V_\ast^\top \rangle V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
%     % &=  \sum_{i=1}^N 
%     % \langle A_i, U_\ast \Sigma_\ast V_\ast^\top V_t V_t^\top - F V_t^\top- U_\ast \Sigma_\ast V_\ast^\top \rangle V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
%     % &= \sum_{i=1}^N 
%     % \langle A_i, U_\ast \Sigma_\ast V_\ast^\top V_{t,\perp} - F V_t^\top \rangle V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
%     &= \sum_{i=1}^N \langle A_i, \hat{U}_{t+1}V_t^\top\rangle V_t^\top A_i^\top \hat{U}_{t+1} - \langle A_i, U_\ast \Sigma_\ast V_\ast^\top \rangle V_t^\top A_i^\top \hat{U}_{t+1} \nonumber
%     % &= \sum_{i=1}^N \sum_{\ell=1}^d
%     % a_{i,\ell}^\top M v_{t,\perp,\ell} \left(\sum_{q = 1}^k e_q v_{t,q}^\top\right) A_i^\top \hat{U}_{t+1}
%     % -\sum_{i=1}^N \langle A_i, F V_t^\top \rangle V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
%     % &= \sum_{i=1}^N \sum_{\ell=1}^d
%     %  \left(\sum_{q = 1}^k e_q a_{i,\ell}^\top M v_{t,\perp,\ell} v_{t,q}^\top\right) A_i^\top \hat{U}_{t+1}
%     % -\sum_{i=1}^N \langle A_i, F V_t^\top \rangle V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
% \end{align}
% Next, define {\small 
% \begin{align}
% \Lambda_i \coloneqq \left[\begin{matrix}A_i &\dots&0_{n}\\\vdots&\ddots&\vdots\\0_n&\dots&A_i \end{matrix}\right]
% % \mbox{ , }
% % H\coloneqq \left[\begin{matrix}h_{1,t}I_{n}&\dots&0_{n}\\\vdots&\ddots&\vdots\\0_n&\dots&h_{k,t}I_n\end{matrix}\right] 
% \end{align}}
% for all $i \in [N]$. Further, define  $$  \widetilde{v}^{(t)}=\left[\begin{matrix}\hat{v}_1^{(t+1)}\\\vdots\\\hat{v}_k^{(t+1)}\end{matrix}\right]$$. 

% Consider
% \begin{align}
%     \text{tr}\left(\sum_{i=1}^N \langle A_i, \hat{U}_{t+1}V_t^\top\rangle V_t^\top A_i^\top \hat{U}_{t+1}\right) &= \sum_{i=1}^N \sum_{p=1}^k (v_p^{(t)})^\top A_i^\top \hat{u}_{p}^{(t+1)} \text{tr}\left(V_t^\top A_i^\top \hat{U}_{t+1}\right) \nonumber \\
%     &= \sum_{i=1}^N\sum_{p=1}^k (\hat{u}_{p}^{(t+1)})^\top A_i v_p^{(t)} \sum_{q=1}^k (v_q^{(t)})^\top A_i^\top \hat{u}_{q}^{(t+1)} \nonumber \\
%     &=\sum_{p=1}^k (\hat{u}_{p}^{(t+1)})^\top \sum_{q=1}^k  \left(\sum_{i=1}^N A_i v_p^{(t)}  (v_q^{(t)})^\top A_i^\top\right) \hat{u}_{q}^{(t+1)} \nonumber \\
%     &= \sum_{p=1}^k (\hat{u}_{p}^{(t+1)})^\top \sum_{q=1}^k  \left(\sum_{i=1}^N A_i v_p^{(t)}  (v_q^{(t)})^\top A_i^\top\right) \hat{u}_{q}^{(t+1)} \nonumber \\
%     &= \sum_{p=1}^k (\hat{u}_{p}^{(t+1)})^\top \sum_{q=1}^k  \left(\sum_{i=1}^N A_i v_p^{(t)}  (v_q^{\ast})^\top A_i^\top\right) \sigma_q^\ast {u}_{q}^{\ast} \nonumber
%     % &= \sum_{i=1}^N  \widetilde{v}_t^\top \Lambda_i^\top \widetilde{u}_{t+1} V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
%     % &= \sum_{i=1}^N  \widetilde{v}_t^\top \Lambda_i^\top B^{-1}CS \widetilde{u}_\ast V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
%     % &= \sum_{i=1}^N  \widetilde{u}_\ast^\top S C^\top B^{-\top} \Lambda_i^\top  \widetilde{v}_t V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
% \end{align}
% where the last equality follows by definition of $\hat{u}_{q}^{(t+1)}$. Meanwhile,
% \begin{align}
%     \text{tr}\left(\sum_{i=1}^N \langle A_i, {U}_{\ast}\Sigma_\ast V_\ast^\top\rangle V_t^\top A_i^\top \hat{U}_{t+1}\right) &= \sum_{i=1}^N \sum_{q=1}^k \sigma_q^\ast (v_q^{\ast})^\top A_i^\top \hat{u}_{q}^{\ast} \text{tr}\left(V_t^\top A_i^\top \hat{U}_{t+1}\right) \nonumber \\
%     &= \sum_{i=1}^N\sum_{q=1}^k \sigma_q^\ast ({u}_{p}^{\ast})^\top A_i v_q^{\ast} \sum_{p=1}^k (v_p^{(t)})^\top A_i^\top \hat{u}_{p}^{(t+1)} \nonumber \\
%     &= \sum_{i=1}^N\sum_{p=1}^k (\hat{u}_{p}^{(t+1)})^\top  A_i v_p^{(t)} \sum_{q=1}^k \sigma_q^\ast (v_q^{\ast})^\top A_i^\top {u}_{p}^{\ast} \nonumber \\
%     % &=\sum_{p=1}^k (\hat{u}_{p}^{(t+1)})^\top \sum_{q=1}^k  \left(\sum_{i=1}^N A_i v_p^{(t)}  (v_q^{(t)})^\top A_i^\top\right) \hat{u}_{q}^{(t+1)} \nonumber \\
%     % &= \sum_{p=1}^k (\hat{u}_{p}^{(t+1)})^\top \sum_{q=1}^k  \left(\sum_{i=1}^N A_i v_p^{(t)}  (v_q^{(t)})^\top A_i^\top\right) \hat{u}_{q}^{(t+1)} \nonumber \\
%     &= \sum_{p=1}^k (\hat{u}_{p}^{(t+1)})^\top \sum_{q=1}^k  \left(\sum_{i=1}^N A_i v_p^{(t)}  (v_q^{\ast})^\top A_i^\top\right) \sigma_q^\ast {u}_{q}^{\ast} \nonumber \\
%     &= \text{tr}\left(\sum_{i=1}^N \langle A_i, \hat{U}_{t+1}V_t^\top\rangle V_t^\top A_i^\top \hat{U}_{t+1}\right) 
%     % &= \sum_{i=1}^N  \widetilde{v}_t^\top \Lambda_i^\top \widetilde{u}_{t+1} V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
%     % &= \sum_{i=1}^N  \widetilde{v}_t^\top \Lambda_i^\top B^{-1}CS \widetilde{u}_\ast V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
%     % &= \sum_{i=1}^N  \widetilde{u}_\ast^\top S C^\top B^{-\top} \Lambda_i^\top  \widetilde{v}_t V_t^\top A_i^\top \hat{U}_{t+1} \nonumber \\
% \end{align}
% Thus 
% \begin{align}
%     \text{tr}(V_t^\top S_t^\top \hat{U}_{t+1}) = \text{tr}(\sum_{i=1}^N \langle A_i, \hat{U}_{t+1}V_t^\top\rangle V_t^\top A_i^\top \hat{U}_{t+1} - \langle A_i, U_\ast \Sigma_\ast V_\ast^\top \rangle V_t^\top A_i^\top \hat{U}_{t+1}) = 0
% \end{align}
% Likewise,
% \begin{align}
%     \text{tr}( \hat{U}_{t+1}^\top S_t V_t)  = 0
% \end{align}


% noting that since $ a_{i,\ell}^\top M v_{t,\perp,\ell}$ is a scalar, it commutes with every other term.

----------------------------------------

{\color{red} old:}

Multiplying both sides by $V_{\ast,\perp}^\top$ and taking the squared spectral norm, we have 
\begin{align}
    \| V_{\ast,\perp}^\top \hat{V}_{t+1}\|_2^2 &= \| V_{\ast,\perp}^\top V_t - \eta V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1} \|_2^2 \nonumber \\
    &= \lambda_{\max}\big( V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top V_t - \eta ( V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1} + \hat{U}_{t+1}^\top S_t V_{\ast,\perp} V_{\ast,\perp}^\top V_t) \nonumber \\
    &\quad \quad \quad \quad \eta^2 \hat{U}_{t+1}^\top S_t V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1}\big) \nonumber \\
    &\leq \lambda_{\max}( V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top V_t) - \eta \lambda_{\min}( V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1} + \hat{U}_{t+1}^\top S_t V_{\ast,\perp} V_{\ast,\perp}^\top V_t) \nonumber \\
    &\quad \quad \quad \quad \eta^2 \lambda_{\max}(\hat{U}_{t+1}^\top S_t V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1}) \label{weyl} \\
    &= \text{dist}^2(V_t, V_\ast) - \eta \lambda_{\min}( V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1} + \hat{U}_{t+1}^\top S_t V_{\ast,\perp} V_{\ast,\perp}^\top V_t) \nonumber \\
    &\quad \quad \quad \quad \eta^2 \lambda_{\max}(\hat{U}_{t+1}^\top S_t V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1}) \label{3termsk}
\end{align}
where \eqref{weyl} follows by Weyl's inequality, noting that each of the three matrices involved is symmetric. Next we lower bound the cross term. Consider
\begin{align}
    \lambda_{\min}( V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1} ) &= \min_{x: \|x\|_2 =1} x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1} x \nonumber \\
    &= \min_{x: \|x\|_2 =1} \langle (\hat{U}_{t+1}x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top)^\top,  S_t^\top\rangle \nonumber \\
    &= \min_{x: \|x\|_2 =1} \langle \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top,  \mathcal{A}^\ast \mathcal{A}( \hat{U}_{t+1} V_t^\top - U_\ast \Sigma_\ast V_\ast^\top )\rangle \nonumber \\
    &= \min_{x: \|x\|_2 =1} \langle \mathcal{A} (\hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top), \mathcal{A}( \hat{U}_{t+1} V_t^\top - U_\ast \Sigma_\ast V_\ast^\top )\rangle \nonumber \\
    &\geq \min_{x: \|x\|_2 =1} \langle \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top, \hat{U}_{t+1} V_t^\top - U_\ast \Sigma_\ast V_\ast^\top \rangle \nonumber \\
    &\quad \quad \quad \quad - \delta_{2k} \| \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top \|_F \| \hat{U}_{t+1} V_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F \label{krip1} 
\end{align}
%\left(\mathcal{A}^\ast \mathcal{A}( \hat{U}_{t+1} V_t^\top - U_\ast \Sigma_\ast V_\ast^\top )\right)^\top\right
where \eqref{krip1} follows by the RIP. We first consider the term $\| \hat{U}_{t+1} V_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F$:
% $$\|\hat{U}_{t+1}  \hat{V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F \leq \|U_\ast \Sigma_\ast R_t^\top {V}_t - U_\ast \Sigma_\ast V_\ast^\top \|_F$$
\begin{align}
    \|\hat{U}_{t+1}  {V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F &\leq  \frac{1}{1-\delta_{2k}}\|\mathcal{A}(\hat{U}_{t+1}  {V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top) \|_F \label{krip2} \\
    &\leq \frac{1}{1-\delta_{2k}}\|\mathcal{A}(U_\ast \Sigma_\ast V_\ast^\top V_t {V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top) \|_F \label{lss} \\
    &\leq \frac{1+\delta_{2k}}{1-\delta_{2k}}\|U_\ast \Sigma_\ast V_\ast^\top V_t {V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F \label{krip3} \\
    &\leq \frac{1+\delta_{2k}}{1-\delta_{2k}} \|U_\ast\|_F \| \Sigma_\ast\|_2 \| (V_\ast^\top V_t {V}_t^\top - V_\ast^\top) \|_2 \label{cs1} \\
    &\leq \sqrt{k}\frac{1+\delta_{2k}}{1-\delta_{2k}} \| \Sigma_\ast\|_2 \| V_\ast^\top (V_t {V}_t^\top - I) \|_2 \label{rtk} \\
    % &= \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \Sigma_\ast\|_2 \| V_\ast^\top (V_t {V}_t^\top - I) \|_2 \nonumber \\
    &= \sqrt{k} \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \Sigma_\ast\|_2 \;\text{dist}(V_t, V_\ast) \label{step1}
\end{align}
where \eqref{krip2} and \eqref{krip3} follow by $2k$-RIP, \eqref{lss} follows by the fact that $\hat{U}_{t+1}$ is the least squares solution, \eqref{cs1} follows by Cauchy-Schwarz, \eqref{rtk} follows since $\|U\|_F \leq \sqrt{k} \|U\|_2$ = $\sqrt{k}$. Next we consider
\begin{align}
    \|\hat{U}_{t+1} x x^\top {V}_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top\|_F &\leq  \|\hat{U}_{t+1} x x^\top\|_F\| {V}_t^\top V_{\ast,\perp}\|_2 \|V_{\ast,\perp}^\top\|_2 \nonumber \\
    &\leq\|\hat{U}_{t+1}\|_2 \|xx^\top \|_F \; \text{dist}(V_t, V_\ast) \nonumber \\
    &= \|\hat{U}_{t+1}\|_2 \; \text{dist}(V_t, V_\ast) \label{step2}
\end{align}
We have 
\begin{align}
    \|\hat{U}_{t+1}\|_2 &\leq 
    % \| B^{-1} C S \tilde{u}^\ast \|_2 \nonumber \\
    \| U_\ast \Sigma_\ast V_\ast^\top V_t \|_2 + \|F\|_2 \nonumber \\
    &\leq \| \Sigma_\ast\|_2  + \|F\|_F  \nonumber \\
    &\leq \| \Sigma_\ast\|_2 + \frac{\sqrt{k}}{1-\delta_{2k}}\|\Sigma_\ast\|_2\|(BD-C)\|_2  \nonumber \\ 
    &\leq \|\Sigma_\ast\|_2 + \frac{k\delta_{2k}}{1-\delta_{2k}}\|\Sigma_\ast\|_2  \nonumber \\
    &= \frac{1 + (k-1)\delta_{2k}}{1-\delta_{2k}}\|\Sigma_\ast\|_2 \label{boundU}
    % &\leq \| B^{-1}\|_2 \| C \|_2 \| S \|_2 \nonumber \\
    %&\leq \sqrt{k}\frac{1+ \sqrt{k}\delta_{2k}}{1-\delta_{2k}} \|\Sigma_\ast\|_2
\end{align}
using Lemmas B.2 to bound $\|B^{-1}\|_2$ and 4.6 to bound $\|(BD-C)\|_2$ in JNS14, recalling that $\hat{U}_{t+1} = U_\ast \Sigma_\ast V_\ast^\top V_t - F$ where $vec(F) = B^{-1}(BD-C)S \tilde{u}^\ast$. Thus we have
    \begin{align}
    \min_{x: \|x\|_2=1} \delta_{2k} \|\hat{U}_{t+1} x x^\top {V}_t^\top {V}_{\ast,\perp}\|_F \|\hat{U}_{t+1}  {V}_t^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F \leq \sqrt{k}\delta_{2k} \frac{(1+\delta_{2k})(1+(k-1)\delta_{2k})}{(1 -\delta_{2k})^2}\|\Sigma_\ast\|_2^2 \; \text{dist}^2(V_t, V_\ast)
\end{align}
Next we consider the inner product in \eqref{krip1}. We have that for any $x \in \mathbb{R}^k$ such that $\|x\|_2 = 1$,
\begin{align}
    \langle \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top, \hat{U}_{t+1} V_t^\top - U_\ast \Sigma_\ast V_\ast^\top \rangle &=  \langle \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top, \hat{U}_{t+1} V_t^\top\rangle - \nonumber \\
    &\quad \quad\langle \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top,  U_\ast \Sigma_\ast V_\ast^\top \rangle \nonumber \\
    &=  \langle \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top, \hat{U}_{t+1} V_t^\top\rangle  \nonumber \\
    &\quad \quad -\text{tr} (V_{\ast,\perp}^\top V_t x x^\top \hat{U}_{t+1}^\top  U_\ast \Sigma_\ast V_\ast^\top V_{\ast,\perp}) \nonumber \\
    &= \langle \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top, \hat{U}_{t+1} V_t^\top\rangle
\end{align}
since $V_\ast^\top V_{\ast,\perp} = 0$. Next,
\begin{align}
    \langle \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top, \hat{U}_{t+1} V_t^\top\rangle &= \text{tr}(V_{\ast,\perp} V_{\ast,\perp}^\top V_t x x^\top\hat{U}_{t+1}^\top \hat{U}_{t+1} V_t^\top) \nonumber \\
    &= \text{tr}(V_{\ast,\perp} V_{\ast,\perp}^\top V_t \hat{U}_{t+1}^\top \hat{U}_{t+1} V_t^\top) + \text{tr}(V_{\ast,\perp} V_{\ast,\perp}^\top V_t (xx^\top - I_k) \hat{U}_{t+1}^\top \hat{U}_{t+1} V_t^\top) \nonumber \\
    &= \|V_{\ast,\perp}^\top V_t \hat{U}_{t+1}^\top\|_F^2 + \langle (xx^\top-I_k) V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top V_t, \hat{U}_{t+1}^\top \hat{U}_{t+1}\rangle \nonumber \\
    &\geq \sigma_{\min}^2(\hat{U}_{t+1}) \; \text{dist}^2(V_t, V_\ast) - \| (I_k - xx^\top) V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top V_t\|_F\| \hat{U}_{t+1}^\top \hat{U}_{t+1}\|_F \nonumber \\
    &\geq \sigma_{\min}^2(\hat{U}_{t+1}) \; \text{dist}^2(V_t, V_\ast) - \|I_k - xx^\top\|_F\| \hat{U}_{t+1}\|_F^2\; \text{dist}^2(V_t, V_\ast)
\end{align}

but this bound is negative....


-------------------------------------------

by repeated applications of the Cauchy-Schwarz inequality. First note that $\|I_k - xx^\top\|_F^2 = \text{tr}(I_k - xx^\top) = k - 1$. Next, we have using similar analysis as in \eqref{boundU} that
\begin{align}
    \|\hat{U}_{t+1}\|_F &\leq 
    % \| B^{-1} C S \tilde{u}^\ast \|_2 \nonumber \\
    \| U_\ast \Sigma_\ast V_\ast^\top V_t \|_F + \|F\|_F \nonumber \\
    &\leq \sqrt{k}\| \Sigma_\ast\|_2  + \|F\|_F  \nonumber \\
    % &\leq \sqrt{k}\| \Sigma_\ast\|_2 + \frac{\sqrt{k}}{1-\delta_{2k}}\|\Sigma_\ast\|_2\|(BD-C)\|_2  \nonumber \\ 
    &\leq \sqrt{k}\|\Sigma_\ast\|_2 + \frac{k\delta_{2k}}{1-\delta_{2k}}\|\Sigma_\ast\|_2  \nonumber \\
    &= (1+\frac{k\delta_{2k}}{1-\delta_{2k}})\|\Sigma_\ast\|_2  %\frac{\sqrt{k} + (k-\sqrt{k})\delta_{2k}}{1-\delta_{2k}}\|\Sigma_\ast\|_2
\end{align}
Thus 
\begin{align}
\|\hat{U}_{t+1}\|_F^2 &\leq  \big(2+\frac{2k^2 \delta_{2k}^2}{(1-\delta_{2k})^2}\big)\|\Sigma_\ast\|_2^2
\end{align}
For the lower bound, note that
\begin{align}
    \|\hat{U}_{t+1}\|_F^2 &= \|B^{-1}C S \tilde{u}^\ast\|_2^2 \nonumber \\
    &\geq \sigma_{\min}^2(B^{-1}) \sigma_{\min}^2(C) \sigma_{\min}^2(\Sigma) \nonumber \\
    &\geq (1 - \text{dist}^2(V_t, V_{\ast,\perp}) - \delta_{2k}(1 + \sqrt{k} + k\delta_{2k}))\sigma_{\min}^2(\Sigma)
\end{align}
using Lemmas \ref{lem:bmin} and \ref{lem:cmin}.

Putting these parts together, we have:
\begin{align}
    \langle \hat{U}_{t+1} x x^\top V_t^\top V_{\ast,\perp} V_{\ast,\perp}^\top, \hat{U}_{t+1} V_t^\top - U_\ast \Sigma_\ast V_\ast^\top \rangle &\geq  \sigma_{\min}^2(\Sigma) - \sqrt{k-1}\big(2+\frac{2k^2 \delta_{2k}^2}{(1-\delta_{2k})^2}\big)\|\Sigma_\ast\|_2^2
\end{align}




Next we upper bound the $O(\eta^2)$ term in \eqref{3termsk}. We have
\begin{align}
    \lambda_{\max}(\hat{U}_{t+1}^\top S_t V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1}) &= \|V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1}\|_2^2 \nonumber \\
    &\leq \|V_{\ast,\perp}\|_2^2 \|S_t\|_2^2 \|\hat{U}_{t+1}\|_2^2 \nonumber \\
    &\leq \|S_t\|_2^2 \frac{(1 + (k-1)\delta_{2k})^2}{(1-\delta_{2k})^2}\|\Sigma_\ast\|_2^2 \label{boundUu}
\end{align}
where \eqref{boundUu} follows from \eqref{boundU}.
Next,
\begin{align}
    \|S_t\|_2^2 &= \| \mathcal{A}^\ast \mathcal{A}( \hat{U}_{t+1} V_t - U_\ast \Sigma_\ast V_\ast^\top)\|_2^2 \nonumber \\
    &\leq (1+ \sqrt{2k}\delta_{2k})\|\hat{U}_{t+1} V_t - U_\ast \Sigma_\ast V_\ast^\top\|_2^2 \nonumber \\
    &\leq k(1+ \sqrt{2k}\delta_{2k}) \frac{(1+\delta_{2k})^2}{(1-\delta_{2k})^2} \| \Sigma_\ast\|_2^2 \;\text{dist}^2(V_t, V_\ast) \label{dif1}
\end{align}
where \eqref{dif1} follows from \eqref{step1}. As a result we have
\begin{align}
    \lambda_{\max}(\hat{U}_{t+1}^\top S_t V_{\ast,\perp} V_{\ast,\perp}^\top S_t^\top \hat{U}_{t+1}) &\leq k(1+ \sqrt{2k}\delta_{2k}) \frac{(1+\delta_{2k})^2(1 + (k-1)\delta_{2k})^2}{(1-\delta_{2k})^4} \| \Sigma_\ast\|_2^2 \;\text{dist}^2(V_t, V_\ast)
\end{align}




\section{$\mathcal{A}$ satisfies RIP}

Recall that our measurements are $\mathbf{A}_{i,j} = e_{i} (x_{i}^j)^\top$, where $i \in [n]$ is an index over users and $j \in [m]$ is an index over the samples for each user.
% In particular,
% \begin{align}
%     f(\mathbf{W},\mathbf{\hat{B}}) = \sum_{i=1}^N \langle A_i, \hat{W}\hat{B}^\top \rangle^2
% \end{align}
% need to include $1/m$ factor above
% We assume that each $x_{j_i}^{(h_i)}$ is sub-gaussian with each element being iid with mean 0 and variance 1. For any rank-$k$ matrix $S \in \mathbb{R}^{n\times d}$, we have
% \begin{align}
%     \mathcal{A}(S) &= \sum_{i =1}^N \langle e_{j_i} x_{j_i}^{(h_i)^\top}, S \rangle^2 = \sum_{i =1}^N \langle x_{j_i}, s_{j_i} \rangle^2 \nonumber \\
%     &= \sum_{i =1}^N \sum_{\ell =1}^d \sum_{\ell' =1}^d x_{j_i}(\ell) s_{j_i}(\ell)  x_{j_i}(\ell') s_{j_i}(\ell') \label{rip:sum}
% \end{align}
% where $s_{j_i}$ is the $j_i$-th row of $S$, and $x_{j_i}(\ell)$ is the $\ell$-th element of $x_i$. Note that \eqref{rip:sum} is the sum of sub-exponential random variables with mean
% \begin{align}
%     \mathbb{E}[\sum_{i =1}^N \sum_{\ell =1}^d \sum_{\ell' =1}^d x_{j_i}(\ell) s_{j_i}(\ell)  x_{j_i}(\ell') s_{j_i}(\ell')] &= \sum_{i =1}^N \sum_{\ell =1}^d  s_{j_i}(\ell)^2  \\
%     &= m \|S\|_F^2
% \end{align}
% where $m$ is the number of samples per user. variance must be 1/m
% Note: of course it satisfies RIP by decomposing per user
% We can decompose the operator $\mathcal{A}$ into the per-user operators ${A}_i \in \mathbb{R}^{m \times d}$.
% % \begin{align}
% %     \mathcal{A}_i(z) &= A_{i,j} z]_j
% % \end{align}
% We need to show that each $\mathcal{A}_i$ satisfies RIP.
% Each $z$ of interest can be written as $B u$ for a universal $B \in \mathbb{O}^{d \times k}$ and some $u \in \mathbb{R}^{k}$. We need $\|A_i z\|_2^2 \leq (1+\delta)\|\mathbf{z}\|_2^2$. We have
% \begin{align}
%     \|{A}_i z\|_2^2 &= \sum_{j=1}^m ( \sum_{\ell =1}^d a_{i,j,\ell} \langle v_\ell, u \rangle)^2 \nonumber \\
%     &= 
% \end{align}
% we have that each operator per user is RIP if m > d 
% so in total would need nd samples
% where does k come in?
% centralized setting, full gaussian measurements: would need (n+d)k samples
% 

{\color{red} \textbf{OLD PROOF:} (see new proof below)}

Let the data matrix for user $i$ be denoted as 
\begin{align}
    \mathbf{X}_i \coloneqq \begin{bmatrix} (\mathbf{x}_i^1)^\top \\
    \vdots \\
    (\mathbf{x}_i^m)^\top
    \end{bmatrix} \in \mathbb{R}^{m \times d}
\end{align}
Assume that each element of each data point is sub-gaussian with mean 0 and variance $\frac{1}{m}$. We can assume the variance decays with $\frac{1}{m}$ by moving the $\frac{1}{m}$ factor in the objective inside of the 2-norm, thus multiplying the data by $\frac{1}{\sqrt{m}}$.

Note that any $n \times d$, rank-$k$ matrix $\mathbf{S}$ can be written as $\mathbf{S} = \mathbf{WB}^\top$ for some $\mathbf{W} \in \mathbb{R}^{n \times k}$ and $\mathbf{\hat{B}} \in \mathbb{R}^{d \times k}$. We have
\begin{align}
    \|\mathcal{A}(\mathbf{S})\|_2^2 = \sum_{i =1}^n \| \mathbf{X}_i \mathbf{\hat{B}} \mathbf{w}_i \|_2^2 = \sum_{i =1}^n \sum_{j =1}^m \langle \mathbf{x}_i^j, \mathbf{\hat{B}} \mathbf{w}_i \rangle^2
\end{align}
where $\mathbf{w}_i^\top$ is the $i$-th row of $\mathbf{W}$. Let $\mathbf{u}_i =  \mathbf{\hat{B}} \mathbf{w}_i$ for all $i$, and let $\gamma_{i,j} = \langle \mathbf{x}_i^j, \mathbf{\hat{B}} \mathbf{w}_i \rangle^2$ for all $i,j$. Then the $\gamma_{i,j}$'s are independent because the $\mathbf{x}_i^j$'s are independent and the $\mathbf{u}_i$'s are fixed. Also, $\mathbb{E}[\gamma_{i,j}] = \frac{1}{m}\|\mathbf{u}_i\|_2^2$.
%(\textcolor{red}{I think you can assume that data points have unit norm}).
% Note that each $\gamma_{i,j}$ is the square of a sum of sub-gaussian random variables with sub-gaussian norm $O(\frac{1}{m} z_{i,l})$
To understand the tail properties of each $\gamma_{i,j}$, note that
\begin{align}
    \gamma_{i,j} &= \left(\sum_{l=1}^d x_{i,l}^j z_{i,l} \right)^2
\end{align}
where $x_{i,l}^j$ (respectively $z_{i,l}$) is the $l$-th element of the vector ${x}_{i,l}^j$ (respectively $z_{i,l}$). Each ${x}_{i,l}^j z_{i,l}$ is sub-gaussian with variance $\frac{z_{i,l}^2}{m}$, their sum is sub-gaussian with variance $\frac{\|\mathbf{z}_{i}\|_2^2}{m}$. Thus $\gamma_{i,j}$ is sub-exponential with sub-exponential norm $$\| \gamma_{i,j}\|_{\phi_1} = \|\sum_{l=1}^d x_{i,l}^j z_{i,l}\|_{\phi_2}^2 = \frac{C\|\mathbf{z}_{i}\|_2^2}{m},$$ where $\|\cdot\|_{\phi_1}$ denotes the sub-exponential norm and $\|\cdot\|_{\phi_2}$ denotes the sub-gaussian norm, and $C$ is an absolute constant. 
% Next, note that 
% $\sum_{l=1}^d x_{j,l}^i z_{i,l}$ is sub-gaussian with mean zero and norm $\sqrt{C\|\mathbf{z}_i\|_2^2/m}$ for some absolute constant $C$. Then we have
% \begin{align}
%     \| \gamma_{i,j}\|_{\phi_1}\leq \|\sum_{l=1}^d x_{j,l}^i z_{i,l}\|_{\phi_2}^2 &\leq \frac{C \|\mathbf{z}_{i}\|^2_2}{nm} 
% \end{align}
% Further, by Proposition 2.6.1 in Bershynin, 
% we have
% \begin{align}
%     \|\sum_{l=1}^d x_{j,l}^i z_{i,l}\|_{\phi_2}^2 &\leq C' \sum_{l=1}^d \|x_{j,l}^i z_{i,l}\|_{\phi_2}^2 = \frac{C}{m^2} \|\mathbf{z}_{i}\|^2
% \end{align}
% where $C$ and $C'$ are absolute constants. Thus the sub-exponential norm of $\gamma_{i,j}$ is at most $\frac{C}{m^2} \|\mathbf{z}_{i}\|^2_2$.
Now we have that for any $\mathbf{S} = \mathbf{WB}^\top \in \mathbb{R}^{n\times d}$ with $\mathbf{W} \in \mathbb{R}^{n \times k}$ and $\mathbf{{B}} \in \mathbb{R}^{d \times k}$ such that $\|\mathbf{S}\|_F = 1$,
\begin{align}
    \mathbb{P}(|\|\mathcal{A}(\mathbf{S})\|_F^2 - \|\mathbf{S}\|_F^2| \geq \delta_{k} \|\mathbf{S}\|_F^2) &=   \mathbb{P}(|\sum_{i=1}^n \sum_{j=1}^m (\gamma_{i,j} - \frac{1}{m}\|\mathbf{z}_i\|_2^2)| \geq \delta_{k} \sum_{i=1}^n \|\mathbf{z}_i\|_2^2 ) \nonumber \\
    % &\leq \mathbb{P}\left(\bigcup_{i=1}^n |\sum_{j=1}^m (\gamma_{i,j} - \frac{1}{m}\|\mathbf{z}_i\|_2^2)| \geq \delta_{k} \|\mathbf{z}_i\|_2^2 \right) \nonumber \\
    % &\leq \sum_{i=1}^n \mathbb{P}\left(|\sum_{j=1}^m (\gamma_{i,j} - \frac{1}{m}\|\mathbf{z}_i\|_2^2)| \geq \delta_{k} \|\mathbf{z}_i\|_2^2 \right) \nonumber \\
    % &\leq \sum_{i=1}^n 2 \exp\left({-c_1  \min(\frac{ \delta_{k}^2}{\sum_{j=1}^m \frac{\|\mathbf{z}_{i}\|^4_2}{m^2} } \|\mathbf{z}_i\|_2^4 , \frac{\delta_{k}}{( \frac{\|\mathbf{z}_{i}\|^2_2}{m}) }  \|\mathbf{z}_i\|_2^2) }\right) \nonumber \\
    % &\leq \sum_{i=1}^n 2 \exp\left({-c_1 m\delta_{k} \min({ \delta_{k}}{ } , 1 ) }\right) \nonumber \\
    % &\leq \sum_{i=1}^n 2 \exp\left({-c_1 m\delta_{k}^2}\right) \nonumber \\
    % &= 2n \exp\left({-c_1 m\delta_{k}^2}\right)
    % &\leq  2\mathbb{P}(\sum_{i=1}^n \sum_{j=1}^m \gamma_{i,j} -  \geq (1+\delta_{k} )\|S\|_F^2+\|S\|_F^2) \nonumber \\
    % &=   \mathbb{P}(|\frac{1}{nm}\sum_{i=1}^n \sum_{j=1}^m (\gamma_{i,j} - \frac{1}{m}\|\mathbf{z}_i\|_2^2)| \geq \frac{\delta_{k}}{nm} \sum_{i=1}^n \|\mathbf{z}_i\|_2^2 ) \nonumber \\
    &\leq   2 \exp\left({-c_1  \min(\frac{ \delta_{k}^2}{\sum_{i=1}^n \sum_{j=1}^m \frac{\|\mathbf{z}_{i}\|^4_2}{m^2} } (\sum_{i=1}^n \|\mathbf{z}_i\|_2^2)^2 , \frac{\delta_{k}}{( \frac{\|\mathbf{z}_{i^\ast}\|^2_2}{m}) } \sum_{i=1}^n \|\mathbf{z}_i\|_2^2) }\right)  \\
    &= 2 \exp\left({-c_1 m\delta_k \min(\frac{ \delta_{k}}{\sum_{i=1}^n {\|\mathbf{z}_{i}\|^4_2} } , \frac{1}{ {\|\mathbf{z}_{i^\ast}\|^2_2} }) }\right)  \\
    &\leq 2 \exp\left(-c_1 m\delta_k^2 \right) 
    % &=  2 \exp\left({-c  \min(\frac{m^3 \delta_{k}^2}{\sum_{i=1}^n {\|\mathbf{z}_{i}\|^4_2} } (\sum_{i=1}^n \|\mathbf{z}_i\|_2^2)^2 , \frac{\delta_{k}}{( \frac{\|\mathbf{z}_{i^\ast}\|^2_2}{m^2}) } (\sum_{i=1}^n \|\mathbf{z}_i\|_2^2) }\right) \nonumber \\
    % &=  2 \exp\left({-c_1 nm \min(\frac{ \delta_{k}^2}{\sum_{i=1}^n {\|\mathbf{z}_{i}\|^4_2} }, \frac{{m^2}\delta_{k}}{( {\|\mathbf{z}_{i^\ast}\|^4_2}) } \sum_{i=1}^n \|\mathbf{z}_i\|_2^2 })\right) \nonumber  \\
    % &= 2 \exp\left({-c_1  \min(\frac{m^3 \delta_{k}^2}{\sum_{i=1}^n {\|\mathbf{z}_{i}\|^8_2} }, \frac{{m^2}\delta_{k}}{( {\|\mathbf{z}_{i^\ast}\|^4_2}) } })\right) \nonumber \\
    % &\leq 2 \exp\left({-c_1  \min({m^3 \delta_{k}^2}, {{m^2}\delta_{k}} })\right) \nonumber \\
    % &= 2 \exp\left({-c_1 m \min({m^2 \delta_{k}^2}, {{m}\delta_{k}} })\right) \nonumber
    % &\leq  2 \exp\left({-c  \min({m^3 \delta_{k}^2}, \frac{\delta_{k}}{( \frac{\|\mathbf{z}_{i^\ast}\|^2_2}{m^2}) } (\sum_{i=1}^n \|\mathbf{z}_i\|_2^2) }\right) \nonumber \\
    % &= 2 \exp\left({-c nm^2 \min(\frac{m \delta_{k}^2}{n^2 {\|\mathbf{z}_{i^\ast}\|^4_2} } (\sum_{i=1}^n \|\mathbf{z}_i\|_2^2)^2 , \frac{\delta_{k}}{n  {\|\mathbf{z}_{i^\ast}\|^2_2}} \sum_{i=1}^n \|\mathbf{z}_i\|_2^2 }\right) \nonumber \\
    % &\leq 2 \exp\left({-c nm^2 \min({m \delta_{k}^2}, {\delta_{k}} })\right) \nonumber \\
    % &= 
\end{align}
where we have used Bernstein's inequality, and $\mathbf{z}_{i^\ast}$ have the maximum 2-norm among the $\mathbf{z}_i$'s.

\textbf{Remark:} we really need $e^{-mn\delta_{2k}^2}$. but consider the case where all the $\mathbf{z}_i$'s are zero besides one $\mathbf{z}_{i^\ast}$, which has norm 1. This corresponds to a matrix $\mathbf{S}$ of rank less than $k$ increasing $n$ does not and should not help us with concentration, i.e. we can only expect $e^{-m\delta_{2k}^2}$ in the RHS. So we need some assumption about the norms of the $z_i$'s, but this restricts the class of matrices for which the RIP applies. In our case, we need to to apply to the difference of two matrices (e.g. $\mathbf{W}_{t+1}\mathbf{\hat{B}}_{t}^\top - \mathbf{M}_\ast$)
%, and I don't think we can say anything about the norms of their columns

{\color{blue}\textbf{Remark 12/21:}} We should be able to say that $\mathbf{W}_{t+1}\mathbf{\hat{B}}_{t}^\top - \mathbf{M}_\ast$ has balanced row norms under the standard assumption that the optimal user parameters are normalized. The issue is in bounding $|| \mathbf{F}||_2$ where $\mathbf{F}$ is defined as in \eqref{deff}. In order to bound $|| \mathbf{F}||_2$ we must bound $|| \mathbf{GD - C}||_2$. 
As in JNS14, we can show that
\begin{align}
|| \mathbf{GD - C}||_2 = \max_{\mathbf{U},\mathbf{V} \in \mathbb{R}^{n\times k}: \| \mathbf{U}\|_2 = \| \mathbf{V}\|_2= 1} \sum_{i=1}^n\sum_{j=1}^m \text{tr}( A_{i,j}^\top \mathbf{U}\mathbf{\hat{B}}_t^\top) \text{tr}( A_{i,j}^\top \mathbf{V} \mathbf{\hat{B}}_{\ast}^\top \mathbf{\hat{B}}_{t,\perp})
\end{align}
so we need RIP to apply to the matrix $\mathbf{U}\mathbf{\hat{B}}_t^\top + \mathbf{V} \mathbf{\hat{B}}_{\ast}^\top \mathbf{\hat{B}}_{t,\perp}$. But we cannot say anything about the row norms of this matrix because $\mathbf{U}$ and $\mathbf{V}$ are arbitrary.

% write $\mathcal{A}(\mathbf{WB}^\top) = \frac{1}{\sqrt{nm}} [\langle A_{ij}, WB^\top]_{i,j}$, sub-gaussian with variance 1 doesn't help

% we are trying to show the concentration of $n$ non-iid random variables. The error 


% no it only makes it worse... but column-wise there is still hope? no
%e^{(n+d)k} 
% Next, assume $\|\mathbf{z}_i\|_2^2 = \frac{1}{n}$ for all $i$. Then we have $\|S\|_F = 1$ and
% \begin{align}
%     \mathbb{P}(|\|\mathcal{A}(S)\|_F^2 - \|S\|_F^2| \geq \delta_{k} \|S\|_F^2)
%     &\leq  2 \exp\left({-c nm^2 \delta_k  \min({m \delta_{k}}, 1}\right) \nonumber 
% \end{align}

% where we have used the fact that $\sum_{i=1}^n \|\mathbf{z}_i\|_2^2 = \|S\|_F^2 = 1$. 
Next, by Theorem 2.3 in \cite{candes2010tight} we have that if $m \geq 2(n+d+1)k$, then
$\mathcal{A}$ satisfies RIP with isometry constant $\delta_k \leq \delta$ with probability at least $1 - 2 e^{-c_0 m}$, where 
\begin{align}
    c_0 &\coloneqq c_1 \delta^2 - \frac{\log(36 \sqrt{2}/\delta)}{2}
\end{align}
In order for $c_0 > 0$, we must have 
\begin{align}
    2 >  \frac{\log(36 \sqrt{2}/\delta)}{c_1\delta^2}
\end{align}
This implies, using the lower bound on $m$, that
\begin{align}
    m &\geq 2(n+d+1)k \nonumber \\
    &>\frac{\log(36 \sqrt{2}/\delta)}{c_1 \delta^2} (n+d+1)k
\end{align}
% Next assume that $m\delta \geq1$ (the other case can be shown to be impossible). Then we need 
% \begin{align}
%     m^2
%     &>\frac{\log(36 \sqrt{2}/\delta)}{c_1 \delta} (n+d+1)k
% \end{align}
Since we need $\delta_k \leq c_2/k$ for some small constant $c_2$ for our convergence results, we effectively need
\begin{align}
    m &\geq c_4  (n+d)k^3 {\log(k)}.
\end{align}
Thus, we need $m \geq c_4  (n+d)k^3 {\log(k)}$ samples per user, for a total of $c_4 n(n+d)k^3 {\log(k)}$ samples.

but the number of samples per user should not grow with $n$...

% if each $z_i$ was constrained to have norm 1, we would be fine. but since its norms may vary, we have more n more degrees of freedom? thus more n hurts us


% For covering number $e^{(n+d)k}$, we need 
% $(n+d)k < nm^2 delta$

% thus for delta < k, we need $(n+d)k/(nk) < m^2 $ i.e. $(n+d)/n < m^2$ so more users helps. but... still not sure about covering number, and whether we can assume columns are normalized

% By Lemma 2.7.6 in Bershynin, we have that 

% Each $\gamma_{i,j}$ is sub-exponential with parameter $K = O(\frac{1}{m^2}(\sum_{\ell = 1}^d z_{i,\ell})^2)$.
% *** not sure . This means that their sub has parameter that is not square root... but i think this actually shouldnt matter
% \begin{align}
% \end{align}



% Bia Bernstein inequality and and e-net argument, we obtain that:
% \begin{align}
%     \mathbb{P}(|\|\mathcal{A}(S)\|_F^2 - \|S\|_F^2| \geq \delta_{k} \|S\|_F^2) &\leq  2\mathbb{P}(\sum_{i=1}^n \sum_{j=1}^m \gamma_{i,j} -  \geq (1+\delta_{k} )\|S\|_F^2+\|S\|_F^2) \nonumber \\
%     &\leq   e^{(n+d)k} e^{-\min()}
% \end{align}
% ***assuming covering number of d-by-n rank-k unit norm matrices is $O(e^{(n+d)k})$ 
% for now, for factors with normalized columns this makes sense, see Bershynin book (4.12)

% High-level argument: Based on Lemma 9.5 in ${http://www.princeton.edu/~yc5/ele520_math_data/lectures/compressed_sensing.pdf}$, each user needs $m \geq \frac{1}{\delta}\text{log}(d)$ samples to achieve $\delta_{k} \leq \delta$ for their data matrix. All of the local data matrices being RIP with parameter $\delta_{k}$ implies that the entire linear operator is RIP with parameter $\delta_{k}$, since the squared Frobenius norm is decomposable by columns. Since we need $\delta_{k} \leq 1/k$, we need $m \geq k^2 \text{log} (d)$ samples per user, for a total of $n k^2 \text{log} (d)$ samples.



% But this is not capturing the fact that more users should help, not hurt, with learning the representation. Need to think more about this.

%also fix lemma, square?
% new directions: 
% two-layer relu lift to infinite dims, but will need to remove log d dependence
% how do they avoid the log d  cost? no rip, but how do they show concentration
%compare vs baselines


%to do tonight: figure this out
% finish related works section of draft

% can we show 2.2 in candes?
% does it really make sense the more n helps? i dont think so because each user has to learn their local params. and in general case, you can decompse measurements by row, but doing this should not let you improve sample complexity
% why am i getting m^2?
%our case should reduce to the general case by concatenting for each j across all n users
% no it's not quite the same bc you have a sum of squares vs square of sum difference
% need to get rid of squared m and min
%how do they show concentration for gaussian - may be useful

{\color{blue} \textbf{NEW PROOF:}}

Let the data matrix for user $i$ be denoted as 
\begin{align}
    \mathbf{X}_i \coloneqq \begin{bmatrix} (\mathbf{x}_i^1)^\top \\
    \vdots \\
    (\mathbf{x}_i^m)^\top
    \end{bmatrix} \in \mathbb{R}^{m \times d}
\end{align}
Assume that each element of each data point is sub-gaussian with mean 0 and variance $\frac{1}{m}$. We can assume the variance decays with $\frac{1}{m}$ by moving the $\frac{1}{m}$ factor in the objective inside of the 2-norm, thus multiplying the data by $\frac{1}{\sqrt{m}}$.

Fix a $k \leq \min(n,d)$ and $0 \leq \delta < 1$. Let $\mathbf{S}$ denote an arbitrary matrix in $\mathbb{R}^{n \times d}$, and let $\mathcal{S}_k$ denote the set of matrices in $\mathbb{R}^{n \times d}$ with rank at most $k$.

Let $E$ be the event that $\mathcal{A}$ satisfies $k$-RIP with parameter $\delta$, i.e.
\begin{align}
    E \coloneqq \left\{ (1-\delta)\|\mathbf{S}\|_F^2 \leq \|\mathcal{A}(\mathbf{S})\|_2^2 \leq (1+\delta)\|\mathbf{S}\|_F^2 \; \forall \; \mathbf{S} \in \mathcal{S}_k \right\}
\end{align}

Note that any $\mathbf{S} \in \mathcal{S}_k$ can be written as $\mathbf{S} = \mathbf{W} \mathbf{\hat{B}}^\top$ where $\mathbf{W} \in \mathbb{R}^{n \times k}$ and $\mathbf{\hat{B}} \in \mathbb{R}^{d \times k}$ has orthonormal columns, for example by taking the SVD. 

Now, note that for any $\mathbf{S} = \mathbf{W} \mathbf{\hat{B}}^\top \in \mathcal{S}_k$, we have that 
\begin{align}
    \|\mathcal{A}(\mathbf{S})\|_2^2 = \sum_{i =1}^n \| \mathbf{X}_i \mathbf{\hat{B}} \mathbf{w}_i \|_2^2
\end{align}
% Bernstein:
% Let $t_i = \| \mathbf{X}_i \mathbf{\hat{B}} \mathbf{w}_i \|_2^2$
% \begin{align}
%     P( \frac{1}{n} \sum_{i=1}^n (t_i - \bar{t}_i) \geq h) \leq \exp( -c n \min ( \frac{h^2}{\sum_{i=1}^n K_i^2} , \frac{h}{K_{i*}} )  )  
% \end{align}
%(\delta \frac{1}{n}\sum_{i=1}^n \bar{t}_i)^2
where $\mathbf{w}_i^\top$ is the $i$-th row of $\mathbf{W}$. Pick any $i$. Note that $\mathbf{w}_i$ is a $k$-dimensional vector, and $\mathbf{\hat{B}}$ is an orthogonal basis of a $k$-dimensional subspace of $\mathbb{R}^d$. Thus the vector $\mathbf{\hat{B}} \mathbf{w_i}$ is sparse in the basis $\mathbf{\hat{B}}$, so we can use can use compressed sensing results to control $\| \mathbf{X}_i \mathbf{\hat{B}} \mathbf{w}_i \|_2^2$, noting that $\mathbf{X}_i$ is sufficiently isometric. In particular, for fixed orthonormal basis $\mathbf{\hat{B}} \in \mathbb{R}^{d \times k}$, define the events $E_1(\mathbf{\hat{B}}), \dots, E_n(\mathbf{\hat{B}})$ as follows:
\begin{align}
E_i(\mathbf{\hat{B}}) \coloneqq \left\{ (1-\delta)\|\mathbf{\hat{B}} \mathbf{w}_i\|_2^2 \leq \|\mathbf{X}_i \mathbf{\hat{B}} \mathbf{w}_i \|_2^2 \leq (1+\delta)\|\mathbf{\hat{B}} \mathbf{w}_i\|_2^2 \; \forall \; \mathbf{w}_i \in \mathbb{R}^k \right\}
\end{align}
for all $i \in [n]$. By Theorem 5.2 in \cite{baraniuk2008simple} and the sub-gaussian construction of $\mathbf{X}_i$, we have that as long as $m \geq c_1 k \log(d/k)$, we have 
\begin{align}
    \mathbb{P}(E_i(\mathbf{\hat{B}})) \geq 1-e^{-c_2 m}
\end{align}
Now, let $\mathcal{O}^{d \times k}$ denote the set of matrices in $\mathbb{R}^{d\times k}$ with orthogonal columns. Notice that
\begin{align}
    \bigcap_{\mathbf{\hat{B}} \in \mathcal{O}^{d \times k}} \bigcap_{i=1}^n E_i(\mathbf{\hat{B}}) \subset E \label{subset}
\end{align}
Next, we can construct an $\epsilon$-net of $\mathcal{O}^{d \times k}$ with cardinality $e^{c_3 dk}$ for some constant $c_1$ depending only on $\epsilon$. Let ${A}^\mathbf{c}$ denote the complement of the event $A$. By \eqref{subset} and a union bound, we have
\begin{align}
    \mathbb{P}(E) &\geq \mathbb{P}\left(\bigcap_{\mathbf{\hat{B}} \in \mathcal{O}^{d \times k}} \bigcap_{i=1}^n E_i(\mathbf{\hat{B}})\right) \nonumber \\
    &= 1 - \mathbb{P}\left(\bigcup_{\mathbf{\hat{B}} \in \mathcal{O}^{d \times k}} \bigcup_{i=1}^n E_i(\mathbf{\hat{B}})^\mathbf{c}\right) \nonumber \\
    &\geq 1 - e^{c_3 dk} \sup_{\mathbf{\hat{B}} \in \mathcal{O}^{d \times k}} \left( \sum_{i=1}^n \mathbb{P}( E_i(\mathbf{\hat{B}})^\mathbf{c})\right) \nonumber \\
    &\geq 1 - e^{c_3 dk} \sum_{i=1}^n e^{-c_2 m} \nonumber \\
    &= 1 - \exp({-(c_2m - c_3dk - \log n)})
\end{align}
Thus we have that if $m \geq c_1 k \log(d/k) + 2(c_3 dk + \log n)$, then 
\begin{align}
    \mathbb{P}(E) &\geq 1 - \exp({-c_2m/2})
\end{align}
The constant $c_1$ hides $1/\delta^2$, so we must have $m \geq c_1' \frac{1}{\delta^2} k \log(d/k) + 2(c_3 dk + \log n)$, i.e. $m = \Omega(dk + \frac{1}{\delta^2} k \log(nd/k))$. Since we need $\delta_k \leq 1/(k\kappa^2)$ (where $\kappa = \frac{\sigma_{\max}(\mathbf{\Sigma_\ast})}{\sigma_{\min}(\mathbf{\Sigma_\ast})}$), this means $m \geq O(dk + k^3 \kappa^4 \log(nd/k))$ in order for $\mathcal{A}$ to satisfy $k$-RIP with probability at least $1 - e^{-\Omega(m)}$. Thus, we need a total of 
\begin{align}
    nm \geq O(ndk + nk^3 \kappa^4 \log(nd/k))
\end{align}
samples.


% \textbf{Remarks}. The $d$ factor I think is unavoidable. Even in the Lee and Jin papers, they need $O(d)$ samples for training. For fixed basis we don't need $d$, but since we need RIP to hold for $\mathcal{A}$ for all rank-$k$ matrices, i.e. for all $k$-dimensional bases in $\mathbb{R}^d$, I think the $d$ is unavoidable.

% One remaining question is whether we can show that larger $n$ actually helps with learning the representation, as in the Lee and Jin papers.

The reason that we don't have concentration in $n$ right now is that only a constant fraction of the columns of the matrix may have non-trivial norm. We cannot show that the RIP inequality holds for all rank-$k$ matrices. But it should hold for all nice matrices in the sense that their column norms are balanced. If this is true, then we have concentration with $n$, and the number of samples we need per user is smaller for larger $n$. But, the question is, can we show that the matrices we need the RIP inequality for balanced? Is this akin to making the assumption that the users' vectors have norm 1 as in the Lee paper? But we need the inequality for the difference of two matrices, is the assumption sufficient to ensure that the columns of this difference are balanced?





\begin{lemma} \label{lem:cmax}
Suppose $\mathcal{A}$ satisfies $2k$-RIP with parameter $\delta_{2k}$. Then the following holds:
\begin{align}
    \|\mathbf{C}\|_2 \leq 1+\sqrt{k} \delta_{2k} 
\end{align}
\end{lemma}
\begin{proof}
{C}onsider any $\mathbf{u} \in \mathbb{R}^{nk}$ such that $\|\mathbf{u}\|_2=1$. Let 
\begin{align}
    \mathbf{u} =\left[\begin{matrix} \mathbf{u}_1\\\vdots\\\mathbf{u}_k\end{matrix}\right],
\end{align}  
where each $\mathbf{u}_p \in \mathbb{R}^{n}$. Denote $\mathbf{U} = [\mathbf{u}_1,\dots, \mathbf{u}_k] \in \mathbb{R}^{n \times k}$, i.e. $\mathbf{u} = \text{vec}(\mathbf{U})$. Similarly, let $\mathbf{z} = \mathbf{C}\mathbf{u}$ and denote $\mathbf{Z} =  [\mathbf{z}_1,\dots, \mathbf{z}_k]$. Then we have
\begin{align}
     \mathbf{u}^\top \mathbf{C}^\top \mathbf{C} \mathbf{u} &= \sum_{p,q=1}^k \mathbf{u}_p^\top \mathbf{C}_{qp}^\top \mathbf{z}_q = \sum_{i=1}^N \sum_{p,q=1}^k \mathbf{u}_p^\top \mathbf{A}_{i,j} \mathbf{\hat{b}}_p^\ast (\mathbf{\hat{b}}_q^t)^\top \mathbf{A}_{i,j}^\top \mathbf{z}_q = \sum_{i=1}^N \left(\sum_{p=1}^k \mathbf{u}_p^\top \mathbf{A}_{i,j} \mathbf{\hat{b}}_p^\ast \right)\left(\sum_{q=1}^k(\mathbf{\hat{b}}_q^t)^\top \mathbf{A}_{i,j}^\top \mathbf{z}_q\right) \nonumber \\
    &= \sum_{i=1}^N \text{tr}
    (\mathbf{A}_{i,j}^\top \mathbf{U} \mathbf{\hat{B}}_\ast^\top )\text{tr}
    (\mathbf{A}_{i,j}^\top \mathbf{Z} \mathbf{\hat{B}}_t^\top ) \nonumber \\
    &= \langle \mathcal{A}(\mathbf{U} \mathbf{\hat{B}}_\ast^\top),  \mathcal{A}(\mathbf{Z} \mathbf{\hat{B}}_t^\top) \rangle \nonumber \\
    &\leq \langle \mathbf{U} \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{\hat{B}}_t^\top \rangle + \delta_{2k} \|\mathbf{U} \mathbf{\hat{B}}_\ast^\top\|_{F}\|\mathbf{Z} \mathbf{\hat{B}}_t^\top\|_{F} \label{cmin00} \\
    &\leq \langle \mathbf{U} \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{\hat{B}}_t^\top \rangle + \delta_{2k} \|\mathbf{U}\|_{F}\|\mathbf{Z}\|_{F}\nonumber \\
    &\leq \langle \mathbf{U} \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{\hat{B}}_t^\top \rangle + \delta_{2k} \sqrt{k} \|\mathbf{C}\|_2 \label{cmin000}
\end{align}
where \eqref{cmin00} follows from the RIP. Next, let $\mathbf{\Gamma}_t =\mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast$. We have
\begin{align}
    \langle \mathbf{U} \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{\hat{B}}_t^\top \rangle &= \text{tr}( \mathbf{U}^\top \mathbf{Z} \mathbf{\Gamma}_t) = \sum_{p=1}^k \mathbf{u}_p^\top \mathbf{Z} \mathbf{\gamma}^t_p  = \sum_{p=1}^k \sum_{q=1}^k \mathbf{u}_p^\top \mathbf{z}_q \gamma^t_{q,p}  \nonumber \\
    &= \sum_{p=1}^k \sum_{q=1}^k \mathbf{u}_p^\top \sum_{j=1}^k \mathbf{C}_{qj} \mathbf{u}_j \gamma^t_{q,p}  \nonumber \\
    % &= \sum_{p=1}^k \sum_{q=1}^k \sum_{j=1}^k \mathbf{u}_p^\top  \mathbf{C}_{qj} \mathbf{u}_j \gamma_{q,p}  \nonumber \\
    % &= \sum_{p=1}^k \sum_{q=1}^k \mathbf{u}_p^\top \sum_{j=1}^k \mathbf{C}_{qj} \mathbf{u}_j \gamma_{q,p}  \nonumber \\
    &= \sum_{i=1}^N \sum_{p=1}^k \sum_{q=1}^k \sum_{j=1}^k  \mathbf{u}_p^\top  \mathbf{A}_{i,j} \mathbf{\hat{b}}_q^t (\mathbf{\hat{b}}_j^\ast)^\top \mathbf{A}_{i,j}^\top \mathbf{u}_j \gamma_{q,p}^t  \nonumber \\
    &= \sum_{i=1}^N \sum_{p=1}^k  \sum_{j=1}^k  \mathbf{u}_p^\top  \mathbf{A}_{i,j}  \left( \sum_{q=1}^k \mathbf{\hat{b}}_q^t \gamma_{q,p}^t\right) (\mathbf{\hat{b}}_j^\ast)^\top \mathbf{A}_{i,j}^\top \mathbf{u}_j   \nonumber \\
    &= \sum_{i=1}^N \sum_{p=1}^k  \sum_{j=1}^k  \mathbf{u}_p^\top  \mathbf{A}_{i,j}  \left(  \mathbf{\hat{B}}_t \gamma_{p}\right) (\mathbf{\hat{b}}_j^\ast)^\top \mathbf{A}_{i,j}^\top \mathbf{u}_j   \nonumber \end{align}
    Now we can proceed as previously:
    \begin{align}
    \langle \mathbf{U} \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{\hat{B}}_t^\top \rangle &= \sum_{i=1}^N \left(\sum_{p=1}^k    \mathbf{u}_p^\top  \mathbf{A}_{i,j}  \left(  \mathbf{\hat{B}}_t \gamma_{p}^t \right)\right)\left( \sum_{j=1}^k (\mathbf{\hat{b}}_j^\ast)^\top \mathbf{A}_{i,j}^\top \mathbf{u}_j  \right) \nonumber \\
    &= \sum_{i=1}^N \text{tr}\left(\mathbf{A}_{i,j}^\top \mathbf{U} \left(\mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top \mathbf{\hat{B}}_\ast \right)^\top\right)\text{tr}(\mathbf{A}_{i,j}^\top \mathbf{U} \mathbf{\hat{B}}_\ast^\top ) \nonumber \\
    &= \langle \mathcal{A}(\mathbf{U} \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top),  \mathcal{A}(\mathbf{U} \mathbf{\hat{B}}_\ast^\top) \rangle \nonumber \\
    &\leq \langle \mathbf{U} \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top,  \mathbf{U} \mathbf{\hat{B}}_\ast^\top \rangle + \delta_{2k} \|\mathbf{U} \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top\|_F\|\mathbf{U} \mathbf{\hat{B}}_\ast^\top\|_F \nonumber \\
    &\leq \langle \mathbf{U} \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t ,  \mathbf{U} \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \rangle + \delta_{2k} \|\mathbf{U}\|_F^2 \|\mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top\|_2 \nonumber \\
    &\leq \|\mathbf{U} \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t\|_F^2 + \delta_{2k}\nonumber \\
    &\leq \|\mathbf{U} \|_F^2 + \delta_{2k}\nonumber \\
    &= 1 +\delta_{2k}
\end{align}
{C}ombining this with \eqref{cmin000} yields
\begin{align}
     \mathbf{u}^\top \mathbf{C}^\top \mathbf{C} \mathbf{u} 
    &\leq 1+\delta_{2k} + \delta_{2k} \sqrt{k} \|\mathbf{C}\|_2 \label{cmin20}
\end{align}
Since $$\|\mathbf{C}\|_2^2 = \lambda_{\max}(\mathbf{C}^\top \mathbf{C}) = \min_{\mathbf{u}: \|\mathbf{u}\|_2 = 1}\mathbf{u}^\top \mathbf{C}^\top \mathbf{C} \mathbf{u}$$ and \eqref{cmin20} holds for any $\mathbf{u}\in \mathbb{R}^{nk}: \|\mathbf{u}\|_2 = 1$, we have 
\begin{align}
    \|\mathbf{C}\|_2^2 \leq 1+\delta_{2k} + \delta_{2k} \sqrt{k} \|\mathbf{C}\|_2.
\end{align}
By the quadratic formula, we have
\begin{align}
    \|\mathbf{C}\|_2 \leq \frac{1}{2} \left( \delta_{2k} \sqrt{k} + \sqrt{\delta_{2k}^2 k + 4\delta_{2k} + 4}   \right) \leq 1+\sqrt{k} \delta_{2k} 
\end{align}
\end{proof}

\begin{comment}
\begin{lemma} \label{lem:cmin}
Suppose $\mathcal{A}$ satisfies $2k$-RIP with parameter $\delta_{2k}$. Then the following holds:
\begin{align}
    \sigma_{\min}^2(\mathbf{C}) \geq 1 - \text{dist}^2(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_{\ast}) - \delta_{2k}(1 + \sqrt{k} + k\delta_{2k}) 
\end{align}
\end{lemma}

\begin{proof}
As in Lemma \ref{lem:cmax}, consider any $\mathbf{u}\in \mathbb{R}^{nk}$ such that $\|\mathbf{u}\|_2=1$. Let 
\begin{align}
    \mathbf{u} =\left[\begin{matrix} \mathbf{u}_1\\\vdots\\\mathbf{u}_k\end{matrix}\right],
\end{align}  
where each $\mathbf{u}_p \in \mathbb{R}^{n}$. Denote $\mathbf{U} = [\mathbf{u}_1,\dots, \mathbf{u}_k] \in \mathbb{R}^{n \times k}$, i.e. $\mathbf{u}= vec(\mathbf{U})$. Similarly, let $z = \mathbf{C}w$ and denote $\mathbf{Z} =  [\mathbf{z}_1,\dots, \mathbf{z}_k]$. Using similar analysis as in Lemma \ref{lem:cmax}, we have
\begin{align}
    \mathbf{u}^\top \mathbf{C}^\top \mathbf{C} w 
    &= \langle \mathcal{A}(W \mathbf{\hat{B}}_\ast^\top),  \mathcal{A}(\mathbf{Z} \mathbf{\hat{B}}_t^\top) \rangle \nonumber \\
    &\geq \langle W \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{B}_t^\top \rangle - \delta_{2k} \|W \mathbf{\hat{B}}_\ast^\top\|_F\|\mathbf{Z} \mathbf{B}_t^\top\|_F \label{cmin0} \\
    &\geq \langle W \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{B}_t^\top \rangle - \delta_{2k} \|W\|_F\|\mathbf{Z}\|_F\nonumber \\
    &\geq \langle W \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{B}_t^\top \rangle - \delta_{2k} \sqrt{k} \|\mathbf{C}\|_2 \nonumber \\
    &\geq \langle W \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{B}_t^\top \rangle - \delta_{2k} \sqrt{k} (1+\sqrt{k} \delta_{2k}) \label{cmin1}
\end{align}
where \eqref{cmin0} follows from the RIP and \eqref{cmin1} follows by Lemma \ref{lem:cmax}.
Next, let $\mathbf{\Gamma}_t =\mathbf{B}_t^\top \mathbf{\hat{B}}_\ast$. Again proceeding as in Lemma \ref{lem:cmax}, we have
\begin{align}
    \langle W \mathbf{\hat{B}}_\ast^\top,  \mathbf{Z} \mathbf{B}_t^\top \rangle 
    &= \langle \mathcal{A}(W \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t \mathbf{B}_t^\top),  \mathcal{A}(W \mathbf{\hat{B}}_\ast^\top) \rangle \nonumber \\
    &\geq \langle W \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t \mathbf{B}_t^\top,  W \mathbf{\hat{B}}_\ast^\top \rangle - \delta_{2k} \|W \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t \mathbf{B}_t^\top\|_F\|W \mathbf{\hat{B}}_\ast^\top\|_F \nonumber \\
    &\geq \langle W \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t ,  W \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t \rangle - \delta_{2k} \|W\|_F^2 \|\mathbf{B}_\ast^\top \mathbf{B}_t \mathbf{B}_t^\top\|_2 \nonumber \\
    &\geq \|W \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t\|_F^2 - \delta_{2k}\nonumber \\
    &\geq \sigma_{\min}^2(\mathbf{B}_\ast^\top \mathbf{B}_t) \|W \|_F^2 - \delta_{2k} \nonumber \\
    &=\sigma_{\min}^2((I - \mathbf{\hat{B}}_{\ast,\perp} \mathbf{\hat{B}}_{\ast,\perp}^\top) \mathbf{B}_t) - \delta_{2k} \nonumber \\
    &=\lambda_{\min}(\mathbf{B}_t^\top(I - \mathbf{\hat{B}}_{\ast,\perp} \mathbf{\hat{B}}_{\ast,\perp}^\top) \mathbf{B}_t) - \delta_{2k} \nonumber \\
    &\geq 1 - \|\mathbf{\hat{B}}_{\ast,\perp}^\top) \mathbf{B}_t\|_2^2 - \delta_{2k}  \nonumber \\
    &= 1 - \text{dist}^2(\mathbf{B}_t, \mathbf{\hat{B}}_{\ast,\perp}) - \delta_{2k}
\end{align}
{C}ombining this with \eqref{cmin1}, we have 
\begin{align}
    \mathbf{u}^\top \mathbf{C}^\top \mathbf{C} w &\geq 1 - \text{dist}^2(\mathbf{B}_t, \mathbf{\hat{B}}_{\ast,\perp}) - \delta_{2k} -\delta_{2k} \sqrt{k} (1+\sqrt{k} \delta_{2k} ) \label{cmin2}
\end{align}
Since $$\sigma_{\min}^2(\mathbf{C}) = \lambda_{\min}(\mathbf{C}^\top \mathbf{C}) = \min_{\mathbf{u}: \|\mathbf{u}\|_2 = 1}\mathbf{u}^\top \mathbf{C}^\top \mathbf{C} w$$ and \eqref{cmin2} holds for any $\mathbf{u}\in \mathbb{R}^{nk}: \|\mathbf{u}\|_2 = 1$, we have 
\begin{align}
    \sigma_{\min}^2(\mathbf{C}) &\geq 1 - \text{dist}^2(\mathbf{B}_t, \mathbf{\hat{B}}_{\ast,\perp}) - \delta_{2k} -\delta_{2k} \sqrt{k} (1+\sqrt{k} \delta_{2k})  \nonumber \\
    &= 1 - \text{dist}^2(\mathbf{B}_t, \mathbf{\hat{B}}_{\ast,\perp}) - \delta_{2k}(1 + \sqrt{k} + k\delta_{2k}) 
\end{align}
completing the proof.
\end{proof}
\end{comment}




\section{Consequences of RIP}

We will repeatedly use the following result, which is a well-known consequence of the RIP.
\begin{lemma}[Candes 2008] \label{lem:rip1}
If $\mathcal{A}$ satisfies $2k$-RIP with parameter $\delta_{2k}$, then for any rank-$k$ matrices $\mathbf{X}$ and $\mathbf{Y}$ in $\mathbb{R}^{n\times d}$, then
\begin{align}
    \mid \langle \mathcal{A}(\mathbf{X}), \mathcal{A}(\mathbf{Y}) \rangle - \langle \mathbf{X}, \mathbf{Y} \rangle \mid \leq \delta_{2k} \|\mathbf{X}\|_F \|\mathbf{Y}\|_F
\end{align}
\end{lemma}
% Note that this result is tighter, by a factor of 3, than Lemma B.1 in JNS14. Anywhere JNS14 uses their Lemma B.1, we will replace it with Lemma \ref{lem:rip1} to obtain a tighter bound. 

We now show another useful consequence of the RIP.
\begin{lemma} \label{lem:rip2}
If $\mathcal{A}$ satisfies $2k$-RIP with parameter $\delta_{2k}$, then for any rank-$k$ matrices $\mathbf{X}\in\mathbb{R}^{n\times d}$, then
\begin{align}
   \|\mathcal{A}^\ast \mathcal{A}(\mathbf{X}) -  \mathbf{X}\|_2 \leq \delta_{2k} \|\mathbf{X}\|_F,
\end{align}
where $\mathcal{A}^\ast$ is the adjoint operator of $\mathcal{A}$.
\end{lemma}
\begin{proof}
% First note that by Cauchy-Schwarz:
% \begin{align}
%     \|\mathcal{A}^\ast \mathcal{A}(\mathbf{X}) -  \mathbf{X}\|_2 &= \|(\mathcal{A}^\ast \mathcal{A}-\mathbf{I}_n) \mathbf{X}\|_2 \nonumber \\
%     &\leq \|\mathcal{A}^\ast \mathcal{A}-\mathbf{I}_n \|_2 \| \mathbf{X}\|_2
% \end{align}
Let $\mathcal{I}: \mathbb{R}^{n\times d} \rightarrow \mathbb{R}^{n\times d}$ be the identity operator in $\mathbb{R}^{n\times d}$.
For ease of notation we will sometimes use $\mathbf{U} = (\mathcal{A}^\ast \mathcal{A} - \mathcal{I}) (\mathbf{X})$.
We have 
\begin{align}
    \|\mathcal{A}^\ast \mathcal{A}(\mathbf{X}) -  \mathbf{X}\|_2^2 &=\|(\mathcal{A}^\ast \mathcal{A}- \mathcal{I}) (\mathbf{X})\|_2^2  \nonumber \\
    &= \max_{\mathbf{v}:\|\mathbf{v}\|_2 = 1}  \mathbf{v}^\top \mathbf{U}^\top (\mathcal{A}^\ast \mathcal{A}- \mathcal{I}) (\mathbf{X}) \mathbf{v} \nonumber \\
    &= \max_{\mathbf{v}:\|\mathbf{v}\|_2 = 1}  \text{tr} ( \mathcal{A}^\ast \mathcal{A}(\mathbf{X}) \mathbf{v}\mathbf{v}^\top \mathbf{U}^\top) -  \text{tr}( \mathbf{X} \mathbf{v} \mathbf{v}^\top \mathbf{U}^\top) \nonumber \\
    &= \max_{\mathbf{v}:\|\mathbf{v}\|_2 = 1}  \langle \mathcal{A}( \mathbf{U} \mathbf{v}\mathbf{v}^\top),  \mathcal{A}(\mathbf{X}) \rangle - \langle   \mathbf{U} \mathbf{v} \mathbf{v}^\top , \mathbf{X} \rangle \nonumber \\
    &\leq \max_{\mathbf{v}:\|\mathbf{v}\|_2 = 1} \delta_{2k} \|\mathbf{X}\|_F \|\mathbf{U} \mathbf{v} \mathbf{v}^\top \|_F \label{rip22} \\
    &\leq \max_{\mathbf{v}:\|\mathbf{v}\|_2 = 1} \delta_{2k} \|\mathbf{X}\|_F \|\mathbf{U}\|_2 \|\mathbf{v} \mathbf{v}^\top \|_F \nonumber \\
    &= \delta_{2k} \|\mathbf{X}\|_F \|(\mathcal{A}^\ast \mathcal{A} - \mathcal{I}) (\mathbf{X})\|_2 \label{divide}
\end{align}
where \eqref{rip22} follows from Lemma \ref{lem:rip1}.
Dividing both sides of \eqref{divide} by $\|(\mathcal{A}^\ast \mathcal{A} - \mathcal{I}) \mathbf{X}\|_2$ completes the proof.
% \begin{align}
%     \|\mathcal{A}^\ast \mathcal{A}(\mathbf{X}) -  \mathbf{X}\|_2^2 &= \|\mathcal{A}^\ast \mathcal{A}(\mathbf{X}) -  \mathbf{X}\|_2^2 \sup_{\mathbf{Y} \in \mathbb{R}^{n \times d}: \|\mathbf{Y}\|_F = 1} \langle \mathcal{A}^\ast \mathcal{A}(\mathbf{X}) -  \mathbf{X}, \mathbf{Y} \rangle \nonumber \\
%     &= \sup_{\mathbf{Y} \in \mathbb{R}^{n \times d}: \|\mathbf{Y}\|_F = 1} \langle \mathcal{A}^\ast \mathcal{A}(\mathbf{X}), \mathbf{Y} \rangle  - \langle \mathbf{X}, \mathbf{Y} \rangle \nonumber \\
%     &= \sup_{\mathbf{Y} \in \mathbb{R}^{n \times d}: \|\mathbf{Y}\|_F = 1} \langle  \mathcal{A}(\mathbf{X}), \mathcal{A}(\mathbf{Y}) \rangle  - \langle \mathbf{X}, \mathbf{Y} \rangle \nonumber \\
%     &\leq \sup_{\mathbf{Y} \in \mathbb{R}^{n \times d}: \|\mathbf{Y}\|_F = 1} \delta_{2k} \|\mathbf{X}\|_F\| \mathbf{Y}\|_F  \label{rip22}\\
%     &= \delta_{2k} \|\mathbf{X}\|_F^2 \nonumber
% \end{align}
\end{proof}



\begin{lemma}\label{lem:qt}
The following holds 
\begin{align}
    \|\mathbf{{W}}_{t+1} \mathbf{\hat{B}}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top\|_F\leq \sqrt{k} \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \mathbf{\Sigma}_\ast\|_2 \;\text{dist}(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_\ast) 
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    \|\mathbf{{W}}_{t+1}  \mathbf{\hat{B}}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \|_{F}&\leq  \frac{1}{1-\delta_{2k}}\|\mathcal{A}(\mathbf{W}_{t+1}  \mathbf{\hat{B}}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top) \|_{F}\label{krip2} \\
    &\leq \frac{1}{1-\delta_{2k}}\|\mathcal{A}(\mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top) \|_{F}\label{lss} \\
    &\leq \frac{1+\delta_{2k}}{1-\delta_{2k}}\|\mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \|_{F}\label{krip3} \\
    &\leq \frac{1+\delta_{2k}}{1-\delta_{2k}} \|\mathbf{\hat{W}}_\ast\|_{F}\| \mathbf{\Sigma}_\ast\|_2 \| (\mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top - \mathbf{\hat{B}}_\ast^\top) \|_2 \label{cs1} \\
    &\leq \sqrt{k}\frac{1+\delta_{2k}}{1-\delta_{2k}} \| \mathbf{\Sigma}_\ast\|_2 \| \mathbf{\hat{B}}_\ast^\top (\mathbf{\hat{B}}_t \mathbf{\hat{B}}_t^\top - \mathbf{I}_d) \|_2 \label{rtk} \\
    % &= \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \mathbf{\Sigma}_\ast\|_2 \| \mathbf{\hat{B}}_\ast^\top (\mathbf{B}_t {B}_t^\top - I) \|_2 \nonumber \\
    &= \sqrt{k} \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \mathbf{\Sigma}_\ast\|_2 \;\text{dist}(\mathbf{\hat{B}}_t, \mathbf{\hat{B}}_\ast) \label{step1}
\end{align}
where \eqref{krip2} and \eqref{krip3} follow by $2k$-RIP, \eqref{lss} follows by the fact that $\mathbf{W}_{t+1}$ is the least squares solution, \eqref{cs1} follows by {C}auchy-Schwarz, \eqref{rtk} follows since $\|\mathbf{\hat{W}}_\ast\|_{F}\leq \sqrt{k} \|\mathbf{\hat{W}}_\ast\|_2$ = $\sqrt{k}$. 
\end{proof}



For any fixed $\mathbf{z} \in \mathbb{R}^n: \|\mathbf{z}\|_2=1 $, we have
\begin{align}
    \mathbf{z}^\top (\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast &= \sum_{i=1}^n z_i u_{\ast,i} H^i \nonumber \\
    &= \sum_{i=1}^n z_i u_{\ast,i} \sum_{j=1}^m  (\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle) \nonumber \\
    &\leq \sum_{i=1}^n \sum_{j=1}^m \frac{z_i \mu}{\sqrt{n}}   ( \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle)
\end{align}
by the incoherence of $\mathbf{u}_\ast$. Next, note that $\mathbf{z}^\top (\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast$ is the sum of $nm$ sub-exponential random variables with mean 0 and norm $O(1/(m \sqrt{n}))$. But the $\sqrt{n}$ is not strong enough for us since we must union bound over all $\mathcal{S}^n$.... we don't have the extra 1/rt(d) term because we cannot use the incoherence of v... so we must use higher-order concentration argument
----------------------------







% Now we deal with higher-order moments...

% We need to upper bound the sum of $nm^2$ random variables that are not independent, whose sum has mean $\frac{\mu^2}{m} \text{dist}(\mathbf{v},\mathbf{v}_\ast)$, and which have variance $1/(n^2 m^4)$.

% Non-independence is a problem but ignore it for now.

% The variance is sufficient. We need the truncation level to be $O(1/(nm^2))$, can we say this?
% \begin{align}
% \mathbb{P}( X_i > R) &\leq e^{-\sqrt{R}} \nonumber
% \end{align}
% according to lemma 29 in Jin, we need $R > (\log(nm^2/(\delta )))^2$. 
% but what do we need t to be? we need $t < \delta$. Thus we need
% $$\frac{nm^2 \delta }{(\log(nm^2/\delta))^2} \gg \log(d) \implies nm^2  \gg 
% \frac{\log(d) (\log(nm^2/\delta))^2}{\delta} $$

% Ok, now deal with non-independence: fix j. then the set of RV's {Xjj'}j' is independent. 

% P(Xj Yj < delta) > P(Yj < delta/Xj | Xj < rt(delta) ) P( Xj < rt(delta) )
% > P(Yj < delta/Xj | Xj < rt(delta) ) (1-e2)
% > P(Yj < rt(delta) ) (1-e2)
% then substitute delta=delta/m
% We have

% Let $E_j$ be the event:
% $$ E_j \coloneqq \{ \frac{1}{nm}\sum_{i=1}^n \sum_{j'=1}^m X_{i,j} X_{i,j'} \geq \delta \}  $$
% We have
% \begin{align}
%     \mathbb{P}(\frac{1}{nm^2} \sum_{i=1}^n \sum_{j=1}^m \sum_{j'=1}^m X_{i,j} X_{i,j'} \geq \delta) &=  \mathbb{P}(\frac{1}{m}\sum_{j=1}^m ( \frac{1}{nm}\sum_{i=1}^n  \sum_{j'=1}^m X_{i,j} X_{i,j'}) \geq \delta) \nonumber \\
%     &\leq \mathbb{P}(\cup_{j=1}^m E_j)\nonumber \\
%     &\leq \sum_{j=1}^m \mathbb{P}(E_j)
% \end{align}
% So we just need a bound on the $E_j$. With probability at least $1 - e^{-c \delta^{1/4}}$ we have that  $X_{i,j} $
% We have
% \begin{align}
%     \mathbb{P}(E_j) &= \mathbb{P}( \frac{1}{nm}\sum_{i=1}^n \sum_{j'=1}^m X_{i,j} X_{i,j'} \geq \delta ) \nonumber \\
% \end{align}

% (see above...)






% we get the 1/rt(n) factor from incoherence of u* and the 1/m factor from subgaussian. but really we need the 1/m factor to be 1/rt(n). in sujay's paper the 1/m factor is 1/rt(d) by incoherence of v. does this mean that they need m > rt(d)? they need pd > 1, so no they do not need m > rt(d). 

%note: instead of this higher order moments stuff, we could instead union bound over Sn, because we do have a 1/n factor. either will work, and will only require m > f(k). but i think with clipping we can actually get m > f(k)/n. but do we even need the incoherence of u* in this proof? we need it for the union bound. but in the proof without union bound, do we need it?? no, we don't even need it for the union bound; we can take max over n, then union bound over n, obtain m > log n as previously. but maybe things do not break down like this for k > 1, i.e. H is not block diagonal? it is block diagonal but the blocks are n by n, not k by k, so this is why we need the 1/n. no that is false, the matrices are k by k, the proof is inconsistent. note they still do maximize over n later. but why need incoherence? maybe we need should we be seeing a rt(d) factor somewhere as in lemma C.4? yes after cancelling p's that's why they need incoherence... but where does the rt(d) i.e. rt(m) factor come from? somehow the incoherence of u* must be necessary for us....






% but still, where does their dimension-dependence come in? it is because there is no nd factor in the denominator of p. but why not? for us m = pd, and there is a 1/min(n,d) factor in p, so their analysis gives us m = d/min(n,d), which is close enough to what we want..... and the 1/min(n,d) factor comes from incoherence ..... but right now we are getting away with p<Omega(1/nd), we should really only be able to say p<Omega(1/min(n,d)) .... 

% p > 1/d --> pd > 1 --> m > d/d 

% p > 1 would be a problem

% they get the 1/d by incoherence, we get it automatically because v is norm 1 and we are taking a subgaussian measurement, not just observing one entry

% and likewise for the second result

% so the m > d/min(n,d) is implicit. but if n << d, we should see it...

% p > 1/n --> pd > d/n --> m > d/n 

% but this is not what we show. we actually show 
% p > 1/d because the incoherence/subgaussian measurement is over a d-dimensional vector. so implicitly, we actually have m > d/d.

% if we needed to show the analogous inequalities for U,  we would implicitly need m > d/n

% but we do not need a descent result in U

% ok! i think i understand it now

% when they minimize V, they require incoherence of V* and Ut. thus when they minimize U, they would require incoherence of U* and Vt. In our case, we get away without requiring incoherence of Vt because we have `half' subgaussian measurements. We only require incoherence of U*. Also, we do not minimize V, so we do not require incoherence of V* and Ut from that step. The only remaining question is what do we require to bound (2.)

% We have that for any $\mathbf{z} \in \mathbb{R}^n:\|z\|_2=1$, $\mathbf{z}^\top \mathbf{H} \hat{\mathbf{v}}$ is sum of $n$ sub-exponential random variables with norm $O(1/(mn))$ and mean 0 (the 1/n factor is due to incoherence of the rows of $\mathbf{U}_\ast$, elements of $\mathbf{u}_\ast$). 




% In summary, we need (analogous to Lemma C.4 in Sujay's paper) the bound
% \begin{align}
%     \| (\mathbf{GD} - \mathbf{C})\hat{\mathbf{u}}_\ast\|_2^2 \leq \delta_2 \text{dist}(\mathbf{v}, \mathbf{v}_*)
% \end{align}
% to hold with high probability over the samples $\mathbf{x}_i^j$,
% where $\mathbf{GD} - \mathbf{C} = \mathbf{H}$ is a diagonal matrix in $\mathbb{R}^{n\times n}$ whose $i$-th diagonal entry is:
% \begin{align}
%     H^i 
%     &= \sum_{j=1}^m  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle 
% \end{align}
% There are two approaches:
% \begin{enumerate}
% \item Variational approach (as in Sujay's paper):
%  Obtain
%  \begin{align}
%     \mathbf{z} (\mathbf{GD} - \mathbf{C})\hat{\mathbf{u}}_\ast &\leq \delta_2 \text{dist}(\mathbf{v}, \mathbf{v}_*)
%  \end{align}
%  for all $\mathbf{z}\in \mathbb{R}^n: \|\mathbf{z}\|_2 = 1$ with high probability. We have:
%  \begin{align}
%     \mathbf{z}^\top (\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast &= \sum_{i=1}^n z_i \hat{u}_{\ast,i} H^i \nonumber \\
%     &= \sum_{i=1}^n z_i \hat{u}_{\ast,i} \sum_{j=1}^m  (\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle) \nonumber \\
%     &\leq \sum_{i=1}^n \sum_{j=1}^m \frac{z_i \mu}{\sqrt{n}}   ( \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle)
% \end{align}
% by the incoherence of $\hat{\mathbf{u}}_\ast$ ($\mu$ is the incoherence parameter, a constant) (I believe the incoherence of $\hat{\mathbf{u}}_\ast$ is a reasonable assumption, we can discuss this). Note that $\mathbf{z}^\top (\mathbf{GD} - \mathbf{C})\hat{\mathbf{u}}_\ast$ is the sum of $nm$ sub-exponential random variables with mean 0 and norm $O(1/(m \sqrt{n}))$. But the $\sqrt{n}$ is not strong enough for us since we must union bound over all $\mathcal{S}^n$.... in Sujay's paper, they upper bound each $( \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle)$ term with an $O(1/\sqrt{d})$ factor by the incoherence of $\mathbf{v}$, but we cannot use this.

  % \|\hat{\mathbf{B}}^\top\|_2^2\; \mathbb{E}[\|\mathbf{\Pi}_i\|_2^2]\; \|(\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\hat{\mathbf{B}}_\ast\|_2^2 \nonumber \\
    % &=  \mathbb{E}[\|\mathbf{\Pi}_i\|_F^2]\; \text{dist}^2(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast) \nonumber  \\
    % &= \mathbb{E}\left[\sum_{j=1}^m \sum_{j'=1}^m \text{Tr} \left(\mathbf{x}_i^j (\mathbf{x}_i^{j})^\top \mathbf{x}_i^{j'} (\mathbf{x}_i^{j'})^\top\right)  \right]\; \text{dist}^2(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast) \nonumber \\
    % \hat{\mathbf{B}}^\top \mathbb{E}[ \mathbf{\Pi}] (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\hat{\mathbf{B}}_\ast = \frac{1}{m}\hat{\mathbf{B}}^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\hat{\mathbf{B}}_\ast = \mathbf{0}
    % &= \left(\sum_{j=1}^m \sum_{j'=1, j' \neq j}^m \mathbb{E}\left[\text{Tr} \left(\mathbf{x}_i^j (\mathbf{x}_i^{j})^\top \mathbf{x}_i^{j'} (\mathbf{x}_i^{j'})^\top\right) \right] + \sum_{j=1}^m \mathbb{E}\left[\text{Tr} \left(\mathbf{x}_i^j (\mathbf{x}_i^{j})^\top \mathbf{x}_i^{j} (\mathbf{x}_i^{j})^\top\right) \right] \right)\; \text{dist}^2(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast) \nonumber \\
    % &= \left(\sum_{j=1}^m \sum_{j'=1, j' \neq j}^m  + \sum_{j=1}^m \mathbb{E}\left[\text{Tr} \left(\mathbf{x}_i^j (\mathbf{x}_i^{j})^\top \mathbf{x}_i^{j} (\mathbf{x}_i^{j})^\top\right) \right] \right)\; \text{dist}^2(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast) \nonumber \\
    
    
    % Hence Proved.

% Next, the gradient update for $\hat{B}$ is:
% \begin{align}
%     \hat{v}^{t+1}_p &= {v}^t_p - \eta \sum_{i=1}^N \left(\sum_{q=1}^k {({v}_q^{(t)}})^\top  \mathbf{A}_{i,j}^\top \hat{u}_q^{(t+1)} - \sum_{q=1}^k \sigma_q^*({{v}_q^*})^\top  \mathbf{A}_{i,j}^\top u_q^* \right)
% 	\mathbf{A}_{i,j}^\top \hat{u}^{(t+1)}_p \\
% 	&= {v}^t_p - \eta \sum_{i=1}^N \left(\sum_{q=1}^k {({v}_q^{(t)}})^\top  \mathbf{A}_{i,j}^\top  (\mathbf{B}^{-1}\mathbf{C}Su^*)_q - \sum_{q=1}^k \sigma_q^*({{v}_q^*})^\top  \mathbf{A}_{i,j}^\top u_q^* \right)
% 	\mathbf{A}_{i,j}^\top (\mathbf{B}^{-1}\mathbf{C}Su^*)_p
% \end{align}

% The problem boils down to showing
% \begin{align}
%     \min_{\mathbf{x}: \|\mathbf{x}\|_2=1}\text{tr}(\mathbf{\hat{B}}_{\ast,\perp}\mathbf{\hat{B}}_{\ast,\perp}^\top {B}_t\mathbf{x}\mathbf{x}^\top \mathbf{W}_{t+1}^\top \mathbf{W}_{t+1} {B}_{t}^\top )- \delta_{2k} \|\mathbf{W}_{t+1}\mathbf{x}\mathbf{x}^\top {B}_t^\top {B}_{\ast,\perp}\|_F\|\mathbf{W}_{t+1}  {B}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \|_F\geq c > 0
% \end{align}
% for some constant $c$.

% Note that
% % $$\|\mathbf{W}_{t+1}  \hat{B}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \|_F\leq \|\mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{R}_t^\top {B}_t - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \|_F$$
% \begin{align}
%     \|\mathbf{W}_{t+1}  {B}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \|_F&\leq  \frac{1}{1-\delta_{2k}}\|\mathcal{A}(\mathbf{W}_{t+1}  {B}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top) \|_F\nonumber \\
%     &\leq \frac{1}{1-\delta_{2k}}\|\mathcal{A}(\mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t {B}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top) \|_F\nonumber \\
%     &\leq \frac{1+\delta_{2k}}{1-\delta_{2k}}\|\mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t {B}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \|_F\nonumber \\
%     &\leq \frac{1+\delta_{2k}}{1-\delta_{2k}} \|\mathbf{\hat{W}}_\ast\|_F\| \mathbf{\Sigma}_\ast (\mathbf{B}_\ast^\top \mathbf{B}_t {B}_t^\top - \mathbf{\hat{B}}_\ast^\top) \|_2 \nonumber \\
%     &\leq \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \mathbf{\Sigma}_\ast\|_2 \| \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t {B}_t^\top - \mathbf{\hat{B}}_\ast^\top \|_2 \nonumber \\
%     &= \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \mathbf{\Sigma}_\ast\|_2 \| \mathbf{\hat{B}}_\ast^\top (\mathbf{B}_t {B}_t^\top - I) \|_2 \nonumber \\
%     &= \frac{1+\delta_{2k}}{1-\delta_{2k}} \| \mathbf{\Sigma}_\ast\|_2 \;\text{dist}(\mathbf{B}_t, \mathbf{\hat{B}}_\ast) 
% \end{align}
% by RIP, the fact that $\mathbf{W}_{t+1}$ is the least squares solution, and \mathbf{C}auchy-Schwarz. 

% Next we consider
% \begin{align}
%     \|\mathbf{W}_{t+1}\mathbf{x}\mathbf{x}^\top {B}_t^\top \mathbf{\hat{B}}_{\ast,\perp}\|_F&\leq  \|\mathbf{W}_{t+1}\mathbf{x}\mathbf{x}^\top\|_F\| {B}_t^\top \mathbf{\hat{B}}_{\ast,\perp}\|_2 \nonumber \\
%     &\leq\|\mathbf{W}_{t+1}\|_2\text{dist}(\mathbf{B}_t, \mathbf{\hat{B}}_\ast) \nonumber
% \end{align}
% We have 
% \begin{align}
%     \|\mathbf{W}_{t+1}\|_2 &\leq \| \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t \|_2 - \|\mathbf{F}\|_F\nonumber \\
%     &\leq \| \mathbf{\Sigma}_\ast\|_2  + \|\mathbf{F}\|_2  \nonumber \\
%     &\leq \| \mathbf{\Sigma}_\ast\|_2 + \frac{\sqrt{k}}{1-\delta_{2k}}\|\mathbf{\Sigma}_\ast\|_2\|(BD-\mathbf{C})\|_2  \nonumber \\ 
%     &\leq \| \mathbf{\Sigma}_\ast\|_2  + \frac{\delta_{2k}k}{1-\delta_{2k}}\|\mathbf{\Sigma}_\ast\|_2  \nonumber 
% \end{align}
% using Lemmas B.2 to bound $\|\mathbf{B}^{-1}\|_2$ and 4.6 to bound $\|(BD-\mathbf{C})\|_2$ in JNS14. 
% Next,
% \begin{align}
%     \| \mathbf{B}_t J_t^{-1}\mathbf{x}\mathbf{x}^\top \mathbf{R}_t^\top\|_2 &\leq \|J_t^{-1}\|_2 \|\mathbf{R}_t^\top\|_2
% \end{align}
% $\|J_t^{-1}\|_2$ should be related to $\|\mathbf{R}_t^{-1}\|_2$, which we should be able to show is upper bounded by $\|\mathbf{R}_0^{-1}\|_2$ using similar techniques as before.

% $J_t$ should be $\mathbf{R}_t$...

% We can assume WLOG that the updates in $B$ are orthogonolized. 
% doing so means that the new update $\widetilde{W}_{t+1} = \mathbf{W}_{t+1} \widetilde{R}_{t+1}$. then the column space of $\sum_{i=1}^N \langle \mathbf{A}_{i,j}, \widetilde{W}_{t+1} \mathbf{B}_t^\top - M_\ast\rangle \mathbf{A}_{i,j}^\top$ equals that of $\sum_{i=1}^N \langle \mathbf{A}_{i,j}, \mathbf{W}_{t+1} \hat{B}_t^\top - M_\ast\rangle \mathbf{A}_{i,j}^\top$, does it? is $\widetilde{R}_{t+1} = \mathbf{R}_{t}^{\top}$? yes

% but do we need to consider another R as in JNS14? yes because the algorithms have different histories. but it should still go through. use arg in JNS14. we should always have $\widetilde{W}_{t+1} \mathbf{B}_t^\top = \overline{W}_{t+1} \overline{B}_t^\top$, bar is original alg, thus column spaces of grad descent update should be the same.


\begin{comment}
Next, let $X^i \coloneqq \|\mathbf{H}^i\|_2^2$ and define the truncated variables $\bar{X}^i \coloneqq X^i \chi_{\{X^i \leq R\}}$ for all $i \in [n]$ and some truncation level $R$. An appropriate $\Delta$ value is computed as follows, letting $\tau = \frac{m}{k\;\text{dist}(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast)}$ for ease of notation:
\begin{align}
    |\mathbb{E}[X^i] - \mathbb{E}[\bar{X}^i]|
    &= \mathbb{E}[X^i \chi_{\{X^i \geq R\}}]\nonumber \\
    &\leq \int_R^\infty z e^{-c \sqrt{\tau z}} dz  \nonumber \\
    &= - \frac{2 e^{-c\sqrt{\tau z}}(  \tau^2 z^2 + 3 \tau z (\sqrt{\tau z} + 2)+ 6\sqrt{\tau z} )}{\tau^2 \sqrt{z\tau}} \Big|_{z=R}^\infty \nonumber\\
    &= - \frac{2 e^{-c\sqrt{R\tau }}(  R^2 \tau^2  + 3 \tau  (\sqrt{R \tau } + 2)+ 6\sqrt{R \tau } )}{\tau^2 \sqrt{R\tau}}  \nonumber\\
    % &= \frac{2 e^{-\sqrt{Rm}}( R^2 m^2 + 3 Rm (\sqrt{Rm} + 2)+ 6\sqrt{Rm} )}{m^2 \sqrt{Rm}} \nonumber \\
    &\leq \frac{R^{1.5}}{\sqrt{\tau}}e^{-\sqrt{R\tau}} \nonumber \\
    &= \frac{R^{1.5}\sqrt{k}\;\text{dist}(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast)}{\sqrt{m}}e^{-c\sqrt{Rm}/\sqrt{k\;\text{dist}(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast)}} =: \Delta
\end{align} 
Now we can apply Lemma \ref{lem:tbscalar} to obtain:
\begin{align}
    \mathbb{P}[|\frac{1}{n}\sum_{i=1}^n X^i - \mathbb{E}[{X}^i]| > t_{2k}] &\leq 2 \exp \left(-\frac{n^2(t_{2k}-\Delta)^2}{\sigma^2 + 2Rn(t_{2k}-\Delta)/3} \right) + n \mathbb{P}[| X^i| \geq R] \nonumber \\
    &\leq 2 \exp \left(-\frac{c n(t_{2k}-\Delta)^2}{k^4/m^2 + R(t_{2k}-\Delta)} \right) + n \exp \left(\frac{-c \sqrt{R m}}{\sqrt{k}
    %\; \text{dist}(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast)}
    }\right) 
\end{align}
for any $t_{2k} \geq \Delta$. Set the truncation level $R = 100^2 \text{dist}^3(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast) k \log^2(n)/(cm)$ and $t_{2k} = \text{dist}^2(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)/k$

and let $t_{2k} = O(1/k)$, then $\Delta = O(\frac{k^2}{m^2 n^2})$ and $\Delta < \delta_{2k}$ as long as ${m^2 n^2} \gg k^3$. Thus we have
\begin{align}
    \mathbb{P}[|\frac{1}{n}\sum_{i=1}^n X^i - \mathbb{E}[{X}^i]| > \delta_{2k}] 
    &\leq 2 \exp \left(\frac{c m^2 n}{k^6 + 100^2 mk^3 \log^2(n)/c'} \right) + e^{-100}
\end{align}
Finally, since $\mathbb{E}[{X}^i] \leq $, we have that
\begin{align}
    \frac{1}{n}\sum_{i=1}^n \|\mathbf{H}^i\|_2^2  = \frac{1}{n}\sum_{i=1}^n X^i \leq \frac{1}{n}\sum_{i=1}^n \mathbb{E}[{X}^i] + \delta_{2k} \leq \frac{ck^2}{m} + \delta_{2k}
\end{align}
\end{comment}




\begin{comment}
-------------------------

 We have
\begin{align}
    \|(\mathbf{GD} - \mathbf{C})\hat{\mathbf{u}}_\ast\|_2^2
    &= \sum_{i=1}^n \hat{u}_{\ast,i}^2 (H^i)^2 \nonumber \\
    &= \sum_{i=1}^n \hat{u}_{\ast,i}^2 \sum_{j=1}^m  \sum_{j'=1}^m H_j^i H_{j'}^i \nonumber
\end{align}
Assume that $\mathbf{u}_{\ast}$ is incoherent, then we have
\begin{align}
    \|(\mathbf{GD} - \mathbf{C})\hat{\mathbf{u}}_\ast\|_2^2
    &\leq \frac{\mu^2}{n} \sum_{i=1}^n  \sum_{j=1}^m  \sum_{j'=1}^m H_j^i H_{j'}^i \nonumber 
\end{align}
where $H_j^i = \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle$ is a sub-exponential random variable with mean zero and norm $O(1/m)$. 

Assume temporarily that the data is Gaussian (** obviously if the data is generically sub-gaussian then we will not have this exact result but we will still have that the below expectation is $O(1/m)$, which is sufficient for our proof.).
Note that since $\mathbb{E}[H_j^i]=0$ and $H_j^i$ and $H_{j'}^i$ are independent for $j\neq j'$, we have that 
\begin{align}
    \mathbb{E}[\sum_{j=1}^m  \sum_{j'=1}^m H_j^i H_{j'}^i]&= \sum_{j=1}^m  \mathbb{E}[( H_j^i)^2] \nonumber \\
    &= \sum_{j=1}^m  \mathbb{E}[ \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2
     - 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle  + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 ] \nonumber \\
%      &= \sum_{j=1}^m  \mathbb{E}[ \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2
%   + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 ]  \nonumber \\
  &= \sum_{j=1}^m \bigg( \sum_{\ell=1}^d \frac{3\hat{{v}}_\ell^4}{m^2} \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 + \sum_{\ell=1}^d \sum_{\ell'=1, \ell' \neq \ell}^d \frac{3 \hat{{v}}_\ell^2 \hat{{v}}_{\ell'}^2}{m^2} \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 + \sum_{\ell=1}^d \frac{3\hat{{v}}_\ell^2\hat{{v}}_{\ast,\ell}^2}{m^2}  
  + \sum_{\ell=1}^d \sum_{\ell'\neq\ell, \ell'=1}^d \frac{\hat{{v}}_\ell^2\hat{{v}}_{\ast,\ell'}^2 + 2 \hat{{v}}_\ell \hat{{v}}_{\ell'}\hat{{v}}_{\ast,\ell}\hat{{v}}_{\ast,\ell'}}{m^2} \nonumber \\
  &\quad - \frac{2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle}{m^2} \sum_{\ell=1}^d 3 v_\ell^3 v_{\ast,\ell} - \frac{2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle}{m^2} \sum_{\ell=1}^d \sum_{\ell'\neq\ell, \ell'=1}^d 3v_\ell^2 v_{\ell'} v_{\ast,\ell'} \bigg) \nonumber \\
  &= \frac{1}{m^2} \sum_{j=1}^m \bigg(  3\langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 
  + 1 + 2\langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2  - 6 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 \bigg) \nonumber \\
  &= \frac{1}{m} ( 1 - \langle\hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 ) \nonumber \\
  &= \frac{1}{m} \text{dist}^2(\hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast)
\end{align}
So $\mathbf{F}$ gets smaller as we have more samples and as $\mathbf{v}$ approaches $\mathbf{v}_\ast$, this makes sense. With many samples we can easily see from \eqref{hi} that $H^i \rightarrow 0$. On the other hand, when $m=1$, we have that $|\langle \hat{\mathbf{b}}, \hat{\mathbf{b}}_\ast\rangle| = 1  \implies \hat{\mathbf{v}} = \pm \hat{\mathbf{v}}_\ast \implies H^i = 0$.

We have
\begin{align}
    \mathbb{E}[\|(\mathbf{GD} - \mathbf{C})\mathbf{\Lambda}\hat{{\mathbf{w}}}_\ast\|_2^2]&\leq  \frac{\mu^2}{nm}\text{dist}^2(\hat{\mathbf{b}}, \hat{\mathbf{b}}_\ast)
\end{align}
We need to show that $\|(\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast\|_2^2$ concentrates about its mean as $m$ and $n$ increase. In particular, let $r \coloneqq \mathbb{E}[\|(\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast\|_2^2]$, then we need
\begin{align}
    \|(\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast\|_2^2 - r \leq \epsilon
\end{align}
with high probability, which implies $\|(\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast\|_2^2 \leq \frac{\mu^2}{nm}\text{dist}^2(\hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast) + \epsilon$ with high probability. This bound is slightly different than what we originally used in the linear convergence proof but it is essentially similar and will still work.

Note that $\|(\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast\|_2^2$ is weighted sum of $nm^2$ random variables $H^i_{j} H^i_{j'}$. We have
\begin{align}
    \mathbb{E}[(H^i_{j})^2 (H^i_{j'})^2] &\leq \mathbb{E}[(H^i_{j})^4] \nonumber \\
    &= \mathbb{E}[(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle )^4] \nonumber \\
    &= \mathbb{E}[(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 - 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle +  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2)(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle )^2] \nonumber \\
    &\leq \mathbb{E}[(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 - 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle +  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2) \nonumber \\
    &\quad \quad \quad \quad \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 (\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 - 2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 )] \nonumber \\
    &\leq \mathbb{E}[(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 - 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2) \nonumber \\
    &\quad \quad \quad \quad \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 (\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2  - 2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 )] \nonumber \\
    &= \mathbb{E}[\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 
    - 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle 
    - 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^3 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle 
    + 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2
    \nonumber \\
    &\quad \quad \quad \quad \quad \quad + 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2
    + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^4) \nonumber \\
    &\leq \mathbb{E}[\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 
    - 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle 
    - 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^3 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle 
    + 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2
    \nonumber \\
    &\quad \quad \quad \quad \quad \quad + 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2
    + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^4)  \nonumber \\
    &\leq 16 \mathbb{E}[\langle \mathbf{x}_{i}^j, \tilde{\mathbf{v}}\rangle^8] \nonumber
\end{align}
where $\tilde{\mathbf{v}} = \arg \max_{\mathbf{v} \in \{  \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \}} \langle \mathbf{x}_{i}^j, {\mathbf{v}} \rangle^2$. 
Note that $\langle \mathbf{x}_{i}^j, \tilde{\mathbf{v}}\rangle$ is subgaussian with norm $\|\tilde{\mathbf{v}}\|_2/\sqrt{m}= 1/\sqrt{m}$ (variance $1/m$). So we have 
\begin{align}
    \mathbb{E}[(H^i_{j})^2 (H^i_{j'})^2]
&\leq \frac{c}{m^4} \nonumber
\end{align}
for some absolute constant $c$. Therefore, $X^i \coloneqq \sum_{j=1}^m \sum_{j'=1}^m H^i_{j} H^i_{j'}$ has variance
\begin{align}
    \text{Var}(X^i) &= \mathbb{E}[ (\sum_{j=1}^m \sum_{j'=1}^m H^i_{j} H^i_{j'} - \bar{r})^2 ] \nonumber \\
    &\leq \left( {m \choose 2}{4 \choose 2} + {m\choose 1}  \right) \mathbb{E}[(H_{j}^i)^4] \nonumber \\
    &\leq \frac{c}{m^2}
\end{align}
where the first inequality follows by a simple counting argument: there are at most $ {m \choose 2}{4 \choose 2} + {m\choose 1}  $ terms in the square with even-order powers of the $H_j^i$'s, which have expectation bounded above by $\mathbb{E}[(H_{j}^i)^4]$. All other terms have expectation zero.
% by sub-gaussian property, we have
% \begin{align}
%     \mathbb{P}[]
% \end{align}
Next, let $\bar{X}^i = X^i \chi_{\{X^i \leq R\}}$ for some constant truncation level $R$. Since the $X^i$'s are independent, we have, ignoring constant factors,
\begin{align}
    \mathbb{P}(\|(\mathbf{GD}- \mathbf{C})\mathbf{u}_\ast\|_2^2 \geq \delta_2 + \frac{\mu}{nm} \text{dist}^2(\mathbf{v}, \mathbf{v}_\ast) ) &\leq \mathbb{P}( \frac{1}{n} \sum_{i=1}^n X^i - \mathbb{E}[X^i] \geq \delta_2 ) \nonumber \\
    &\leq \mathbb{P}( \frac{1}{n} \sum_{i=1}^n \bar{X}^i - \mathbb{E}[\bar{X}^i] \geq \delta_2  - \Delta) + n \mathbb{P} [{X}^i > R] \label{split0} \\
    &\leq  \exp \left(- \frac{n (\delta - \Delta)^2}{ 1/m^2 + R (\delta - \Delta)} \right) + n \mathbb{P} [{X}^i > R] \label{split}
\end{align}
 for any $\delta \geq \Delta$, where $\delta \coloneqq | \mathbb{E}[X^i] - \mathbb{E}[\bar{X}^i]$ and \eqref{split0} follows by splitting on the event $\{X^i \leq R\}$, as in Lemma 29 in \cite{tripuraneni2020provable} (Jin paper). Recall that each $H^i_j$ is sub-exponential with norm $O(1/m)$, so $\sum_{j=1}^m H^i_j$ is sub-exponential with norm $O(1/\sqrt{m})$. Also, $X^i = (\sum_{j=1}^m H^i_j)^2$. So by sub-exponential tail bound, we have
\begin{align}
    \mathbb{P}( X^i \geq R  ) \leq \mathbb{P}(|\sum_{j=1}^m H^i_j| \geq \sqrt{R} ) \leq O(e^{-\sqrt{Rm}})
\end{align}
Plugging this back into \eqref{split}, we have
\begin{align}
    \mathbb{P}\left(\|(\mathbf{GD}- \mathbf{C})\mathbf{u}_\ast\|_2^2 \geq \delta + \frac{\mu^2}{nm} \text{dist}^2(\mathbf{v}, \mathbf{v}_\ast) \right) &\leq \exp \left( -\frac{n (\delta - \Delta)^2}{ 1/m^2 + R (\delta - \Delta)} \right) + n \exp (-\sqrt{Rm})
\end{align}
All that remains is to show $\Delta$ is small. We have
\begin{align}
    \Delta &= \mid \mathbb{E}[X^i]  - \mathbb{E}[\bar{X}^i] \mid \nonumber \\
    &= \mathbb{E}[X^i \chi_{\{X^i \geq R\}}] \nonumber \\
    &\leq \int_R^\infty z e^{- \sqrt{zm}} dz \nonumber \\
    &= - \frac{2 e^{-\sqrt{zm}}( z^2 m^2 + 3 zm (\sqrt{zm} + 2)+ 6\sqrt{zm} )}{m^2 \sqrt{zm}} \Big|_{z=R}^\infty \nonumber \\
    &= \frac{2 e^{-\sqrt{Rm}}( R^2 m^2 + 3 Rm (\sqrt{Rm} + 2)+ 6\sqrt{Rm} )}{m^2 \sqrt{Rm}} \nonumber \\
    &\leq \tfrac{cR^{1.5}}{\sqrt{m}}e^{-\sqrt{Rm}} \nonumber
\end{align}
for some constant factor $c$. Thus it is safe to assume that $\delta \gg \Delta$. Putting everything together, we have, up to absolute constants and assuming $nm \geq 1/\delta$,
\begin{align}
    \mathbb{P}\left(\|(\mathbf{GD}- \mathbf{C})\mathbf{u}_\ast\|_2^2 \geq \delta\right)
    &\leq \exp \left( -c\frac{n \delta^2}{ 1/m^2 + R \delta} \right) + n \exp (-\sqrt{Rm}) \nonumber \\
    &\leq \exp \left( -c'{n\delta^2 \min(m^2, 1/\delta)} \right) +  \exp (-(\sqrt{Rm} - \log(n))) \nonumber %\\
    % &\leq \exp \left( -c'{n\delta } \right) +  \exp (-(\sqrt{Rm} - \log(n))) 
\end{align}
% Since we need $\delta \leq \frac{1}{k^2}$, we can easily set $m$ large enough such that $\delta \geq \Delta$ (we only require $m \geq O(\log^2(k))$). Finally, let $\delta = O(1/k^2)$ and assume $nm \geq O(k^2)$, then we have
% \begin{align}
%     \mathbb{P}\left(\|(\mathbf{GD}- \mathbf{C})\mathbf{u}_\ast\|_2^2 \geq O\left(\frac{1}{k^2}\right)\right) &\leq \mathbb{P}\left(\|(\mathbf{GD}- \mathbf{C})\mathbf{u}_\ast\|_2^2 \geq O\left(\frac{1}{k^2}\right) + \frac{\mu^2}{nm} \text{dist}^2(\mathbf{v}, \mathbf{v}_\ast) \right) \nonumber \\
%     &\leq \exp \left( c\frac{n /k^4}{ 1/m^2 + R /k^2} \right) + n \exp (-\sqrt{Rm}) \nonumber \\
%     &\leq \exp \left( c'\frac{n \max(m^2, k^2)}{k^4} \right) + n \exp (-\sqrt{Rm}) 
% \end{align}
% where $R$ and $\mu$ are absolute constants. So, including our earlier bound on $\Delta$, we require $m \geq O(\log^2(n) + \log^2 (k))$
So we have what we need as long as $m \gg \log^2(n)$, $n\delta^2 \min(m^2, 1/\delta) \gg 1$, and $m \gg \log^2 (1/\delta)$ (so that $\delta \gg \Delta$).

Note that we will need $\delta_{2k} \leq O(1/k)$. So if a similar result above holds in the rank-$k$ case, we will need $n \min(m^2, k) \gg k^2$.

Remark on lack of dependence on $d$: the heart of the result is showing that $ ( \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle)$ concentrates. Although the vectors here are $d$-dimensional, the tails of this quantity do not depend on $d$ because $\hat{\mathbf{v}}$ and $\hat{\mathbf{v}}_\ast$ are normalized. The analogous bound in Sujay's matrix completion does have sample complexity dependence on $d$, but I think this part is loose, because the quantity they need to show concentrates does not scale with $d$ either.

This completes the bound on $\|\mathbf{F}\|_F$.
\end{comment}



\begin{comment}
Next we upper bound the variance of $\|\mathbf{H}_i\|_2^2$. We have
\begin{align}
    \text{Var}(\|\mathbf{H}_i\|_2^2) &\leq \mathbb{E}[\|\mathbf{H}^i\|_2^4] \nonumber \\
    &= \sum_{j=1}^m \sum_{j'=1}^m \sum_{j''=1}^m \sum_{j'''=1}^m  \mathbb{E}\Big[\text{Tr}\left(  \hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \hat{\mathbf{B}}\hat{\mathbf{B}}^\top \mathbf{x}_i^{j'} (\mathbf{x}_i^{j'})^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\hat{\mathbf{B}}_\ast\right) \nonumber \\
    &\quad \quad \quad \quad \quad \quad \quad \quad\quad\quad\quad \text{Tr}\left( \hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^{j''} (\mathbf{x}_i^{j''})^\top \hat{\mathbf{B}}\hat{\mathbf{B}}^\top \mathbf{x}_i^{j'''} (\mathbf{x}_i^{j'''})^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\hat{\mathbf{B}}_\ast \right)\Big] \nonumber \\
    &= \sum_{j=1}^m   \sum_{j'=1}^m \sum_{j''=1}^m \sum_{j'''=1}^m  \mathbb{E}\left[ \langle \mathbf{u}_i^j, \mathbf{u}_i^{j'} \rangle \langle \mathbf{v}_i^j, \mathbf{v}_i^{j'} \rangle \langle \mathbf{u}_i^{j''}, \mathbf{u}_i^{j'''} \rangle \langle \mathbf{v}_i^{j''}, \mathbf{v}_i^{j'''} \rangle \right] \nonumber \\
    &= \sum_{j=1}^m   \mathbb{E}\left[ \|\mathbf{u}_i^j\|_2^4 \|\mathbf{v}_i^j\|_2^4\right] +  2 \sum_{j=1}^m \sum_{j'=1, j'\neq j}^m \mathbb{E}\left[ \|\mathbf{u}_i^j\|_2^2 \|\mathbf{v}_i^j\|_2^2 \|\mathbf{u}_i^{j'}\|_2^2 \|\mathbf{v}_i^{j'}\|_2^2 \right] + 2 \sum_{j=1}^m \sum_{j'=1, j' \neq j}^m \mathbb{E}\left[ \langle \mathbf{u}_i^j, \mathbf{u}_i^{j'} \rangle^2 \langle \mathbf{v}_i^j, \mathbf{v}_i^{j'} \rangle^2 \right] \nonumber 
    %\\
    %&\leq \sum_{j=1}^m   \mathbb{E}\left[ \|\mathbf{u}_i^j\|_2^4 \|\mathbf{v}_i^j\|_2^4\right] + 2m^2
    % &\leq \left( {m \choose 2}{4 \choose 2} + {m\choose 1}  \right) \mathbb{E}\Big[\text{Tr}\left(  \hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \hat{\mathbf{B}}\hat{\mathbf{B}}^\top \mathbf{x}_i^{j} (\mathbf{x}_i^{j})^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\hat{\mathbf{B}}_\ast\right) \nonumber \\
    % &\quad \quad \quad \quad \quad \quad \quad \quad\quad\quad\quad \text{Tr}\left( \hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^{j} (\mathbf{x}_i^{j})^\top \hat{\mathbf{B}}\hat{\mathbf{B}}^\top \mathbf{x}_i^{j} (\mathbf{x}_i^{j})^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\hat{\mathbf{B}}_\ast \right)\Big] \label{choose}
\end{align}
The middle term in the above equation can be bounded as in \eqref{sg2}. The third term can be similarly bounded using Cauchy Schwarz and \eqref{sg2}:
\begin{align}
\mathbb{E}\left[ \langle \mathbf{u}_i^j, \mathbf{u}_i^{j'} \rangle^2 \langle \mathbf{v}_i^j, \mathbf{v}_i^{j'} \rangle^2 \right] &\leq \mathbb{E}\left[ \|\mathbf{u}_i^j\|_2^2 \|\mathbf{v}_i^j\|_2^2 \|\mathbf{u}_i^{j'}\|_2^2 \|\mathbf{v}_i^{j'}\|_2^2\right] \nonumber \\
&= \mathbb{E}\left[ \|\mathbf{u}_i^j\|_2^2 \|\mathbf{v}_i^j\|_2^2 \right] \mathbb{E}\left[ \|\mathbf{u}_i^{j'}\|_2^2 \|\mathbf{v}_i^{j'}\|_2^2\right] \nonumber \\
&\leq \frac{ck^4}{m^4}  \text{dist}^4(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast)
\end{align}
Next, notice that
\begin{align}
    \mathbb{E}\left[ \|\mathbf{u}_i^j\|_2^4 \|\mathbf{v}_i^j\|_2^4 \right] 
%    &=           \nonumber \\
    &= \mathbb{E}\left[\left(\sum_{p,q=1}^k \langle \mathbf{u}_i^j, \mathbf{e}_p\rangle^2 \; \langle \mathbf{v}_i^j, \mathbf{e}_q\rangle^2\right)^2\right] \nonumber \\
    &= \mathbb{E}\left[\sum_{p,q=1}^k \sum_{p',q'=1}^k \langle \mathbf{u}_i^j, \mathbf{e}_p\rangle^2 \; \langle \mathbf{v}_i^j, \mathbf{e}_q\rangle^2 \langle \mathbf{u}_i^j, \mathbf{e}_{p'}\rangle^2 \; \langle \mathbf{v}_i^j, \mathbf{e}_{q'}\rangle^2 \right] \nonumber \\
    &\leq k^4 \left( \max_{p,p'\in [k]} \mathbb{E}\left[ \langle \mathbf{u}_i^j, \mathbf{e}_p\rangle^4 \langle \mathbf{u}_i^j, \mathbf{e}_{p'}\rangle^4\right] \;\max_{q,q'\in [k]} \mathbb{E}\left[ \langle \mathbf{v}_i^j, \mathbf{e}_q\rangle^4   \langle \mathbf{v}_i^j, \mathbf{e}_{q'}\rangle^4 \right]\right)^{1/2} \nonumber \\
    &\leq k^4 \left( \max_{p,p'\in [k]} \left(\mathbb{E}\left[ \langle \mathbf{u}_i^j, \mathbf{e}_p\rangle^8 \right] \mathbb{E}\left[\langle \mathbf{u}_i^j, \mathbf{e}_{p'}\rangle^8\right]\right)^{1/2} \;\max_{q,q'\in [k]}\left( \mathbb{E}\left[ \langle \mathbf{v}_i^j, \mathbf{e}_q\rangle^8\right]\mathbb{E}\left[ \langle \mathbf{v}_i^j, \mathbf{e}_{q'}\rangle^8 \right]\right)^{1/2}\right)^{1/2} \nonumber \\
    &\leq c k^4 \left( \frac{1}{m^4}  \| \mathbf{I}_k - \hat{\mathbf{B}}_\ast^\top \hat{\mathbf{B}} \hat{\mathbf{B}}^\top \hat{\mathbf{B}}_\ast\|_2^8 \;\frac{1}{m^4} \right)^{1/2} \label{sg3} \\
    &\leq c \frac{k^4}{m^4} \text{dist}^4(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast) \nonumber
\end{align}
where \eqref{sg3} again follows by sub-gaussian properties. Thus we have 
\begin{align}
    \text{Var}(\|\mathbf{H}_i\|_2^2) &\leq (c_1 m + c_2m^2) \frac{k^4}{m^4} \text{dist}^4(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast) \leq c \frac{k^4}{m^2} \text{dist}^4(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast)
\end{align}
for some absolute constant $c$. 
\end{comment}


% a similar argument as in Proposition 2.6.1 in \cite{vershynin2018high},  the sum of independent sub-exponential random variables (not necessarily with mean zero) is sub-exponential with norm equal to the sum of the norms. In particular, since the sub-exponential random variables $\|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2$ are independent, 
% \begin{align}
%     \left\|\sum_{j=1}^m  \|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2 \right\|_{\phi_1} &\leq C \sum_{j=1}^m \left\| \|\mathbf{u}_i^j\|_2\; \|\mathbf{v}_i^j\|_2 \right\|_{\phi_1}  \label{versh1}  \leq {C' k} \; \text{dist}(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast). \nonumber
% \end{align}
% Finally, combining the sub-exponential property of $\sum_{j=1}^m  \|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2$ with \eqref{hii} yields

    % \mathbb{P}\left( \|\mathbf{H}^i\|_2^2 - \mathbb{E}[\|\mathbf{H}^i\|_2^2] > t \right) &\leq \mathbb{P}\left( \left(\sum_{j=1}^m  \|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\right) > \sqrt{t} \right) \leq \exp \left(\frac{-c \sqrt{t m}}{\sqrt{k}\; \text{dist}(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast)}\right) \label{hii}
    
            % \leq \exp \left(\frac{-c \sqrt{t m}}{\sqrt{k}\; \text{dist}(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast)}\right) 
            
            % Next, the sub-exponential norm of $ \|\mathbf{u}_i^j\|_2^2$ is bounded as:
% \begin{align}
%     \left\| \|\mathbf{u}_i^j\|_2^2 \right\|_{\phi_2} &= \left\| \sum_{\ell} \right\|_{\phi_2} \nonumber \\
%     &= \left\| \|\mathbf{u}_i^j\|_2^2 \right\|_{\phi_2} \nonumber \\
% \end{align}




\subsection{Restricted Isometry Property}

In order for AltMinGD to converge,  the linear operator $\mathcal{A}$ must be nearly isometric. We formalize this via the well-known Restricted Isometry Property (RIP).
\begin{definition} (Restricted Isometry Property \cite{})
An operator $\mathcal{A}: \mathbb{R}^{n \times d} \rightarrow \mathbb{R}^{mn}$ satisfies the $k$-RIP with constant $\delta_k < 1$ if 
\begin{equation}
    (1-\delta_r) \|\mathbf{M}\|_{F}^2 \leq \|\mathcal{A}(\mathbf{M})\|_2^2 \leq (1+\delta_r) \|\mathbf{M}\|_{F}^2
\end{equation}
holds simultaneously for all $\mathbf{M}$ of rank at most $k$.
\end{definition}
The following lemma characterizes the number of samples $m$ needed by each user in order for $\mathcal{A}$ to satisfy the RIP:

\begin{lemma} (Sample Complexity for RIP)
Let $\kappa = \frac{\sigma_{\max}(\mathbf{B}_\ast\mathbf{W}_\ast^\top)}{\sigma_{\min}(\mathbf{B}_\ast\mathbf{W}_\ast^\top)}$. Under Assumption \ref{assump:subgauss}, $\mathcal{A}$ satisfies $k$-RIP
 with parameter $\delta_k$ as long as 
 \begin{align}
     m \geq O(dk + k^3 \kappa^4 \log(nd/k))
 \end{align}
\end{lemma}



% note that we can only do as well as the noise floor, i.e. w^\ast (B^\ast) = w^\ast + noise


%For now, ignore evaluation of the learned model on new data and/or tasks.

%We measure the quality of our solution $\phi$ by the excess expected risk $\mathcal{E}(\phi)$, defined as
%\begin{align}
 %   \mathcal{E}(\phi) \coloneqq \frac{1}{n} \sum_{i=1}^n \mathbb{E}_{(\mathbf{x}_i, y_i) \sim \mu_i}[(\langle \mathbf{w}_i^\ast(\phi),  \phi(\mathbf{x}_i) \rangle - \langle \mathbf{w}_i^\ast, \phi^\ast(\mathbf{x}_i) \rangle)^2]\label{er}
%\end{align}

% different from admm in many ways, one is that we are executing GD over phi, not solving for the optimal phi each time


% Our work introduces a novel representation learning scheme for federated learning. We prove that our algorithm efficiently learns a globally optimal representation 


% provides a framework for developing distributed learning algorithms subject to communication and privacy constraints.
% the importance of learning systems that efficiently leverage all of the data collected across devices while preserving user privacy is becoming more apparent. 
% Often, the amount of data available locally on each device is insufficient for users to solve their tasks using only local data, necessitating further information that may be supplied by other users.
% {\em Federated learning} \cite{mcmahan2017communication} provides a framework for developing distributed learning algorithms subject to communication and privacy constraints.
% Federated learning aims to address this issue by supplementing each user's local data with global information extracted from all users. 
% The hope is that the data across all users may share features that are useful for each user, even if the data is non-i.i.d.

% tomorrow: test new users with femnist and shakespeare
% may neeed to download from elsewhere

% to do for cifar:
% reduce local accuracy --> reduce lg n=1000
% for n=100, recover baselines - done
% --- with 1200 iters of fedavg for init: 
% --- amg gets 90, lg 88 on 200th iter. but best lg is 91 vs 90 for amg. but i think we can point out that this evaluation method favors lg. can also still tune amg. also, note that amg does need a good initialization, so running fedavg first is fine i think
% test

% left off: need to increase number of test samples in femnist. right now, we are only testing one sample per new user. for cifar, we have 200 total samples in each test
% need to fix acc decreasing for cifar
% get shakespeare working

% summary of some results:
% local with 100 usrrs, 2000 iters gets 77 best acc with fed-sgd.
% n=1000 amg outperforms lg with 1200 fed-sgd iters for initialization, 200 for fine-tuning, according to per-iter best acc metric (88 to 81, roughly). on new data it is also better but worse for ensemble (not surprising). but lg wins when taking the best models over all iters, again this is not surprising because you have more parameters to choose when doing this for lg

% where is paper that tests on new users -- need baseline for femnist
% feddane gives number of users in femnist, shakespeare datasets
% plots
% to do tonight: 
% get shakespeare working
% decide on eval metric for new users
% create datasets for emnist and shakespeare with new samples
% fix code for these
% fix and finalize cifar
% issue: acc of avg model much higher than avg acc of local models. fixed: was taking weighted average. Which is what we want? i think non-weighted. so must edit test_img_avg_all...check - actually fedane weights by local dataset size
% must use 0.01 step size for femnist
% current issues: tune makes worse, cifar gets worse
% for cifar, why is new acc so good?
% fixed cifar convergence
% next: make sure accs make sense, make sure accs make sense for femnist and shakespeare, update other algs with femnist and shakespeare, collect results
% left off: still issue with cifar lg: only the first 10 clients improve... fixed
% next to do:
% 1. get shakespeare usersplit working for amg, lg, local, fed -femnist done
% 2. get femnist and shakespeare datasplit working for amg, lg, local, fed
% 3. get final results for cifar
%    a. n = 10, 100, 1000, 5000
%    b. implement other baselines
% 4. get final results for shakespeare (maybe, since we can't vary n, instead vary the total amount of training data)
% 5. get final results for femnist
% 6. reddit
% 7. mnist if time
% meanwhile: synthetic

%tonight:
%1. fix tune - done
%2. compare to alt gd gd, make sure relative accs make sense
%   a. accs are not good enough. increasing lr helps but accs are still too low. need to see if better initialization helps
%   b. measures are still weird. why is post-tune worse?
%   c. check on femnist datasplit-small first
%3. get shakespeare usersplit working
%4. work on intro

% should we compare against localized versions of these algs? i.e. fed avg after local update

% fedavg femnistus: Round 199, Average loss 1.161, Test loss 1.206, Test accuracy: 64.92
%Best model, iter: 197, acc: 65.1730690221857, acc new: 52.13074247687366

% amg: Round 199, Test acc pre: 47.79, Test acc post: 37.01
% 8493.775048017502
% Acc (new users, pre adapt): 49.13973940740872, acc (new users, post adapt): 35.400709443765614

% issue: fedsgd seems tough to beat for femnist

% implement reptile
% questions: how much data does charles use? what kind of model do they use for shakespeare? tf

% today: 
% get initial shakespeare table
% start to collect final cifar results
%   - the metrics are consistent, just need to run script
%   - verify they make sense while getting initial shakespeare results
% plot convergence trajectories
%   - verify how to extract from results
% plot accs vs num_users
% fix synthetic

%next commands: 
% shakespeare fed21 - done
% shakespeare amg, shakespeare lg, shakespeare local - done
% then test plot script
%then run cifar
% then fix synthetic

% for shakespeare, somehow need to select more users with fewer samples

% this weekend:
% get initial shakespeare usersplit table
% finalize cifar
% finalize synthetic

% next run: local shakespeare. then cifar
% would be nice to get some better femnist usersplit results before tuesday
% then goals: edit shakespeare dataset, fix femnist just run cifar

% We use the original test set in CIFAR-10 as our global test set for comparing performance of all method -FEDERATED LEARNING WITH MATCHED AVERAGING, same for us

% femnist debugging questions:
% why is local acc so low? why does test acc get worse for amg even though traing acc decereases? need more users to prevent overfitting? how do other baselines do? how much data per user?
% todo: get additional femnist results. get shakespeare local
% tonight: answer these q's, read papers

% fundamental issue of federated learning is resolving the trade-off between leveraging the similarity of data shared across users and catering user models to unique local data.

% The factors informing this trade-off are statistical, such as the local and global data variance, as well as systematic, such as communication costs and privacy concerns. To interpolate between the two extremes of totally global and local learning, several recent works have 

%using a novel result of interest beyond
%




The key is to show that $\|\mathbf{H}^i\|_F^2$ is bounded above by a squared sub-exponential random variable. Note that 
\begin{align}
    \|\mathbf{H}^i\|_F^2 &= \text{Tr}\left(\hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)  \mathbf{\Pi}^i\hat{\mathbf{B}}\hat{\mathbf{B}}^\top \mathbf{\Pi}^i (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\hat{\mathbf{B}}_\ast \right) \nonumber \\
    &= \sum_{j=1}^m \sum_{j'=1}^m \text{Tr}\left(\hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \hat{\mathbf{B}}\hat{\mathbf{B}}^\top \mathbf{x}_i^{j'} (\mathbf{x}_i^{j'})^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\hat{\mathbf{B}}_\ast \right) \nonumber \\
    &= \sum_{j=1}^m \sum_{j'=1}^m \text{Tr}\left( \mathbf{u}_i^j (\mathbf{v}_i^j)^\top \mathbf{v}_i^{j'} (\mathbf{u}_i^{j'})^\top \right) \nonumber \\
    &\leq \sum_{j=1}^m \sum_{j'=1}^m \sigma_{\max}( \mathbf{u}_i^j (\mathbf{v}_i^j)^\top)\sigma_{\max}( \mathbf{v}_i^{j'} (\mathbf{u}_i^{j'})^\top) \label{vn} \\
    &= \sum_{j=1}^m \sum_{j'=1}^m \|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2 \| \mathbf{u}_i^{j'}\|_2  \|\mathbf{v}_i^{j'}\|_2 \nonumber \\
    &= \left(\sum_{j=1}^m  \|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\right)^2 
\end{align}
where \eqref{vn} holds almost surely by the von Neumann trace inequality and the fact that $\mathbf{u}_i^j (\mathbf{v}_i^j)^\top$ and $\mathbf{u}_i^{j'} (\mathbf{v}_i^{j'})^\top$ are rank-1. 

---------



Thus, we have that 
for any $t\geq0$,
\begin{align}
        \mathbb{P}\left( \|\mathbf{H}^i\|_2^2 > t \right) &\leq \mathbb{P}\left( \left(\sum_{j=1}^m  \|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\right) > \sqrt{t} \right) \nonumber \\
        \implies \mathbb{P}\left( \|\mathbf{H}^i\|_2^2 > \left(\sqrt{t} + \sum_{j=1}^m\mathbb{E}\left[\|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\right]\right)^2 \right) &\leq \mathbb{P}\left( \|\mathbf{H}^i\|_2^2 > \left(\sqrt{t} + \sum_{j=1}^m\mathbb{E}\left[\|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\right]\right)^2 \right) \nonumber \\
        &\leq \mathbb{P}\left( \sum_{j=1}^m  \|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2 -\mathbb{E}\left[  \|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\right]  > \sqrt{t} \right) \label{hii}
\end{align}
Thus the problem reduces to showing concentration of the random variables $\|\mathbf{u}_i^j\|_2\|\|\mathbf{v}_i^j\|_2$. Recall that $\mathbf{u}_i^j = \hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)\mathbf{x}_{i}^j$, where the elements of $\mathbf{x}_{i}^j$ are independent, mean zero, variance $1/m$, and sub-gaussian with norm $c/\sqrt{m}$. 
Then, by Theorem 2.1 in \citet{rudelson2013hanson} (an extension of the Hanson-Wright inequality), the random variable $Z \coloneqq \|\mathbf{u}_i^j\|_2 - \|\frac{1}{\sqrt{m}}\hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d) \|_{F}$ is sub-gaussian with norm bounded as
\begin{align}
    \|Z \|_{\phi_2} \leq c \frac{1}{\sqrt{m}} \|\hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)  \|_2 \nonumber
\end{align}
Therefore, by the triangle inequality, we have
\begin{align}
    \left\| \|\mathbf{u}_i^j\|_2 \right\|_{\psi_2} &\leq \|Z \|_{\psi_2} + \left\|\left\|\frac{1}{\sqrt{m}}\hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)  \right\|_F \right\|_{\psi_2} \nonumber \\
    &\leq c \frac{1}{\sqrt{m}} \left\|\hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d) \right\|_2 + \frac{1}{\sqrt{m}}\left\|\hat{\mathbf{B}}_\ast^\top (\hat{\mathbf{B}} \hat{\mathbf{B}}^\top -  \mathbf{I}_d)  \right\|_F \nonumber \\
    &\leq \frac{c + \sqrt{k}}{\sqrt{m}} \text{dist}(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)
\end{align}
A similar argument shows that the sub-gaussian norm of $ \|\mathbf{v}_i^j\|_2$ is bounded as: 
\begin{align*}
    \left\| \|\mathbf{v}_i^j\|_2 \right\|_{\psi_2} 
    &\leq \frac{c + \sqrt{k}}{\sqrt{m}} \|\hat{\mathbf{B}}\|_2 = \frac{c + \sqrt{k}}{\sqrt{m}}
\end{align*}
Thus, by Lemma 2.7.7 in \citet{vershynin2018high}, the product $ \|\mathbf{u}_i^j\|_2 \|\mathbf{v}_i^j\|_2$ is sub-exponential with norm
\begin{align}
    \left\| \|\mathbf{u}_i^j\|_2 \|\mathbf{v}_i^j\|_2 \right\|_{\psi_1} &\leq \left\| \|\mathbf{u}_i^j\|_2 \right\|_{\psi_2}\left\|\|\mathbf{v}_i^j\|_2 \right\|_{\psi_2} \leq \frac{c' k}{m} \; \text{dist}(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)
\end{align}
for an absolute constant $c'$. Further, by the centering inequality (Excercise 2.7.10 in \citet{vershynin2018high}), we have 
$$  \left\| \|\mathbf{u}_i^j\|_2 \|\mathbf{v}_i^j\|_2 - \mathbb{E}\big[ \|\mathbf{u}_i^j\|_2 \|\mathbf{v}_i^j\|_2 \big]  \right\|_{\psi_1} \leq \frac{c k}{m} \; \text{dist}(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)$$ for an absolute constant $c$.
Thus, we can use Bernstein's Inequality to upper bound \eqref{hii}, namely:
\begin{align}
\mathbb{P}\left( \|\mathbf{H}^i\|_2^2 > \left(\sqrt{t} + \sum_{j=1}^m \mathbb{E}\big[\|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\big]\right)^2 \right) 
&\leq \mathbb{P}\left( \sum_{j=1}^m  \|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2 - \mathbb{E}\big[\|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\big]  > \sqrt{t} \right) \nonumber \\
&\leq \exp\left(-c \min \left( \frac{t}{\sum_{j=1}^m \frac{k^2}{m^2} \; \text{dist}^2(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)} , \frac{\sqrt{t}}{\frac{k}{m}\; \text{dist}(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)} \right) \right) \nonumber \\
&= \exp\left(-c \min \left( \frac{m t}{ {k^2}\; \text{dist}^2(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)} , \frac{m\sqrt{t}}{{k}\; \text{dist}(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)} \right) \right) \label{bern1}
\end{align}
 Next, note that
\begin{align}
\sum_{j=1}^m \mathbb{E}\big[\|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\big]
    &= m \mathbb{E}\left[\| \mathbf{u}_1^j\|_2 \; \|\mathbf{v}_1^{j} \|_2\right] \label{iid} \\
&\leq m \left( \mathbb{E}\left[\| \mathbf{u}_1^j\|_2^2\right] \mathbb{E}\left[ \|\mathbf{v}_1^{j} \|_2^2\right] \right)^{1/2} \label{cau0} \\
&= m \Big( \text{Tr}\left( (\mathbf{I}_k - \hat{\mathbf{B}} \hat{\mathbf{B}}^\top) \hat{\mathbf{B}}_\ast \hat{\mathbf{B}}_\ast^\top (\mathbf{I}_k - \hat{\mathbf{B}} \hat{\mathbf{B}}^\top) \mathbb{E}\left[\mathbf{x}_1^{j} (\mathbf{x}_1^{j})^\top\right] \right) \nonumber \\
&\quad \quad \quad \quad \text{Tr}\left( \hat{\mathbf{B}} \hat{\mathbf{B}}^\top \mathbb{E}\left[\mathbf{x}_1^{j} (\mathbf{x}_1^{j})^\top\right] \right)  \Big)^{1/2} \label{cau5} \\
&=  \Big( \text{Tr}\left( (\mathbf{I}_k - \hat{\mathbf{B}} \hat{\mathbf{B}}^\top) \hat{\mathbf{B}}_\ast \hat{\mathbf{B}}_\ast^\top (\mathbf{I}_k - \hat{\mathbf{B}} \hat{\mathbf{B}}^\top) \right)  \text{Tr}\left( \hat{\mathbf{B}} \hat{\mathbf{B}}^\top \right)  \Big)^{1/2} \nonumber \\
&= \| (\mathbf{I}_k - \hat{\mathbf{B}} \hat{\mathbf{B}}^\top) \hat{\mathbf{B}}_\ast\|_F \; \| \hat{\mathbf{B}} \|_F \nonumber \\
&\leq k \; \| (\mathbf{I}_k - \hat{\mathbf{B}} \hat{\mathbf{B}}^\top) \hat{\mathbf{B}}_\ast\|_2 \; \| \hat{\mathbf{B}} \|_2 \label{raankk} \\
&= k \; \text{dist}(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast) \label{raankk2}
\end{align}
where \eqref{iid} follows from the fact that the random variables $\| \mathbf{u}_1^j\|_2 \; \|\mathbf{v}_1^{j} \|_2$ are i.i.d., \eqref{cau0} follows from the Cauchy-Schwarz inequality, and \eqref{raankk} follows from the fact that both 
$(\mathbf{I}_k - \hat{\mathbf{B}} \hat{\mathbf{B}}^\top) \hat{\mathbf{B}}_\ast$ and $\hat{\mathbf{B}}$ are rank-$k$. Define the truncation level $R_t \coloneqq  2t + 2k^2 \; \text{dist}^2(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)$, then using \eqref{bern1} and \eqref{raankk2}, we have
\begin{align}
 \mathbb{P}\left( \|\mathbf{H}^i\|_2^2 > R_t \right) &\leq   \mathbb{P}\left( \|\mathbf{H}^i\|_2^2 > \left(\sqrt{t} + \sum_{j=1}^m \mathbb{E}\big[\|\mathbf{u}_i^j\|_2\|\mathbf{v}_i^j\|_2\big]\right)^2 \right) \leq \exp\left(-c \min \left( \frac{m t}{ {k^2}\; \text{dist}^2(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)} , \frac{m\sqrt{t}}{{k}\; \text{dist}(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)} \right) \right)
\end{align}
using the numerical inequality $2a^2 + 2b^2 \geq (a+b)^2 $.


% \begin{align}
%     \text{dist}(\hat{B}_{t+1}, \mathbf{\hat{B}}_\ast) \leq \sqrt{1 - \eta} \text{dist}(\hat{B}_{t}, \mathbf{\hat{B}}_\ast) 
% \end{align}
% \begin{align}
%     \text{dist}(\mathbf{B}_t, \mathbf{\hat{B}}_\ast)
%     &\leq  \frac{\left(1 - \eta \mathcal{O}(1-k\delta_{2k}) \right)}{\sqrt{1- \eta \mathcal{O}(k^2 \delta_{2k}^2)}}  \text{dist}(\mathbf{B}_t,\mathbf{B}_\ast) 
% \end{align}
% which corresponds to linear convergence for $\delta_{2k} = \mathcal{O}(\nicefrac{1}{k})$ and for any step size $\eta$ satisfying
% \begin{equation}
%   0 < \eta \leq 1 -\mathcal{O}(k \delta_{2k} - k^2 \delta_{2k}^2).
% %   \frac{ \|\hat{v}_{0}\|_2^2}{4\sigma_\ast^2} \frac{(1-\delta_4)^2}{(1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2}\left( \frac{(\langle \mathbf{\hat{b}}_0, \mathbf{\hat{b}}_\ast \rangle( \langle \mathbf{\hat{b}}_0, \mathbf{\hat{b}}_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4))(1-\delta_4)^4}{(1+\delta_4)^4} - {2\sqrt{2} \delta_4 } \right), 
% \end{equation}
% Alternatively,
% \begin{align}
%   \eta \leq \frac{c_1 - c_1 k \delta_{2k} - c_2 k^2 \delta_{2k}^2}{c_1^2(1 -  k \delta_{2k})^2}
% \end{align}
% for some constants $c_1$, $c_2$.

% note that sigma1 is O(1) by normalization of objective and normalization of parameter vectors\|\mathbf{W}_\ast \mathbf{B}_\ast^\top\|. otherwise we have additional sigma factor in objective
%that
%the iterates in $\mathbf{B}$ of FedRep satisfy
% \begin{align}
%     \text{dist}(\hat{V}_{t+1}, V_\ast) \leq \sqrt{1 - \eta} \text{dist}(\hat{V}_{t}, V_\ast)
% \end{align}
% \begin{align}
%     \text{dist}(B_T, B_\ast)
%     &\leq  \frac{\left(1 - \eta \mathcal{O}(1-k\delta_{2k}) \right)^T}{\left(1- \eta \mathcal{O}(k^2 \delta_{2k}^2)\right)^{T/2}}  \text{dist}(B_0,B_\ast) 
% \end{align}



% Given pairs of samples $\{\mathbf{x}_i^j, y_i^j\}_{j=1}^m$ and a fixed representation $\mathbf{B}$, the $i$-th client attempts to learn the head $\mathbf{w}_i \in \mathbb{R}^k$ that solves the following least-squares problem:
% %
% \begin{align} \label{obj:client}
%      f_i(\mathbf{w}_i \circ \mathbf{B}) \coloneqq  \frac{1}{2m}\sum_{j=1}^m ({y}_i - \mathbf{w}_i^\top  \mathbf{B}^\top \mathbf{x}_i^j)^2 \big\}
% \end{align}
% The benefit of learning a representation is that it reduces each client's least squares problem from $\mathbb{R}^d$ to $\mathbb{R}^k$. Of course, this only makes sense if an accurate representation exists for $k \ll d$. Thus,
% Predictions are made by first mapping samples $\mathbf{x} \in \mathbb{R}^d$ to low-dimensional feature vectors $\mathbf{B^\top x} \in \mathbb{R}^k$. Then, a linear regressor $\mathbf{w}\in \mathbb{R}^k$ is applied in the low-dimensional space.
% Thus predictions are given by $q_i(\mathbf{x}_i) = \mathbf{w}_i^\top \mathbf{B}^\top \mathbf{x}_i$. 
% In order to make the learning problem significant, 
% we assume that the data is generated by an unobserved ground-truth orthogonal representation $\mathbf{B}_{\ast}\in \mathbb{R}^{d \times k}$ and unobserved ground-truth heads $\mathbf{w}_{1,\ast},\dots,\mathbf{w}_{n,\ast} \in \mathbb{R}^k$, where $k \ll d$. 
% % In other words, for all $i \in [n]$, each client's optimal solution $\mathbf{B}_\ast \mathbf{w}_{i,\ast}$ belongs to the same $k$-dimensional subspace of $\mathbb{R}^d$, which is spanned by the columns of $\mathbf{B}_\ast$. 
% For simplicity, we consider the noiseless case, i.e.,
% $
% y_i^j = \mathbf{w}_{i,\ast}^\top \mathbf{B}_{\ast}^\top
% \mathbf{x}_i
% $
% for all $i \in [n]$ and $j \in [m]$, as adding noise does not fundamentally change our analysis. 
% The global objective can be written as
% Now, $f_i$ can be rewritten using matrix notation as
% \begin{align}
%     f_i( \mathbf{w}_i \circ \mathbf{B}) = \frac{1}{2m} \| \mathbf{y}_i -  \mathbf{X}_i \mathbf{B} \mathbf{w}_i \|_2^2 
% \end{align}
% where $\mathbf{X}_i = [\mathbf{x}_i^1, \dots, \mathbf{x}_i^m]^\top \in \mathbb{R}^{m \times d}$ contains the feature vectors $\mathbf{x}_i^j$ for the $i$-th user and $\mathbf{y}_i \in \mathbb{R}^m$ contains their corresponding labels, which means that the global objective is equal to
% \begin{align}
%     \min_{\mathbf{B} \in \mathbb{R}^{d \times k}}   \frac{1}{2nm} \sum_{i=1}^n \min_{\mathbf{w}_i \in \mathbb{R}^k} \sum_{j=1}^m ({y}_i - \mathbf{w}_i^\top  \mathbf{B}^\top \mathbf{x}_i^j)^2   \label{linear_obj}
% \end{align}
%, \mathbf{W} \in \mathbb{R}^{n \times k}



% LG-Fed (Salakhutdinov paper) and Fed-MTL are trained with their default learning rates, although unlike in the Salakhutdinov paper, they are not pretrained with FedAvg. 

Define $\mathbf{H} = \mathbf{GD} - \mathbf{C}$ and 
% Then
% Recall that for $k=1$, $\mathbf{D} = \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle \mathbf{I}_n$. Define $D^i = \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle$ for all $i \in [n]$, and
\begin{align}
    \mathbf{H}^i &\coloneqq \mathbf{G}^i \mathbf{D}^i - \mathbf{C}^i = \mathbf{\hat{B}}^\top \mathbf{\Pi} \mathbf{\hat{B}} \mathbf{\hat{B}}^\top \mathbf{\hat{B}}^\ast- \mathbf{\hat{B}}^\top \mathbf{\Pi} \mathbf{\hat{B}}^\ast = \mathbf{\hat{B}}^\top \mathbf{\Pi} (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast, 
\end{align}
for all $i \in [rn]$.
Then we have
\begin{align}
    \|(\mathbf{GD} - \mathbf{C}) \mathbf{w}_\ast\|_2^2
    &= \sum_{i=1}^{rn} \| \mathbf{H}^i  \mathbf{w}_\ast^i\|_2^2 \nonumber \\
    &\leq \sum_{i=1}^{rn} \| \mathbf{H}^i \|_2^2 \|\mathbf{w}^\ast_i\|_2^2\nonumber \\
    &\leq \frac{k}{rn} \|\mathbf{W}^\ast\|_2^2  \sum_{i=1}^{rn}  \| \mathbf{H}^i \|_2^2  \label{rw1}
\end{align}
where the last inequality follows almost surely from Assumption \ref{assump:norm} (the $1$-row-wise incoherence of $\mathbf{{W}}^\ast$) and the fact that $\|\mathbf{W}^\ast\|_F^2 \leq k\|\mathbf{W}^\ast\|_2^2$ as $\mathbf{W}^\ast$ has rank $k$. It remains to bound $\frac{1}{rn}\sum_{i=1}^{rn} \|\mathbf{H}^i\|_2^2$. 
The $\|\mathbf{H}^i\|_2^2$ are i.i.d., but since each $\|\mathbf{H}^i\|_2^2$ is unbounded with possibly heavier-than-exponential tails, we will use a truncated version of the Bernstein inequality, similar to Lemma 29 in \cite{tripuraneni2020provable}. 
%Letting $X^i=\|\mathbf{H}^i\|_2^2$. 
We first state and prove the truncated Bernstein inequality. 
\begin{lemma}[Truncated Matrix Bernstein Inequality \cite{tripuraneni2020provable}]\label{lem:tb}
Suppose $X^1,\dots,X^n$ are independent random variables. Consider a truncation level $R > 0$ and define $\bar{X}^i \coloneqq X^i \chi_{\{X^i \leq R\}}$. Also let $\Delta \geq | \mathbb{E}[X^i] - \mathbb{E}[\bar{X}^i]|$. Then for any $t\geq \Delta$,
\begin{align}
    \mathbb{P}[|\frac{1}{n}\sum_{i=1}^n X^i - \mathbb{E}[{X}^i]| > t] \leq \mathbb{P}[|\frac{1}{n}\sum_{i=1}^n \bar{X}^i - \mathbb{E}[\bar{X}^i]| > t-\Delta] + n \mathbb{P}[| X^i| \geq R]
\end{align}
and 
\begin{align}
 \mathbb{P}[|\frac{1}{n}\sum_{i=1}^n \bar{X}^i - \mathbb{E}[\bar{X}^i]| > t-\Delta] \leq 2 \exp \left(\frac{n^2(t-\Delta)^2}{\sigma^2 + 2Rn/3} \right)
\end{align}
where $\sigma^2 = \sum_{i=1}^n \mathbb{E}[\text{Var}(X^i)] \leq \left|\sum_{i=1}^n \mathbb{E}[(X^i)^2]\right|$.
\end{lemma}
\begin{proof}
The proof is identical to the proof of Lemma 29 in \cite{tripuraneni2020provable} with matrix-valued random variables replaced by scalars.
\end{proof}



To use this lemma we first bound the tail of the distribution of $\|\mathbf{H}^i\|_2^2$.
Then, we upper bound the expected value and variance of $\|\mathbf{H}^i\|_2^2$. Next, we set the truncation level $R$, upper bound the difference between the mean of the original and truncated variables, and finally apply the truncated Bernstein inequality.


\textbf{1. Tail bound:} 
We must compute a tail bound for
$\|\mathbf{H}^i\|_2^2$. 
% \begin{align}
%     \|\mathbf{H}^i\|_F^2 &= \text{Tr}\left(\mathbf{\hat{B}}^\ast^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)  \mathbf{\Pi}^i\mathbf{\hat{B}}\mathbf{\hat{B}}^\top \mathbf{\Pi}^i (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast \right) \nonumber \\
%     &= \sum_{j=1}^m \sum_{j'=1}^m \text{Tr}\left(\mathbf{\hat{B}}^\ast^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \mathbf{\hat{B}}\mathbf{\hat{B}}^\top \mathbf{x}_i^{j'} (\mathbf{x}_i^{j'})^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast \right) \nonumber \\
%     &= \sum_{j=1}^m \sum_{j'=1}^m \text{Tr}\left( \mathbf{u}_i^j (\mathbf{v}_i^j)^\top \mathbf{v}_i^{j'} (\mathbf{u}_i^{j'})^\top \right) \nonumber \\\
%     &= \sum_{l=1}^k \sum_{j=1}^m \sum_{j'=1}^m \langle \mathbf{e}_l,  \mathbf{v}_i^j \rangle \langle  \mathbf{u}_i^j, \mathbf{u}_i^{j'} \rangle \langle \mathbf{v}_i^{j'}, \mathbf{e}_l \rangle \nonumber \\\
%     &= \sum_{l=1}^k \| \sum_{j=1}^m  (\mathbf{v}_i^j)_l \mathbf{u}_i^j \|_2^2 \nonumber \\
%     &=  \sum_{l=1}^k \|\mathbf{\hat{B}}^\ast^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{X}_i^\top \mathbf{X}_i \mathbf{b}_l \|_2^2 \nonumber
% \end{align}
Note that $\| \mathbf{H}^i\|_2^2 = \|\frac{1}{m}(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{X}_i^\top \mathbf{X}_i  \mathbf{\hat{B}}\|_2^2$. Let $\mathbf{U} \coloneqq \frac{1}{\sqrt{m}}\mathbf{X}_i(\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast$ then the $j$-th row of $\mathbf{U}$ is given by $$\mathbf{u}_j = \frac{1}{\sqrt{m}} \mathbf{\hat{B}}^{\ast^\top}(\mathbf{\hat{B}}\mathbf{\hat{B}}^\top - \mathbf{I}_d)\mathbf{x}_i^j,$$ and is $\frac{1}{\sqrt{m}} \|\mathbf{\hat{B}}^{\ast^\top}(\mathbf{\hat{B}}\mathbf{\hat{B}}^\top - \mathbf{I}_d)\|_2=\frac{1}{\sqrt{m}}\text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)$-sub-gaussian. Likewise, define $\mathbf{V} \coloneqq \frac{1}{\sqrt{m}} \mathbf{X}_i \mathbf{\hat{B}}$, then the $j$-th row of $\mathbf{V}$ is $$ \mathbf{v}_j = \frac{1}{\sqrt{m}} \mathbf{\hat{B}}^\top\mathbf{x}_i^j,$$ therefore is $\frac{1}{\sqrt{m}} \|\mathbf{\hat{B}}\|_2= \frac{1}{\sqrt{m}}$-sub-gaussian. 
We aim to upper bound $\mathbb{P}(\|(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{X}_i^\top \mathbf{X}_i  \mathbf{B}\|_2^2 > t ) = \mathbb{P}(\|\mathbf{U}^\top \mathbf{V} \|_2^2 > t ) $. 
% Note that $\mathbb{E} [\mathbf{U}^\top \mathbf{V} ] = (\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{B} =\mathbf{0}$, so we alternatively desire an upper bound on $\mathbb{P}(\|\mathbf{U}^\top \mathbf{V}  - \mathbb{E}[\mathbf{U}^\top \mathbf{V}]\|_2^2 > t )$. 

We leverage the sub-gaussianity of the rows of $\mathbf{U}$ and $\mathbf{V}$ to make a similar argument as in Proposition 4.4.5 in \cite{vershynin2018high}. First, let $\mathcal{S}^{k-1}$ denote the unit sphere in $k$ dimensions, and let $\mathcal{N}_k$ be a $\frac{1}{4}$-th net of cardinality $|\mathcal{N}|\leq 9^k$, which exists by Corollary 4.2.13 in \cite{vershynin2018high}. Next, using equation 4.13 in \cite{vershynin2018high}, we obtain
\begin{align}
  \|(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{X}_i^\top \mathbf{X}_i  \mathbf{B}\|_2=  \left\| \mathbf{U}^\top \mathbf{V}  \right\|_2 &\leq 2 \max_{\mathbf{z},\mathbf{y}  \in \mathcal{N}_k}  \mathbf{z}^\top \left( \mathbf{U}^\top \mathbf{V} \right)\mathbf{y} \nonumber \\
    &= 2 \max_{\mathbf{z}, \mathbf{y} \in \mathcal{N}_k} \mathbf{z}^\top\left(\sum_{j=1}^m  \mathbf{u}_j  \mathbf{v}_j^\top\right)\mathbf{y} \nonumber \\
    &= 2 \max_{\mathbf{z}, \mathbf{y} \in \mathcal{N}_k} \sum_{j=1}^m \langle \mathbf{z},  \mathbf{u}_j\rangle \langle \mathbf{v}_j,\mathbf{y} \rangle \nonumber 
\end{align}
By definition of sub-gaussianity, $\langle \mathbf{z},  \mathbf{u}_j\rangle$ and $\langle \mathbf{v}_j,\mathbf{y} \rangle$ are sub-gaussian with norms $\frac{1}{\sqrt{m}}\text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)$ and $\frac{1}{\sqrt{m}}$, respectively. Thus for all $j\in [m]$, $\langle \mathbf{z},  \mathbf{u}_j\rangle \langle \mathbf{v}_j,\mathbf{z} \rangle $ is sub-exponential with norm $\frac{c}{m} \text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)$ for some absolute constant $c$.  
Note that for any $j \in [m]$ and any $\mathbf{z}$, $\mathbb{E}[\langle \mathbf{z},  \mathbf{u}_j\rangle \langle \mathbf{v}_j,\mathbf{y} \rangle] = \mathbf{z}^\top ((\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{B}) \mathbf{y} = 0$. Thus we have a sum of $m$ mean-zero, independent sub-exponential random variables. We can now use Bernstein's inequality to obtain, for any fixed $\mathbf{z}, \mathbf{y} \in \mathcal{N}_k$,
\begin{align}
    \mathbb{P}\left(\sum_{j=1}^m \langle \mathbf{z},  \mathbf{u}_j\rangle \langle \mathbf{v}_j,\mathbf{y} \rangle \geq s  \right) \leq \exp \left(-c' m \min\left(\frac{s^2}{\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast) }, \frac{s}{\text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)} \right)\right)
\end{align}
Now union bound over all $\mathbf{z}, \mathbf{y} \in \mathcal{N}_k$ to obtain
\begin{align}
\mathbb{P}\left( \|(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{X}_i^\top \mathbf{X}_i  \mathbf{\hat{B}}\|_2 \geq 2s \right) &\leq 9^{2k} \exp \left(-c' m \min(s^2/\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast) , s/\text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast) )\right)
\end{align}
Let $\frac{s}{\text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)} = \max(\varepsilon, \varepsilon^2)$ for some $\epsilon > 0$, then it follows that $\min(s^2/\text{dist}^2(\mathbf{\hat{B}},\mathbf{\hat{B}}^\ast), s/\text{dist}(\mathbf{\hat{B}},\mathbf{\hat{B}}^\ast)) = \varepsilon^2$. So we have
\begin{align}
    \mathbb{P}\left( \|(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{X}_i^\top \mathbf{X}_i  \mathbf{\hat{B}}\|_2 \geq 2\text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)\max(\varepsilon, \varepsilon^2) \right) &\leq 9^{2k} e^{-c' m \varepsilon^2 }
\end{align}
Moreover, letting $\varepsilon^2 = \frac{ck^2\log(rn)}{4m}$ for some constant $c$, and $m \geq ck^2\log(rn)$, we have
\begin{align}
    \mathbb{P}\left( \|(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{X}_i^\top \mathbf{X}_i  \mathbf{\hat{B}}\|_2 \geq \text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast) \sqrt{\frac{ck^2\log(rn)}{m}} \right)&\leq 9^{2k} e^{-c_1 k^2 
    \log(rn)}\nonumber \\
    &\leq e^{ - 100 k^2 
    \log(rn)}
\end{align}
for large enough constant $c_1$. Thus, noting that $\|\mathbf{H}^i \|_2^2 =\|(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{X}_i^\top \mathbf{X}_i  \mathbf{\hat{B}}\|_2^2$, we obtain
\begin{align}
    \mathbb{P}\left( \|\mathbf{H}^i\|_2^2 \geq c\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast) {\frac{k^2\log(rn)}{m}} \right)
    &\leq e^{ - 100 k^2 \log(rn)}
\end{align}
%Using this notation, we have
% \begin{align}
    % \mathbb{P}(\|(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{X}_i^\top \mathbf{X}_i  \mathbf{B}\|_2^2 > t ) &= \mathbb{P}(\|\mathbf{U}^\top \mathbf{V} - \mathbb{E}[\mathbf{U}^\top \mathbf{V}] \|_2^2 > t ) \nonumber \\
    % &= \mathbb{P}(\|\mathbf{U}^\top \mathbf{V} - \mathbb{E}[\mathbf{U}^\top \mathbf{V}] \|_2^2 > t )
% \end{align}
% use Vershynin 4.6.1, covering and Bernstein, the key is that our sub-exponential rvs have mean 0.
% We obtain, letting $D$ be the distance,
% \begin{align}
%     \mathbb{P}(\|\mathbf{H}_i\|_2^2 > D^2 (\frac{k+t^2}{m}) ) \leq e^{-t^2}
% \end{align}
Now we set the truncation level $R = c\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)\frac{k^2 \log(rn)}{m}$.
% $= D^2\frac{k+t^2}{m}$. 
% Then $t^2 = k^2 \log^2(n) - k \equiv k^2\log^2(n)$ and $e^{-t^2} = e^{-k^2\log^2(n)}$.

% We need
% \begin{align}
%     \mathbb{P}\left( \| (\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{X} \mathbf{X} \mathbf{b}_l \|_2^2 \right)
% \end{align}

%Since $\mathbf{u}_i^j$ is $\frac{1}{\sqrt{m}}(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)$-sub-gaussian, $\|\mathbf{u}_i^j\|_2^2$ is sub-exponential with norm $\frac{c'\sqrt{k}}{m}\; \text{dist}^{2}(\mathbf{\hat{B}},\mathbf{\hat{B}}_\ast)$, and $\|\mathbf{u}_i^j\|_2$ is sub-gaussian with norm $\frac{c{k}^{1/4}}{\sqrt{m}} \text{dist}(\mathbf{\hat{B}},\mathbf{\hat{B}}_\ast)$, for some absolute constants $c, c'$. Similarly, $\|\mathbf{v}_i^j\|_2$ is sub-exponential with norm $\frac{c{k}^{1/4}}{\sqrt{m}}$. Therefore, $\|\mathbf{u}_i^j\|_2\|\|\mathbf{v}_i^j\|_2$ is sub-exponential with norm $\frac{c\sqrt{k}\;\text{dist}(\mathbf{\hat{B}},\mathbf{\hat{B}}_\ast)}{{m}}$. Further, $\sum_{j=1}^m  \|\mathbf{u}_i^j\|_2\|\|\mathbf{v}_i^j\|_2$ is sub-exponential with norm $\frac{c\sqrt{k}\;\text{dist}(\mathbf{\hat{B}},\mathbf{\hat{B}}_\ast)}{\sqrt{m}}$. 




\textbf{2. Bound on } $\Delta$\textbf{:}
Recall 

We have
\begin{align}
    \Delta &= \mid \mathbb{E}[X_i]  - \mathbb{E}[\bar{X}^i] \mid \nonumber \\
    &= \mathbb{E}[X^i \chi_{\{X^i \geq R\}}] \nonumber \\
    &\leq \int_R^\infty z \mathbb{P}(X^i \geq z) dz \nonumber \\
    &\leq \int_R^\infty z e^{-100k^2\log(rn)} dz \nonumber \\
    &= - \frac{2 e^{-100k^2\log(rn)}( z^2 m^2 + 3 zm (\sqrt{zm} + 2)+ 6\sqrt{zm} )}{m^2 \sqrt{zm}} \Big|_{z=R}^\infty \nonumber \\
    &= \frac{2 e^{-\sqrt{Rm}}( R^2 m^2 + 3 Rm (\sqrt{Rm} + 2)+ 6\sqrt{Rm} )}{m^2 \sqrt{Rm}} \nonumber \\
    &\leq \tfrac{cR^{1.5}}{\sqrt{m}}e^{-\sqrt{Rm}} \nonumber
\end{align}
for some constant factor $c$.

Replace $e^{-\sqrt{Rm}}$ by $e^{-100k^2\log(rn)}$ and set $R$ appropriately. Then we have that $\Delta$ is order-wise less than $t$.






\textbf{4. Bound on } $\mathbb{E}\left[\|\mathbf{H}^i\|_2^2\right]$\textbf{:}
We bound $\mathbb{E}\left[\|\mathbf{H}^i\|_2^2\right]$ using similar analysis as in the bound on $\mathbb{E}[\|\mathbf{u}^i\|_2 \|\mathbf{v}^i\|_2 ]$ in $\eqref{raankk2}$. In particular, observe that
\begin{align}
    \mathbb{E}[\|\mathbf{H}^i\|_2^2] &=\mathbb{E}[\|\mathbf{\hat{B}}^\top \mathbf{\Pi}^i (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}_\ast\|_2^2]  \nonumber \\
    &\leq \mathbb{E}[\|\mathbf{\hat{B}}^\top \mathbf{\Pi}^i (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}_\ast\|_F^2] \nonumber \\
    &= \mathbb{E}\left[\text{Tr}\left((\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)  \mathbf{\Pi}^i\mathbf{\hat{B}}\mathbf{\hat{B}}^\top \mathbf{\Pi}^i (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast\right)\right] \nonumber \\
    &= \sum_{j=1}^m \sum_{j'=1, j' \neq j}^m  \mathbb{E}\left[\text{Tr}\left((\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \mathbf{\hat{B}}\mathbf{\hat{B}}^\top \mathbf{x}_i^{j'} (\mathbf{x}_i^{j'})^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast\right)\right] \nonumber \\
    &\quad \quad \quad \quad +\sum_{j=1}^m  \mathbb{E}\left[\text{Tr}\left((\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \mathbf{\hat{B}}\mathbf{\hat{B}}^\top \mathbf{x}_i^{j} (\mathbf{x}_i^{j})^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast\right)\right]  \nonumber \\
    &= \sum_{j=1}^m  \mathbb{E}\left[\text{Tr}\left((\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^j (\mathbf{x}_i^j)^\top \mathbf{\hat{B}}\mathbf{\hat{B}}^\top \mathbf{x}_i^{j} (\mathbf{x}_i^{j})^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast\right)\right] \label{exp1}
\end{align}
Since the random vectors $\mathbf{x}_i^j$ are $\frac{1}{\sqrt{m}}\mathbf{I}_d$-sub-gaussian, 
%with covariance $\frac{1}{m}\mathbf{I}_d$, 
the random vectors $\mathbf{u}_i^j \coloneqq (\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) \mathbf{x}_i^j$ are $\frac{1}{\sqrt{m}}(\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{I}_d (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast= \frac{1}{\sqrt{m}}(\mathbf{I}_k - (\mathbf{\hat{B}}^\ast)^\top \mathbf{\hat{B}} \mathbf{\hat{B}}^\top \mathbf{\hat{B}}_\ast)$-sub-gaussian.
%with covariance $\frac{1}{{m}}(\mathbf{I}_k - (\mathbf{\hat{B}}^\ast)^\top \mathbf{\hat{B}} \mathbf{\hat{B}}^\top \mathbf{\hat{B}}_\ast)$.
Similarly, the random vectors $\mathbf{v}_i^j \coloneqq \mathbf{\hat{B}}^\top \mathbf{x}_i^{j}$
are $\frac{1}{\sqrt{m}}\mathbf{I}_k$-sub-gaussian. 
%with covariance $\frac{1}{{m}}\mathbf{I}_k$).
Thus, arguing similarly as in Lemma 27 in \citep{tripuraneni2020provable}, we have
\begin{align}
    \mathbb{E}\Big[\text{Tr}\Big((\mathbf{\hat{B}}^\ast)^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d) &\mathbf{x}_i^j (\mathbf{x}_i^j)^\top \mathbf{\hat{B}}\mathbf{\hat{B}}^\top \mathbf{x}_i^{j} (\mathbf{x}_i^{j})^\top (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top -  \mathbf{I}_d)\mathbf{\hat{B}}^\ast\Big)\Big] \nonumber \\
    &= \mathbb{E}\left[\text{Tr}\left( \mathbf{u}_i^j (\mathbf{v}_i^j)^\top \mathbf{v}_i^{j} (\mathbf{u}_i^{j})^\top \right)\right] \nonumber \\
    &= \mathbb{E}\left[\| \mathbf{u}_i^j\|_2^2 \; \|\mathbf{v}_i^{j} \|_2^2\right] \nonumber \\
    &= \mathbb{E}\left[\sum_{p,q=1}^k \langle \mathbf{u}_i^j, \mathbf{e}_p\rangle^2 \; \langle \mathbf{v}_i^j, \mathbf{e}_q\rangle^2\right] \nonumber \\
    &\leq \sum_{p,q=1}^k \left( \mathbb{E}\left[\langle \mathbf{u}_i^j, \mathbf{e}_p\rangle^4\right] \; \mathbb{E}\left[\langle \mathbf{v}_i^j, \mathbf{e}_q\rangle^4\right] \right)^{1/2} \label{cau1} \\
    &\leq \frac{c}{m^2} \sum_{p,q=1}^k  \| \mathbf{I}_k - (\mathbf{\hat{B}}^\ast)^\top \mathbf{\hat{B}} \mathbf{\hat{B}}^\top \mathbf{\hat{B}}_\ast\|_2^2 \label{sg1}  \\
    &= \frac{ck^2}{m^2}  \text{dist}^2(\mathbf{\hat{B}},\mathbf{\hat{B}}_\ast) \label{sg2}
\end{align}
where \eqref{cau1} follows from the Cauchy-Schwarz inequality and \eqref{sg1} follows because the sub-gaussian norm of $\mathbf{u}_i^j$ (respectively $\mathbf{v}_i^j$) is at most $\frac{c}{\sqrt{m}}\|\mathbf{I}_k - (\mathbf{\hat{B}}^\ast)^\top \mathbf{\hat{B}} \mathbf{\hat{B}}^\top \mathbf{\hat{B}}_\ast\|_2$ (respectively $\frac{c}{\sqrt{m}}\| \mathbf{I}_k \|_2 = \frac{c}{\sqrt{m}}$) for some absolute constant $c$, and finally \eqref{sg2} follows because $\| \mathbf{I}_k - (\mathbf{\hat{B}}^\ast)^\top \mathbf{\hat{B}} \mathbf{\hat{B}}^\top \mathbf{\hat{B}}_\ast\|_2 = \|(\mathbf{\hat{B}}^\ast)^\top( \mathbf{I}_d - \mathbf{\hat{B}} \mathbf{\hat{B}}^\top) \mathbf{\hat{B}}_\ast\|_2 \leq \|(\mathbf{\hat{B}}^\ast)^\top( \mathbf{I}_d -  \mathbf{\hat{B}} \mathbf{\hat{B}}^\top)\|_2 = \text{dist}(\mathbf{\hat{B}},\mathbf{\hat{B}}_\ast)$. Substituting this back into \eqref{exp1} yields
\begin{align}
    \mathbb{E}[\|\mathbf{H}^i\|_2^2] &\leq \frac{ck^2}{m}  \text{dist}^2(\mathbf{\hat{B}},\mathbf{\hat{B}}_\ast) \label{exphi}
\end{align}
We have
\begin{align}
    \mathbb{E}[\|\mathbf{H}^i\|_2] &\leq \frac{ck^2}{m}  \text{dist}^2(\mathbf{\hat{B}},\mathbf{\hat{B}}_\ast) \label{exphi1}
\end{align}

\textbf{3. Bound on } $\text{Var} \left[\|\mathbf{H}^i\|_2^2\right]$\textbf{:}

 We have
\begin{align}
    \|(\mathbf{GD} - \mathbf{C})\hat{\mathbf{u}}_\ast\|_2^2
    &= \sum_{i=1}^n \hat{u}_{\ast,i}^2 (H^i)^2 \nonumber \\
    &= \sum_{i=1}^n \hat{u}_{\ast,i}^2 \sum_{j=1}^m  \sum_{j'=1}^m H_j^i H_{j'}^i \nonumber
\end{align}
Assume that $\mathbf{u}_{\ast}$ is incoherent, then we have
\begin{align}
    \|(\mathbf{GD} - \mathbf{C})\hat{\mathbf{u}}_\ast\|_2^2
    &\leq \frac{\mu^2}{n} \sum_{i=1}^n  \sum_{j=1}^m  \sum_{j'=1}^m H_j^i H_{j'}^i \nonumber 
\end{align}
where $H_j^i = \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle$ is a sub-exponential random variable with mean zero and norm $O(1/m)$. 

Assume temporarily that the data is Gaussian. 
% (** obviously if the data is generically sub-gaussian then we will not have this exact result but we will still have that the below expectation is $O(1/m)$, which is sufficient for our proof.).
Note that since $\mathbb{E}[H_j^i]=0$ and $H_j^i$ and $H_{j'}^i$ are independent for $j\neq j'$, we have that 
\begin{align}
    \mathbb{E}[\sum_{j=1}^m  \sum_{j'=1}^m H_j^i H_{j'}^i]&= \sum_{j=1}^m  \mathbb{E}[( H_j^i)^2] \nonumber \\
    &= \sum_{j=1}^m  \mathbb{E}[ \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2
     - 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle  + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 ] \nonumber \\
%      &= \sum_{j=1}^m  \mathbb{E}[ \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2
%   + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 ]  \nonumber \\
  &= \sum_{j=1}^m \bigg( \sum_{\ell=1}^d \frac{3\hat{{v}}_\ell^4}{m^2} \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 + \sum_{\ell=1}^d \sum_{\ell'=1, \ell' \neq \ell}^d \frac{3 \hat{{v}}_\ell^2 \hat{{v}}_{\ell'}^2}{m^2} \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 + \sum_{\ell=1}^d \frac{3\hat{{v}}_\ell^2\hat{{v}}_{\ast,\ell}^2}{m^2}  
  + \sum_{\ell=1}^d \sum_{\ell'\neq\ell, \ell'=1}^d \frac{\hat{{v}}_\ell^2\hat{{v}}_{\ast,\ell'}^2 + 2 \hat{{v}}_\ell \hat{{v}}_{\ell'}\hat{{v}}_{\ast,\ell}\hat{{v}}_{\ast,\ell'}}{m^2} \nonumber \\
  &\quad - \frac{2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle}{m^2} \sum_{\ell=1}^d 3 v_\ell^3 v_{\ast,\ell} - \frac{2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle}{m^2} \sum_{\ell=1}^d \sum_{\ell'\neq\ell, \ell'=1}^d 3v_\ell^2 v_{\ell'} v_{\ast,\ell'} \bigg) \nonumber \\
  &= \frac{1}{m^2} \sum_{j=1}^m \bigg(  3\langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 
  + 1 + 2\langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2  - 6 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 \bigg) \nonumber \\
  &= \frac{1}{m} ( 1 - \langle\hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 ) \nonumber \\
  &= \frac{1}{m} \text{dist}^2(\hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast)
\end{align}
So $\mathbf{F}$ gets smaller as we have more samples and as $\mathbf{v}$ approaches $\mathbf{v}_\ast$, this makes sense. With many samples we can easily see from \eqref{hi} that $H^i \rightarrow 0$. On the other hand, when $m=1$, we have that $|\langle \mathbf{\hat{B}}, \mathbf{\hat{B}}_\ast\rangle| = 1  \implies \hat{\mathbf{v}} = \pm \hat{\mathbf{v}}_\ast \implies H^i = 0$.

Note that $\|(\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast\|_2^2$ is weighted sum of $nm^2$ random variables $H^i_{j} H^i_{j'}$. We have
\begin{align}
    \mathbb{E}[(H^i_{j})^2 (H^i_{j'})^2] &\leq \mathbb{E}[(H^i_{j})^4] \nonumber \\
    &= \mathbb{E}[(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle )^4] \nonumber \\
    &= \mathbb{E}[(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 - 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle +  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2)(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle )^2] \nonumber \\
    &\leq \mathbb{E}[(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 - 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle +  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2) \nonumber \\
    &\quad \quad \quad \quad \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 (\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2 - 2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 )] \nonumber \\
    &\leq \mathbb{E}[(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 - 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2) \nonumber \\
    &\quad \quad \quad \quad \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 (\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2  - 2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 )] \nonumber \\
    &= \mathbb{E}[\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 
    - 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle 
    - 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^3 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle 
    + 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2
    \nonumber \\
    &\quad \quad \quad \quad \quad \quad + 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2
    + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^4) \nonumber \\
    &\leq \mathbb{E}[\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4(\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^4 
    - 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^3 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle 
    - 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^3 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle 
    + 4\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2
    \nonumber \\
    &\quad \quad \quad \quad \quad \quad + 2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^2
    + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle^4)  \nonumber \\
    &\leq 16 \mathbb{E}[\langle \mathbf{x}_{i}^j, \tilde{\mathbf{v}}\rangle^8] \nonumber
\end{align}
where $\tilde{\mathbf{v}} = \arg \max_{\mathbf{v} \in \{  \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \}} \langle \mathbf{x}_{i}^j, {\mathbf{v}} \rangle^2$. 
Note that $\langle \mathbf{x}_{i}^j, \tilde{\mathbf{v}}\rangle$ is subgaussian with norm $\|\tilde{\mathbf{v}}\|_2/\sqrt{m}= 1/\sqrt{m}$ (variance $1/m$). So we have 
\begin{align}
    \mathbb{E}[(H^i_{j})^2 (H^i_{j'})^2]
&\leq \frac{c}{m^4} \nonumber
\end{align}

for some absolute constant $c$. Therefore, $X^i \coloneqq \sum_{j=1}^m \sum_{j'=1}^m H^i_{j} H^i_{j'}$ has variance
\begin{align}
    \text{Var}(X^i) &= \mathbb{E}[ (\sum_{j=1}^m \sum_{j'=1}^m H^i_{j} H^i_{j'} - \bar{r})^2 ] \nonumber \\
    &\leq \left( {m \choose 2}{4 \choose 2} + {m\choose 1}  \right) \mathbb{E}[(H_{j}^i)^4] \nonumber \\
    &\leq \frac{c}{m^2}
\end{align}
where the first inequality follows by a simple counting argument: there are at most $ {m \choose 2}{4 \choose 2} + {m\choose 1}  $ terms in the square with even-order powers of the $H_j^i$'s, which have expectation bounded above by $\mathbb{E}[(H_{j}^i)^4]$. All other terms have expectation zero.


\textbf{5. Conclusion:}
% $t = \frac{\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}_\ast) \sigma_{\min}^2(\mathbf{\Sigma}_\ast)}{k^2\|\mathbf{\Sigma}_\ast\|_2^4}$
Setting $t = \frac{ k^2}{m}\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}_\ast) \log^{2}(n)$, 
\begin{align}
 \mathbb{P}[|\frac{1}{n}\sum_{i=1}^n \bar{X}^i - \mathbb{E}[\bar{X}^i]| > t-\Delta] &\leq 2 \exp \left(\frac{n^2(t-\Delta)^2}{\sigma^2 + 2Rn/3} \right) \nonumber \\
 &\leq 2 \exp \left(\frac{n^2(t-\Delta)^2}{\sigma^2 + 2Rn/3} \right) \nonumber \\
\end{align}



We finally obtain
\begin{align}
    \|(\mathbf{GD}-\mathbf{C}) \mathbf{\Lambda} \mathbf{w}_\ast \|_2^2 \leq \frac{\mu^2 \|\mathbf{\Sigma}_\ast\|_2^2 k^3 \log^2(n) D^2}{m}
\end{align}
with probability at least $1-e^{-n} - ne^{-k^2 \log^2(n)}$. 

% --------

% and using a union bound over $i \in [n]$, we obtain:
% \begin{align}
%     \mathbb{P}\left(\frac{1}{n} \sum_{i=1}^n \|\mathbf{H}^i\|_2^2 >  \frac{10^4 k^2}{m}\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}_\ast) \log^{2}(n)  \right) \leq n \exp \left(-100 c  \log(rn)\right) = n^{-100}
% \end{align}
% Plugging this back into \eqref{rw1},
% %and 
% %letting 
% % $m = C\frac{\sigma_{\max}^4(\mathbf{\Sigma}_\ast) }{\sigma_{\min}^2(\mathbf{\Sigma}_\ast)}k^4 \log^2(n)$ for some sufficiently large constant $C$, 
% we have
% \begin{align}
%     \|(\mathbf{GD} - \mathbf{C}) \mathbf{\Lambda}\mathbf{w}_\ast\|_2^2
%     &\leq {\mu^2 k} \|\mathbf{\Sigma}_\ast\|_2^2 \left(\mathbb{E}[\|\mathbf{H}^1\|_2^2] + \frac{k^2}{m}\delta_k\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}_\ast) \log^{2}(n)\right) \nonumber \\
%     &\leq {\mu^2 k} \|\mathbf{\Sigma}_\ast\|_2^2 \left(\frac{ck^2\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}_\ast)}{m} + \frac{k^2}{m}\delta_k\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}_\ast) \log^{2}(n)\right) \nonumber \\
%     &\leq \frac{c\mu^2 k^3  \log^2(n) \|\mathbf{\Sigma}_\ast\|_2^2 }{m}\text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}_\ast)
% \end{align}
% with probability at least $n^{\left(-(c \sqrt{k}-1)\right)}$. Taking the square root of both sides completes the proof.
% % Combining this with \eqref{} via a union bound completes the proof. 


Returning to \eqref{inco0}, we have
\begin{align}
    \frac{1}{n}\| \mathcal{A}^\ast \mathcal{A}(\mathbf{Q}) - \mathbf{Q}\|_F^2 &= \frac{1}{n}\sum_{i=1}^n  \left( \sum_{j=1}^m \left( \sum_{i'=1}^n \sum_{j'=1}^m \left(\langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle \langle \mathbf{x}_{i'}^{j'}, \mathbf{q}_{i'} \rangle \langle \mathbf{x}^{j}_i, \mathbf{x}^{j'}_{i'} \rangle\right) - 2 \langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle^2  \right) + \langle \mathbf{q}_i, \mathbf{q}_i \rangle\right) \nonumber \\
    &= \frac{1}{n}\sum_{i=1}^n   \sum_{j=1}^m  \sum_{i'=1}^n \sum_{j'=1}^m \left(\langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle \langle \mathbf{x}_{i'}^{j'}, \mathbf{q}_{i'} \rangle \langle \mathbf{x}^{j}_i, \mathbf{x}^{j'}_{i'} \rangle - \frac{2}{nm} \langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle^2 + \frac{1}{nm^2}\langle \mathbf{q}_i, \mathbf{q}_i \rangle\right) \nonumber \\
    &= \frac{1}{n}\sum_{i=1}^n   \sum_{j=1}^m  \sum_{i'=1}^n \sum_{j'=1}^m \left(\langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle \langle \mathbf{x}_{i'}^{j'}, \mathbf{q}_{i'} \rangle \langle \mathbf{x}^{j}_i, \mathbf{x}^{j'}_{i'} \rangle - \frac{2}{nm} \langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle^2 + \frac{1}{n^2m^2}\right) \nonumber \\
    &= \frac{1}{n}\sum_{i=1}^n   \sum_{j=1}^m  \sum_{i'=1}^n \sum_{j'=1}^m H_{i,i'}^{j,j'} \nonumber %\\
    %\sum_{i=1}^n   \sum_{j=1}^m  \sum_{i'=1}^n \sum_{j'=1}^m H_i^j H_{} 
\end{align}
We show that the above quantity is close to zero with high probability in two steps: 1) show the mean goes to zero; 2) show concentration to the mean. For the first step, we have
\begin{align}
    \mathbb{E}[ \tfrac{1}{n} \| \mathcal{A}^\ast \mathcal{A}(\mathbf{Q}) - \mathbf{Q}\|_F^2 ] &=  \frac{1}{n}\sum_{i=1}^n   \sum_{j=1}^m  \sum_{i'=1}^n \sum_{j'=1}^m \mathbb{E}\left[\langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle \langle \mathbf{x}_{i'}^{j'}, \mathbf{q}_{i'} \rangle \langle \mathbf{x}^{j}_i, \mathbf{x}^{j'}_{i'} \rangle - \frac{2}{nm} \langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle^2 + \frac{1}{n^2m^2}\right] \nonumber \\  
    &= -\frac{1}{n} + \frac{1}{n}\sum_{ij=1}^{nm}  \mathbb{E}\left[\langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle \langle \mathbf{x}_{i}^{j}, \mathbf{q}_{i} \rangle \langle \mathbf{x}^{j}_i, \mathbf{x}^{j}_{i} \rangle\right] + \frac{1}{n}\sum_{ij=1}^{nm}  \sum_{i'j'=1, i'j' \neq ij}^{nm} \mathbb{E}\left[\langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle \langle \mathbf{x}_{i'}^{j'}, \mathbf{q}_{i'} \rangle \langle \mathbf{x}^{j}_i, \mathbf{x}^{j'}_{i'} \rangle\right] \label{tthree}
\end{align}
We bound the second term as follows:
\begin{align}
    \frac{1}{n}\sum_{ij=1}^{nm}  \mathbb{E}\left[\langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle \langle \mathbf{x}_{i}^{j}, \mathbf{q}_{i} \rangle \langle \mathbf{x}^{j}_i, \mathbf{x}^{j}_{i} \rangle\right] &\leq \frac{c}{n}\sum_{ij=1}^{nm} \frac{\|\mathbf{q}_i\|_2^2 d}{m^2}  %\frac{c}{n}\sum_{ij=1}^{nm}  \mathbb{E}[\|\mathbf{x}_i^j\|_2^4]
  \label{subg1} \\
    &\leq  \frac{c}{n}\sum_{ij=1}^{nm} \frac{\tilde{\mu} d}{nm^2}  %\frac{c}{n}\sum_{ij=1}^{nm}  \mathbb{E}[\|\mathbf{x}_i^j\|_2^4]
 \label{subg2} \\
    &= \frac{c \tilde{\mu} d}{nm}  %\frac{c}{n}\sum_{ij=1}^{nm}  \mathbb{E}[\|\mathbf{x}_i^j\|_2^4]
\end{align}
where \eqref{subg1} follows from the sub-gaussian property of $\mathbf{x}_i^j$ and \eqref{subg2} follows from the incoherence of $\mathbf{q}_i$ as shown in Lemma \ref{lem:incoherent}. The third term of \eqref{tthree} can be bounded as follows, using the covariance of $\mathbf{x}_{i}^j$ and the fact that $\|\mathbf{Q}\|_F^2 = 1$.
\begin{align}
\frac{1}{n}\sum_{ij=1}^{nm}  \sum_{i'j'=1, i'j' \neq ij}^{nm} \mathbb{E}\left[\langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle \langle \mathbf{x}_{i'}^{j'}, \mathbf{q}_{i'} \rangle \langle \mathbf{x}^{j}_i, \mathbf{x}^{j'}_{i'} \rangle\right] 
    &=  \frac{1}{nm^2} \sum_{ij=1}^{nm}  \sum_{i'j'=1, i'j' \neq ij}^{nm} \mathbb{E}\left[\mathbf{q}_i^\top \mathbf{x}_i^{j}  (\mathbf{x}^{j}_i)^\top \mathbf{x}^{j'}_{i'} (\mathbf{x}_{i'}^{j'})^\top \mathbf{q}_{i'} \right]   \nonumber \\
    &=  \frac{1}{nm^2} \sum_{ij=1}^{nm}  \sum_{i'j'=1, i'j' \neq ij}^{nm} \langle \mathbf{q}_i, \mathbf{q}_{i'} \rangle   \nonumber \\
    &= \frac{1}{n} \sum_{i=1}^{n}  \sum_{i'=1}^{n} \langle \mathbf{q}_i, \mathbf{q}_{i'} \rangle \nonumber \\
    &= \frac{1}{n} \sum_{i=1}^{n} \|\mathbf{Q} \mathbf{q}_i\|_F^2 \nonumber \\
     &\leq \frac{1}{n} \sum_{i=1}^{n} \|\mathbf{Q}\|_F^2 \| \mathbf{q}_i\|_F^2 \nonumber \\
     &=  \frac{1}{n} 
\end{align}
We thus have
\begin{align}
    \mathbb{E}[ \tfrac{1}{n} \| \mathcal{A}^\ast \mathcal{A}(\mathbf{Q}) - \mathbf{Q}\|_F^2 ] 
     &\leq \frac{c \tilde{\mu} d}{nm}  
\end{align}




% Now we show concentration to the mean. Each $H_{i,i'}^{j,j'}$ is a degree-4 polynomial of sub-gaussians. 



We next bound the Frobenius norm of the error matrix $\mathbf{Q}^{t+1}$.
% \textbf{Bound on (1.):}
\begin{lemma} \label{lem:qt}
The Frobenius norm of $\mathbf{Q}^{t+1} \coloneqq \mathbf{W}_{t+1}\hat{\mathbf{B}}_{t} - \mathbf{M}_\ast$, i.e. the difference between the current iterates of FedRep and the ground-truth matrix, is bounded above as follows
\begin{align}
    \| \mathbf{Q}^{t+1} \|_F = \| \mathbf{W}^{t+1} \hat{\mathbf{B}}_t^\top - \mathbf{M}_\ast \|_F &\leq  \frac{\sqrt{k}}{1-\delta_{k}}\; \|\mathbf{\Sigma}_\ast\|_2 \; \text{dist}(\hat{\mathbf{B}}_t, \hat{\mathbf{B}}_\ast)
\end{align}
with probability at least $1 - e^{}$
\end{lemma}

\begin{proof}
We use the definition of $\hat{\mathbf{W}}_{t+1}$, the triangle and Cauchy Schwarz inequalities, and the concentration of $\mathbf{F}$ from Lemma \ref{lem:f}:
\begin{align}
    \| \mathbf{W}_{t+1} \hat{\mathbf{B}}_t^\top - \mathbf{M}_\ast \|_F &= \| \mathbf{M}_{\ast} \hat{\mathbf{B}}_t \hat{\mathbf{B}}_t^\top  - \mathbf{F}\hat{\mathbf{B}}_t^\top - \mathbf{M}_\ast \|_F \nonumber \\
    &\leq  \| \mathbf{M}_{\ast} \hat{\mathbf{B}}_t \hat{\mathbf{B}}_t^\top  - \mathbf{M}_\ast \|_F + \| \mathbf{F}\hat{\mathbf{B}}_t^\top\|_F \nonumber \\
    &= \| \hat{\mathbf{W}}_{\ast} \mathbf{\Sigma}_\ast \hat{\mathbf{B}}_\ast (\hat{\mathbf{B}}_t \hat{\mathbf{B}}_t^\top  - \mathbf{I}_d) \|_F + \| \mathbf{F}\hat{\mathbf{B}}_t^\top\|_F \nonumber \\
    &\leq \sqrt{k}\|\mathbf{\Sigma}_\ast\|_2 \| \mathbf{B}_\ast^\top(\hat{\mathbf{B}}_t \hat{\mathbf{B}}_t^\top  - \mathbf{I})\|_2 + \| \mathbf{F}\|_F \label{rtk} \\
    &\leq \sqrt{k}\|\mathbf{\Sigma}_\ast\|_2 \text{dist}(\hat{\mathbf{B}}_t, \hat{\mathbf{B}}_\ast) + \frac{\delta_{k}}{1-\delta_k}\|\mathbf{\Sigma}_\ast\|_2 \; \text{dist}(\hat{\mathbf{B}}_t, \hat{\mathbf{B}}_\ast) \label{qqq} \\
    &\leq \frac{\sqrt{k}}{1-\delta_k}\|\mathbf{\Sigma}_\ast\|_2\;\text{dist}(\hat{\mathbf{B}}_t, \hat{\mathbf{B}}_\ast) \label{lastt},
\end{align}
where \eqref{rtk} follows by Cauchy-Schwarz and the fact that $\|\mathbf{A}\|_F \leq \sqrt{k} \|\mathbf{A}\|_2$ for any rank-$k$ matrix $\mathbf{A}$, \eqref{qqq} follows with probability at least $1- e^{}$ by Lemma \ref{lem:f}, and \eqref{lastt} follows since $\delta_k \leq 1$.
%note that we have removed a sqrt(k) factor from previously. are we sure of this? just need from norm of orthogonal matrix=1, right?
\end{proof}

% why do we not need d?
% we should have d for that same reason that sujay cannot have 1/mn

% Note that $\hat{\mathbf{v}}$ is really $\hat{\mathbf{v}}_t$, and we need to apply our bound for each $t$. Since we have linear convergence, we only need to apply it logarithmically many times, i.e., we do not need our bound to hold for all $\hat{\mathbf{v}} \in \mathbb{R}^d:\|\hat{\mathbf{v}}\|=1$. Thus we do not need to deal with an $e^d$ in the final union bound, and this is where we escape the $d$ factor? If we must union bound over $\mathcal{S}^d$, we are in trouble because in the first bound (minimum singular value) we would need $m > d$, unless we can say that $(\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast$ is itself balanced, but I don't think we can show this, because it would require control of all $n$ $H^i$'s.

We will use Lemma \ref{lem:tb} in order to control the error term resulting from the gradient descent step. Before doing so, we must establish the incoherence of $\mathbf{W}^{t+1}$ and $\mathbf{Q}^{t+1} \coloneqq \mathbf{W}^{t+1}\mathbf{\hat{B}}^{{t}^\top} - \mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top}$.
% Experiments status:
% fixed fem/shakes issue i think, but accs still weird. why is test loss sometimes smaller than train loss for fedavg
% why is train loss so small for amg, yet test loss so large
% -----------------------------
% \textbf{Bound on (2.):}
% We let $\mathbf{Q} \coloneqq \mathbf{W}_{t+1}\hat{\mathbf{B}}_t - \mathbf{M}_\ast$. In the proof of linear convergence we have used 
% \begin{align}
%     \| \mathcal{A}^\ast \mathcal{A}(\mathbf{Q}) - \mathbf{Q}\|_2 &\leq \delta_k \|\mathbf{Q}\|_F
% \end{align}
% with high probability, 
% but we could instead use 
% \begin{align}
%     \frac{1}{\sqrt{n}}\| \mathcal{A}^\ast \mathcal{A}(\mathbf{Q}) - \mathbf{Q}\|_F &\leq \delta_k \sqrt{k} \|\mathbf{Q}\|_F
% \end{align}
% as this is easier to show. 
We have
\begin{align}
\mathcal{A}^\ast \mathcal{A}(\mathbf{Q}) &= \sum_{i=1}^n \sum_{j=1}^m \langle \mathbf{e}_{i} (\mathbf{x}_{i}^j)^\top , \mathbf{Q}\rangle \mathbf{e}_{i} (\mathbf{x}_{i}^j)^\top = \sum_{i=1}^n \sum_{j=1}^m \langle \mathbf{x}_{i}^j , \mathbf{q}_i \rangle \mathbf{e}_{i} (\mathbf{x}_{i}^j)^\top  \nonumber \\
   \frac{1}{n} \| \mathcal{A}^\ast \mathcal{A}(\mathbf{Q}) - \mathbf{Q}\|_F^2 &= \frac{1}{n} \sum_{i=1}^n\left(   \sum_{j=1}^m \left( \sum_{i'=1}^n \sum_{j'=1}^m \langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle \langle \mathbf{x}_{i'}^{j'}, \mathbf{q}_{i'} \rangle \langle \mathbf{x}^{j}_i, \mathbf{x}^{j'}_{i'} \rangle - 2 \langle \mathbf{x}_i^{j}, \mathbf{q}_i \rangle^2  \right) + \langle \mathbf{q}_i, \mathbf{q}_i \rangle \right) \label{inco0}
\end{align}
% Assume WLOG that $\|\mathbf{Q}\|_F=1$, i.e. $\sum_{i=1}^n \langle \mathbf{q}_i, \mathbf{q}_i \rangle = 1$.
% We must show that $\mathbf{Q}$ is incoherent across its rows, otherwise we would need $m > d$.


\begin{lemma} \label{lem:incoherent}
    % Assume that $\mathbf{W}_t$ is $\mu$-row-wise incoherent, then 
    For all $t$, the matrix $\mathbf{Q}^{t+1} = \mathbf{W}^{t+1}\mathbf{\hat{B}}^{{t}^\top} - \mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top}\in \mathbb{R}^{n \times d}$ is row-wise incoherent with parameter $\tilde{\mu} = \kappa$, i.e.
    \begin{align}
        \max_{i \in [n]} \left\|\frac{\mathbf{q}^{t+1}_i}{\|\mathbf{Q}^{t+1}\|_F} \right\|_2 \leq \frac{\tilde{\mu}\sqrt{2k}}{\sqrt{n}}
    \end{align}
    with probability at least $1  - e^{-100k^2 \log(n)}$, and where $\mathbf{q}_i^{t+1} \in \mathbb{R}^d$ is the $i$-th row of $\mathbf{Q}^{t+1}$.
\end{lemma}
\begin{proof}
For simplicity we drop superscripts $t$.
Recall $\mathbf{W}$ and the $i$-th row of $\mathbf{W}$:
\begin{align}
    \mathbf{W} &= {\mathbf{W}}_\ast  \hat{\mathbf{B}}_\ast^\top \hat{\mathbf{B}} - \mathbf{F} \nonumber \\
    \mathbf{w}_i^\top &= (\hat{\mathbf{w}}_{i}^\ast)^\top \mathbf{\hat{B}}_\ast^\top \mathbf{\hat{B}}- \mathbf{f}_i^\top \nonumber
\end{align}
Thus
\begin{align}
    \|\mathbf{q}_i\|_2^2 
    &= \| \mathbf{\hat{B}} \mathbf{\hat{B}}^\top \mathbf{\hat{B}}^\ast \hat{\mathbf{w}}_{i}^\ast  - \mathbf{\hat{B}}\mathbf{f}_i - \mathbf{\hat{B}}^\ast \hat{\mathbf{w}}_{i}^\ast\|_2^2 \nonumber \\
    &= \| (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top - \mathbf{I}_d)\mathbf{\hat{B}}^\ast \hat{\mathbf{w}}_{i}^\ast - \mathbf{\hat{B}}\mathbf{f}_i\|_2^2 \nonumber \\
    &\leq 2\| (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top - \mathbf{I}_d)\mathbf{\hat{B}}^\ast \hat{\mathbf{w}}_{i}^\ast\|_2^2  + 2\| \mathbf{\hat{B}} \mathbf{f}_i\|_2^2 \nonumber \\
    &\leq 2\| (\mathbf{\hat{B}} \mathbf{\hat{B}}^\top - \mathbf{I}_d)\mathbf{\hat{B}}^\ast\|_2^2 \| \mathbf{\hat{w}}_{i}^\ast\|_2^2  + 2\| \mathbf{f}_i\|_2^2 \nonumber \\
    &=2k \text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast) + 2\| \mathbf{f}_i\|_2^2
    % &\leq \frac{2\mu^2 k}{n}\; \text{dist}^2(\mathbf{B}, \hat{\mathbf{B}}_\ast) \; \| \mathbf{\Sigma}_\ast \|_2^2  + 2\| \mathbf{f}_i\|_2^2 \nonumber \\
    % &= \| \hat{\mathbf{V}} \mathbf{u}_i \|_2^2 - \mathbf{u}_i^\top \hat{\mathbf{V}}^\top \hat{\mathbf{V}}_\ast \mathbf{\Sigma}_\ast \hat{\mathbf{u}}_{\ast,i}  + \|\hat{\mathbf{V}}_\ast \mathbf{\Sigma}_\ast \hat{\mathbf{u}}_{\ast,i}\|_2^2 \nonumber \\
    % &\leq 2\| \hat{\mathbf{V}} \mathbf{u}_i \|_2^2  + 2\|\hat{\mathbf{V}}_\ast \mathbf{\Sigma}_\ast \hat{\mathbf{u}}_{\ast,i}\|_2^2 \nonumber \\
    % &\leq 2\| \hat{\mathbf{V}} \mathbf{u}_i \|_2^2  + \frac{2\mu^2 \| \mathbf{\Sigma}_\ast\|_2^2}{n}  
\end{align}
% Thus
% \begin{align}
%  \|\mathbf{q}_i\|_2^2 &\leq 4\| \hat{\mathbf{V}} \hat{\mathbf{V}}^\top  \hat{\mathbf{V}}_\ast \mathbf{\Sigma}_\ast \hat{\mathbf{u}}_{\ast,i} \|_2^2 + 4\| \hat{\mathbf{V}} \mathbf{f}_i\|_2^2 + \frac{2\mu^2 \| \mathbf{\Sigma}_\ast\|_2^2}{n} \nonumber \\
%  &\leq \frac{6\mu^2 \| \mathbf{\Sigma}_\ast\|_2^2}{n}+ 4\|\mathbf{f}_i\|_2^2 \label{inco1}
% \end{align}
Recall that $\text{vec}(\mathbf{F}) =  \mathbf{G}^{-1}(\mathbf{GD} - \mathbf{C})  \mathbf{\hat{w}}_\ast$. From equation \eqref{fi}, the $i$-th row of $\mathbf{F}$ is given by:
\begin{align}
    \mathbf{f}^i = (\mathbf{G}^i)^{-1} (\mathbf{G}^i \mathbf{D}^i - \mathbf{C}^i){\mathbf{w}}^{\ast}_i \nonumber
\end{align}
Thus, using the Cauchy-Schwarz inequality and our previous bounds, 
\begin{align}
    \|\mathbf{f}_i\|_2^2 &\leq \| (\mathbf{G}^i)^{-1}\|_2^2\; \|\mathbf{G}^i \mathbf{D}^i - \mathbf{C}^i\|_2^2\;  \;\|{\mathbf{w}}^{\ast}_i\|_2^2 \nonumber \\
    &\leq \| (\mathbf{G}^i)^{-1}\|_2^2 \; \|\mathbf{G}^i \mathbf{D}^i - \mathbf{C}^i\|_2^2 \; k  
    % \|\mathbf{W}^\ast\|_2^2\frac{k}{rn} 
    \label{inco10}  \\
    &\leq \| (\mathbf{G}^i)^{-1}\|_2^2 \; \|\mathbf{G}^i \mathbf{D}^i - \mathbf{C}^i\|_2^2 \; \|\mathbf{W}^\ast\|_2^2 \; \frac{k}{rn}  \label{llast}
    % \left\| [ (\mathbf{G}^{-1}(\mathbf{GD} - \mathbf{C}))_{pn + i} \hat{\mathbf{u}}_\ast]_{1\leq p \leq k} \right\|_2^2 \nonumber \\
    % &= \sum_{p=1}^k (\mathbf{e}_{pn + i}^\top \mathbf{G}^{-1}(\mathbf{GD} - \mathbf{C}) \hat{\mathbf{u}}_\ast)^2 \nonumber \\
    % &\leq \sum_{p=1}^k \|\mathbf{G}^{-1}\|_2^2 \|\mathbf{GD} - \mathbf{C}\|_2^2 
\end{align}
where \eqref{inco10} follows by Assumption \ref{assump:norm}, and \eqref{llast} follows since $krn = \|\mathbf{W}^\ast\|_F^2 \leq k \|\mathbf{W}^\ast\|_2^2$. From \eqref{hiii}, we have that
\begin{align}
         \mathbb{P}\left( \|\mathbf{G}^i\mathbf{D}^i - \mathbf{C}^i\|_2^2 \geq \delta_k^2 \; \text{dist}^2(\mathbf{\hat{B}},\mathbf{\hat{B}}^\ast)  \right)
    &\leq e^{ - 101 k^2 \log(rn)} \nonumber %\\
    %  \implies \mathbb{P}(\|\mathbf{G}^i \mathbf{D}^i - \mathbf{C}^i \|_2^2 > t +\frac{ck^2}{m} \text{dist}^2(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast) ) \leq
     %\exp\left(\frac{-c\sqrt{tm}}{\sqrt{k}\text{dist}(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)} \right) 
    % &\leq \frac{}{} \|\mathbf{\Sigma}_\ast\|_2^2 \frac{\mu^2 k}{n} \label{inco11}
\end{align}
% where the last relation follows from the bound in \eqref{exphi}: $\mathbb{E}[\|\mathbf{G}^i \mathbf{D}^i - \mathbf{C}^i \|_2^2]\leq \frac{ck^2}{m} \text{dist}^2(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast)$. Setting $t=\frac{k^2}{m}\text{dist}^2(\hat{\mathbf{B}}, \hat{\mathbf{B}}_\ast)$, we have 
% \begin{align}
%  \mathbb{P}(\|\mathbf{G}^i \mathbf{D}^i - \mathbf{C}^i \|_2^2 > \frac{ck^2}{m} \text{dist}^2(\hat{\mathbf{B}},\hat{\mathbf{B}}_\ast) ) \leq e^{-ck}
%     % &\leq \frac{}{} \|\mathbf{\Sigma}_\ast\|_2^2 \frac{\mu^2 k}{n} \label{inco11}
% \end{align}




% \begin{align}
%     \|\mathbf{f}_i\|_2^2 &= \sum_{p=1}^k ((\mathbf{G}^{-1}(\mathbf{GD} - \mathbf{C}))_{pn + i} \hat{\mathbf{u}}_\ast)^2 \nonumber \\
%     &= \sum_{p=1}^k \left(\sum_{q=1}^k ((\mathbf{G}^{-1}(\mathbf{GD} - \mathbf{C}))_{pn + i,q} \hat{\mathbf{u}}_{\ast,q }\right)^2
% \end{align}
% where $(\mathbf{G}^{-1}(\mathbf{GD} - \mathbf{C}))_{pn + i}$ is the $(pn + i)$-th row of the matrix   $\mathbf{G}^{-1}(\mathbf{GD} - \mathbf{C})$. 
% For $k=1$, we have
% \begin{align}
%     | f_i | &= \Bigg| \frac{\hat{u}_{\ast, i}\sum_{j=1}^m  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle}{\sum_{j=1}^m  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2} \Bigg| \nonumber \\
%     &\leq \frac{\mu}{\sqrt{n}} \Bigg| \frac{\sum_{j=1}^m  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle}{\sum_{j=1}^m  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2} \Bigg|
% \end{align}
% Both the numerator and denominator within the absolute value are sub-exponential with norm $1/\sqrt{m}$ (variance $1/m$). Also, the numerator has mean $0$ and the denominator has mean 1.
% {\color{blue} need sub-exponential parameter of the numerator to scale with the distance. indeed we have it. now just show for k g 1}
% steps:
% 1. 
% 2. complete this incoherence proof
%
% So we have 
% \begin{align}
%     &\mathbb{P}(\{ |\sum_{j=1}^m  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 - 1| > \nu_1\}  \cup \{|\sum_{j=1}^m  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle  | > \nu_2\}) \nonumber \\
%     &\leq \mathbb{P}( |\sum_{j=1}^m  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 - 1| > \nu_1 ) + \mathbb{P}( |\sum_{j=1}^m  \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle  | > \nu_2)  \nonumber \\
%     &\leq e^{-\nu_1 \sqrt{m}} + e^{-\nu_2 \sqrt{m}}
% \end{align}
% Thus 
% \begin{align}
% | f_i | &\leq \frac{\mu \nu}{\sqrt{n}(1-\nu)} 
% \end{align}
% with probability at least $1-2e^{-c\nu \sqrt{m}}$ for some absolute constant $c$. 

Similarly, from equations \eqref{omd} and \eqref{omd_prob}, we have that 
\begin{align}
    \mathbb{P}\left(\|(\mathbf{G}^i)^{-1}\|_2^2 \geq \frac{1}{(1-\delta_k)^2}\right) \leq e^{-121 k^3 \log(rn)}
\end{align}

Now plugging this back into \eqref{inco10} and assuming $\delta_k \leq \frac{1}{5}$, we obtain
\begin{align}
 \|\mathbf{q}_i\|_2^2
 &\leq 2k\; \text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)\;\left(1+\frac{\delta_k^2}{(1-\delta_k)^2}\right) \leq \frac{5}{4}k\; \text{dist}^2(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)\label{recal}
%  \frac{6\mu^2 \| \mathbf{\Sigma}_\ast\|_2^2}{n}+ \frac{4\mu^2 \nu^2 \| \mathbf{\Sigma}_\ast\|_2^2}{n (1-\nu)^2} = \frac{\mu^2 \| \mathbf{\Sigma}_\ast\|_2^2 (6 - 12\nu + 10\nu^2)}{n (1-\nu)^2}
\end{align}
with probability at least $1-e^{-100k^2\log(rn)}$. Finally, we must lower bound $\|\mathbf{Q}^{t+1}\|_F$. Similarly as in Lemma \ref{lem:qt}, we have
\begin{align}
    \| \mathbf{W}\mathbf{\hat{B}}^{\top} - \mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top} \|_F^2 &= \| \mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top}\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} -\mathbf{F}\mathbf{\hat{B}}^\top - \mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top} \|_F^2 \nonumber \\
    &= \| \mathbf{W}^{\ast} \mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d)\|_F^2 - 2\; \text{Tr}\left(\mathbf{W}^{\ast} \mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d) \mathbf{F}\hat{\mathbf{B}}^\top\right)  +  \|\mathbf{F}\hat{\mathbf{B}}^\top\|_F^2 \nonumber \\
    % &= \| \mathbf{\Sigma}_{\ast}(\hat{\mathbf{B}}_\ast( \hat{\mathbf{B}}_t \hat{\mathbf{B}}_t^\top - \mathbf{I}_n))\|_F^2 -  2\; \text{Tr}\left((\mathbf{M}_{\ast} \hat{\mathbf{B}}_t \hat{\mathbf{B}}_t^\top - \mathbf{M}_\ast)^\top \mathbf{F}\hat{\mathbf{B}}_t^\top\right)  +  \|\mathbf{F}\hat{\mathbf{B}}_t^\top\|_F^2 \nonumber \\
    &\geq  \sigma^2_{\min}(\mathbf{W}^{\ast})\| \mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d) \|_F^2 -  2\; \text{Tr}\left(\mathbf{W}^{\ast} \mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d) \mathbf{F}\hat{\mathbf{B}}^\top\right) \label{theineq}
\end{align}
where \eqref{theineq} follows by the fact that $\|\mathbf{XY}\|_F \geq \sigma_{\min}(\mathbf{X})\|\mathbf{Y}\|_F$ for any two matrices $\mathbf{X}$ and $\mathbf{Y}$. Next we upper bound the cross term:
\begin{align}
   2 \;\text{Tr}\left(\mathbf{W}^{\ast} \mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d) \mathbf{F}\hat{\mathbf{B}}^\top\right)   &\leq 2 \|\mathbf{W}^{\ast} \mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d) \|_F\; \|\mathbf{F}\hat{\mathbf{B}}^\top\|_F \nonumber \\
%   &\leq 2\|\mathbf{M}_{\ast} \hat{\mathbf{B}}_t \hat{\mathbf{B}}_t^\top - \mathbf{M}_\ast\|_2 \; \|\mathbf{F}\|_F \; \|\hat{\mathbf{B}}^\top\|_2\; \nonumber \\
   &\leq  2 \|\mathbf{W}^\ast\|_2 \;  \|\mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d)\|_F \; \|\mathbf{F}\|_F \nonumber \\
   &\leq \frac{2\delta_k}{1-\delta_k} \|\mathbf{W}^\ast\|_2^2  \;  \text{dist}(\mathbf{\hat{B}},\mathbf{\hat{B}}^\ast)
   \|\mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d)\|_F \label{notlast} \\
   &\leq \frac{2\delta_k}{1-\delta_k} \|\mathbf{W}^\ast\|_2^2  \;  
   \|\mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d)\|_F^2 \nonumber \\
   &\leq {\frac{5}{2}\delta_k} \|\mathbf{W}^\ast\|_2^2  \;  
   \|\mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d)\|_F^2 \label{laast}
\end{align}
where \eqref{notlast} follows with probability at least $1-e^{-100k^2 \log(rn)}$ from Lemma \ref{lem:bound_f}, and \eqref{laast} follows as long as $\delta_{k}\leq 1/5$. Next, combining \eqref{theineq} and \label{laast} and assuming that $\sigma_{\min}^2(\mathbf{W}^\ast) \geq \frac{5\delta_k}{2} \|\mathbf{W}^\ast\|_2^2$, we have
\begin{align}
    \| \mathbf{W}\mathbf{\hat{B}}^{\top} - \mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top} \|_F^2 &\geq \left(\sigma^2_{\min}(\mathbf{W}^{\ast})-{\frac{5}{2}\delta_k} \|\mathbf{W}^\ast\|_2^2 \right) \;  
   \|\mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d)\|_F^2 \nonumber \\
   &\geq \left(\sigma^2_{\min}(\mathbf{W}^{\ast})-{\frac{5}{2}\delta_k} \|\mathbf{W}^\ast\|_2^2 \right) \;  
   \|\mathbf{\hat{B}}^{*^\top} (\mathbf{\hat{B}}\mathbf{\hat{B}}^{\top} - \mathbf{I}_d)\|_2^2 \nonumber \\
   &\geq \left(\sigma^2_{\min}(\mathbf{W}^{\ast})-{\frac{5}{2}\delta_k} \|\mathbf{W}^\ast\|_2^2 \right) \;  
   \text{dist}^2(\mathbf{\hat{B}},\mathbf{\hat{B}}^{*}) 
\end{align}
% $\delta_k \leq \frac{c \sigma_{\min}^2(\|\mathbf{\Sigma}_\ast) }{k\|\mathbf{\Sigma}_\ast\|_2^2}$, 
%letting $\kappa^2 = \frac{\|\mathbf{\Sigma}_\ast\|_2^2}{\sigma_{\min}^2(\|\mathbf{\Sigma}_\ast)}$ 
Now recalling \eqref{recal}, we have
\begin{align}
\left\|\frac{\mathbf{q}_i}{\|\mathbf{Q}_i\|_F^2} \right\|_2^2 &\leq \frac{\frac{5}{4}\|\mathbf{W}^\ast\|_2^2\; k}{\left(\sigma^2_{\min}(\mathbf{W}^{\ast})-{\frac{5}{2}\delta_k} \|\mathbf{W}^\ast\|_2^2\right)rn } 
% \nonumber \\
% &\leq  \frac{\frac{5}{4}\|\mathbf{W}^\ast\|_2^2\; k}{(1-\frac{5}{2}\delta_k)\sigma^2_{\min}(\mathbf{W}^{\ast})rn } \nonumber \\
% &\leq \frac{{5}\|\mathbf{W}^\ast\|_2^2\; k}{2\sigma^2_{\min}(\mathbf{W}^{\ast})rn } \nonumber \\
% &\leq   \frac{\frac{5}{2}\kappa^2\; k}{rn} \leq \frac{4\kappa^2\; k}{rn}
\end{align}
where we have again used the assumption that $\delta_k \leq 1/5$.
We further require $\delta_k \leq \frac{\sigma^2_{\min}(\mathbf{W}^{\ast})}{3\|\mathbf{W}^\ast\|_2^2} \leq \frac{1}{3\kappa}$. Then, we have
\begin{align}
\left\|\frac{\mathbf{q}_i}{\|\mathbf{Q}_i\|_F^2} \right\|_2^2 &\leq \frac{\frac{15}{2}\|\mathbf{W}^\ast\|_2^2\; k}{\sigma^2_{\min}(\mathbf{W}^{\ast})rn } \leq \frac{8k}{\kappa rn}
% \nonumber \\
% &\leq  \frac{\frac{5}{4}\|\mathbf{W}^\ast\|_2^2\; k}{(1-\frac{5}{2}\delta_k)\sigma^2_{\min}(\mathbf{W}^{\ast})rn } \nonumber \\
% &\leq \frac{{5}\|\mathbf{W}^\ast\|_2^2\; k}{2\sigma^2_{\min}(\mathbf{W}^{\ast})rn } \nonumber \\
% &\leq   \frac{\frac{5}{2}\kappa^2\; k}{rn} \leq \frac{4\kappa^2\; k}{rn}
\end{align}
 Thus $\tilde{\mu} = 2\kappa$.

% \begin{align}
%     \| \mathbf{W}_{t+1} \hat{\mathbf{B}}_t^\top - \mathbf{M}_\ast \|_F^2 &\geq  \left( \frac{\sigma^2_{\min}(\mathbf{\Sigma}_\ast)  - 3\delta_k \|\mathbf{\Sigma}_\ast\|_2^2 }{1-\delta_k}  \right)\text{dist}^2(\hat{\mathbf{B}}_t,\hat{\mathbf{B}}_\ast)
% \end{align}
% for some absolute constant $c < 1$. Putting everything together and using a union bound, we have 
% \begin{align}
%  \left\| \frac{\mathbf{q}_i}{\|\mathbf{Q}\|_F} \right\|_2^2
%  &\leq \frac{\mu^2 \| \mathbf{\Sigma}_\ast\|_2^2 (6 - 12\nu + 10\nu^2)}{n  \sigma^2_{\min}(\mathbf{\Sigma}_\ast)\left(1- \frac{c }{k}\right)\text{dist}^2(\hat{\mathbf{B}}_t,\hat{\mathbf{B}}_\ast)(1-\nu)^2}
% \end{align}
% \begin{align}
%  \left\| \frac{\mathbf{q}_i}{\|\mathbf{Q}\|_F} \right\|_2^2
%  &\leq \frac{k \; \| \mathbf{\Sigma}_\ast\|_2^2  }{n  ({\sigma^2_{\min}(\mathbf{\Sigma}_\ast)}- 3 \delta_k \|\mathbf{\Sigma}\|_2^2)} \leq \frac{k \kappa^2}{n} %(1-\nu)^2
% \end{align}
% with probability at least $1-2e^{-c\nu \sqrt{m}} - e^{-}$.
    % &\leq  \| \mathbf{M}_{\ast} \hat{\mathbf{B}}_t \hat{\mathbf{B}}_t^\top  - \mathbf{M}_\ast \|_F + \| \mathbf{F}\hat{\mathbf{B}}_t^\top\|_F \nonumber \\
    % &\leq \|\mathbf{\Sigma}_\ast\|_2 \| \mathbf{B}_\ast^\top(\hat{\mathbf{B}}_t \hat{\mathbf{B}}_t^\top  - \mathbf{I})\|_2 + \| \mathbf{F}\|_F \nonumber \\
    % &\leq \|\mathbf{\Sigma}_\ast\|_2\text{dist}(\hat{\mathbf{B}}_t, \hat{\mathbf{B}}_\ast) + \frac{\delta_k}{1-\delta_k}\|\mathbf{\Sigma}_\ast\|_2\text{dist}(\hat{\mathbf{B}}_t, \hat{\mathbf{B}}_\ast) \nonumber \\
    % &= \frac{1}{1-\delta_k}\|\mathbf{\Sigma}_\ast\|_2\text{dist}(\hat{\mathbf{B}}_t, \hat{\mathbf{B}}_\ast)
% Define $\tilde{\mu} \coloneqq \sqrt{\frac{\mu^2 \| \mathbf{\Sigma}_\ast\|_2^2 (6 - 12\nu + 10\nu^2)}{(1-\nu)^2}}$, completing the proof for the $k=1$ case.


\end{proof}


\begin{lemma}
\label{lem:wincoherent}
    For any $t$, the matrix $\mathbf{W}_{t+1} \in \mathbb{R}^{n \times k}$ is row-wise incoherent with parameter $\mu = \kappa$, 
    % $\mu = \|\mathbf{\Sigma}_\ast\|_2(1+ \frac{\delta_kD}{1-\delta_k})\leq  \frac{\|\mathbf{\Sigma}_\ast\|_2}{1-\delta_k}$, 
    $\mu = \frac{\|\mathbf{\Sigma}_\ast\|_2}{\sigma_{\min}(\mathbf{\Sigma}_\ast)-\delta_k \|\mathbf{\Sigma}_\ast\|_2} \leq \kappa$, 
    i.e.
    \begin{align}
        \max_{i \in [n]} \left\|\frac{\mathbf{w}^{t+1}_i}{\|\mathbf{W}_{t+1}\|_F} \right\|_2 \leq \frac{\mu\sqrt{k}}{\sqrt{n}}
    \end{align}
    with probability at least $1 -  e^{-100k^2 \log(n)}$, where $\mathbf{w}_i^{t+1} \in \mathbb{R}^k$ is the $i$-th row of $\mathbf{W}^{t+1}$.
\end{lemma}
\begin{proof} The argument proceeds similarly as in Lemma \ref{lem:incoherent}. For ease of notation we drop superscripts $t$.
From Lemma \ref{lem:defu}, we have:
\begin{align}
    \mathbf{W} &= {\mathbf{W}}^\ast  \mathbf{\hat{B}}^{\ast^\top} \hat{\mathbf{B}} - \mathbf{F} \nonumber \\
    \mathbf{w}_i^\top &= {\mathbf{w}}_{i}^{\ast^\top} \mathbf{\hat{B}}^{\ast^\top} \mathbf{\hat{B}} - \mathbf{f}_i^\top \nonumber
\end{align}
Thus 
\begin{align}
    \|\mathbf{w}_i\|_2^2 &\leq 2\| \mathbf{\hat{B}}^\top\mathbf{\hat{B}}^{\ast}\mathbf{w}_{i}^\ast \|_2^2 + 2 \|\mathbf{f}_i\|_2^2 \nonumber \\
    &\leq 2 \| \mathbf{\hat{B}}^\top\mathbf{\hat{B}}^{\ast}\|_2^2 \| \mathbf{w}_{i}^\ast \|_2^2  + 2 \|\mathbf{f}_i\|_2^2 \nonumber \\
    &\leq 2 \| \mathbf{\hat{B}}^\top\mathbf{\hat{B}}^{\ast}\|_2^2 \| \mathbf{W}^\ast \|_2^2 \frac{k}{rn} + 2 \frac{\delta_k^2}{(1-\delta_k)^2}\text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^{\ast})\| \mathbf{W}^\ast \|_2^2 \frac{k}{rn} \label{toppp}
    %\nonumber \\
    %&\leq  \| \mathbf{W}^\ast \|_2^2 \frac{5k}{2rn} 
\end{align}
with probability at least $1-e^{-100k^2\log(n)}$ by similar analysis as in Lemma \ref{lem:incoherent}.
% , and under the assumption that $\delta_k \leq 1/5$. 
Next,
\begin{align}
\|\mathbf{W}\|_F^2 &= \|  \mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top} \mathbf{\hat{B}} \|_F^2 -2\text{Tr}(\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast \mathbf{W}^{\ast^\top}  \mathbf{F}) + \|\mathbf{F}\|^2_F \nonumber \\
&\geq \|\mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top} \mathbf{\hat{B}} \|_F^2 - 2 \|\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast \mathbf{W}^{\ast^\top} \|_F \|\mathbf{F}\|_F \nonumber \\
&\geq  \|\mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top} \mathbf{\hat{B}} \|_F^2 - \frac{2\delta_k}{1-\delta_k} \text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)\| \mathbf{W}^{\ast} \|_2 \|\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast \mathbf{W}^{\ast^\top} \|_F \nonumber \\
&\geq  \|\mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top} \mathbf{\hat{B}} \|_F^2 - \frac{5\delta_k}{2} \| \mathbf{W}^{\ast} \|_2 \|\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast \mathbf{W}^{\ast^\top} \|_F \nonumber \\
% &\geq  \nonumber \\
&\geq \sigma_{\min}(\mathbf{W}^\ast)\sigma_{\min}(\mathbf{\hat{B}}^{\ast^\top} \mathbf{\hat{B}})\|\mathbf{W}^\ast \mathbf{\hat{B}}^{\ast^\top} \mathbf{\hat{B}} \|_F - \frac{2\delta_k}{1-\delta_k} \text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)\| \mathbf{W}^{\ast} \|_2 \|\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast \mathbf{W}^{\ast^\top} \|_F \nonumber \\
&\geq \left( \sigma_{\min}(\mathbf{W}^\ast)\sqrt{E_0} - \frac{2\delta_k}{1-\delta_k} \text{dist}(\mathbf{\hat{B}}, \mathbf{\hat{B}}^\ast)\| \mathbf{W}^{\ast} \|_2 \right)\|\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast \mathbf{W}^{\ast^\top} \|_F    \label{lasttt} \\
&\geq \left( \sigma_{\min}(\mathbf{W}^\ast)\sqrt{E_0} - \frac{5\delta_k}{2} \| \mathbf{W}^{\ast} \|_2 \right)\|\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast \mathbf{W}^{\ast^\top} \|_F \label{lastttt}
\end{align}
where \eqref{lasttt} follows by the definition of $E_0$, and \eqref{lastttt} follows under the assumption that $\delta_{k} \leq 1/5$. Next, assuming that $\delta_k \leq \frac{\sqrt{E_0}}{3\kappa}$, we have 
\begin{align}
\|\mathbf{W}\|_F^2 &\geq \left( \frac{1}{6}\sigma_{\min}(\mathbf{W}^\ast)\sqrt{E_0}\right)\; \|\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast \mathbf{W}^{\ast^\top} \|_F \nonumber \\
% &\geq \left( \sigma_{\min}(\mathbf{W}^\ast)\sqrt{E_0}- \frac{5\delta_k}{2} \| \mathbf{W}^{\ast} \|_2 \right)\|\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast \mathbf{W}^{\ast^\top} \|_F \nonumber  \\
&\geq \frac{1}{6}\sigma_{\min}(\mathbf{W}^\ast)\sqrt{E_0}{\sigma}_{\min}(\mathbf{\hat{B}}^\top  \mathbf{\hat{B}}^\ast) {\sigma}_{\min}(\mathbf{W}^{\ast}) \nonumber \\
% &\geq \frac{1}{6}\sigma_{\min}(\mathbf{W}^\ast)\sqrt{E_0}\sqrt{E_0} \;{\sigma}_{\min}(\mathbf{W}^{\ast}) \nonumber \\
&=  \frac{1}{6}\sigma_{\min}^2(\mathbf{W}^\ast)E_0
\end{align}
Combining this with \eqref{toppp} yields 
\begin{align}
    \left\|\frac{\mathbf{w}_i}{\|\mathbf{W}\|_F} \right\|_2^2 &\leq \frac{8\kappa^2 E_0k}{rn}
\end{align}
thus $\mathbf{W}$ is incoherent with parameter 

\end{proof}

We next use our bound on $\|\mathbf{F}\|_F$ to bound $\|\mathbf{W}_{t+1}\|_2$.
\begin{lemma}\label{lem:uhat}
The following holds with probability at least $1-e^{}$:
\begin{align}
    \|\mathbf{{W}}^{t+1}\|_F
    % \| \mathbf{B}^{-1} \mathbf{C} S \tilde{u}^\ast \|_2 \nonumber \\
    &\leq \frac{\sqrt{k}}{1-\delta_{2k}}\; \|\mathbf{\Sigma}_\ast\|_2 
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align}
    \|\mathbf{W}_{t+1}\|_F &\leq 
    % \| \mathbf{B}^{-1} \mathbf{C} S \tilde{u}^\ast \|_2 \nonumber \\
    \| \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast (\mathbf{\hat{B}}^\ast)^\top \mathbf{\hat{B}}^t \|_F + \|\mathbf{F}\|_F \nonumber \\
    &\leq \sqrt{k} \; \| \mathbf{\Sigma}_\ast\|_2  + \|\mathbf{F}\|_F \nonumber \\
    % &\leq \| \mathbf{\Sigma}_\ast\|_2 + \frac{\sqrt{k}}{1-\delta_{2k}}\|\mathbf{\Sigma}_\ast\|_2\|(\mathbf{GD}-\mathbf{C})\|_2  \nonumber \\ 
    &\leq \sqrt{k}\| \mathbf{\Sigma}_\ast\|_2+ \frac{\delta_{2k}}{1-\delta_{2k}}\; \|\mathbf{\Sigma}_\ast\|_2  \label{boundWw} \\
    &\leq \frac{\sqrt{k} }{1-\delta_{2k}}\; \|\mathbf{\Sigma}_\ast\|_2 \nonumber
\end{align}
where \eqref{boundWw} holds with probability at least $1- $ from Lemma \ref{lem:f}.
\end{proof}


\begin{table}[H]
\caption{CIFAR10 classification test accuracies for \textbf{2 classes/user}.
%, with 95\% confidence intervals over 5 random trials. 
All algorithms are executed for $T=200$ communication rounds, excluding initialization. $L$ is the number of neurons in the final layer of the network. By default, $L=100$.}
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccr}
\toprule
Algorithm & $n=100$  &  $n=1000$ \\
\midrule
AltMinSGD  & 86.54  & $\mathbf{77.46}$ \\ %87.53 /79 all 1 loc epoch. for 1 loc step: 79.86 & 
%AltMinGD20-Fix     & 87.17 $\pm$ & 1533 \\
% AltMinSGD, $L=20$  &  86.01 &  \\
% AltMinSGD, $L=15$  & 86.30  &  \\
% AltMinSGD, $L=10$  & 86.67  &  \\
% AltMinSGD, $L=5$  & 85.17  &  \\
AltMinGD &  81.98 & 76.16 \\
AltSGD-SGD   & 80.26  & 58.23    \\
% AltGD-GD    &  &     \\ %83.16 &   76.07 old 1 loc epoch. for 1 loc step: 70.54 & 
LG-Fed & 78.23 & 68.43  \\
% FedAvg, $E=20$, 1800 rds   & 52.01 & 39.70 \\
% FedAvg, $E=1$, 1800 rds   & 60.67 & 31.75 \\
FedAvg, $E=1$  & 34.56 & 32.81 \\
FedAvg, $E=10$  & 46.85 & 41.70 \\
FedAvg, $\tau=1, B=50$  & 26.16 & 32.89 \\
FedAvg, $\tau=1, B=200$  & 39.22 & N/A \\ %\tau = 10, B = 200 --> 
FedAvg, $\tau=10, B=50$  & 45.41 & 43.08 \\
FedProx, $E=1$ & 31.89 & 32.95\\
FedAvg-FT, $E=10$ & (46.24) 62.60 & \\ %batch size 100 for n=100
% Per-FedAvg-FT (MAML), $E=10$ & (36.45) 63.25 & \\
Per-FedAvg-FT (MAML), $E=5$ & (39.20) 64.77 & \\
Fed-MTL     & 71.18 & 61.67 \\ %65.41  \\
Local     & $\mathbf{87.11}$ & 70.43  \\%77.81
% \midrule
% AltMinSGD$^{*}$     &  90.56 & 84.88 \\ %/79
% AltMinSGD$^{*}$     &  90.15 &  \\ %/79
% AltSGD-SGD$^{*}$     & 87.11  & 84.48 \\ %/79
% % AltSGD-SGD$^{*}$     &   &  \\%685 574 3542
% SCAFFOLD  & 48.0 & &  \\
% LG-Fed$^*$     & 88.49  & 82.27 \\ %/79
% % FedAvg$^*$, $E=20$   &   &   \\
% % FedAvg$^*$, $E=1$    &  & 54.84 \\
% Fed-MTL$^*$     & 88.56 &  \\
% Local$^*$     &  &  \\ % 93.82  & 84.22 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
%  
% \begin{table}[t]
% \caption{Same table as above but instead of taking the accuracy of the final model after 200 iterations, we store the best local model for each user over the course of the 200 iterations, then compute the test accuracy using these best local models after 200 iterations.}
% \label{table1}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lccr}
% \toprule
% Algorithm & Acc., $n=100$  &  Acc., $n=1000$ \\
% \midrule
% AltMinGD      &  & 79.54 \\ %/79
% %AltMinGD20-Fix     & 87.17 $\pm$ & 1533 \\
% AltGD-GD    &  &        \\
% LG-Fed &  & 74.67  \\
% FedAvg ($E=20$)   &  &   \\
% FedSGD   &  &  \\
% Fed-MTL     & 76.64 &  65.41 \\
% AltMinGD$^*$     & 90.62  & 88.03 \\ %/79
% AltGD-GD$^*$     &   &   \\ %/79
% LG-Fed$^*$     & 91.24  & 86.51  \\ %/79
% FedAvg$^*$ ($E=20$)   &   &   \\
% FedSGD$^*$   &  &  \\
% Fed-MTL$^*$     & 91.76 & 83.58   \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

\begin{table}[H]
\caption{CIFAR10 classification test accuracies for \textbf{5 classes/user}
%, with 95\% confidence intervals over 5 random trials. 
% Unless otherwise noted, the algorithms are initialized randomly, unless they are denoted with a $^\ast$, in which case they are initialized with the result of 1200 rounds of FedSGD. 
All algorithms are executed for $T=200$ communication rounds, excluding initialization. $L$ is the number of neurons in the final layer of the network. By default, $L=100$.}
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Algorithm & $n=100$  &   $n=1000$ & $n=2000$ \\
\midrule
Only Head     & 37.59 & & \\
AltMinSGD, $L=100$     & 70.24 & 48.95 &  \\
AltMinSGD, $L=10$  & 74.03 & 52.20 &  \\ %lr = 0.1/1.2, 0.08
AltMinGD      & 63.08 & 49.17 & 43.51  \\ %/79
% AltMinSGD, 2 loc layers      & 60.46  &  &  \\
% AltMinGD, 2 loc layers      & 63.35 &  &   \\
%AltMinGD20-Fix     & 87.17 $\pm$ & 1533 \\
AltSGD-SGD    & 49.06 &   34.38 &   \\
SCAFFOLD  & 50.5  & &  \\
LG-Fed & 58.01  & 35.10 & \\
% FedProx, $\mu=0.1$ & 49.34  &  & \\
% FedProx, $\mu=0.5$ & 47.74  &  & \\
% FedProx, $\mu=1$ & 46.19  &  & \\
% FedNova & 50.22 &  & \\
% FedAvg, $E=20$   &  &  \\
FedAvg, $\tau=1, B=50$   &  & 31.03 &  \\
{ FedAvg, $\tau=10, B=50$ }  &  & 50.1  &   \\ %61.45? 47.69?53.03
FedProx, $\mu=1$   &  & 32.94 &  \\
FedAvg-FT, $E=10$ & (58.23) 61.54 & \\ %batch size 100 for n=100
Per-FedAvg-FT (MAML), $E=10$ & () & \\
Fed-MTL     & 60.01 & 35.24 \\ %65.41  \\
Local     & 65.81 & 48.54 & 41.78  \\%77.81
% AltMinGD$^*$     &  90.56 & 84.88 \\ %/79
% AltGD-GD$^*$     & 86.95  & 84.48 \\ %/79
% LG-Fed$^*$     & 88.41  & 82.27 \\ %/79
% FedAvg$^*$, $E=20$   &   &   \\
% FedAvg$^*$, $E=1$    &  & 54.84 \\
% Fed-MTL$^*$     & 88.56 &  \\
% Local$^*$     & 93.82  & 84.22  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

% {\color{red} \textbf{TODO, besides tuning and testing on current datasets:} 
% \begin{enumerate}
%     \item Consider alternative evaluation metrics? Right now we are measuring the average local accuracy at the last iterate.
%     \begin{enumerate}
%         \item Performance on a new user? Not well-defined for MNIST and CIFAR datasets.
%         \item Performance on corrupted data in which the representation is invariant? e.g. testing on rotated MNIST images as in the LG-Fed paper.
%     \end{enumerate}
%     \item  SCAFFOLD/FedGATE
%     \item Plots: convergence trajectories? statistics of datasets?
% \end{enumerate}}

% \begin{table}[t]
% \caption{FEMNIST-usersplit image classification test accuracies with 95\% confidence intervals over 5 random trials. Number of training users: $n=1596$. Number of testing users: 178. Number of training communication rounds: $T=200$.}
% \label{table1}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lccr}
% \toprule
% Algorithm & Pre-Adapt & Post-Adapt \\
% \midrule
% AltMinGD      & 57.95  & 60.23 \\
% AltGD-GD    &   52.29   &  55.37  \\
% LG-Fed & 34.50  &  41.45 \\
% % FedAvg + LG-Fed & $\pm$   \\
% % FedAvg   &  &  \\
% FedSGD   &  69.36 & 70.95 \\
% % Fed-MTL     & $\pm$    \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}


% \begin{table}[t]
% \caption{MNIST image classification test accuracies, 2 classes per user, $T=100$, three-layer MLP.
% %with 95\% confidence intervals over 5 random trials.
% }
% \label{table1}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Algorithm & $n=100$ &$n=500$ & $n=1000$ \\%& Post-Adapt  \\
% \midrule
% %AltMinSGD-{\em small}      &   & \\%34.18 & 55.34  \\
% AltMinSGD, $L=128$      & 97.95  &  & \\
% AltMinSGD, $L=10$     & 97.10  & & \\
% %AltGD-GD    &  & \\%43.78 &  62.27   \\
% LG-Fed& 98.79 &  & \\%500 is even with removing the middle layer of network, batch_size 5, 11 loc epochs for amtminsgd \\
% % FedAvg + LG-Fed & $\pm$   \\
% % FedAvg   &   &  \\
% FedAvg, $E=1$  & 91.29 & 86.25 & 63.01  \\%77.18 & 77.83 \\
% % FedAvg, $E=1$, 1000 rounds  & 98.01 & & \\
% % Fed-MTL     & $\pm$    \\
% Local, $L=128$    &  98.44 & 96.98 &  \\%35.06 & 49.99   \\
% Local, $L=10$    & 98.36  &  &  \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

\begin{table}[H]
\caption{MNIST image classification test accuracies, 2 classes per user, and the learning model is a two-layer MLP. All methods are trained for $T=100$ rounds. 
%with 95\% confidence intervals over 5 random trials.
}
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccr}
\toprule
Algorithm & $n=100$ &$n=500$  \\%& Post-Adapt  \\
\midrule
%AltMinSGD-{\em small}      &   & \\%34.18 & 55.34  \\
AltMinSGD      &  $\mathbf{98.93}$ & $\mathbf{98.02}$  \\
AltSGD-SGD      &   & 96.73  \\
%AltGD-GD    &  & \\%43.78 &  62.27   \\
LG-Fed  & 98.23 & 97.16  \\%19.20 &  19.83  \\
% FedAvg + LG-Fed & $\pm$   \\
% FedAvg   &   &  \\
FedAvg, $\tau=10, B=10$ &   & 90.02    \\%77.18 & 77.83 \\ corresponds to E=1
FedAvg, $\tau=100, B=10$ &  96.19 &  95.36  \\ %E=10
FedAvg, $\tau=50, B=50$ &  95.43 & 92.94   \\
FedProx, $\mu=0.05$ (best) &   & 89.52    \\
% FedProx, $\mu=0.1$ &   & 89.48    \\
% FedProx, $\mu=0.5$ &   & 85.10    \\
% FedAvg, $E=1$, 1000 rounds  &  & & \\
Fed-MTL     & 98.61 &  --  \\
Local     &  98.08 & 97.37    \\%35.06 & 49.99   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[H]
\caption{MNIST image classification test accuracies, 5 classes per user. The learning model is a two-layer MLP. All methods are run for $T=100$ rounds. Unless otheriwse noted, the batch size $B=10$.
%with 95\% confidence intervals over 5 random trials.
}
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccr}
\toprule
Algorithm & $n=100$ &$n=500$  \\%& Post-Adapt  \\
\midrule
%AltMinSGD-{\em small}      &   & \\%34.18 & 55.34  \\
AltMinSGD      &  96.44 & 92.75   \\ %old three-layer mlp: 93.91 for n=100
AltSGD-SGD      &   &   \\
%AltGD-GD    &  & \\%43.78 &  62.27   \\
LG-Fed &  & 89.03 \\%19.20 &  19.83  \\%old three-layer mlp: 93.71 for n=100
% FedAvg + LG-Fed & $\pm$   \\
% FedAvg   &   &  \\
FedAvg, $\tau=10, B=10$  &   & 88.68    \\
FedAvg, $\tau=100, B=10$  &  $\mathbf{97.47}$ & $\mathbf{96.31}$    \\%77.18 & 77.83 \\%old three-layer mlp: 95.97 for n=100
FedAvg, $\tau=1, B=200$  &   & 40.31     \\ %40.31
FedAvg, $\tau=10, B=50$  & 96.06  & 94.47     \\
% FedAvg, $E=1$, 1000 rounds  &  & & \\
Fed-MTL     &92.03 &  -- \\
Local     &  94.14 & 89.37   \\%35.06 & 49.99   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[H]
\caption{FEMNIST-datasplit image classification test accuracies .
%with 95\% confidence intervals over 5 random trials. 
Number of users: $n=284$. All algorithms are executed for $T=200$ communication rounds.}
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcr}
\toprule
Algorithm & Accuracy \\%& Post-Adapt  \\
\midrule
AltMinSGD, $L=10$    &  60.40 \\%34.18 & 55.34  \\
AltMinSGD, $L=100$    &  34.18 \\
% AltMinGD      &   \\
% AltGD-GD    &   \\%43.78 &  62.27   \\
LG-Fed & 42.02  \\%19.20 &  19.83  \\
% FedAvg + LG-Fed & $\pm$   \\
% FedAvg   &   &  \\
FedAvg, $E=1$ & 77.63 \\%77.18 & 77.83 \\
FedAvg, $\tau=10, B=10$ & 72.03 \\
% Fed-MTL     & $\pm$    \\
Local     &    \\%35.06 & 49.99   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}



%todo:
% scaffold, fedgate, fednova, fedprox
% mnist: more classes per user - no good, fewer samples per user - promising
% cifar: fedavg with many loc updates is too good
% femnist: try 200-user partintion, as in fedprox, fed dane
% shakespeare
% sent-140

% For FEMNIST, we use a two-layer MLP with ReLU activations.

\begin{table}[H]
\caption{Shakespeare next word prediction test accuracies.
%with 95\% confidence intervals over 5 random trials. 
Number of classes: 80.
Number of users: $n=34$. Communication rounds: $T=100$. Average samples per user: 3000. Local params: 20,000. Global params: 300,000.}
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcr}
\toprule
Algorithm & $n=34$ & $n=$\\
\midrule
AltMinSGD      &  42.04 &    \\
% AltMinSGD-{small-80}      & 45.44  &    \\
% AltMinSGD-{small-10}      & 45.42  &    \\
% AltMinSGD-{$\ell_2$ reg.}      &   &    \\
% AltMinSGD-{dropout}      &   &    \\
% 11 Loc epochs, lr 0.1/1.2 and 0.8
AltSGD-SGD    &  45.35  &      \\
% LG-Fed &    &    \\
% FedAvg + LG-Fed & $\pm$   \\
FedAvg   & 50.77 &  \\
% FedSGD   &  &  \\
% Fed-MTL     & $\pm$    \\
Local     & 30.03  &   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[H]
\caption{Shakespeare accuracies on new users. Number of training users: $n=178$. Communication rounds: $T=100$. Average samples per user: }
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccr}
\toprule
Algorithm & Pre-Fine-Tune & Post-Fine-Tune  \\
\midrule
AltMinSGD      &   45.5  & 47.0  \\
% AltMinSGD-{small-80}      & 45.44  &    \\
% AltMinSGD-{small-10}      & 45.42  &    \\
% AltMinSGD-{$\ell_2$ reg.}      &   &    \\
% AltMinSGD-{dropout}      &   &    \\
% 11 Loc epochs, lr 0.1/1.2 and 0.8
% AltSGD-SGD    &    &      \\
% LG-Fed &    &    \\
% FedAvg + LG-Fed & $\pm$   \\
FedAvg   &  46.0 & 48.0  \\
% FedSGD   &  &  \\
% Fed-MTL     & $\pm$    \\
Local     & 30.0 &     \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[H]
\caption{Sent140 accuracies. Number of training users: $n=183$. Communication rounds: $T=50$. Average samples per user: $60$. Min samples per user: $50$. Local params: 200. Global params: 10,000,000. }
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcr}
\toprule
Algorithm & $n=183$ & $n=$\\
\midrule
AltMinSGD, $E=1$ for rep.      & 71.3 &    \\ %for 100 rounds: 71.5
% AltMinSGD, $E=10$ for rep.     & 70.5 &    \\
% AltMinSGD-{small-80}      & 45.44  &    \\
% AltMinSGD-{small-10}      & 45.42  &    \\
% AltMinSGD-{$\ell_2$ reg.}      &   &    \\
% AltMinSGD-{dropout}      &   &    \\
% 11 Loc epochs, lr 0.1/1.2 and 0.8
AltSGD-SGD    &  69.7   &      \\ %for 100 rounds: 71.5
LG-Fed &    &    \\
% FedAvg + LG-Fed & $\pm$   \\
FedAvg, $E=1$   & 51.5 &  \\ %52.8
FedAvg, $E=10$   & 55.0 &  \\ %100 rounds 59.8 
% FedSGD   &  &  \\
% Fed-MTL     & $\pm$    \\
Local     & 70.2  &   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{table}[H]
\caption{Sent140 new-user accuracies. Number of training users: $n= $. Communication rounds: $T=100$. Average samples per user: $60$. Min samples per user: $50$. Local params: 200. Global params: 10,000,000. }
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcr}
\toprule
Algorithm & Pre-Fine-Tune & Post-Fine-Tune\\
\midrule
AltMinSGD, $E=1$ for rep.      & &    \\
AltMinSGD, $E=10$ for rep.     & &    \\
% AltMinSGD-{small-80}      & 45.44  &    \\
% AltMinSGD-{small-10}      & 45.42  &    \\
% AltMinSGD-{$\ell_2$ reg.}      &   &    \\
% AltMinSGD-{dropout}      &   &    \\
% 11 Loc epochs, lr 0.1/1.2 and 0.8
AltSGD-SGD    &     &      \\
LG-Fed &    &    \\
% FedAvg + LG-Fed & $\pm$   \\
FedAvg, $E=1$   &  &  \\
FedAvg, $E=10$   &  &  \\
% FedSGD   &  &  \\
% Fed-MTL     & $\pm$    \\
Local     &   &   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}



\begin{table}[H]
\caption{CIFAR100 accuracies. Communication rounds: $T=200$. Training samples per user: $50,000/n$. 20 classes per user.}
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcr}
\toprule
Algorithm & $n=100$ & $n=500$\\
\midrule
AltMinSGD      & 38.23  & 20.88    \\
% AltMinSGD-{small-80}      & 45.44  &    \\
% AltMinSGD-{small-10}      & 45.42  &    \\
% AltMinSGD-{$\ell_2$ reg.}      &   &    \\
% AltMinSGD-{dropout}      &   &    \\
% 11 Loc epochs, lr 0.1/1.2 and 0.8
AltSGD-SGD    &    &      \\
LG-Fed &  31.11  &    \\
% % FedAvg + LG-Fed & $\pm$   \\
% FedAvg, $\tau=10, B=50$   &  &  \\
FedAvg, $\tau=100, B=50$   & 22.21 & 19.55 \\
% FedSGD   &  &  \\
Fed-MTL     & &    \\
Local     & 32.60  & 19.62  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}




\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{cifar.pdf}}
\vskip -0.17in
\caption{CIFAR10 local test errors for different numbers of local epochs $E$.}
\label{fig:cifar}
\end{center}
\end{figure}

%  We also test the algorithm that only executes one descent step for the final layer on each iteration \cite{arivazhagan2019federated}. 


% MNIST, EMNIST, FMINST, CIFAR, 

\begin{table*}[ht]
\caption{Average local test accuracies.
%with 95\% confidence intervals over 5 random trials.
}
\label{table1}
\vskip 0.15in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lcccccccc}
\toprule
Dataset & FedRep & AltGD-GD & FedAvg &  Fed-MTL & PerFedAvg &  LG-Fed  & Local \\%& Post-Adapt  \\
\midrule
CIFAR10, $S=2$, $n=100$ & $86.08\pm .3$ & $83.52 \pm .4$ & $44.29\pm 1.3$ & $70.44 \pm .2$  & $64.54 \pm .4$ &$78.12 \pm 1.1$  & $87.28 \pm .6$ \\
CIFAR10, $S=2$, $n=1000$ &$76.41\pm .5$ & $73.07 \pm .5$ & $41.11\pm 1.6$ & $56.90 \pm .1$ & $57.81\pm .3$ & $68.32 \pm 1.4$  &$72.17 \pm .3$\\
CIFAR10, $S=5$, $n=100$ & $72.19 \pm .9$  &$72.26 \pm 1.0$ & $58.14 \pm 1.5$ & $54.21\pm .3$& $51.97 \pm .3$ & $57.83 \pm 1.2$  & $67.76 \pm .5$\\ %$72.66 \pm .2$
CIFAR10, $S=5$, $n=1000$ & $53.41 \pm .7$ & $52.27 \pm .8$ & $50.40 \pm .9$ & $34.58 \pm .5$ & $52.77 \pm .5$ & $35.05 \pm .9$ &  $47.56 \pm .4$\\ %$48.63\pm .7$
CIFAR100, $S=20$, $n=100$ & $38.17 \pm .8$ & $37.41 \pm .5$ & $15.74 \pm .8$ & $23.38 \pm .3$ & $20.05 \pm .3$ &$31.06 \pm .5$ & $32.04 \pm .7$ \\
CIFAR100, $S=20$, $n=500$ & $24.30 \pm .6^*$ & $21.92 \pm .6$ & $19.43 \pm .7$  & $10.56 \pm .3$ & $41.80$ & $8.98\pm .3$ & $21.06 \pm .6$ \\
% CIFAR100, $S=50$, $n=100$ & $23.71 \pm .7$ & $23.45 \pm .6$ & $20.25\pm .8$ & $14.72 \pm .3$ & $25.07 \pm .4$ & & $17.10\pm 1.1$ \\
% CIFAR100, $S=50$, $n=500$ & $13.33^*$ & $11.50 \pm .3$ & $18.82\pm.4$ & $6.09 \pm .2$ & $45.56$& &  $11.66 \pm 1.4$\\
FEMNIST, $n=$ & $m$ & & $60.11 \pm 1.6$ & & &  &$19.12 \pm .9$ \\
Sent140, $n=183$ & $72.13 \pm .2$ &$69.57 \pm .8$ & $56.82 \pm 1.4$ & & & $70.84 \pm 1.4$ & $70.22 \pm .8$\\%$70.64 \pm .9$
% FEMNIST, $n=100$ & & &  & & & & &\\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}







==> proof_main.tex <==
\section{Proof of Main Result} \label{app:proof_main}

% We next generalize the previous result from rank-1 to rank-$k$ matrices.
\subsection{Preliminaries.}
\begin{definition}
For a random vector $\mathbf{x} \in \mathbb{R}^d$ and a fixed matrix $\mathbf{A} \in \mathbb{R}^{d_1 \times d_2}$, the vector $\mathbf{A}^\top \mathbf{x}$  is called {\em $\|\mathbf{A}\|_2$-sub-gaussian} if $\mathbf{y}^\top \mathbf{A}^\top \mathbf{x}$ is sub-gaussian with sub-gaussian norm $\|\mathbf{A}\|_2  \|\mathbf{y}\|_2$ for all $\mathbf{y} \in \mathbb{R}^{d_2}$, i.e. $\mathbb{E}[\exp({\mathbf{y}^\top \mathbf{A}^\top \mathbf{x}})] \leq \exp\left({\|\mathbf{y}\|_2^2 \|\mathbf{A}\|_2^2/2}\right)$.
\end{definition}

\begin{definition}
A rank-$k$ matrix $
\mathbf{M} \in \mathbb{R}^{d_1 \times d_2}$ is {\em $\mu$-row-wise incoherent} if 
  $ \max_{i \in [d_1]} \|\mathbf{m}_i\|_2 \leq (\nicefrac{\mu \sqrt{d_2}}{\sqrt{d_1}}) \|\mathbf{M}\|_F$, 
where $\mathbf{m}_i \in \mathbb{R}^{d_2}$ is the $i$-th row of $\mathbf{M}$.
\end{definition}

We use hats to denote orthonormal matrices (a matrix is called orthonormal if its set of columns is an orthonormal set). By Assumption \ref{assump:norm}, the ground truth representation $\mathbf{B}^\ast$ is orthonormal, so from now on we will write it as $\hat{\mathbf{B}}^\ast$. 

For a matrix $\mathbf{W} \in \mathbb{R}^{n \times k}$ and a random set of indices $\mathcal{I} \in [n]$ of cardinality $rn$, define $\mathbf{W}_\mathcal{I} \in \mathbb{R}^{rn \times k}$ as the matrix formed by taking the rows of $\mathbf{W}$ indexed by $\mathcal{I}$. Define $\bar{\sigma}_{\max, \ast} \coloneqq \max_{\mathcal{I} \in [n], |\mathcal{I}| = rn} \sigma_{\max} (\frac{1}{\sqrt{rn}}\mathbf{W}^\ast_{\mathcal{I}})$ and $\bar{\sigma}_{\min, \ast} \coloneqq \min_{\mathcal{I} \in [n], |\mathcal{I}| = rn} \sigma_{\min}(\frac{1}{\sqrt{rn}} \mathbf{W}^\ast_{\mathcal{I}})$, i.e. the maximum and minimum singular values of any matrix that can be obtained by taking $rn$ rows of $\frac{1}{\sqrt{rn}}\mathbf{W}^\ast$. Note that by Assumption \ref{assump:norm}, each row of $\mathbf{W}^\ast$ has norm $\sqrt{k}$, so $\frac{1}{\sqrt{rn}}$ acts as a normalizing factor such that $\|\frac{1}{\sqrt{rn}}\mathbf{W}^\ast_{\mathcal{I}}\|_F = \sqrt{k}$.  In addition, define $\kappa = \bar{\sigma}_{\max, \ast}/\bar{\sigma}_{\min, \ast}$.

Let $i$ now be an index over $[rn]$, and let $i'$ be an index over $[n]$.
% First, assume without loss of generality that $\mathcal{I}=[rn]$. 
For random batches of samples $\{ \{ (\mathbf{x}_{i}^{j},y_i^j ) \}_{j=1}^m \}_{i=1}^{rn}$,
% \footnote{With slight abuse of notation, we now use $i$ as an index over the selected clients, and assume that $rn$ is an integer.}
% , 
define the random linear operator $\mathcal{A}: \mathbb{R}^{rn \times d} \rightarrow \mathbb{R}^{rnm}$ as 
$
    \mathcal{A}(\mathbf{M}) = [\langle \mathbf{A}_{i}^{j}, \mathbf{M} \rangle]_{1\leq i \leq rn, 1\leq j \leq m} \in \mathbb{R}^{rnm}.
$
Here, $\mathbf{A}_{i}^{j} \coloneqq \mathbf{e}_i  ({\mathbf{x}_i^{j}})^\top $, where $\mathbf{e}_i$ is the $i$-th standard vector in $\mathbb{R}^{rn}$, and $\mathbf{M} \in \mathbb{R}^{rn \times d}$. 
Then, the loss function in \eqref{obj:glob_linear} is equivalent to 
\begin{align}
    \min_{\mathbf{B} \in \mathbb{R}^{d \times k}, \mathbf{W} \in \mathbb{R}^{n \times k}} \{ &
    F(\mathbf{B},\mathbf{W}) \coloneqq \frac{1}{2rnm} \mathbb{E}_{\mathcal{A}, \mathcal{I}} \left[\| \mathbf{Y} - \mathcal{A}(\mathbf{W}_\mathcal{I}\mathbf{B}^\top)\|_2^2 \right] \}, \label{linop_app} 
\end{align}
where $\mathbf{Y}  =\mathcal{A}(\mathbf{W}^\ast_\mathcal{I} \hat{\mathbf{B}}^{\ast^\top}) \in \mathbb{R}^{rnm}$ is a concatenated vector of labels. It is now easily seen that the problem of recovering $\mathbf{W}_\ast \hat{\mathbf{B}}^{\ast^\top}$ from finitely-many measurements $\mathcal{A}(\mathbf{W}^\ast_\mathcal{I} \hat{\mathbf{B}}^{\ast^\top})$ is an instance of matrix sensing. 
Moreover, the updates of FedRep satisfy the following recursion:
\begin{align}
    {\mathbf{W}}^{t+1}_{\mathcal{I}^t} &= 
    % \argmin_{{\mathbf{W}}_{\mathcal{I}^t} \in \mathbb{R}^{rn\times k}} \frac{1}{2rnm}\|\mathbf{Y} - \mathcal{A}^t({\mathbf{W}}_{\mathcal{I}^t}\mathbf{B}^{t^\top})\|_2^2 = 
    \argmin_{{\mathbf{W}}_{\mathcal{I}^t} \in \mathbb{R}^{rn\times k}} \frac{1}{2rnm}\| \mathcal{A}^t({\mathbf{W}}_{\mathcal{I}^t}^\ast\hat{\mathbf{B}}^{\ast^\top} -  {\mathbf{W}}_{\mathcal{I}^t}\mathbf{B}^{t^\top})\|_2^2 \label{up_ww} \\
  \mathbf{B}^{t+1} &= \mathbf{B}^t - \!\frac{\eta}{rnm} 
  \left((\mathcal{A}^t)^\dagger \mathcal{A}^t({\mathbf{W}}^{t+1}_{\mathcal{I}^t}\mathbf{B}^{t^\top}- {\mathbf{W}}_{\mathcal{I}^t}^\ast\hat{\mathbf{B}}^{\ast^\top})\right)^\top {\mathbf{W}}^{t+1}_{\mathcal{I}^t} \label{up_b}
  %\sum_{i=1}^{rn}\sum_{j=1}^m (\langle \mathbf{A}^{t,j}_{i}, {\mathbf{W}}_{\mathcal{I}^t}^{t+1}\mathbf{B}^{t^\top} \rangle - y_{i}^{j}) \mathbf{A}_i^{{t,j}^\top} {\mathbf{W}}_{\mathcal{I}^t}^{t+1} \label{up_b}
\end{align}
where $\mathcal{A}^t$ is an instance of $\mathcal{A}$, and $(\mathcal{A}^t)^\dagger$ is the adjoint operator of $\mathcal{A}^t$, i.e. $(\mathcal{A}^t)^\dagger \mathcal{A}(\mathbf{M}) = \sum_{i=1}^{rn}\sum_{j=1}^m (\langle \mathbf{A}^{t,j}_{i},  {\mathbf{M}} \rangle) \mathbf{A}_i^{{t,j}}$.
% the measurement matrices $\mathbf{A}_{i}^{t,j} = \mathbf{e}_i (\mathbf{x}_i^{t,j})^\top$ for $i \in \mathcal{I}^t, j \in [m]$. 
Note that for the purposes of analysis, it does not matter how $\mathbf{w}_{i'}^{t+1}$ is computed for all $i' \notin \mathcal{I}^t$, as these vectors do not affect the computation of $\mathbf{B}^{t+1}$. Moreover, our analysis does not rely on any particular properties of the batches $\mathcal{I}^1,\dots, \mathcal{I}^T$ other than the fact that they have cardinality $rn$, so without loss of generality we assume $\mathcal{I}^t = [rn]$ for all $t=1,...T$ and drop the subscripts $\mathcal{I}^t$ on $\mathbf{W}^t$.   

% For simplicity, we move the $\frac{1}{m}$ factor inside the measurement matrices $\mathbf{A}_i^j$, and define the 

% \input{proof_challenges}

% Next we consider only the $t$-th update, and drop the superscript on $t$ in the measurements for ease of notation.
\subsection{Auxilliary Lemmas}

We start by showing that we can assume without loss of generality that $\mathbf{B}^t$ is orthonormalized at the end of every communication round.

\input{proofLemmas}



\subsection{Main Result}

Now we are ready to show Theorem \ref{thrm:linear}, which follows immediately from the following descent lemma.

\begin{lemma} \label{lem:main}
Define $E_0 \coloneqq 1- \dist^2(\mathbf{\hat{B}}^0,\mathbf{\hat{B}}^\ast)$ and $\bar{\sigma}_{\max, \ast} \coloneqq \max_{\mathcal{I} \in [n], |\mathcal{I}| = rn} \sigma_{\max} (\frac{1}{\sqrt{rn}}\mathbf{W}^\ast_{\mathcal{I}})$ and $\bar{\sigma}_{\min, \ast} \coloneqq \min_{\mathcal{I} \in [n], |\mathcal{I}| = rn} \sigma_{\min}(\frac{1}{\sqrt{rn}} \mathbf{W}^\ast_{\mathcal{I}})$, i.e. the maximum and minimum singular values of any matrix that can be obtained by taking $rn$ rows of $\frac{1}{\sqrt{rn}}\mathbf{W}^\ast$.

Suppose that $m \geq c(\kappa^4 k^3\log(rn)/E_0^2 + \kappa^4 k^2 d/(E_0^2 rn))$ for some absolute constant $c$. 
Then for any $t$ and any $\eta \leq 1/(4 \bar{\sigma}_{\max,\ast}^2)$, we have 
\begin{align}
    \dist(\mathbf{\hat{B}}^{t+1}, \mathbf{\hat{B}}^\ast)
    &\leq \left(1 -  \eta E_0\bar{\sigma}_{\min,\ast}^2 /2\right)^{1/2}\; \dist(\mathbf{\hat{B}}^t,\mathbf{\hat{B}}^\ast), \nonumber
\end{align}
with probability at least $1 - e^{-100\min(k^2\log(rn),d)}$.
\end{lemma}
% Note that from the analysis point of view, it does not matter how $\mathbf{w}_{i}^{t+1}$ is computed for all $i \notin \mathcal{I}$, as these vectors do not affect the update of $\mathbf{B}^{t+1}$. Thus, for ease of notation we will 
% Now the proof of Theorem \ref{thrm:linear} follows immediately by recursively applying Lemma \ref{lem:main} and union bounding over $t$. It remains to show Lemma \ref{lem:main}.

% \subsection{Proof of Lemma \ref{lem:main} }
\begin{proof}
% We first show that problem \eqref{obj:glob_linear} is an instance of matrix sensing. 
% For ease of notation, we drop the superscripts $t$ on the measurements and  the subscripts $\mathcal{I}^t$, e.g. $\mathbf{W}^t \coloneqq \mathbf{W}^t_{\mathcal{I}^t}$. Further, by Lemma \ref{lem:ortho},  we can assume without loss of generality that $\mathbf{B}^t$ is orthogonal, i.e. $\hat{\mathbf{B}}^t$. Then, the updates of FedRep are written as:

% Further,  we define the new notation: $\mathbf{\overline{W}} = \frac{1}{\sqrt{rn}} \mathbf{W}_{1:rn}$ denotes the matrix formed by taking the first $rn$ rows of $\mathbf{W}$ and dividing them by $\frac{1}{\sqrt{rn}}$. By Assumption \ref{assump:norm}, we have that ${\mathbf{\overline{W}}}_\ast$ is $1$-row-wise incoherent and has Frobenius norm $\|\mathbf{\overline{W}}\|_F = \sqrt{k}$.
% We also bring $m$ inside
% Thus, by bringing the $1/rn$ factor in \eqref{linop_app} inside the norm, we obtain the following update rule for FedRep:
% Recall that $y_{i}^j = \langle \mathbf{A}_{i}^{j}, \mathbf{W}^\ast \mathbf{B}^{\ast^\top}$ where $\mathbf{W}^\ast$ and $\mathbf{B}^{\ast}$ are the ground-truth set of client-specific parameters and representation, respectively. Without loss of generality, we bring the 

Recall that $\mathbf{W}^{t+1} \in\mathbb{R}^{rn \times k}$ and $\mathbf{B}^{t+1} \in\mathbb{R}^{d \times k}$ are computed as follows:
\begin{align}
    {\mathbf{{W}}}^{t+1} &= 
    \argmin_{{\mathbf{{W}}} \in \mathbb{R}^{rn\times k}} \frac{1}{2rnm}\| \mathcal{A}({\mathbf{{W}}}^\ast\mathbf{\hat{B}}^{\ast^\top} -  {\mathbf{{W}}}\mathbf{\hat{B}}^{t^\top})\|_2^2 \label{up_w} \\
  \mathbf{B}^{t+1} &= \mathbf{\hat{B}}^t - \!\frac{\eta}{rnm} 
  \left(\mathcal{A}^{\dagger} \mathcal{A}({\mathbf{W}}^{t+1}\mathbf{\hat{B}}^{t^\top}- {\mathbf{{W}}}^\ast\mathbf{\hat{B}}^{\ast^\top})\right)^\top {\mathbf{{W}}}^{t+1}
\end{align}
% By Lemma \ref{lem:uhat}, we can assume without loss of generality that $\mathbf{B}^{t+1}$ is orthogonalized at the end of each round, and we denote the orthogonalized matrix by $\hat{\mathbf{B}}^{t+1} = {\mathbf{B}}^{t+1} (\mathbf{R}^{t+1})^{-1}$, 



\input{proofA}

% Recall the computation of $\mathbf{W}_{t+1}$ in Lemma \ref{lem:defu}. The update for $\mathbf{B}$ is given by:
% \begin{align}
%     \mathbf{B}_{t+1} &= \hat{\mathbf{B}}_t - \eta \left(\mathcal{A}^\ast \mathcal{A}( \mathbf{W}_{t+1} \mathbf{\hat{B}}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top ) \right)^\top \mathbf{{W}}_{t+1}
% \end{align}

% We let $\hat{\mathbf{W}}_\ast \mathbf{\Sigma}_\ast \hat{\mathbf{B}}_\ast^\top = \mathbf{M}_\ast$ denote the SVD of $\mathbf{M}_\ast$. 
%In the immediately following proof, matrices with bars are also orthogonal, e.g. $\mathbf{\overline{X}}$.
% Let $\mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top = \mathbf{{W}}_\ast \mathbf{{B}}_\ast^\top$ be the SVD of $\mathbf{{W}}_\ast \mathbf{{B}}_\ast^\top$. 






\end{proof}


% \textbf{Outline of Proof.}
% Recall the global objective:
% \begin{align}
% %     \min_{\mathbf{W} \in \mathbb{R}^{n\times k}, \mathbf{B}\in \mathbb{R}^{d\times k}} \left\{ F(\mathbf{W}, \mathbf{B}) = \frac{1}{2nm}\sum_{i=1}^n \sum_{j=1}^m \langle \mathbf{A}_{i,j}, \mathbf{{W} {B}}^\top - \mathbf{M}_\ast  \rangle^2 \right\} \label{rank1sg:obj}
% % \end{align}
% % AltMinGD takes alternating minimization steps with respect to $\mathbf{W}$ and gradient descent steps with respect to $\mathbf{B}$, as detailed in Algorithm \ref{alg1}.


% The proof of Theorem \ref{thrm:linear} involves multiple steps. First, we show that we can assume {\em for analysis only} that each iterate in $\mathbf{B}$ is orthogonalized at the end of the iteration, which helps to simplify the analysis. Then, we upper bound the norms of two error matrices - one representation a perturbation in the minimization step and the other representing a perturbation in the gradient descent step.
% The bound on the latter term requires the row-wise incoherence of the matrices $\mathbf{Q}_t = \mathbf{W}_t \hat{\mathbf{B}}_t - \mathbf{M}_\ast$ and $\mathbf{W}_t$, which we establish with high probability in an auxiliary result. We also employ a truncated version of the matrix Bernstein inequality similar to Lemma 29 in \cite{tripuraneni2020provable} to bound the gradient descent perturbation term. The bound on the minimization perturbation term requires $m = O(k^3 \log^2(n))$ samples per user per iteration to hold with high probability, and the bound on the gradient descent perturbation term requires $m=O(\nicefrac{d}{n})$ samples, for a total of $m = O(k^3 \log^2(n) + \nicefrac{d}{n})$ samples per user. On each iteration we must sample fresh samples, which multiplies the total number of samples per user required to achieve $\epsilon$ error by $O(\log(1/\epsilon))$. 

% Using these bounds, it is not hard to show the linear convergence of $\mathbf{B}_t$ to $\mathbf{B}_\ast$ in principal angle distance.

% This analysis will require upper bounds on the following terms to hold with with high probability over the samples $\{ \mathbf{x}_i^j\}_{i,j}$:
% \begin{enumerate}
%     \item 
% \end{enumerate}





% Wsing results in JNS14, it is not hard to show
% \begin{align}
%     \min_{\mathbf{x}: \|\mathbf{x}\|_2=1} -\delta_{2k} \|\mathbf{W}_{t+1}\mathbf{x}\mathbf{x}^\top {B}_t^\top {B}_{\ast,\perp}\|_F\|\mathbf{W}_{t+1}  {B}_t^\top - \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \|_F\geq -\delta_{2k} \frac{(1+\delta_2k)(1+(k-1)\delta_{2k})}{(1 -\delta_{2k})^2}\|\mathbf{\Sigma}_\ast\|_2^2 \; \text{dist}^2(\mathbf{B}_t, \mathbf{\hat{B}}_\ast)
% \end{align}
% So now all that remains is to lower bound
% \begin{align}
%     \min_{\mathbf{x}: \|\mathbf{x}\|_2=1} \text{tr}(\mathbf{\hat{B}}_{\ast,\perp}\mathbf{\hat{B}}_{\ast,\perp}^\top {B}_t\mathbf{x}\mathbf{x}^\top \mathbf{W}_{t+1}^\top \mathbf{W}_{t+1} {B}_{t}^\top )
% \end{align}
% where $\mathbf{W}_{t+1} = \mathbf{\hat{W}}_\ast \mathbf{\Sigma}_\ast \mathbf{\hat{B}}_\ast^\top \mathbf{B}_t - F$.

Finally, Theorem \ref{thrm:linear} follows by recursively applying Lemma \ref{lem:main} and taking a union bound over all $t\in [T]$.

% \vspace{3mm}
% \begin{customthm}{1} \label{thrm:main}
% Define $E_0 \coloneqq 1- \text{dist}^2(\mathbf{\hat{B}}^0,\mathbf{\hat{B}}^\ast)$ and $\bar{\sigma}_{\max, \ast} \coloneqq \max_{\mathcal{I} \in [n], |\mathcal{I}| = rn} \sigma_{\max} (\frac{1}{\sqrt{rn}}\mathbf{W}^\ast_{\mathcal{I}})$ and $\bar{\sigma}_{\min, \ast} \coloneqq \min_{\mathcal{I} \in [n], |\mathcal{I}| = rn} \sigma_{\min}(\frac{1}{\sqrt{rn}} \mathbf{W}^\ast_{\mathcal{I}})$, i.e. the maximum and minimum singular values of any matrix that can be obtained by taking $rn$ rows of $\frac{1}{\sqrt{rn}}\mathbf{W}^\ast$.
% Suppose that $m \geq c(\kappa^4 k^3\log(rn)/E_0^2 + \kappa^4 k^2 d/(E_0^2 rn))$ for some absolute constant $c$. 
% Then for any $t$ and any $\eta \leq 1/(4  \bar{\sigma}_{\max,\ast}^2)$, we have 
% \begin{align}
%     \text{dist}(\mathbf{\hat{B}}^T, \mathbf{\hat{B}}^\ast)
%     &\leq \left(1 -  \eta E_0\bar{\sigma}_{\min,\ast}^2 /2\right)^{T/2}\; \text{dist}(\mathbf{\hat{B}}^0,\mathbf{\hat{B}}^\ast), \nonumber
% \end{align}
% with probability at least $1 - Te^{-100\min(k^2\log(rn),d)}$.
% \end{customthm}





%Note that the proofs for the minimization step in JNS14 all go through because the do not rely on how $\mathbf{B}_t$ is computed. 



% Assume that $\mathbf{u}_{\ast}$ is $\mu/\sqrt{n}$-incoherent (I think this is reasonable, since this does not imply that the user parameter vectors have norm $O(1/\sqrt{n})$, since we still have $\mathbf{\Sigma}$. Also see Lemma 17 in Jin paper), then we have
% \begin{align}
%     \|(\mathbf{GD} - \mathbf{C})\mathbf{u}_\ast\|_2^2
%     &\leq \frac{\mu^2}{n} \sum_{i=1}^n  \sum_{j=1}^m  \sum_{j'=1}^m H_j^i H_{j'}^i \nonumber 
    % &= \frac{\mu^2}{n} \sum_{i=1}^n  \sum_{j=1}^m  \sum_{j'=1}^m (\langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle )(\langle \mathbf{x}_{i}^{j'}, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle - \langle \mathbf{x}_{i}^{j'}, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^{j'}, \hat{\mathbf{v}}_\ast \rangle ) \nonumber \\
    % &= \frac{\mu^2}{n} \sum_{i=1}^n  \sum_{j=1}^m  \sum_{j'=1}^m \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle^2
    % \langle \mathbf{x}_{i}^{j'}, \hat{\mathbf{v}} \rangle^2
    % - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle\langle \mathbf{x}_{i}^{j'}, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle \nonumber \\
    % &\quad \quad \quad \quad - \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle^2 \langle \hat{\mathbf{v}}, \hat{\mathbf{v}}_\ast \rangle \langle \mathbf{x}_{i}^{j'}, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^{j'}, \hat{\mathbf{v}}_\ast \rangle + \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^j, \hat{\mathbf{v}}_\ast \rangle \langle \mathbf{x}_{i}^{j'}, \hat{\mathbf{v}} \rangle \langle \mathbf{x}_{i}^{j'}, \hat{\mathbf{v}}_\ast \rangle \nonumber
% \end{align}

% \textbf{Non-symmetric updates.} 
% % To the best of our knowledge, all previously-studied algorithms for nonconvex matrix sensing use the {\em same} update scheme (either minimization or gradient descent) to update both factors,  
% % % take either minimization \cite{Jain_2013, } or gradient descent steps \cite{tu2016low, } to update {\em both} factors, 
% % unlike our method. 
% Existing analyses for nonconvex matrix sensing study algorithms with symmetric update schemes for the factors $\mathbf{W}$ and $\mathbf{B}$, either alternating minimization \cite{Jain_2013} or alternating gradient descent \cite{tu2016low}. 
% %Here we show contraction due to the gradient descent step in principal angle distance, differing from the standard result for gradient descent using Procrustes distance  \cite{tu2016low, }. 
% We combine aspects of both types of analysis in our proof. Nevertheless, we would like to emphasize that this difficulty is in {\em analysis only}, as we present extensive experiments demonstrating the advantage of taking a more local update steps for the head than the representation in Section \ref{sec:experiments}.


% \newpage

% \citet{smith2017federated} applied multi-task learning techniques to the federated setting, but did not attempt to reduce the problem dimension by learning a global representation. Instead, the proposed objective encodes global information in the form of a learnable weight matrix enabling clustering of the local parameters. 

% Contextualization:

% Personalized FL via Regularization:


% \citet{huang2020personalized} also considers a  regularizer that encourages closeness of the local models.

% \citet{liang2020think} proposed a framework and algorithm for learning local low-dimensional representations and a global predictor. Although our works share a motivation of reducing the problem dimension in federated learning, their work differs from ours in multiple key ways. First, since they attempt to learn many local representations as opposed to a single global representation, their incorporation of global parameters only serves as a regularizer to prevent local over-fitting, not as a means to learn and utilize global features present in the data across devices. Second, while our algorithm takes advantage of the reduced problem dimension from the client perspective by performing a local parameter minimization step on each iteration, their proposed algorithm takes gradient descent steps with respect to both the global and local parameters on each iteration.

\subsection{Initialization}

% \textbf{Initialization for linear representation:}

As mentioned in the main body, our interpretation of Theorem \ref{thrm:linear} assumes that the initial distance is bounded above by a constant less than one, i.e., $E_0$ is bounded below by a constant greater than zero. We can achieve such an initialization without increasing the overall sample complexity via the Method-of-Moments algorithm, ignoring log factors.  To show this, we adapt a result from \cite{tripuraneni2020provable}.

\begin{customthm}{2}
[Theorem 3, \cite{tripuraneni2020provable}] Suppose that each client $i \in [n]$ sends the server $\mathbf{Z}_i\! \coloneqq\!\frac{1}{m}\sum_{j=1}^m (y_i^{0,j})^2 \mathbf{x}_i^{0,j} (\mathbf{x}_i^{0,j})^\top$ and the server computes $\mathbf{\hat{U}} \mathbf{D}\mathbf{\hat{U}}^\top\!\leftarrow\! \text{rank-}k \text{ SVD}(\tfrac{1}{n}\textstyle{\sum_{i=1}^n\mathbf{Z}_i)}$ and sets $\mathbf{B}^0 =\mathbf{\hat{U}}$. Then, if $m \geq c \polylog(d,mn) kd/(\sigma_{\min,\ast}^4 n)$,
\begin{align}
    \dist\left(\mathbf{B}, \mathbf{\hat{B}}^\ast\right) &\leq \tilde{O}\left(\frac{kd}{\sigma_{\min,\ast}^4 mn} \right)
\end{align}
with probability at least $1 - O((mn)^{-100})$ for some absolute constant $c$, where $\sigma_{\min,\ast} \coloneqq \frac{1}{\sqrt{n}}\mathbf{W}^\ast$ and $\tilde{O}(\cdot)$ hides log factors.
\end{customthm}

The above result is a direct adaptation of Theorem 3 in \cite{tripuraneni2020provable} so we omit the proof. This result shows that $m = \tilde{\Omega}(\frac{kd}{\sigma_{\min,\ast}^4n})$ are required for proper initialization.
Since $\kappa \gtrsim 1/\sigma_{\min,\ast}$, the overall sample complexity is not increased up to log factors.


% The result follows directly from Theorem 2 in \cite{tripuraneni2020provable} so we omit the proof.


% If each user can sends the following weighted sum of their data: $\frac{1}{M}\sum_{j=1}^M %\mathbf{e}_i 
% y_i^j \mathbf{x}_i^j $ to the server, then we can use the SVD strategy from Jain et al 2013.

% This should be secure for any $M>1$...


















\input{proof_init}

% \input{proof_noise}


\input{proof_challenges}


% \section{Further Discussion of Related Works}
% The majority of methods for personalized federated learning do not involve dimensionality-reduction at the local level. For instance,
% \citet{jiang2019improving} and \citet{fallah2020personalized} obtain full-dimensional models advantageous for local fine-tuning via SGD by applying model-agnostic meta-learning (MAML) methods to federated learning. On the other hand, many works propose to learn multiple full-dimensional models, typically a single global model and unique local models for each client.
% \citet{hanzely2020federated}, 
% \citet{t2020personalized}, and \citet{li2020federated} add a regularization term to the standard federated learning objective which penalizes local models from being too far from a global model. \citet{huang2020personalized} takes a similar approach but uses a regularizer with an attention-inducing function to encode relationships between the local models, similar to \cite{smith2017federated}.
% % \cite{yu2020salvaging} investigates the trade-off between robustness and accuracy for fine-tuning and multi-task learning federated learning techniques.
% Meanwhile, \citet{deng2020adaptive} and \citet{mansour2020three} also use full-dimensional local and global models, and propose to linearly combine them to obtain the model for each client, a framework for which they are able to provide generalization bounds on new client data. \citet{mansour2020three} additionally analyzes two other methods for personalization, but these methods require combining client data and hence are not applicable to federated learning.

% Multiple concurrent works have also proposed to learn local heads and a global representation for federated learning, via hypernetworks \cite{shamsian2021personalized} or meta-learning \cite{singhal2021federated}, mostly from experimental perspectives.  Another recent paper \cite{thekumparampil2021sample}, which first appeared on arxiv several months later than this paper, proved a similar sample complexity result as ours for learning the representation in the context of meta-learning for mixed linear regression. Their result in the noiseless case achieves improved dependence on condition number ($mn = \Omega(\kappa)$ for theirs and $mn = \Omega(\kappa^4)$ dependence for ours) and does not require a $\log(rn)$
%  term in the complexity of $mn$. However, their results are for alternating minimization, as opposed to the more difficult-to-analyze alternating descent-minimization.
 
 
 


==> rank1fm.tex <==
\textbf{Rank-1, population case:}

Here $k=1$,
\begin{align}
    \mathbf{w}_{t+1} &= \mathbf{w}_{\ast} \frac{\langle \mathbf{b}_t, \mathbf{\hat{b}}_\ast\rangle}{\|\mathbf{b}_t\|_2^2}, \nonumber \\
    \mathbf{b}_{t+1} &= \mathbf{b}_{t} - \eta \|\mathbf{w}_t\|_2^2 \mathbf{b}_t + \eta  \langle \mathbf{w}_\ast, \mathbf{w}_t \rangle \mathbf{\hat{b}}_\ast \nonumber \\
\end{align}
Choose $\eta= 1/\|\mathbf{w}_t\|_2^2$, then the algorithm becomes Alt-Min. We have 
\begin{align}
    \mathbf{b}_{t+1} &= \frac{ \langle \mathbf{w}_\ast, \mathbf{w}_t \rangle}{\|\mathbf{w}_t\|_2^2}\mathbf{\hat{b}}_\ast \nonumber \\
    \langle \frac{\mathbf{b}_{t+1}}{\|\mathbf{b}_{t+1}\|_2}, \mathbf{\hat{b}}_\ast\rangle &= 1
\end{align}


==> rank1sg.tex <==
\section{Rank-$1$, Sub-gaussian Measurements}
\begin{comment}
The problem we aim to solve is
\begin{align}
    F(\hat{u}, \hat{v}) &= \frac{1}{2}\sum_{i=1}^N \langle A_i, \hat{u} \hat{v}^T - \sigma_\ast u_\ast v_\ast^\top \rangle^2 \label{rank1sg:obj}
\end{align}

% \begin{theorem}

% \end{theorem}

\begin{proof}
Setting the gradient of \eqref{rank1sg:obj} with respect to $\hat{u}$ equal to 0, we obtain that the update for $\hat{u}_{t+1}$ is:
\begin{align}
    \hat{u}_{t+1} &= \frac{\sigma_{\ast}}{\|\hat{v}_t \|} B^{-1} C u_\ast
\end{align}
where
\begin{align}
    B &\coloneqq \sum_{i=1}^N A_i {v}_t {v}_t^\top A_i^\top \\
    C &\coloneqq \sum_{i=1}^N A_i {v}_t v_\ast^\top A_i^\top 
\end{align}
Plugging this back into the objective, we obtain
\begin{align}
    F(\hat{u}_{t+1}, \hat{v}) &= \frac{1}{2}\sum_{i=1}^N \langle A_i, \frac{\sigma_{\ast}}{\|\hat{v}_t \|} B^{-1} C u_\ast \hat{v}^T - \sigma_\ast u_\ast v_\ast^\top \rangle^2 \\
    &= \frac{1}{2}\sum_{i=1}^N \sigma_\ast^2 \left( \hat{v}^T A_i^\top \frac{1}{\|\hat{v}_t \|} B^{-1} C u_\ast - v_\ast^\top A_i^\top u_\ast \right)^2 
%eliminate u_\ast?
\end{align}
Then the gradient with respect to $\hat{v}$ is
\begin{align}
    \nabla_{\hat{v}} F(\hat{u}_{t+1}, \hat{v}) = \sum_{i=1}^N \sigma_\ast^2 \left(  u_\ast^\top C^\top B^{-\top} A_i \frac{1}{\|\hat{v}_t \|}  \hat{v}  -  u_\ast^\top A_i v_\ast \right) A_i^\top \frac{1}{\|\hat{v}_t \|} B^{-1} C u_\ast 
    =: S_t
\end{align}
and we have
\begin{align}
    \hat{v}_{t+1} = \hat{v}_{t} - \eta \sum_{i=1}^N \sigma_\ast^2 \left(  u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) A_i^\top \frac{1}{\|\hat{v}_t \|} B^{-1} C u_\ast 
\end{align}
Using operator notation, this is
\begin{align}
    \hat{v}_{t+1} = \hat{v}_t - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast
\end{align}
where $\mathcal{A}^\ast$ is the adjoint of the operator $\mathcal{A}$.


Next, we have 
\begin{align}
    \hat{v}_{t+1}^\top \hat{v}_{t+1} &= \hat{v}_{t}^\top \hat{v}_{t} - 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_t \|} \sum_{i=1}^N  \left(  u_\ast^\top C^\top B^{-\top}  A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) \hat{v}_{t}^\top A_i^\top  B^{-1} C u_\ast \nonumber \\
    &\quad \quad + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_t \|^2}  \sum_{i=1}^N  \sum_{i'=1}^N  \left(u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right)\left(u_\ast^\top C^\top B^{-\top} A_{i'} {v}_t  -  u_\ast^\top A_{i'} v_\ast \right) u_\ast^\top C^\top B^{\top}A_i A_{i'}^\top B^{-1} C u_\ast  \label{rank1sg:square}
\end{align}
We expect the cross terms to be close to zero:
\begin{align}
    \frac{\sigma_\ast^2}{\|\hat{v}_t \|}& \sum_{i=1}^N  \left(  u_\ast^\top C^\top B^{-\top}  A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) \hat{v}_{t}^\top A_i^\top  B^{-1} C u_\ast  \nonumber \\
    &= {\sigma_\ast^2} \sum_{i=1}^N  u_\ast^\top C^\top B^{-\top}  A_i {v}_t {v}_{t}^\top A_i^\top B^{-1} C u_\ast -  u_\ast^\top A_i v_\ast{v}_{t}^\top A_i^\top  B^{-1} C u_\ast \nonumber \\
    &= {\sigma_\ast^2} u_\ast^\top C^\top B^{-\top} \left(\sum_{i=1}^N A_i {v}_t {v}_{t}^\top A_i^\top\right) B^{-1} C u_\ast  -  {\sigma_\ast^2} u_\ast^\top \left(\sum_{i=1}^N A_i v_\ast{v}_{t}^\top A_i^\top \right) B^{-1} C u_\ast\nonumber \\
    &= {\sigma_\ast^2} u_\ast^\top C^\top B^{-\top} C u_\ast  -  {\sigma_\ast^2} u_\ast^\top C^\top  B^{-1} C u_\ast\nonumber \\
    &= 0 \label{rank1sq:cross}
\end{align}
where \eqref{rank1sq:cross} follows because $B$ is symmetric.
Next, we expect the last term of \eqref{rank1sg:square} to monotonically increase with the distance $1-\langle v_t, v_\ast \rangle^2$:
\begin{align}
\Psi &\coloneqq \frac{\sigma_\ast^4}{\|\hat{v}_t \|^2} \sum_{i=1}^N  \sum_{i'=1}^N  \left(u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right)\left(u_\ast^\top C^\top B^{-\top} A_{i'} {v}_t  -  u_\ast^\top A_{i'} v_\ast \right) u_\ast^\top C^\top B^{-\top}A_i A_{i'}^\top B^{-1} C u_\ast  \nonumber \\
&= \frac{\sigma_\ast^4}{\|\hat{v}_t \|^2} \sum_{i=1}^N  \sum_{i'=1}^N  \left(u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) u_\ast^\top C^\top B^{-\top}A_i A_{i'}^\top B^{-1} C u_\ast \left(u_\ast^\top C^\top B^{-\top} A_{i'} {v}_t  -  u_\ast^\top A_{i'} v_\ast \right) \nonumber \\
&= 
\end{align}
% the u stars should be irrelevant - remove them
Define $\Delta_t = B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top$ and $\bar{u}_t = B^{-1} C u_\ast$. An initial bound for $\Psi$ is:
\begin{align} \label{norm-a*a}
    \Psi &= \frac{\sigma_\ast^2}{\|\hat{v}_t \|} \left\|\left(\mathcal{A}^\ast \mathcal{A} (B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1}C u_\ast \right\|_2^2 \\
    &= \frac{\sigma_\ast^2}{\|\hat{v}_t \|} \left\|\left(\mathcal{A}^\ast \mathcal{A} (B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1}C \right\|_2^2 \nonumber \\
    &\leq \frac{\sigma_\ast^2}{\|\hat{v}_t \|} \left\|\mathcal{A}^\ast \mathcal{A} (B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top)\right\|_2^2 \|B^{-1}\|_2^2\|C\|_2^2
\end{align}
Each of the three norms can be controlled with RIP. The term $\left\|\mathcal{A}^\ast \mathcal{A} (B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top)\right\|_2^2$ will yield an upper bound in terms of $\|B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top\|_F^2$. This question now is whether we can write this in terms of the distance. We have
\begin{align}
\|B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top\|_F^2 &= \|B^{-1}(C u_\ast v_t^\top - B u_\ast v_\ast^\top) \|_F^2 \nonumber \\
&\leq \frac{1}{(1- 3 \delta_{2k})^2} \|(C u_\ast v_t^\top - B u_\ast v_\ast^\top) \|_F^2  \label{c-b-u-u*}\\
&= \frac{1}{(1- 3 \delta_{2k})^2} tr((C u_\ast v_t^\top - B u_\ast v_\ast^\top)^\top (C u_\ast v_t^\top - B u_\ast v_\ast^\top)) \nonumber \\
&=\frac{1}{(1- 3 \delta_{2k})^2} (u_\ast^\top C^\top C u_\ast - tr(v_t u_\ast^\top C^\top B u_\ast v_\ast^\top) - tr(v_\ast u_\ast^\top B^\top C u_\ast v_t^\top) + u_\ast^\top B^\top B u_\ast )
\end{align}
Lemma B.1. is crucial.
Using it, we have
\begin{align}
    u_\ast^\top C^\top C u_\ast &= \sum_{j=1}^n u_\ast^\top C^\top e_j e_{j}^\top C u_\ast \\
    &= \sum_{j=1}^n (\sum_{i=1}^N u_\ast^\top A_i v_\ast v_t^\top A_i^\top e_j) (\sum_{i=1}^N e_{j}^\top A_i v_t v_\ast^\top A_i^\top u_\ast) \\
    &= \sum_{j=1}^n (\sum_{i=1}^N \text{tr}(A_i^\top u_\ast v_\ast^\top )\text{tr}(A_i^\top e_j v_t^\top)) (\sum_{i=1}^N \text{tr}( A_i^\top e_j v_t^\top)\text{tr}( A_i^\top u_\ast v_\ast^\top)) \\
    &=  \sum_{j=1}^n \langle \mathcal{A}( u_\ast v_\ast^\top), \mathcal{A}(e_j v_t^\top)\rangle \langle \mathcal{A}(e_j v_t^\top),\mathcal{A}(u_\ast v_\ast^\top)\rangle \\
    &\leq \sum_{j=1}^n \left( \langle u_\ast, e_j \rangle  \langle v_t, v_\ast \rangle + 3\delta_4 \right)^2 \label{rank1sg:b11} \\
    &= \sum_{j=1}^n \langle u_\ast, e_j \rangle^2  \langle v_t, v_\ast \rangle^2 + 6 \delta_4 \langle u_\ast, e_j \rangle  \langle v_t, v_\ast \rangle + 9\delta_2^2 \nonumber \\
    &\leq \langle v_t, v_\ast \rangle^2 + 6 \delta_2 \sqrt{n}\langle v_t, v_\ast \rangle + 9\delta_2^2 \label{rank1sg:rtn} \\
    &\leq 1 - \text{dist}(v_t, v_\ast) + 6 \delta_2 \sqrt{n} + 9\delta_2^2
    % \sum_{i=1}^N \sum_{i'=1}^N u_\ast^\top A_i^\top v_\ast v_t^\top A_i A_{i'} v_t v_\ast^\top A_{i'}^\top u_\ast \nonumber \\
    % &=         \nonumber \\
    % &= \sum_{i=1}^N \text{tr}( A_i^\top u_\ast v_t^\top)  \text{tr}(A_i^\top u_\ast v_\ast^\top) \nonumber \\
    % &= \langle \mathcal{A}(u_\ast v_t^\top) , \mathcal{A}(u_\ast v_\ast^\top) \rangle  \nonumber \\
    % &= \langle \mathcal{A}(u_\ast v_t^\top) , \mathcal{A}(u_\ast v_\ast^\top) \rangle 
\end{align}
where \eqref{rank1sg:b11} follows from Lemma B.1 and \eqref{rank1sg:rtn} follows since for any $u \in \mathbb{R}^n$ such that $\|u\|_2 = 1$, $\sum_{j=1}^n u_j \leq \sqrt{n}$. Similarly, we have
\begin{align}
    u_\ast^\top B^\top B u_\ast &= \sum_{j=1}^n u_\ast^\top B^\top e_j e_j^\top B u_\ast \nonumber \\
    &= 
\end{align}

Aside
\begin{align}
    u_\ast^\top C u_\ast &= \sum_{i=1}^N u_\ast^\top A_i v_\ast v_t^\top A_i^\top u_\ast \nonumber \\
    &= \sum_{i=1}^N \text{tr}( A_i^\top u_\ast v_t^\top)  \text{tr}(A_i^\top u_\ast v_\ast^\top) \nonumber \\
    &= \langle \mathcal{A}(u_\ast v_t^\top) , \mathcal{A}(u_\ast v_\ast^\top) \rangle  \nonumber \\
    &\leq \langle v_t, v_\ast \rangle  + 3 \delta_{2k}
\end{align}

% Note that
% \begin{align}
%     \|C\|
% \end{align}
Using Lemma B.1 we have
\begin{align}
    \| C\|_2^2 \leq \left( \langle v_t, v_\ast \rangle + 3 \delta_{2k} \right)^2
    &= 1- \text{dist}(v_t, v_\ast) + 6 \delta_{2k} \langle v_t, v_\ast \rangle + 9 \delta_{2k}^2 \\
    &\leq  (1+3 \delta_{2k})^2 - \text{dist}(v_t, v_\ast)
\end{align}
and this is the tightest we can do using Lemma B.1.
Meanwhile we have
\begin{align}
    \|B^{-1} \|_2^2 \leq \frac{1}{(1- 3 \delta_{2k})^2}
\end{align}
by directly taking results from the proof of Lemma 4.3.

Combining these, we have
\begin{align}
    a
\end{align}
%is $\|\Delta_t\|$ a function of the distance? yes



\textcolor{red}{Another way to bound \eqref{c-b-u-u*} could be as follows:}

First note that using $2k$-RIP we have for any rank-$2k$ matrix $x$ that:
$$ ||\mathcal{A}^*\mathcal{A}(x) - x||_2 \leq \delta_{2k} ||x||_F,$$
and we thus obtain
$$||\mathcal{A}^*\mathcal{A}(x)||_2 \leq (1 + \sqrt{2k} \delta_{2k}) ||x||_2,$$
as $||x||_F \leq \sqrt{2k}||x||_2$ when $\text{rank}(x) \leq 2k$.

Continuing from \eqref{norm-a*a} and noting that has at most rank 2, we obtain 
$$|| \mathcal{A}^*\mathcal{A}(C u_\ast v_t^\top - B u_\ast v_\ast^\top) ||_2^2 \leq (1 + \sqrt{2}\delta_2)^2   \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|_2^2 $$
and 
\begin{align} \label{alternative}
  \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|_2^2 
  &=  \|C u_\ast v_t^\top - C u_\ast v_\ast^\top + C u_\ast v_\ast^\top - B u_\ast v_\ast^\top \|_2^2 \\
  & = || Cu_\ast(v_t - v_\ast)^\top + (C-B)u_\ast v_\ast^\top)||_2^2
\end{align}
Now, let's first bound the norm of $Cu_\ast(v_t - v_\ast)^\top$. We have: 
\begin{align*}
||Cu_\ast(v_t - v_\ast)^\top||_2 & \leq 
||Cu_\ast ||_2 ||(v_t - v_\ast)^\top||_2 \\
&\leq ||Cu_\ast ||_2 \sqrt{2(1 - \langle v_t, v_\ast\rangle)}\\
&\leq ||C ||_2 \sqrt{2(1 - \langle v_t, v_\ast \rangle^2)} \\
&\leq (1+\delta_k)  \sqrt{2\text{dist}(v_t, v_\ast)},
\end{align*}
Where we have used 
$$|| C||_2 \leq (1+\delta_k) || v_t v_\ast^\top||_2 \leq  (1+\delta_2).$$
In the same manner, by using RIP we can write
\begin{align*}
    || C - B ||_2 \leq (1+\delta_k) || v_t (v_t - v_\ast)^\top ||_2 \leq || v_t||_2 || v_t - v_\ast||_2 \leq \sqrt{2 \text{dist}(v_t, v_\ast)}.
\end{align*}
And thus: 
$$ ||(C-B) u_\ast v_\ast^\top||_2 \leq ||(C-B) u_\ast||_2 u_\ast v_\ast^\top||_2 \leq (1+\delta_k)  \sqrt{2 \text{dist}(v_t, v_\ast)} . $$
Putting these together, we obtain: 
\begin{equation}
    \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|_2^2 
    \leq 8(1+\delta_2)^2\text{dist}(v_t, v_\ast).
\end{equation}
and
\begin{equation}
    || \mathcal{A}^*(\mathcal{A}(C u_\ast v_t^\top - B u_\ast v_\ast^\top) ||_2^2 \leq
    8((1+\delta_2)^2(1+ \sqrt{2} \delta_2))^2\text{dist}(v_t, v_\ast).
\end{equation}
Thus, this term goes to zero as the distance goes to zero, as desired.


Note that in the rank-$k$ case the term $\sqrt{2}\delta_2$ will be changed to $\sqrt{2k}\delta_{2k}$, which is fine. 


Next, we need to show that $\langle v_t, v_\ast \rangle^2$ strictly increases:
\begin{align}
    \langle v_{t+1}, v_\ast \rangle^2 &= \frac{1}{\|\hat{v}_{t+1}\|_2^2} \langle \hat{v}_t - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast, v_\ast \rangle^2 \\
    &= \frac{\|\hat{v}_{t}\|_2^2}{\|\hat{v}_{t+1}\|^2_2} \langle {v}_t, v_\ast \rangle^2  - 2\frac{\eta \sigma_\ast^2 \langle {v}_t, v_\ast \rangle}{\|\hat{v}_{t+1}\|_2^2}\langle  \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast, v_\ast \rangle \nonumber \\
    &\quad \quad \quad \quad + \frac{\eta^2 \sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_t\|_2^2}\langle  \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast, v_\ast \rangle^2
\end{align}
Note that
\begin{align}
&\langle  \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast, v_\ast \rangle \nonumber \\
&= \langle  \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top, v_\ast u_\ast^\top C^\top B^{-\top} \rangle \nonumber \\
&=\langle B^{-1}C u_\ast v_\ast^\top,  \mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top)\rangle \nonumber \\
&= \langle \mathcal{A}( B^{-1}C u_\ast v_\ast^\top),  \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top)\rangle \label{rank1sg:rip}
\end{align}
Next, let $b = \langle  B^{-1}C u_\ast v_\ast^\top, B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top\rangle$ and $c = \delta \| B^{-1}C u_\ast v_\ast^\top\|_F\|B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top\|_F$. Using RIP and \eqref{rank1sg:rip}, we have 
\begin{align}
    |\left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast, v_\ast \rangle| &\geq \max \left\{ 0, -b-c, b-c\right\}
\end{align}
We need to show that either $b-c$ or $-b-c$ is strictly greater than 0. Seems strange..

We first bound $c$:
    \begin{align}
    \|B^{-1} C u_\ast v_\ast^\top\|_F &= \|B^{-1} C\|_2 \\
    &\leq \frac{1}{1-3\delta} \|C\|_2 \\
    &\leq \frac{1+\delta}{1-3\delta}
\end{align}
by Cauchy-Schwarz and earlier bounds (note that the constant numbers may be off, may need $3\delta$ in numerator). For a lower bound, we have
\begin{align}
   \|B^{-1} C u_\ast v_\ast^\top\|_F &= \|B^{-1} C\|_2 \\
    &\geq \sigma_{\min}(B^{-1}) \sigma_{\min}(C) \\
    &\geq \frac{1-\delta}{1+3\delta} 
\end{align}
Next, we have from earlier analysis:
\begin{align}
    \|B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top\|_F &\leq \sqrt{2}\|B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top\|_2 \nonumber \\
    &\leq \frac{4(1+\delta)(\sqrt{1-\langle v_t, v_\ast \rangle})}{1-3\delta}
\end{align}
Also, 
\begin{align}
    \|B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top\|_F &\geq \|B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top\|_2 \nonumber \\
    &\geq \frac{1}{1+3\delta} \sigma_{\min} (C u_\ast v_t^\top - B u_\ast v_\ast^\top)
\end{align}
Nevermind, we only need an upper bound on $c$. 
We have
\begin{align}
c &\leq \frac{4\delta(1+\delta)^2\sqrt{1-\langle v_t, v_\ast \rangle}}{(1-3\delta)^2}
\end{align}
Now for $b$:
\begin{align}
    b &= \langle  B^{-1}C u_\ast v_\ast^\top, B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top\rangle \nonumber \\
    &= \text{tr}( v_\ast u_\ast^\top C^\top B^{-\top}  B^{-1} C u_\ast v_t^\top ) - \text{tr}( v_\ast u_\ast^\top C^\top B^{-\top} u_\ast v_\ast^\top ) \nonumber \\
    &= \text{tr}( u_\ast^\top C^\top B^{-\top}  B^{-1} C u_\ast )\langle v_t, v_\ast \rangle - \text{tr}( u_\ast^\top C^\top B^{-\top} u_\ast  ) \nonumber\\
    &= \text{tr}( u_\ast^\top C^\top B^{-\top}  B^{-1} C u_\ast )\langle v_t, v_\ast \rangle - \text{tr}( u_\ast^\top C^\top B^{-\top}  u_\ast )\langle v_t, v_\ast \rangle + \text{tr}( u_\ast^\top C^\top B^{-\top}  u_\ast )\langle v_t, v_\ast \rangle - \text{tr}( u_\ast^\top C^\top B^{-\top} u_\ast  ) \nonumber \\
    &= \langle v_t, v_\ast \rangle  u_\ast^\top C^\top B^{-\top}  (B^{-1} C-I)u_\ast - u_\ast^\top C^\top B^{-\top}u_\ast(1- \langle v_t, v_\ast \rangle) \nonumber 
    \end{align}
    For an upper bound, we have
    \begin{align}
    b &\leq \langle v_t, v_\ast \rangle  \| C^\top B^{-\top}  (B^{-1} C-I)\|_2 -\sigma_{\min}(C^\top B^{-\top})(1- \langle v_t, v_\ast \rangle) \nonumber \\
    &\leq \langle v_t, v_\ast \rangle \frac{1+\delta}{1-3\delta} \|B^{-1}C - I\|_2 - \frac{1-\delta}{1+3\delta} (1- \langle v_t, v_\ast \rangle) \\
    &\leq \langle v_t, v_\ast \rangle \frac{1+\delta}{1-3\delta} \max (\frac{1+\delta}{1-3\delta} - 1 , 1 - \frac{1-\delta}{1+3\delta})- \frac{1-\delta}{1+3\delta} (1- \langle v_t, v_\ast \rangle) \nonumber \\
    &= \langle v_t, v_\ast \rangle \frac{1+\delta}{1-3\delta} \frac{4\delta}{1-3\delta}- \frac{1-\delta}{1+3\delta} (1- \langle v_t, v_\ast \rangle) \nonumber \\
    &=  \langle v_t, v_\ast \rangle\left( \frac{4\delta(1+\delta)}{(1-3\delta)^2} + \frac{1-\delta}{1+3\delta} \right)- \frac{1-\delta}{1+3\delta}
\end{align}
For $\delta$ sufficiently small, this bound is negative. So I think we are done. Let \\ $\psi = \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast, v_\ast \rangle$. We have by RIP that $\psi \leq b + c$ and $|\psi| \geq -b - c$. Combining our bounds on $b$ and $c$ yields
\begin{align}
b+c &\leq \langle v_t, v_\ast \rangle\left( \frac{4\delta(1+\delta)}{(1-3\delta)^2} + \frac{1-\delta}{1+3\delta} \right)- \frac{1-\delta}{1+3\delta} + \frac{4\delta(1+\delta)^2\sqrt{1-\langle v_t, v_\ast \rangle}}{(1-3\delta)^2}
\end{align}
For sufficiently small $\delta$ this is again negative. So for small enough $\delta$ we have 
\begin{align}
   \psi \leq \theta \quad \text{and} \quad \psi^2 \geq \theta^2
\end{align}
where $\theta = \langle v_t, v_\ast \rangle\left( \frac{4\delta(1+\delta)}{(1-3\delta)^2} + \frac{1-\delta}{1+3\delta} \right)- \frac{1-\delta}{1+3\delta} + \frac{4\delta(1+\delta)^2\sqrt{1-\langle v_t, v_\ast \rangle}}{(1-3\delta)^2}$. 
Now we have
\begin{align}
    \langle v_{t+1}, v_\ast \rangle^2 &= \frac{\|\hat{v}_{t}\|_2^2}{\|\hat{v}_{t+1}\|^2_2} \langle {v}_t, v_\ast \rangle^2  - 2\frac{\eta \sigma_\ast^2 \langle {v}_t, v_\ast \rangle}{\|\hat{v}_{t+1}\|_2^2 }\psi + \frac{\eta^2 \sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_t\|_2^2}\psi^2 \nonumber \\
    &\geq \frac{\|\hat{v}_{t}\|_2^2}{\|\hat{v}_{t+1}\|^2_2} \langle {v}_t, v_\ast \rangle^2  - 2\frac{\eta \sigma_\ast^2 \langle {v}_t, v_\ast \rangle}{\|\hat{v}_{t+1}\|_2^2 }\theta + \frac{\eta^2 \sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_t\|_2^2}\theta^2 \nonumber
\end{align}
Since we are assuming $\delta$ is small enough such that $\theta$ is negative, we must have that: $\frac{1-\delta}{1+3\delta} \geq \frac{4\delta(1+\delta)^2\sqrt{1-\langle v_t, v_\ast \rangle}}{(1-3\delta)^2}$ for all $t$. Then
\begin{align}
    \langle v_{t+1}, v_\ast \rangle^2 
    &\geq \frac{\|\hat{v}_{t}\|_2^2}{\|\hat{v}_{t+1}\|^2_2} \langle {v}_t, v_\ast \rangle^2  - 2\frac{\eta \sigma_\ast^2 }{\|\hat{v}_{t+1}\|_2^2 } \left( \frac{4\delta(1+\delta)}{(1-3\delta)^2} + \frac{1-\delta}{1+3\delta} \right) \langle {v}_t, v_\ast \rangle^2 + \frac{\eta^2 \sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_t\|_2^2}\theta^2 \nonumber \\
    &=  \nonumber \\
\end{align}
For now assume $\delta=0$. Then
we get
\begin{align}
    \langle v_{t+1}, v_\ast \rangle^2 
    &\geq (\frac{\|\hat{v}_t\|_2^2}{\|\hat{v}_{t+1}\|_2^2} - \frac{\eta^2 \sigma^4}{\|\hat{v}_t\|_2^2\|\hat{v}_{t+1}\|_2^2}) \langle v_t, v_\ast \rangle^2 + \frac{\eta^2 \sigma^4}{\|\hat{v}_t\|_2^2\|\hat{v}_{t+1}\|_2^2}
\end{align}
%which is no help.


Then
\begin{align}
    1-  \langle v_{t+1}, v_\ast \rangle^2  &\leq 1 - \frac{\eta^2 \sigma^4}{\|\hat{v}_t\|_2^2\|\hat{v}_{t+1}\|_2^2} - (\frac{\|\hat{v}_t\|_2^2}{\|\hat{v}_{t+1}\|_2^2} - \frac{\eta^2 \sigma^4}{\|\hat{v}_t\|_2^2\|\hat{v}_{t+1}\|_2^2}) \langle v_t, v_\ast \rangle^2
\end{align}
almost... need rt/rt+1 to be at least 1 but it is at most 1

instead, try multiplying both sides of 256 with $V_{\ast,\perp}$ and taking $\| \|_2^2$

% {Ok I think we have it:}





--------

Different approach: Re-write $u_\ast$.

Note that
\begin{align}
    u_\ast &= \frac{\sigma_\ast}{\| \hat{v}_t\|} B^{-1} Cu_\ast\nonumber \\
    &= \frac{\sigma_\ast}{\| \hat{v}_t\|} \langle v_t, v_\ast \rangle u_\ast  - \frac{\sigma_\ast}{\| \hat{v}_t\|} B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast \nonumber
\end{align}
Now, the gradient update for $v$ is:

% \begin{align}
%     \hat{v}_{t+1} = \hat{v}_{t} - \eta \sum_{i=1}^N \sigma_\ast^2 \left(  u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) A_i^\top \frac{1}{\|\hat{v}_t \|} B^{-1} C u_\ast 
% \end{align}
% Using operator notation, this is
\begin{align}
    \hat{v}_{t+1} &= \hat{v}_t - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} \left(\mathcal{A}^\ast \mathcal{A} (u_\ast v_\ast^\top v_t v_t^\top  -  B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top ( \langle v_t, v_\ast \rangle u_\ast  - B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast) \nonumber \\
    &= \hat{v}_t - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} \left(\mathcal{A}^\ast \mathcal{A} (u_\ast v_\ast^\top v_t v_t^\top - u_\ast v_\ast^\top) \right)^\top  \langle v_t, v_\ast \rangle u_\ast  \nonumber \\
    &\quad \quad + \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} \left(\mathcal{A}^\ast \mathcal{A} ( B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast v_t^\top)\right)^\top  \langle v_t, v_\ast \rangle u_\ast   \nonumber \\
    &\quad \quad - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} \left(\mathcal{A}^\ast \mathcal{A} ( B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast v_t^\top)\right)^\top B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast \nonumber \\
    &\quad \quad + \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} \left(\mathcal{A}^\ast \mathcal{A} (u_\ast v_\ast^\top v_t v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast
\end{align}
Here we have $V_{\ast, \perp} = I - v_\ast v_\ast^\top$. Multiplying both sides by this matrix and taking the spectral norm yields
\begin{align}
    \text{dist}({v}_{t+1}, v_\ast)
    &=\frac{1}{\|\hat{v}_{t+1}\|_2} \Big\| \|\hat{v}_{t}\|_2 V_{\ast, \perp}^\top {v}_t - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|_2} V_{\ast, \perp}^\top\left(\mathcal{A}^\ast \mathcal{A} (u_\ast v_\ast^\top v_t v_t^\top - u_\ast v_\ast^\top) \right)^\top  \langle v_t, v_\ast \rangle u_\ast  \nonumber \\
    &\quad \quad + \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} V_{\ast, \perp}^\top\left(\mathcal{A}^\ast \mathcal{A} ( B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast v_t^\top)\right)^\top  \langle v_t, v_\ast \rangle u_\ast   \nonumber \\
    &\quad \quad - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} V_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} ( B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast v_t^\top)\right)^\top B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast \nonumber \\
    &\quad \quad + \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} V_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (u_\ast v_\ast^\top v_t v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast \Big\|_2
\end{align}


Steps: 1. show the first line contracts distance. 2. show the error terms are sufficiently small.. but they must also be a function of the distance.

Consider the second term:
\begin{align}
    &\|V_{\ast, \perp}^\top\left(\mathcal{A}^\ast \mathcal{A} ( B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast v_t^\top)\right)^\top  \langle v_t, v_\ast \rangle u_\ast\|_2\nonumber\\ 
    &\leq \langle v_t, v_\ast \rangle \|\left(\mathcal{A}^\ast \mathcal{A} ( B^{-1}(\langle v_t, v_\ast \rangle B - C)u_\ast v_t^\top)\right) V_{\ast, \perp}\|_2 \nonumber \\
    &= 
\end{align}



%\begin{align} \label{alternative}
%  \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|^2 
%  &=  \| (C - I) u_\ast v_t^\top - (B-I) u_\ast v_\ast^\top %+
%   (u_\ast v_t^\top  - u_\ast v_\ast^\top) \|^2,
%\end{align}
%Recall that $ B \coloneqq \sum_{i=1}^N A_i {v}_t {v}_t^\top A_i^\top$.  Using RIP, we know that $|\lambda_{\min} (B - I)|$ and $|\lambda_{\max} (B - I)|$ are less than $\delta_{2k}$ (note that $B$ is PSD). Hence, $||(B - I)u_\ast v_\ast^\top|| \leq ||(B - I)||_2 ||u_\ast v_\ast^\top||_2 $.  To bound $C - I$ we can write:
% \begin{align*}
%    C - I &=\sum_{i=1}^N A_i {v}_t v_\ast^\top A_i^\top - I \\
%    &= \sum_{i=1}^N A_i {v}_t v_\ast^\top A_i^\top  -  \sum_{i=1}^N A_i {v}_\ast v_\ast^\top A_i^\top + \sum_{i=1}^N A_i {v}_\ast v_\ast^\top A_i^\top - I
% \end{align*}
%and hence
%\begin{align*}
%    ||C - I|| \leq ||\sum_{i=1}^N A_i {v}_t v_\ast^\top A_i^\top  -  \sum_{i=1}^N A_i {v}_\ast v_\ast^\top A_i^\top ||  + \delta_{2k}
%    \leq (1+\delta_{2k})\sqrt{2(1 - \text{dist}(v_t, v_\ast)^2)} + \delta_{2k}.
%\end{align*}
%Also, the third term can be bounded by $\sqrt{1 - \text{dist}(v_\ast, v_t)^2}$.


\end{proof}
\end{comment}

-------------------------------------

{\color{blue} \textbf{Full Proof of Rank-1, Sub-gaussian case:}}

First we establish some basic definitions.

The problem we aim to solve is
\begin{align}
    F(\hat{u}, \hat{v}) &= \frac{1}{2}\sum_{i=1}^N \langle A_i, \hat{u} \hat{v}^T - \sigma_\ast u_\ast v_\ast^\top \rangle^2 \label{rank1sg:obj}
\end{align}




The distance between the iterates $\hat{v}_t$ and the optimal solution $v_\ast$ is given by
\begin{align}
    \text{dist}(\hat{v}_t, v_\ast) &\coloneqq \text{dist}(v_t, v_\ast) \coloneqq \|V_{\ast,\perp}^\top v_t\|_2 = \|(I - v_\ast v_\ast^\top)^\top v_t\|_2 = \sqrt{v_t^\top (I - v_\ast v_\ast^\top)v_t} = \sqrt{1 - \langle v_t, v_\ast \rangle^2 }
\end{align}


Next we make the following assumption.
\begin{assumption} \label{assump:rank1sg}
$\mathcal{A}$ satisfies $4$-RIP with parameter $\delta_{4}$, and the initial iterate $\hat{v}_0$ is chosen such that
\begin{equation}
    0< \frac{ \|\hat{v}_{0}\|_2^2}{4\sigma_\ast^2} \frac{(1-\delta_4)^2}{(1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2}\left( \frac{(\langle v_0, v_\ast \rangle( \langle v_0, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4))(1-\delta_4)^4}{(1+\delta_4)^4} - {2\sqrt{2} \delta_4 } \right) 
\end{equation}
\end{assumption}
For example, if $\frac{ \|\hat{v}_{0}\|_2^2}{4\sigma_\ast^2} \geq 1 $ and $\langle v_0, v_\ast \rangle \geq 0.1$, then $\delta_4 <=  2.5 \times 10^{-3}$ will suffice with $\eta \leq 2.8 \times 10^{-5}$ (relevant to theorem). If $\langle v_0, v_\ast \rangle \geq 0.5$, then we can have $\delta_4 \leq 0.04$ with $\eta \leq 0.015$.
%(1-x)^2((0.1(0.1-x) - x(1+x))(1-x)^4  - 2\sqrt{2}x(1+x)^4 )/((1+3x)^2(1+\sqrt{2}x)^2(1+x)^4), x=0.0025

Note that the majority of our results will hold as long as $\mathcal{A}$ satisfies $2$-RIP (a weaker condition), but we need $4$-RIP for one part, so we use $4$-RIP for the whole proof.




Next we prove some additional helpful lemmas specific to our problem:
\begin{lemma} \label{lem:B1}
The following holds:
\begin{equation}
    \| B^{-1} \|_2 \leq \frac{1}{1-\delta_4}
\end{equation}
\end{lemma}

\begin{proof}
See proof of Lemma 4.3, equation 28 in JNS14 (with factor of 3 removed due to Lemma \ref{lem:rip1}).
\end{proof}

\begin{lemma} \label{lem:B2}
The following holds:
\begin{equation}
    \| B^{-1} C\|_2 \leq \frac{1+\delta_4}{1-\delta_4}
\end{equation}
and 
\begin{equation}
    \sigma_{min}(B^{-1} C ) \geq \frac{\sqrt{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}}{1+\delta_4},
\end{equation}
noting that $\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)\geq 0$ from Assumption \ref{assump:rank1sg} (as we will show that $\langle v_t, v_\ast \rangle$ is increasing in $t$).
\end{lemma}

\begin{proof}


We have
\begin{align}
     \| B^{-1} C\|_2 &\leq \| B^{-1}\|\| C\|_2 \leq \frac{1}{1-\delta}\| C\|_2
\end{align}
from Lemma \ref{lem:B1}. To bound $\| C\|_2$ we
use similar analysis as in equation 28 in JNS14. However, since $C$ is not symmetric, its singular values and eigenvalues do not coincide, making the analysis more tedious. We bound $\| C\|_2$ by computing the maximum eigenvalue of $C^\top C$:
\begin{align}
    \| C\|_2^2 &= \max_{z: \|z\|_2 = 1} z^\top C^\top C z \nonumber\\
    &= \max_{z: \|z\|_2 = 1} z^\top \left( \sum_{i=1}^N A_i  v_\ast v_t^\top A_i^\top \right) C z \nonumber\\
    &= \max_{z: \|z\|_2 = 1}  \sum_{i=1}^N \text{tr}(z^\top A_i v_\ast) \text{tr}(v_t^\top A_i^\top C z) \nonumber\\
    &= \max_{z: \|z\|_2 = 1}  \sum_{i=1}^N \text{tr}( A_i v_\ast z^\top) \text{tr}( A_i^\top C z v_t^\top) \nonumber\\
    &= \max_{z: \|z\|_2 = 1} \langle \mathcal{A}(z v_\ast^\top), \mathcal{A}( C z v_t^\top) \rangle \nonumber\\
    &\leq \max_{z: \|z\|_2 = 1} \langle z v_\ast^\top, Cz v_t^\top\rangle + \delta_4 \| z v_\ast^\top\|_F \|C z v_t^\top\|_F \label{uselem11}\\
    &= \max_{z: \|z\|_2 = 1} \langle z v_\ast^\top, Cz v_t^\top\rangle + \delta_4 \|C\|_2 \label{lem12result}
\end{align}
where \eqref{uselem11} follows from \ref{lem:rip1}. Next, we have
\begin{align}
    \max_{z: \|z\|_2 = 1} \langle z v_\ast^\top, Cz v_t^\top\rangle &= \max_{z: \|z\|_2 = 1} z^\top Cz v_t^\top v_\ast \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \sum_{i=1}^N z^\top A_i v_t v_\ast^\top A_i^\top z (v_t^\top v_\ast) \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \langle \mathcal{A}(z v_t^\top), \mathcal{A}(z v_\ast^\top)\rangle (v_t^\top v_\ast) \nonumber \\
    &\leq \max_{z: \|z\|_2 = 1} \langle z v_t^\top, z v_\ast^\top \rangle (v_t^\top v_\ast) + \delta_4 \|z v_t^\top\|_F \|z v_\ast^\top\|_F (v_t^\top v_\ast) \nonumber \\
    &\leq \langle v_t, v_\ast \rangle (\langle v_t, v_\ast \rangle + \delta_4)
\end{align}
Combining this with \eqref{lem12result} yields:
\begin{align}
    \| C\|_2^2 &\leq \langle v_t, v_\ast \rangle (\langle v_t, v_\ast \rangle + \delta_4) + \delta_4 \|C\|_2
\end{align}
Using the quadratic formula, we obtain
\begin{align}
    \| C\|_2 &\leq \frac{1}{2}\left(\delta_4 + \sqrt{\delta_4^2 + 4\langle v_t, v_\ast \rangle(\langle v_t, v_\ast \rangle + \delta_4) } \right) \nonumber \\
    &= \frac{1}{2}\left(\delta_4 + (2 + \delta) \right) \nonumber \\
    &= 1+\delta_4 \label{c2},
\end{align}
completing the first claim.

Likewise, to prove the second claim we have
\begin{align}
   \sigma_{\min}(B^{-1} C) &\geq \sigma_{\min}(B^{-1}) \sigma_{\min}(C)
\end{align}
and, since $B$ is symmetric, the absolute values of its singular values and eigenvalues coincide, so we can write
\begin{align}
    \sigma_{\max}(B)&= \max_{z: \|z\|_2 = 1} z^\top \left( \sum_{i=1}^N A_i v_t v_t^\top A_i^\top \right) z \nonumber\\
    &= \max_{z: \|z\|_2 = 1} \langle \mathcal{A}( z v_t^\top), \mathcal{A}(z v_t^\top)\rangle \nonumber\\
    &\leq \max_{z: \|z\|_2 = 1} \langle  z v_t^\top,  z v_t^\top\rangle + \delta_4 \| z v_t^\top\|_F^2 \\
    &= 1 + \delta_4 
\end{align}
thus $\sigma_{\min}(B^{-1}) \geq \frac{1}{1+\delta_4}$. 

Next, we consider $C$:
\begin{align}
    \sigma_{\min}(C)^2 &= \min_{z: \|z\|_2=1} z^\top C^\top C z \nonumber \\
    &= \min_{z: \|z\|_2=1} \langle \mathcal{A}(z v_\ast^\top), \mathcal{A}(C z v_t^\top) \rangle  \nonumber\\
    &\geq \min_{z: \|z\|_2=1} \langle z v_\ast^\top, C z v_t^\top \rangle - \delta_4 \|z v_\ast^\top\|_F \|C z v_t^\top\|_F  \nonumber \\
    &\geq \min_{z: \|z\|_2=1} \langle z v_\ast^\top, C z v_t^\top \rangle - \delta_4 \|C\|_2  \nonumber
\end{align}
Continuing,
\begin{align}
     \min_{z: \|z\|_2=1} \langle z v_\ast^\top, C z v_t^\top \rangle &= \min_{z: \|z\|_2=1} z^\top C z v_t^\top v_\ast \nonumber \\
     &= \min_{z: \|z\|_2=1} \sum_{i=1}^N z^\top A_i v_t v_\ast^\top A_i^\top z v_t^\top v_\ast \nonumber \\
     &=\min_{z: \|z\|_2=1} \langle \mathcal{A}(z v_t^\top), \mathcal{A}(z v_\ast^\top) \rangle (v_t^\top v_\ast) \nonumber \\
     &\geq \min_{z: \|z\|_2=1} \langle z v_\ast^\top, z v_t^\top \rangle (v_t^\top v_\ast) - \delta_4 \| z v_\ast^\top \|_F \| z v_t^\top \|_F (v_t^\top v_\ast)  \nonumber \\
     &=\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4)
\end{align}
Thus 
\begin{align}
    \sigma_{\min}(C)^2 &\geq \langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 \|C\|_2 \nonumber \\
    &\geq \langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)
\end{align}
Assuming $\delta_4$ is small enough such that the RHS is at least 0 for all $t$, then we have
\begin{align}
     \sigma_{\min}(C)
    &\geq  \sqrt{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}
\end{align}
completing the proof.

\end{proof}

\begin{lemma} \label{lem:B3}
The following holds:
\begin{equation}
    || B^{-1}C u_\ast v_t^\top -  u_\ast v_\ast^\top ||_2^2 \leq  \frac{8 (1+\delta_4)(1 +3\delta_4) }{(1-\delta_4)^2} \text{dist}^2(v_t,v_\ast) %\leq \frac{8(1 +3\delta_4)^2 }{(1-\delta_4)^2} \text{dist}^2(v_t,v_\ast) 
    %\frac{8((1+\delta_4)}{(1-\delta)^2}\text{dist}(v_t, v_\ast)^2.
\end{equation}
% where $\theta \coloneqq 4 (1+\delta_4)^2 (1 - \langle v_t, v_\ast \rangle) + 2(1 - \langle v_t, v_\ast \rangle)^2 + 4\delta_4(1 - \langle v_t, v_\ast \rangle)\sqrt{2(1 - \langle v_t, v_\ast\rangle)} + 4 \delta_4^2 (1 - \langle v_t, v_\ast\rangle)$.
Moreover, this implies the following:
\begin{equation}
    || \mathcal{A}^*\mathcal{A}(B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top ) ||_2^2 \leq
    \frac{8 (1+\delta_4)(1 +3\delta_4)  (1+ \sqrt{2}\delta_4)^2}{(1-\delta_4)^2} \text{dist}^2(v_t,v_\ast) % \leq \frac{8 (1 +3\delta_4)^2  (1+ \sqrt{2}\delta_4)^2}{(1-\delta_4)^2} \text{dist}^2(v_t,v_\ast) 
\end{equation}
\end{lemma}
\begin{proof}
We first show the first claim. Notice
\begin{align}
    || B^{-1}C u_\ast v_t^\top -  u_\ast v_\ast^\top ||_2^2 &= || B^{-1}(C u_\ast v_t^\top - B u_\ast v_\ast^\top) ||_2^2 \nonumber \\
    &\leq \frac{1}{(1- \delta_4)^2}|| (C u_\ast v_t^\top - B u_\ast v_\ast^\top) ||_2^2 \label{B21} \\
    &=\frac{1}{(1- \delta_4)^2} \|C u_\ast v_t^\top - C u_\ast v_\ast^\top + C u_\ast v_\ast^\top - B u_\ast v_\ast^\top \|_2^2 \nonumber\\
  & = \frac{1}{(1- \delta_4)^2} || Cu_\ast(v_t - v_\ast)^\top + (C-B)u_\ast v_\ast^\top)||_2^2 
\end{align}
where \eqref{B21} follows from the Cauchy-Schwarz inequality and Lemma \ref{lem:B1}. 
% First note that using $2k$-RIP we have for any rank-$2k$ matrix $x$ that:
% $$ ||\mathcal{A}^*\mathcal{A}(x) - x||_2 \leq \delta_{2k} ||x||_F,$$
% and we thus obtain
% $$||\mathcal{A}^*\mathcal{A}(x)||_2 \leq (1 + \sqrt{2k} \delta_{2k}) ||x||_2,$$
% as $||x||_F \leq \sqrt{2k}||x||_2$ when $\text{rank}(x) \leq 2k$.
% Continuing from \eqref{norm-a*a} and noting that has at most rank 2, we obtain 
% $$|| \mathcal{A}^*\mathcal{A}(C u_\ast v_t^\top - B u_\ast v_\ast^\top) ||_2^2 \leq (1 + \sqrt{2}\delta_4)^2   \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|_2^2 $$
% and 
% \begin{align} \label{alternative}
%   \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|_2^2 
%   &=  \|C u_\ast v_t^\top - C u_\ast v_\ast^\top + C u_\ast v_\ast^\top - B u_\ast v_\ast^\top \|_2^2 \\
%   & = || Cu_\ast(v_t - v_\ast)^\top + (C-B)u_\ast v_\ast^\top)||_2^2
% \end{align}
Now, let's first bound the norm of $Cu_\ast(v_t - v_\ast)^\top$. We have: 
\begin{align*}
||Cu_\ast(v_t - v_\ast)^\top||_2 & \leq 
||Cu_\ast ||_2 ||(v_t - v_\ast)^\top||_2 \\
&\leq ||C ||_2 \sqrt{2(1 - \langle v_t, v_\ast\rangle)}\\
&\leq (1+\delta_4) \sqrt{2(1 - \langle v_t, v_\ast \rangle)}
% &\leq ||C ||_2 \sqrt{2(1 - \langle v_t, v_\ast \rangle^2)} \\
% &\leq (1+\delta_k)  \sqrt{2\text{dist}(v_t, v_\ast)},
\end{align*}
where we have used 
$$|| C||_2 \leq  (1+\delta_4)$$
from \eqref{c2}.
In the same manner, by using RIP and Lemma \ref{lem:rip1} we can write
\begin{align*}
    || C - B ||_2^2 &= \max_{z: \|z\|_2 = 1} z^\top (C - B)^\top (C - B) z \nonumber \\
    &= \max_{z: \|z\|_2 = 1} z^\top \left(\sum_{i=1}^N A_i  (v_t - v_\ast) v_t^\top A_i^\top \right) (C - B) z \nonumber \\
    &= \max_{z: \|z\|_2 = 1}  \sum_{i=1}^N \text{tr}(z^\top A_i (v_t - v_\ast))\text{tr}(v_t^\top A_i^\top (C - B)z) \nonumber \\
    &= \max_{z: \|z\|_2 = 1}  \langle \mathcal{A}(z (v_t - v_\ast)^\top), \mathcal{A}((C - B) z v_t^\top) \rangle \nonumber \\
    &\leq \max_{z: \|z\|_2 = 1}  \langle z (v_t - v_\ast)^\top, (C-B) z v_t^\top \rangle + \delta_4 \|z (v_t - v_\ast)^\top\|_F \| (C - B)zv_t^\top \|_F \nonumber \\
    &\leq \max_{z: \|z\|_2 = 1}  \langle z (v_t - v_\ast)^\top, (C-B) z v_t^\top \rangle + \delta_4 \sqrt{2(1-\langle v_t, v_\ast\rangle)} \| C - B\|_2 %\nonumber \\
    % &= 1 - \langle v_t, v_\ast \rangle + \delta_4 \sqrt{2(1 - \langle v_t, v_\ast\rangle)} \nonumber \\
    % &\leq \sqrt{2(1 - \langle v_t, v_\ast \rangle)} + \delta_4 \sqrt{2(1 - \langle v_t, v_\ast\rangle)} \nonumber \\
    % &= (1 + \delta_4)\sqrt{2(1 - \langle v_t, v_\ast \rangle)}
    %\leq (1+\delta_k) || v_t (v_t - v_\ast)^\top ||_2 \leq || v_t||_2 || v_t - v_\ast||_2 \leq \sqrt{2 \text{dist}(v_t, v_\ast)}.
\end{align*}
where the last equation follows since $\|(C-B)z v_t^\top\|_F \leq \|(C-B)\|_2 \|z v_t^\top\|_F = \|C-B\|_2$. Next,
\begin{align}
    \max_{z: \|z\|_2 = 1}  \langle z (v_t - v_\ast)^\top, (C-B) z v_t^\top \rangle &= \max_{z: \|z\|_2 = 1} \sum_{i=1}^N \text{tr} ((v_t - v_\ast) z^\top A_i v_t (v_t - v_\ast)^\top A_i^\top z v_t^\top ) \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \sum_{i=1}^N \text{tr} (z^\top A_i v_t (v_t - v_\ast)^\top A_i^\top z v_t^\top (v_t - v_\ast)  ) \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \sum_{i=1}^N \text{tr} (z^\top A_i v_t) \text{tr}( (v_t - v_\ast)^\top A_i^\top z) (1 -  \langle v_t, v_\ast\rangle) \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \langle \mathcal{A}(z v_t^\top) , \mathcal{A}( z (v_t - v_\ast)^\top )\rangle (1 -  \langle v_t, v_\ast\rangle) \nonumber \\
    &\leq  \max_{z: \|z\|_2 = 1} (1 -  \langle v_t, v_\ast\rangle) \langle z v_t^\top, z (v_t - v_\ast)^\top \rangle \nonumber \\
    &\quad \quad+ \delta_4 (1 -  \langle v_t, v_\ast\rangle) \| z v_t^\top\|_F \|z (v_t - v_\ast)^\top\|_F \nonumber \\
    &\leq (1 -  \langle v_t, v_\ast\rangle)^2 + \delta_4 \sqrt{2} (1 -  \langle v_t, v_\ast\rangle)^{3/2}
\end{align}
Putting these together, we have
\begin{align}
    || C - B ||_2^2 &\leq (1 -  \langle v_t, v_\ast\rangle)^2 + \delta_4 \sqrt{2} (1 -  \langle v_t, v_\ast\rangle)^{3/2} + \delta_4 \sqrt{2(1-\langle v_t, v_\ast\rangle)} \| C - B\|_2  \nonumber \\
    &\leq (1 -  \langle v_t, v_\ast\rangle) +\sqrt{2} \delta_4  (1 -  \langle v_t, v_\ast\rangle) + \delta_4 \sqrt{2(1-\langle v_t, v_\ast\rangle)} \| C - B\|_2  \nonumber \\
\end{align}
where the second inequality follows because $(1 -  \langle v_t, v_\ast\rangle) \leq 1$.
Now using the quadratic formula, we have
\begin{align}
     || C - B ||_2 &\leq \frac{1}{2} \left(\sqrt{2} \delta_4 \sqrt{1 - \langle v_t, v_\ast \rangle} + \sqrt{2 \delta_4^2 (1 - \langle v_t, v_\ast \rangle) + 4(1+\delta_4\sqrt{2})(1 -  \langle v_t, v_\ast\rangle) } \right) \nonumber \\
     &= \frac{1}{2} \left( \sqrt{2} \delta_4  + \sqrt{2 \delta_4^2 + 4\sqrt{2} \delta_4 + 4)}\right)\sqrt{1 -  \langle v_t, v_\ast\rangle } \nonumber \\
     &\leq  \left( \sqrt{2} \delta_4  + (1+ \delta_4)\right)\sqrt{1 -  \langle v_t, v_\ast\rangle } \nonumber \\
     &\leq \left( 1+ 3\delta_4 \right)\sqrt{1 -  \langle v_t, v_\ast\rangle }
\end{align}
% Note that
% \begin{align}
%     \| (C - B)zv_t^\top \|_F^2 &= \text{tr}( v_t z^\top (C - B)^\top (C - B) zv_t^\top) \nonumber \\
%     &= \text{tr}( z^\top (C - B)^\top (C - B) z) \nonumber \\
%     &= 
% \end{align}

And thus: 
$$ ||(C-B) u_\ast v_\ast^\top||_2 \leq ||(C-B)||_2|| u_\ast v_\ast^\top||_2 \leq  (1 +3\delta_4) \sqrt{1 - \langle v_t, v_\ast\rangle} . $$
Putting these together and using the inequality $(a+b)^2 \leq 2a^2 + 2b^2$, we obtain: 
\begin{align}
    \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|_2^2 
    &\leq 8 (1+\delta_4)(1 +3\delta_4) (1 - \langle v_t, v_\ast \rangle) 
    % \nonumber \\
    % &\quad \quad + 2(1 - \langle v_t, v_\ast \rangle)^2 + 4\delta_4(1 - \langle v_t, v_\ast \rangle)\sqrt{2(1 - \langle v_t, v_\ast\rangle)} + 4 \delta_4^2 (1 - \langle v_t, v_\ast\rangle)  \nonumber \\
    % &\leq . %8(1+\delta_4)^2\text{dist}(v_t, v_\ast).
\end{align}
Therefore
\begin{align}
    \|B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top \|_2^2 
    &\leq \frac{8 (1+\delta_4)(1 +3\delta_4) }{(1-\delta_4)^2} (1 - \langle v_t, v_\ast \rangle) 
    % \nonumber \\
    % &\quad \quad + 2(1 - \langle v_t, v_\ast \rangle)^2 + 4\delta_4(1 - \langle v_t, v_\ast \rangle)\sqrt{2(1 - \langle v_t, v_\ast\rangle)} + 4 \delta_4^2 (1 - \langle v_t, v_\ast\rangle)  \nonumber \\
    % &\leq . %8(1+\delta_4)^2\text{dist}(v_t, v_\ast).
\end{align}
%Note that the RHS can be simplified to a looser but much cleaner bound, we leave it in messy form for now.
To show the second claim we first note that by RIP, for any rank-$2k$ matrix $X$ we have that:
\begin{equation}
 ||\mathcal{A}^*\mathcal{A}(X) - X||_2 \leq \delta_{2k} ||X||_F,\end{equation}
and we thus obtain
$$||\mathcal{A}^*\mathcal{A}(X)||_2 \leq (1 + \sqrt{2k} \delta_{2k}) ||X||_2,$$
as $||\mathcal{A}^*\mathcal{A}(X) - X||_2 \geq ||\mathcal{A}^*\mathcal{A}(X)||_2 - ||X||_2$, and $||X||_F \leq \sqrt{2k}||X||_2$ when $\text{rank}(X) \leq 2k$. Using this and noting that $B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top$ has rank at most 2, we immediately obtain
\begin{equation}
    || \mathcal{A}^*(\mathcal{A}(B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top ) ||_2^2 \leq
    \frac{8 (1+\delta_4)(1 +3\delta_4)  (1+ \sqrt{2}\delta_4)^2}{(1-\delta_4)^2} (1 - \langle v_t, v_\ast \rangle) 
\end{equation}
Noting that $1-\langle v_t, v_\ast\rangle \leq 1-\langle v_t, v_\ast\rangle^2 = \text{dist}^2(v_t, v_\ast)$
completes the proof.
\end{proof}
\begin{lemma}
The sequence $\{ \|\hat{v}_t\|_2\}_t$ is monotone increasing. Moreover, $\|\hat{v}_t\| \leq c \|\hat{v}_0\|_2$ for some absolute constant $c$. 
\end{lemma}
\begin{proof}
We have
\begin{align}
    \hat{v}_{t+1}^\top \hat{v}_{t+1} &= \hat{v}_{t}^\top \hat{v}_{t} - 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_t \|} \sum_{i=1}^N  \left(  u_\ast^\top C^\top B^{-\top}  A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) \hat{v}_{t}^\top A_i^\top  B^{-1} C u_\ast \nonumber \\
    &\quad \quad + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_t \|^2}  \sum_{i=1}^N  \sum_{i'=1}^N  \left(u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right)\left(u_\ast^\top C^\top B^{-\top} A_{i'} {v}_t  -  u_\ast^\top A_{i'} v_\ast \right) u_\ast^\top C^\top B^{\top}A_i A_{i'}^\top B^{-1} C u_\ast  \label{rank1sg:square}
\end{align}
We expect the cross terms to be close to zero:
\begin{align}
    \frac{\sigma_\ast^2}{\|\hat{v}_t \|}& \sum_{i=1}^N  \left(  u_\ast^\top C^\top B^{-\top}  A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) \hat{v}_{t}^\top A_i^\top  B^{-1} C u_\ast  \nonumber \\
    &= {\sigma_\ast^2} \sum_{i=1}^N  u_\ast^\top C^\top B^{-\top}  A_i {v}_t {v}_{t}^\top A_i^\top B^{-1} C u_\ast -  u_\ast^\top A_i v_\ast{v}_{t}^\top A_i^\top  B^{-1} C u_\ast \nonumber \\
    &= {\sigma_\ast^2} u_\ast^\top C^\top B^{-\top} \left(\sum_{i=1}^N A_i {v}_t {v}_{t}^\top A_i^\top\right) B^{-1} C u_\ast  -  {\sigma_\ast^2} u_\ast^\top \left(\sum_{i=1}^N A_i v_\ast{v}_{t}^\top A_i^\top \right) B^{-1} C u_\ast\nonumber \\
    &= {\sigma_\ast^2} u_\ast^\top C^\top B^{-\top} C u_\ast  -  {\sigma_\ast^2} u_\ast^\top C^\top  B^{-1} C u_\ast\nonumber \\
    &= 0 \label{rank1sq:cross}
\end{align}
where \eqref{rank1sq:cross} follows because $B$ is symmetric.
Next, we expect the last term of \eqref{rank1sg:square} to monotonically increase with the distance $1-\langle v_t, v_\ast \rangle^2$:
\begin{align}
\Psi &\coloneqq \frac{\sigma_\ast^4}{\|\hat{v}_t \|^2} \sum_{i=1}^N  \sum_{i'=1}^N  \left(u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right)\left(u_\ast^\top C^\top B^{-\top} A_{i'} {v}_t  -  u_\ast^\top A_{i'} v_\ast \right) u_\ast^\top C^\top B^{-\top}A_i A_{i'}^\top B^{-1} C u_\ast  \nonumber \\
&= \frac{\sigma_\ast^4}{\|\hat{v}_t \|^2} \sum_{i=1}^N  \sum_{i'=1}^N  \left(u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) u_\ast^\top C^\top B^{-\top}A_i A_{i'}^\top B^{-1} C u_\ast \left(u_\ast^\top C^\top B^{-\top} A_{i'} {v}_t  -  u_\ast^\top A_{i'} v_\ast \right) \nonumber \\
&= 
\end{align}



To be continued....
\end{proof}


We now have all the ingredients necessary to show linear convergence.
\begin{theorem}
Under Assumption \ref{assump:rank1sg}, the iterates of our alternating minimization-descent algorithm satisfy:
\begin{align}
    \text{dist}(\hat{v}_{t+1}, v_\ast) \leq \sqrt{1 - \eta} \text{dist}(\hat{v}_{t}, v_\ast) 
\end{align}
 for any step size $\eta$ satisfying
\begin{equation}
   0 < \eta \leq \frac{ \|\hat{v}_{0}\|_2^2}{4\sigma_\ast^2} \frac{(1-\delta_4)^2}{(1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2}\left( \frac{(\langle v_0, v_\ast \rangle( \langle v_0, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4))(1-\delta_4)^4}{(1+\delta_4)^4} - {2\sqrt{2} \delta_4 } \right), 
\end{equation}
for which some such $\eta$ is guaranteed to exist.
\end{theorem}

\begin{proof}
Setting the gradient of \eqref{rank1sg:obj} with respect to $\hat{u}$ equal to 0, we obtain that the update for $\hat{u}_{t+1}$ is:
\begin{align}
    \hat{u}_{t+1} &= \frac{\sigma_{\ast}}{\|\hat{v}_t \|} B^{-1} C u_\ast
\end{align}
where
\begin{align}
    B &\coloneqq \sum_{i=1}^N A_i {v}_t {v}_t^\top A_i^\top \\
    C &\coloneqq \sum_{i=1}^N A_i {v}_t v_\ast^\top A_i^\top 
\end{align}
Plugging this back into the objective, we obtain
\begin{align}
    F(\hat{u}_{t+1}, \hat{v}) &= \frac{1}{2}\sum_{i=1}^N \langle A_i, \frac{\sigma_{\ast}}{\|\hat{v}_t \|} B^{-1} C u_\ast \hat{v}^T - \sigma_\ast u_\ast v_\ast^\top \rangle^2 \\
    &= \frac{1}{2}\sum_{i=1}^N \sigma_\ast^2 \left( \hat{v}^T A_i^\top \frac{1}{\|\hat{v}_t \|} B^{-1} C u_\ast - v_\ast^\top A_i^\top u_\ast \right)^2 
%eliminate u_\ast?
\end{align}
Then the gradient with respect to $\hat{v}$ is
\begin{align}
    \nabla_{\hat{v}} F(\hat{u}_{t+1}, \hat{v}) = \sum_{i=1}^N \sigma_\ast^2 \left(  u_\ast^\top C^\top B^{-\top} A_i \frac{1}{\|\hat{v}_t \|}  \hat{v}  -  u_\ast^\top A_i v_\ast \right) A_i^\top \frac{1}{\|\hat{v}_t \|} B^{-1} C u_\ast 
    =: S_t
\end{align}
and we have
\begin{align}
    \hat{v}_{t+1} = \hat{v}_{t} - \eta \sum_{i=1}^N \sigma_\ast^2 \left(  u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) A_i^\top \frac{1}{\|\hat{v}_t \|} B^{-1} C u_\ast 
\end{align}
Using operator notation, this is
\begin{align}
    \hat{v}_{t+1} = \hat{v}_t - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast
\end{align}
where $\mathcal{A}^\ast$ is the adjoint of the operator $\mathcal{A}$. Multiplying both sides by $V_{\ast, \perp}^\top$ yields
\begin{align}
    V_{\ast, \perp}^\top \hat{v}_{t+1} = V_{\ast, \perp}^\top \hat{v}_t - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} V_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast
\end{align}
After dividing both sides by $\| \hat{v}_{t+1}\|_2$ and taking the 2-norm squared of both sides, we obtain
\begin{align}
    \text{dist}^2({v}_{t+1}, v_\ast ) &= \frac{1}{\|\hat{v}_{t+1}\|_2^2}\left\|V_{\ast, \perp}^\top \hat{v}_t - \eta \frac{\sigma_\ast^2}{\|\hat{v}_t\|} V_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast)\right\|_2^2 \nonumber \\
    &= \frac{\|\hat{v}_t\|_2^2}{\|\hat{v}_{t+1}\|_2^2}\text{dist}^2({v}_t, v_\ast) - 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2} \langle V_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast, V_{\ast, \perp}^\top v_t \rangle \nonumber \\
    &\quad \quad + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_{t}\|_2^2} \|V_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast \|_2^2 \label{3terms1}
\end{align}
We will control each of the above terms, starting with the cross term:
\begin{align}
    &\langle V_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast, V_{\ast, \perp}^\top v_t \rangle \nonumber \\
    &= \langle  \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top, V_{\ast, \perp} V_{\ast, \perp}^\top v_t u_\ast^\top C^\top B^{-\top} \rangle \nonumber \\
    &= \langle  \mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) , B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \rangle \nonumber \\
    &= \langle\mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) , \mathcal{A}^\ast ( B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top) \rangle \nonumber \\
    &\geq \langle B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top, B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \rangle - \delta_4 \| B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top \|_F \| B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \|_F \label{uselem12}
\end{align}
%note: I should change all $\delta_4 \rightarrow \delta_4$
where \eqref{uselem12} follows from Lemma \ref{lem:rip1} and the fact that the relevant matrices matrices have rank at most 2. Next, note that 
\begin{align}
    \langle u_\ast v_\ast^\top, B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \rangle &= \text{tr}(v_\ast u_\ast^\top B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top ) \nonumber \\
    &=  u_\ast^\top B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top v_\ast  \nonumber \\
    &= 0
\end{align}
since $V_{\ast, \perp}^\top v_\ast = 0$ by definition of $V_{\ast, \perp}$. Thus,
\begin{align}
    \langle B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top, B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \rangle &= \langle B^{-1} C u_\ast v_t^\top V_{\ast, \perp}, B^{-1} C u_\ast v_t^\top V_{\ast, \perp}  \rangle \nonumber \\
    &= \| B^{-1} C u_\ast v_t^\top V_{\ast, \perp} \|_F^2 \nonumber \\
    &\geq  \sigma_{\min}^2( B^{-1} C )  \|v_t^\top V_{\ast, \perp} \|_2^2 \nonumber \\
    &\geq  \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2} \text{dist}^2(v_t, v_\ast) \label{cross1}
\end{align}
where \eqref{cross1} follows from Lemma \ref{lem:B1}. Next, we need to upper bound the negative term in \eqref{uselem12}. We have
\begin{align}
    \| B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \|_F &= \| B^{-1} C u_\ast v_t^\top V_{\ast, \perp} \|_F \nonumber \\
    &\leq \| B^{-1} C\|_2 \| u_\ast\|_F \|v_t^\top V_{\ast, \perp} \|_2 \nonumber \\
    &\leq \frac{1 + \delta_4}{1 - \delta_4} \text{dist}(v_t,v_\ast)
\end{align}
and thus
\begin{align}
    \| B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top \|_F \| B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \|_F &\leq   \frac{2\sqrt{2} (1 + 3\delta_4) (1 + \delta_4)}{(1 - \delta_4)^2} \text{dist}^2(v_t,v_\ast)
\end{align}
using Lemma \ref{lem:B2} and the fact $\langle v_t, v_\ast \rangle \leq 1$.

Thus we have completed our bound on the cross term:
\begin{align}
    \langle V_{\ast, \perp}^\top \big(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top &- u_\ast v_\ast^\top) \big)^\top B^{-1} C u_\ast, V_{\ast, \perp}^\top v_t \rangle \nonumber \\
    &\geq \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)x}{(1+\delta_4)^2} \text{dist}^2(v_t, v_\ast) - \frac{2\sqrt{2} \delta_4 (1 + \delta_4)^2}{(1 - \delta_4)^2} \text{dist}^2(v_t,v_\ast) \label{2ndterm}
\end{align}
We now turn to the final term in \eqref{3terms1}. We have
\begin{align}
    \|V_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast \|_2^2 &\leq \| \mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top)\|_2^2\| V_{\ast, \perp}\|_2^2 \| B^{-1} C \|_2^2 \|u_\ast\|_F^2 \nonumber \\
    &\leq \frac{8 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \text{dist}^2(v_t,v_\ast)  \label{3rdtermm}
\end{align}
where \label{3rdterm} follows from Lemmas \ref{lem:B1} and \ref{lem:B2} and the fact that $\|V_{\ast, \perp}\|_2 = \|u_\ast\|_F = 1$. 

 Combining \eqref{3terms1}, \eqref{2ndterm} and \eqref{3rdtermm} yields
\begin{align}
    &\text{dist}^2({v}_{t+1}, v_\ast ) \nonumber\\
    &= \frac{\|\hat{v}_t\|_2^2}{\|\hat{v}_{t+1}\|_2^2}\text{dist}^2({v}_t, v_\ast) - 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2} \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2} \text{dist}^2(v_t, v_\ast) \nonumber \\ 
    &\quad + 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2}\frac{2\sqrt{2} \delta_4 (1 + \delta_4)^2}{(1 - \delta_4)^2} \text{dist}^2(v_t,v_\ast) 
    + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_{t}\|_2^2} \frac{8 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \text{dist}^2(v_t,v_\ast)  \nonumber \\
    &\leq  \text{dist}^2({v}_t, v_\ast)\Bigg(1 - 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2} \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2}  \nonumber \\ 
    &\quad + 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2}\frac{2\sqrt{2} \delta_4 (1 + \delta_4)^2}{(1 - \delta_4)^2}  
    + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_{t}\|_2^2} \frac{8 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \Bigg) \nonumber 
\end{align}
where we have used the fact that $\|\hat{v}_t\|_2 \leq \|\hat{v}_{t+1}\|_2$ from Lemma \ref{}. In order to ensure linear convergence we must have
\begin{align}
    &2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2} \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2} \geq  2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2}\frac{2\sqrt{2} \delta_4 (1 + \delta_4)^2}{(1 - \delta_4)^2}  \nonumber \\
    &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_{t}\|_2^2} \frac{8 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \nonumber \\
    &\iff \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2} \geq   \frac{2\sqrt{2} \delta_4 (1 + \delta_4)^2}{(1 - \delta_4)^2} + \eta \frac{\sigma_\ast^2}{ \|\hat{v}_{t}\|_2^2} \frac{4 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \nonumber \\
    &\iff \frac{ \|\hat{v}_{t}\|_2^2}{4\sigma_\ast^2} \left( \frac{(\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4))(1-\delta_4)^4}{(1+\delta_4)^4 (1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2} - \frac{2\sqrt{2} \delta_4 (1-\delta_4)^2}{(1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2} \right) \geq  \eta  \nonumber \\
    &\Longleftarrow \frac{ \|\hat{v}_{0}\|_2^2}{4\sigma_\ast^2} \frac{(1-\delta_4)^2}{(1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2}\left( \frac{(\langle v_0, v_\ast \rangle( \langle v_0, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4))(1-\delta_4)^4}{(1+\delta_4)^4} - {2\sqrt{2} \delta_4 } \right) \geq  \eta  
\end{align}
where in the final inequality we used the facts that  $\{\|\hat{v}_t\|\}_t$ is increasing (Lemma \ref{}) and that if $\hat{v}_t$ converges linearly to $v_\ast$, then $\langle v_t, v_\ast \rangle$ is increasing. By Assumption \ref{assump:rank1sg}, we have that the LHS is strictly greater than 0, so we can choose a sufficiently small $\eta$.


% So, all that remains to show is that we can choose a $\delta_4$ small enough such that the above inequality holds (assume for now) (and assume $\langle v_0, v_\ast \rangle$ is large enough).


\end{proof}











==> rank1sg_new.tex <==
\textbf{Rank-1, finite samples:}


{\color{blue} \textbf{From earlier analysis:}}

The problem we aim to solve is
\begin{align}
    F(\hat{u}, \hat{v}) &= \frac{1}{2}\sum_{i=1}^N \langle A_i, \hat{u} \hat{v}^T - \sigma_\ast u_\ast v_\ast^\top \rangle^2 \label{rank1sg:obj}
\end{align}




The distance between the iterates $\hat{v}_t$ and the optimal solution $v_\ast$ is given by
\begin{align}
    \text{dist}(\hat{v}_t, v_\ast) &\coloneqq \|V_{\ast,\perp}^\top v_t\|_2 = \|(I - v_\ast v_\ast^\top)^\top \hat{v}_t\|_2 = \sqrt{\hat{v}_t^\top (I - v_\ast v_\ast^\top)\hat{v}_t} = \sqrt{1 - \langle \hat{v}_t, v_\ast \rangle^2 }
\end{align}

\begin{comment}
Next we make the following assumption.
\begin{assumption} \label{assump:rank1sg}
$\mathcal{A}$ satisfies $4$-RIP with parameter $\delta_{4}$, and the initial iterate $\hat{v}_0$ is chosen such that
\begin{equation}
    0< \frac{ \|\hat{v}_{0}\|_2^2}{4\sigma_\ast^2} \frac{(1-\delta_4)^2}{(1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2}\left( \frac{(\langle v_0, v_\ast \rangle( \langle v_0, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4))(1-\delta_4)^4}{(1+\delta_4)^4} - {2\sqrt{2} \delta_4 } \right) 
\end{equation}
\end{assumption}
For example, if $\frac{ \|\hat{v}_{0}\|_2^2}{4\sigma_\ast^2} \geq 1 $ and $\langle v_0, v_\ast \rangle \geq 0.1$, then $\delta_4 <=  2.5 \times 10^{-3}$ will suffice with $\eta \leq 2.8 \times 10^{-5}$ (relevant to theorem). If $\langle v_0, v_\ast \rangle \geq 0.5$, then we can have $\delta_4 \leq 0.04$ with $\eta \leq 0.015$.
\end{comment}
%(1-x)^2((0.1(0.1-x) - x(1+x))(1-x)^4  - 2\sqrt{2}x(1+x)^4 )/((1+3x)^2(1+\sqrt{2}x)^2(1+x)^4), x=0.0025

Note that the majority of our results will hold as long as $\mathcal{A}$ satisfies $2$-RIP (a weaker condition), but we need $4$-RIP for one part, so we use $4$-RIP for the whole proof.




Next we prove some additional helpful lemmas specific to our problem:
\begin{lemma} \label{lem:B1}
The following holds:
\begin{equation}
    \| B^{-1} \|_2 \leq \frac{1}{1-\delta_4}
\end{equation}
\end{lemma}

\begin{proof}
See proof of Lemma 4.3, equation 28 in JNS14 (with factor of 3 removed due to Lemma \ref{lem:rip1}).
\end{proof}

\begin{lemma} \label{lem:B2}
The following holds:
\begin{equation}
    \| B^{-1} C\|_2 \leq \frac{1+\delta_4}{1-\delta_4}
\end{equation}
and 
\begin{equation}
    \sigma_{min}(B^{-1} C ) \geq \frac{\sqrt{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}}{1+\delta_4},
\end{equation}
noting that $\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)\geq 0$ from Assumption \ref{assump:rank1sg} (as we will show that $\langle v_t, v_\ast \rangle$ is increasing in $t$).
\end{lemma}

\begin{proof}


We have
\begin{align}
     \| B^{-1} C\|_2 &\leq \| B^{-1}\|\| C\|_2 \leq \frac{1}{1-\delta}\| C\|_2
\end{align}
from Lemma \ref{lem:B1}. To bound $\| C\|_2$ we
use similar analysis as in equation 28 in JNS14. However, since $C$ is not symmetric, its singular values and eigenvalues do not coincide, making the analysis more tedious. We bound $\| C\|_2$ by computing the maximum eigenvalue of $C^\top C$:
\begin{align}
    \| C\|_2^2 &= \max_{z: \|z\|_2 = 1} z^\top C^\top C z \nonumber\\
    &= \max_{z: \|z\|_2 = 1} z^\top \left( \sum_{i=1}^N A_i  v_\ast v_t^\top A_i^\top \right) C z \nonumber\\
    &= \max_{z: \|z\|_2 = 1}  \sum_{i=1}^N \text{tr}(z^\top A_i v_\ast) \text{tr}(v_t^\top A_i^\top C z) \nonumber\\
    &= \max_{z: \|z\|_2 = 1}  \sum_{i=1}^N \text{tr}( A_i v_\ast z^\top) \text{tr}( A_i^\top C z v_t^\top) \nonumber\\
    &= \max_{z: \|z\|_2 = 1} \langle \mathcal{A}(z v_\ast^\top), \mathcal{A}( C z v_t^\top) \rangle \nonumber\\
    &\leq \max_{z: \|z\|_2 = 1} \langle z v_\ast^\top, Cz v_t^\top\rangle + \delta_4 \| z v_\ast^\top\|_F \|C z v_t^\top\|_F \label{uselem11}\\
    &= \max_{z: \|z\|_2 = 1} \langle z v_\ast^\top, Cz v_t^\top\rangle + \delta_4 \|C\|_2 \label{lem12result}
\end{align}
where \eqref{uselem11} follows from \ref{lem:rip1}. Next, we have
\begin{align}
    \max_{z: \|z\|_2 = 1} \langle z v_\ast^\top, Cz v_t^\top\rangle &= \max_{z: \|z\|_2 = 1} z^\top Cz v_t^\top v_\ast \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \sum_{i=1}^N z^\top A_i v_t v_\ast^\top A_i^\top z (v_t^\top v_\ast) \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \langle \mathcal{A}(z v_t^\top), \mathcal{A}(z v_\ast^\top)\rangle (v_t^\top v_\ast) \nonumber \\
    &\leq \max_{z: \|z\|_2 = 1} \langle z v_t^\top, z v_\ast^\top \rangle (v_t^\top v_\ast) + \delta_4 \|z v_t^\top\|_F \|z v_\ast^\top\|_F (v_t^\top v_\ast) \nonumber \\
    &\leq \langle v_t, v_\ast \rangle (\langle v_t, v_\ast \rangle + \delta_4)
\end{align}
Combining this with \eqref{lem12result} yields:
\begin{align}
    \| C\|_2^2 &\leq \langle v_t, v_\ast \rangle (\langle v_t, v_\ast \rangle + \delta_4) + \delta_4 \|C\|_2
\end{align}
Using the quadratic formula, we obtain
\begin{align}
    \| C\|_2 &\leq \frac{1}{2}\left(\delta_4 + \sqrt{\delta_4^2 + 4\langle v_t, v_\ast \rangle(\langle v_t, v_\ast \rangle + \delta_4) } \right) \nonumber \\
    &= \frac{1}{2}\left(\delta_4 + (2 + \delta) \right) \nonumber \\
    &= 1+\delta_4 \label{c2},
\end{align}
completing the first claim.

Likewise, to prove the second claim we have
\begin{align}
   \sigma_{\min}(B^{-1} C) &\geq \sigma_{\min}(B^{-1}) \sigma_{\min}(C)
\end{align}
and, since $B$ is symmetric, the absolute values of its singular values and eigenvalues coincide, so we can write
\begin{align}
    \sigma_{\max}(B)&= \max_{z: \|z\|_2 = 1} z^\top \left( \sum_{i=1}^N A_i v_t v_t^\top A_i^\top \right) z \nonumber\\
    &= \max_{z: \|z\|_2 = 1} \langle \mathcal{A}( z v_t^\top), \mathcal{A}(z v_t^\top)\rangle \nonumber\\
    &\leq \max_{z: \|z\|_2 = 1} \langle  z v_t^\top,  z v_t^\top\rangle + \delta_4 \| z v_t^\top\|_F^2 \\
    &= 1 + \delta_4 
\end{align}
thus $\sigma_{\min}(B^{-1}) \geq \frac{1}{1+\delta_4}$. 

Next, we consider $C$:
\begin{align}
    \sigma_{\min}(C)^2 &= \min_{z: \|z\|_2=1} z^\top C^\top C z \nonumber \\
    &= \min_{z: \|z\|_2=1} \langle \mathcal{A}(z v_\ast^\top), \mathcal{A}(C z v_t^\top) \rangle  \nonumber\\
    &\geq \min_{z: \|z\|_2=1} \langle z v_\ast^\top, C z v_t^\top \rangle - \delta_4 \|z v_\ast^\top\|_F \|C z v_t^\top\|_F  \nonumber \\
    &\geq \min_{z: \|z\|_2=1} \langle z v_\ast^\top, C z v_t^\top \rangle - \delta_4 \|C\|_2  \nonumber
\end{align}
Continuing,
\begin{align}
     \min_{z: \|z\|_2=1} \langle z v_\ast^\top, C z v_t^\top \rangle &= \min_{z: \|z\|_2=1} z^\top C z v_t^\top v_\ast \nonumber \\
     &= \min_{z: \|z\|_2=1} \sum_{i=1}^N z^\top A_i v_t v_\ast^\top A_i^\top z v_t^\top v_\ast \nonumber \\
     &=\min_{z: \|z\|_2=1} \langle \mathcal{A}(z v_t^\top), \mathcal{A}(z v_\ast^\top) \rangle (v_t^\top v_\ast) \nonumber \\
     &\geq \min_{z: \|z\|_2=1} \langle z v_\ast^\top, z v_t^\top \rangle (v_t^\top v_\ast) - \delta_4 \| z v_\ast^\top \|_F \| z v_t^\top \|_F (v_t^\top v_\ast)  \nonumber \\
     &=\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4)
\end{align}
Thus 
\begin{align}
    \sigma_{\min}(C)^2 &\geq \langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 \|C\|_2 \nonumber \\
    &\geq \langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)
\end{align}
Assuming $\delta_4$ is small enough such that the RHS is at least 0 for all $t$, then we have
\begin{align}
     \sigma_{\min}(C)
    &\geq  \sqrt{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}
\end{align}
completing the proof.

\end{proof}

\begin{lemma} \label{lem:B3}
The following holds:
\begin{equation}
    || B^{-1}C u_\ast v_t^\top -  u_\ast v_\ast^\top ||_2^2 \leq  \frac{8 (1+\delta_4)(1 +3\delta_4) }{(1-\delta_4)^2} \text{dist}^2(v_t,v_\ast) %\leq \frac{8(1 +3\delta_4)^2 }{(1-\delta_4)^2} \text{dist}^2(v_t,v_\ast) 
    %\frac{8((1+\delta_4)}{(1-\delta)^2}\text{dist}(v_t, v_\ast)^2.
\end{equation}
% where $\theta \coloneqq 4 (1+\delta_4)^2 (1 - \langle v_t, v_\ast \rangle) + 2(1 - \langle v_t, v_\ast \rangle)^2 + 4\delta_4(1 - \langle v_t, v_\ast \rangle)\sqrt{2(1 - \langle v_t, v_\ast\rangle)} + 4 \delta_4^2 (1 - \langle v_t, v_\ast\rangle)$.
Moreover, this implies the following:
\begin{equation}
    || \mathcal{A}^*\mathcal{A}(B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top ) ||_2^2 \leq
    \frac{8 (1+\delta_4)(1 +3\delta_4)  (1+ \sqrt{2}\delta_4)^2}{(1-\delta_4)^2} \text{dist}^2(v_t,v_\ast) % \leq \frac{8 (1 +3\delta_4)^2  (1+ \sqrt{2}\delta_4)^2}{(1-\delta_4)^2} \text{dist}^2(v_t,v_\ast) 
\end{equation}
\end{lemma}
\begin{proof}
We first show the first claim. Notice
\begin{align}
    || B^{-1}C u_\ast v_t^\top -  u_\ast v_\ast^\top ||_2^2 &= || B^{-1}(C u_\ast v_t^\top - B u_\ast v_\ast^\top) ||_2^2 \nonumber \\
    &\leq \frac{1}{(1- \delta_4)^2}|| (C u_\ast v_t^\top - B u_\ast v_\ast^\top) ||_2^2 \label{B21} \\
    &=\frac{1}{(1- \delta_4)^2} \|C u_\ast v_t^\top - C u_\ast v_\ast^\top + C u_\ast v_\ast^\top - B u_\ast v_\ast^\top \|_2^2 \nonumber\\
  & = \frac{1}{(1- \delta_4)^2} || Cu_\ast(v_t - v_\ast)^\top + (C-B)u_\ast v_\ast^\top)||_2^2 
\end{align}
where \eqref{B21} follows from the Cauchy-Schwarz inequality and Lemma \ref{lem:B1}. 
% First note that using $2k$-RIP we have for any rank-$2k$ matrix $x$ that:
% $$ ||\mathcal{A}^*\mathcal{A}(x) - x||_2 \leq \delta_{2k} ||x||_F,$$
% and we thus obtain
% $$||\mathcal{A}^*\mathcal{A}(x)||_2 \leq (1 + \sqrt{2k} \delta_{2k}) ||x||_2,$$
% as $||x||_F \leq \sqrt{2k}||x||_2$ when $\text{rank}(x) \leq 2k$.
% Continuing from \eqref{norm-a*a} and noting that has at most rank 2, we obtain 
% $$|| \mathcal{A}^*\mathcal{A}(C u_\ast v_t^\top - B u_\ast v_\ast^\top) ||_2^2 \leq (1 + \sqrt{2}\delta_4)^2   \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|_2^2 $$
% and 
% \begin{align} \label{alternative}
%   \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|_2^2 
%   &=  \|C u_\ast v_t^\top - C u_\ast v_\ast^\top + C u_\ast v_\ast^\top - B u_\ast v_\ast^\top \|_2^2 \\
%   & = || Cu_\ast(v_t - v_\ast)^\top + (C-B)u_\ast v_\ast^\top)||_2^2
% \end{align}
Now, let's first bound the norm of $Cu_\ast(v_t - v_\ast)^\top$. We have: 
\begin{align*}
||Cu_\ast(v_t - v_\ast)^\top||_2 & \leq 
||Cu_\ast ||_2 ||(v_t - v_\ast)^\top||_2 \\
&\leq ||C ||_2 \sqrt{2(1 - \langle v_t, v_\ast\rangle)}\\
&\leq (1+\delta_4) \sqrt{2(1 - \langle v_t, v_\ast \rangle)}
% &\leq ||C ||_2 \sqrt{2(1 - \langle v_t, v_\ast \rangle^2)} \\
% &\leq (1+\delta_k)  \sqrt{2\text{dist}(v_t, v_\ast)},
\end{align*}
where we have used 
$$|| C||_2 \leq  (1+\delta_4)$$
from \eqref{c2}.
In the same manner, by using RIP and Lemma \ref{lem:rip1} we can write
\begin{align*}
    || C - B ||_2^2 &= \max_{z: \|z\|_2 = 1} z^\top (C - B)^\top (C - B) z \nonumber \\
    &= \max_{z: \|z\|_2 = 1} z^\top \left(\sum_{i=1}^N A_i  (v_t - v_\ast) v_t^\top A_i^\top \right) (C - B) z \nonumber \\
    &= \max_{z: \|z\|_2 = 1}  \sum_{i=1}^N \text{tr}(z^\top A_i (v_t - v_\ast))\text{tr}(v_t^\top A_i^\top (C - B)z) \nonumber \\
    &= \max_{z: \|z\|_2 = 1}  \langle \mathcal{A}(z (v_t - v_\ast)^\top), \mathcal{A}((C - B) z v_t^\top) \rangle \nonumber \\
    &\leq \max_{z: \|z\|_2 = 1}  \langle z (v_t - v_\ast)^\top, (C-B) z v_t^\top \rangle + \delta_4 \|z (v_t - v_\ast)^\top\|_F \| (C - B)zv_t^\top \|_F \nonumber \\
    &\leq \max_{z: \|z\|_2 = 1}  \langle z (v_t - v_\ast)^\top, (C-B) z v_t^\top \rangle + \delta_4 \sqrt{2(1-\langle v_t, v_\ast\rangle)} \| C - B\|_2 %\nonumber \\
    % &= 1 - \langle v_t, v_\ast \rangle + \delta_4 \sqrt{2(1 - \langle v_t, v_\ast\rangle)} \nonumber \\
    % &\leq \sqrt{2(1 - \langle v_t, v_\ast \rangle)} + \delta_4 \sqrt{2(1 - \langle v_t, v_\ast\rangle)} \nonumber \\
    % &= (1 + \delta_4)\sqrt{2(1 - \langle v_t, v_\ast \rangle)}
    %\leq (1+\delta_k) || v_t (v_t - v_\ast)^\top ||_2 \leq || v_t||_2 || v_t - v_\ast||_2 \leq \sqrt{2 \text{dist}(v_t, v_\ast)}.
\end{align*}
where the last equation follows since $\|(C-B)z v_t^\top\|_F \leq \|(C-B)\|_2 \|z v_t^\top\|_F = \|C-B\|_2$. Next,
\begin{align}
    \max_{z: \|z\|_2 = 1}  \langle z (v_t - v_\ast)^\top, (C-B) z v_t^\top \rangle &= \max_{z: \|z\|_2 = 1} \sum_{i=1}^N \text{tr} ((v_t - v_\ast) z^\top A_i v_t (v_t - v_\ast)^\top A_i^\top z v_t^\top ) \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \sum_{i=1}^N \text{tr} (z^\top A_i v_t (v_t - v_\ast)^\top A_i^\top z v_t^\top (v_t - v_\ast)  ) \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \sum_{i=1}^N \text{tr} (z^\top A_i v_t) \text{tr}( (v_t - v_\ast)^\top A_i^\top z) (1 -  \langle v_t, v_\ast\rangle) \nonumber \\
    &= \max_{z: \|z\|_2 = 1} \langle \mathcal{A}(z v_t^\top) , \mathcal{A}( z (v_t - v_\ast)^\top )\rangle (1 -  \langle v_t, v_\ast\rangle) \nonumber \\
    &\leq  \max_{z: \|z\|_2 = 1} (1 -  \langle v_t, v_\ast\rangle) \langle z v_t^\top, z (v_t - v_\ast)^\top \rangle \nonumber \\
    &\quad \quad+ \delta_4 (1 -  \langle v_t, v_\ast\rangle) \| z v_t^\top\|_F \|z (v_t - v_\ast)^\top\|_F \nonumber \\
    &\leq (1 -  \langle v_t, v_\ast\rangle)^2 + \delta_4 \sqrt{2} (1 -  \langle v_t, v_\ast\rangle)^{3/2}
\end{align}
Putting these together, we have
\begin{align}
    || C - B ||_2^2 &\leq (1 -  \langle v_t, v_\ast\rangle)^2 + \delta_4 \sqrt{2} (1 -  \langle v_t, v_\ast\rangle)^{3/2} + \delta_4 \sqrt{2(1-\langle v_t, v_\ast\rangle)} \| C - B\|_2  \nonumber \\
    &\leq (1 -  \langle v_t, v_\ast\rangle) +\sqrt{2} \delta_4  (1 -  \langle v_t, v_\ast\rangle) + \delta_4 \sqrt{2(1-\langle v_t, v_\ast\rangle)} \| C - B\|_2  \nonumber \\
\end{align}
where the second inequality follows because $(1 -  \langle v_t, v_\ast\rangle) \leq 1$.
Now using the quadratic formula, we have
\begin{align}
     || C - B ||_2 &\leq \frac{1}{2} \left(\sqrt{2} \delta_4 \sqrt{1 - \langle v_t, v_\ast \rangle} + \sqrt{2 \delta_4^2 (1 - \langle v_t, v_\ast \rangle) + 4(1+\delta_4\sqrt{2})(1 -  \langle v_t, v_\ast\rangle) } \right) \nonumber \\
     &= \frac{1}{2} \left( \sqrt{2} \delta_4  + \sqrt{2 \delta_4^2 + 4\sqrt{2} \delta_4 + 4)}\right)\sqrt{1 -  \langle v_t, v_\ast\rangle } \nonumber \\
     &\leq  \left( \sqrt{2} \delta_4  + (1+ \delta_4)\right)\sqrt{1 -  \langle v_t, v_\ast\rangle } \nonumber \\
     &\leq \left( 1+ 3\delta_4 \right)\sqrt{1 -  \langle v_t, v_\ast\rangle }
\end{align}
% Note that
% \begin{align}
%     \| (C - B)zv_t^\top \|_F^2 &= \text{tr}( v_t z^\top (C - B)^\top (C - B) zv_t^\top) \nonumber \\
%     &= \text{tr}( z^\top (C - B)^\top (C - B) z) \nonumber \\
%     &= 
% \end{align}

And thus: 
$$ ||(C-B) u_\ast v_\ast^\top||_2 \leq ||(C-B)||_2|| u_\ast v_\ast^\top||_2 \leq  (1 +3\delta_4) \sqrt{1 - \langle v_t, v_\ast\rangle} . $$
Putting these together and using the inequality $(a+b)^2 \leq 2a^2 + 2b^2$, we obtain: 
\begin{align}
    \|C u_\ast v_t^\top - B u_\ast v_\ast^\top \|_2^2 
    &\leq 8 (1+\delta_4)(1 +3\delta_4) (1 - \langle v_t, v_\ast \rangle) 
    % \nonumber \\
    % &\quad \quad + 2(1 - \langle v_t, v_\ast \rangle)^2 + 4\delta_4(1 - \langle v_t, v_\ast \rangle)\sqrt{2(1 - \langle v_t, v_\ast\rangle)} + 4 \delta_4^2 (1 - \langle v_t, v_\ast\rangle)  \nonumber \\
    % &\leq . %8(1+\delta_4)^2\text{dist}(v_t, v_\ast).
\end{align}
Therefore
\begin{align}
    \|B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top \|_2^2 
    &\leq \frac{8 (1+\delta_4)(1 +3\delta_4) }{(1-\delta_4)^2} (1 - \langle v_t, v_\ast \rangle) 
    % \nonumber \\
    % &\quad \quad + 2(1 - \langle v_t, v_\ast \rangle)^2 + 4\delta_4(1 - \langle v_t, v_\ast \rangle)\sqrt{2(1 - \langle v_t, v_\ast\rangle)} + 4 \delta_4^2 (1 - \langle v_t, v_\ast\rangle)  \nonumber \\
    % &\leq . %8(1+\delta_4)^2\text{dist}(v_t, v_\ast).
\end{align}
%Note that the RHS can be simplified to a looser but much cleaner bound, we leave it in messy form for now.
To show the second claim we first note that by RIP, for any rank-$2k$ matrix $X$ we have that:
\begin{equation}
 ||\mathcal{A}^*\mathcal{A}(X) - X||_2 \leq \delta_{2k} ||X||_F,\end{equation}
and we thus obtain
$$||\mathcal{A}^*\mathcal{A}(X)||_2 \leq (1 + \sqrt{2k} \delta_{2k}) ||X||_2,$$
as $||\mathcal{A}^*\mathcal{A}(X) - X||_2 \geq ||\mathcal{A}^*\mathcal{A}(X)||_2 - ||X||_2$, and $||X||_F \leq \sqrt{2k}||X||_2$ when $\text{rank}(X) \leq 2k$. Using this and noting that $B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top$ has rank at most 2, we immediately obtain
\begin{equation}
    || \mathcal{A}^*(\mathcal{A}(B^{-1}C u_\ast v_t^\top - u_\ast v_\ast^\top ) ||_2^2 \leq
    \frac{8 (1+\delta_4)(1 +3\delta_4)  (1+ \sqrt{2}\delta_4)^2}{(1-\delta_4)^2} (1 - \langle v_t, v_\ast \rangle) 
\end{equation}
Noting that $1-\langle v_t, v_\ast\rangle \leq 1-\langle v_t, v_\ast\rangle^2 = \text{dist}^2(v_t, v_\ast)$
completes the proof.
\end{proof}
\begin{lemma}
The sequence $\{ \|\hat{v}_t\|_2\}_t$ is monotone increasing. Moreover, $\|\hat{v}_t\| \leq c \|\hat{v}_0\|_2$ for some absolute constant $c$. 
\end{lemma}
\begin{proof}
We have
\begin{align}
    \hat{v}_{t+1}^\top \hat{v}_{t+1} &= \hat{v}_{t}^\top \hat{v}_{t} - 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_t \|} \sum_{i=1}^N  \left(  u_\ast^\top C^\top B^{-\top}  A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) \hat{v}_{t}^\top A_i^\top  B^{-1} C u_\ast \nonumber \\
    &\quad \quad + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_t \|^2}  \sum_{i=1}^N  \sum_{i'=1}^N  \left(u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right)\left(u_\ast^\top C^\top B^{-\top} A_{i'} {v}_t  -  u_\ast^\top A_{i'} v_\ast \right) u_\ast^\top C^\top B^{\top}A_i A_{i'}^\top B^{-1} C u_\ast  \label{rank1sg:square}
\end{align}
We expect the cross terms to be close to zero:
\begin{align}
    \frac{\sigma_\ast^2}{\|\hat{v}_t \|}& \sum_{i=1}^N  \left(  u_\ast^\top C^\top B^{-\top}  A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) \hat{v}_{t}^\top A_i^\top  B^{-1} C u_\ast  \nonumber \\
    &= {\sigma_\ast^2} \sum_{i=1}^N  u_\ast^\top C^\top B^{-\top}  A_i {v}_t {v}_{t}^\top A_i^\top B^{-1} C u_\ast -  u_\ast^\top A_i v_\ast{v}_{t}^\top A_i^\top  B^{-1} C u_\ast \nonumber \\
    &= {\sigma_\ast^2} u_\ast^\top C^\top B^{-\top} \left(\sum_{i=1}^N A_i {v}_t {v}_{t}^\top A_i^\top\right) B^{-1} C u_\ast  -  {\sigma_\ast^2} u_\ast^\top \left(\sum_{i=1}^N A_i v_\ast{v}_{t}^\top A_i^\top \right) B^{-1} C u_\ast\nonumber \\
    &= {\sigma_\ast^2} u_\ast^\top C^\top B^{-\top} C u_\ast  -  {\sigma_\ast^2} u_\ast^\top C^\top  B^{-1} C u_\ast\nonumber \\
    &= 0 \label{rank1sq:cross}
\end{align}
where \eqref{rank1sq:cross} follows because $B$ is symmetric.
Next, note that the last term of \eqref{rank1sg:square} is a square and thus nonnegative. Thus we have that $\{ \|\hat{v}_t\|_2\}_t$ is monotone increasing. Now, 
\begin{align}
\Psi &\coloneqq \frac{\sigma_\ast^4}{\|\hat{v}_t \|^2_2} \sum_{i=1}^N  \sum_{i'=1}^N  \left(u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right)\left(u_\ast^\top C^\top B^{-\top} A_{i'} {v}_t  -  u_\ast^\top A_{i'} v_\ast \right) u_\ast^\top C^\top B^{-\top}A_i A_{i'}^\top B^{-1} C u_\ast  \nonumber \\
&= \frac{\sigma_\ast^4}{\|\hat{v}_t \|^2} \sum_{i=1}^N  \sum_{i'=1}^N  \left(u_\ast^\top C^\top B^{-\top} A_i {v}_t  -  u_\ast^\top A_i v_\ast \right) u_\ast^\top C^\top B^{-\top}A_i A_{i'}^\top B^{-1} C u_\ast \left(u_\ast^\top C^\top B^{-\top} A_{i'} {v}_t  -  u_\ast^\top A_{i'} v_\ast \right) \nonumber \\
&= 
\end{align}
This term diminishes with $\dist^2$. We just need to show concentration. But since we have linear convergence of $\dist$, the change in the norm from iteration to iteration is exponentially decreasing, so the total change is the sum of a geometric series, converges to a constant.
\end{proof}


We now have all the ingredients necessary to show linear convergence.
\begin{theorem}
Under Assumption \ref{assump:rank1sg}, the iterates of our alternating minimization-descent algorithm satisfy:
\begin{align}
    \text{dist}({v}_{t+1}, v_\ast) \leq \sqrt{1 - \eta} \text{dist}({v}_{t}, v_\ast) 
\end{align}
 for any step size $\eta$ satisfying
\begin{equation}
   0 < \eta \leq \frac{ \|\hat{v}_{0}\|_2^2}{4\sigma_\ast^2} \frac{(1-\delta_4)^2}{(1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2}\left( \frac{(\langle v_0, v_\ast \rangle( \langle v_0, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4))(1-\delta_4)^4}{(1+\delta_4)^4} - {2\sqrt{2} \delta_4 } \right), 
\end{equation}
for which some such $\eta$ is guaranteed to exist.
\end{theorem}

\begin{proof}
Setting the gradient of \eqref{rank1sg:obj} with respect to ${u}$ equal to 0, we obtain that the update for ${u}_{t+1}$ is:
\begin{align}
    {u}_{t+1} &= \frac{\sigma_{\ast}}{\|{v}_t \|} B^{-1} C \hat{u}_\ast
\end{align}
where
\begin{align}
    B &\coloneqq \sum_{i=1}^N A_i \hat{v}_t \hat{v}_t^\top A_i^\top \\
    C &\coloneqq \sum_{i=1}^N A_i \hat{v}_t \hat{v}_\ast^\top A_i^\top 
\end{align}
(note that the vectors above are normalized).
Plugging this back into the objective, we obtain
\begin{align}
    F({u}_{t+1}, {v}) &= \frac{1}{2}\sum_{i=1}^N \langle A_i, \frac{\sigma_{\ast}}{\|{v}_t \|} B^{-1} C \hat{u}_\ast {v}^\top - \sigma_\ast \hat{u}_\ast \hat{v}_\ast^\top \rangle^2 \\
    &= \frac{1}{2}\sum_{i=1}^N \sigma_\ast^2 \left( {v}^\top A_i^\top \frac{1}{\|{v}_t \|} B^{-1} C \hat{u}_\ast - \hat{v}_\ast^\top A_i^\top \hat{u}_\ast \right)^2 
%eliminate u_\ast?
\end{align}
Then the gradient with respect to ${v}$ is
\begin{align}
    \nabla_{{v}} F({u}_{t+1},{v}) = \sum_{i=1}^N \sigma_\ast^2 \left(  \hat{u}_\ast^\top C^\top B^{-\top} A_i \frac{1}{\|{v}_t \|}  {v}  -  \hat{u}_\ast^\top A_i \hat{v}_\ast \right) A_i^\top \frac{1}{\|{v}_t \|} B^{-1} C \hat{u}_\ast 
    =: S_t
\end{align}
and we have
\begin{align}
    {v}_{t+1} = {v}_{t} - \eta \sum_{i=1}^N \sigma_\ast^2 \left(  \hat{u}_\ast^\top C^\top B^{-\top} A_i \hat{v}_t  -  \hat{u}_\ast^\top A_i \hat{v}_\ast \right) A_i^\top \frac{1}{\|{v}_t \|} B^{-1} C \hat{u}_\ast 
\end{align}
Using operator notation, this is
\begin{align}
    {v}_{t+1} = {v}_t - \eta \frac{\sigma_\ast^2}{\|{v}_t\|} \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top) \right)^\top B^{-1} C \hat{u}_\ast
\end{align}
where $\mathcal{A}^\ast$ is the adjoint of the operator $\mathcal{A}$. Multiplying both sides by $V_{\ast, \perp}^\top$ yields
\begin{align}
    \hat{V}_{\ast, \perp}^\top {v}_{t+1} = \hat{V}_{\ast, \perp}^\top {v}_t - \eta \frac{\sigma_\ast^2}{\|{v}_t\|} \hat{V}_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top) \right)^\top B^{-1} C \hat{u}_\ast
\end{align}
After dividing both sides by $\| {v}_{t+1}\|_2$ and taking the 2-norm squared of both sides, we obtain
\begin{align}
    \text{dist}^2({v}_{t+1}, v_\ast ) &= \frac{1}{\|{v}_{t+1}\|_2^2}\left\|\hat{V}_{\ast, \perp}^\top {v}_t - \eta \frac{\sigma_\ast^2}{\|{v}_t\|} \hat{V}_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top) \right)^\top B^{-1} C \hat{u}_\ast)\right\|_2^2 \nonumber \\
    &= \frac{\|{v}_t\|_2^2}{\|{v}_{t+1}\|_2^2}\text{dist}^2({v}_t, v_\ast) - 2\eta \frac{\sigma_\ast^2}{\|{v}_{t+1}\|_2^2} \langle \hat{V}_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top) \right)^\top B^{-1} C \hat{u}_\ast, \hat{V}_{\ast, \perp}^\top \hat{v}_t \rangle \nonumber \\
    &\quad \quad + \eta^2 \frac{\sigma_\ast^4}{\|{v}_{t+1}\|_2^2 \|{v}_{t}\|_2^2} \|\hat{V}_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top) \right)^\top B^{-1} C \hat{u}_\ast \|_2^2 \label{3terms1}
\end{align}
We will control each of the above terms, starting with the cross term:
\begin{align}
    &\langle \hat{V}_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top) \right)^\top B^{-1} C \hat{u}_\ast, \hat{V}_{\ast, \perp}^\top \hat{v}_t \rangle \nonumber \\
    &= \langle  \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top) \right)^\top, \hat{V}_{\ast, \perp} \hat{V}_{\ast, \perp}^\top \hat{v}_t \hat{u}_\ast^\top C^\top B^{-\top} \rangle \nonumber \\
    &= \langle  \mathcal{A}^\ast \mathcal{A} (B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top) , B^{-1} C \hat{u}_\ast \hat{v}_t^\top \hat{V}_{\ast, \perp} \hat{V}_{\ast, \perp}^\top \rangle \nonumber \\
    &= \langle\mathcal{A} (B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top) , \mathcal{A}^\ast ( B^{-1} C \hat{u}_\ast \hat{v}_t^\top \hat{V}_{\ast, \perp} \hat{V}_{\ast, \perp}^\top) \rangle \nonumber \\
    &\geq \langle B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top, B^{-1} C \hat{u}_\ast \hat{v}_t^\top \hat{V}_{\ast, \perp} \hat{V}_{\ast, \perp}^\top \rangle - \delta_4 \| B^{-1} C \hat{u}_\ast \hat{v}_t^\top - \hat{u}_\ast \hat{v}_\ast^\top \|_F \| B^{-1} C \hat{u}_\ast \hat{v}_t^\top \hat{V}_{\ast, \perp} \hat{V}_{\ast, \perp}^\top \|_F \label{uselem12}
\end{align}
%note: I should change all $\delta_4 \rightarrow \delta_4$
where \eqref{uselem12} follows from Lemma \ref{lem:rip1} and the fact that the relevant matrices matrices have rank at most 2. Next, note that 

{\color{red} NOTE: from here onwards, the hat notation is flipped: hats denote non-normalized vectors and matrices, and no hats denote normalized vectors and matrices.}
\begin{align}
    \langle u_\ast v_\ast^\top, B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \rangle &= \text{tr}(v_\ast u_\ast^\top B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top ) \nonumber \\
    &=  u_\ast^\top B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top v_\ast  \nonumber \\
    &= 0
\end{align}
since $V_{\ast, \perp}^\top v_\ast = 0$ by definition of $V_{\ast, \perp}$. Thus,
\begin{align}
    \langle B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top, B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \rangle &= \langle B^{-1} C u_\ast v_t^\top V_{\ast, \perp}, B^{-1} C u_\ast v_t^\top V_{\ast, \perp}  \rangle \nonumber \\
    &= \| B^{-1} C u_\ast v_t^\top V_{\ast, \perp} \|_F^2 \nonumber \\
    &\geq  \sigma_{\min}^2( B^{-1} C )  \|v_t^\top V_{\ast, \perp} \|_2^2 \nonumber \\
    &\geq  \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2} \text{dist}^2(v_t, v_\ast) \label{cross1}
\end{align}
where \eqref{cross1} follows from Lemma \ref{lem:B1}. Next, we need to upper bound the negative term in \eqref{uselem12}. We have
\begin{align}
    \| B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \|_F &= \| B^{-1} C u_\ast v_t^\top V_{\ast, \perp} \|_F \nonumber \\
    &\leq \| B^{-1} C\|_2 \| u_\ast\|_F \|v_t^\top V_{\ast, \perp} \|_2 \nonumber \\
    &\leq \frac{1 + \delta_4}{1 - \delta_4} \text{dist}(v_t,v_\ast)
\end{align}
and thus
\begin{align}
    \| B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top \|_F \| B^{-1} C u_\ast v_t^\top V_{\ast, \perp} V_{\ast, \perp}^\top \|_F &\leq   \frac{2\sqrt{2} (1 + 3\delta_4) (1 + \delta_4)}{(1 - \delta_4)^2} \text{dist}^2(v_t,v_\ast)
\end{align}
using Lemma \ref{lem:B2} and the fact $\langle v_t, v_\ast \rangle \leq 1$.

Thus we have completed our bound on the cross term:
\begin{align}
    \langle V_{\ast, \perp}^\top \big(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top &- u_\ast v_\ast^\top) \big)^\top B^{-1} C u_\ast, V_{\ast, \perp}^\top v_t \rangle \nonumber \\
    &\geq \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2} \text{dist}^2(v_t, v_\ast) - \frac{2\sqrt{2} \delta_4(1 + 3\delta_4)^2}{(1 - \delta_4)^2} \text{dist}^2(v_t,v_\ast) \label{2ndterm}
\end{align}
We now turn to the final term in \eqref{3terms1}. We have
\begin{align}
    \|V_{\ast, \perp}^\top \left(\mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top) \right)^\top B^{-1} C u_\ast \|_2^2 &\leq \| \mathcal{A}^\ast \mathcal{A} (B^{-1} C u_\ast v_t^\top - u_\ast v_\ast^\top)\|_2^2\| V_{\ast, \perp}\|_2^2 \| B^{-1} C \|_2^2 \|u_\ast\|_F^2 \nonumber \\
    &\leq \frac{8 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \text{dist}^2(v_t,v_\ast)  \label{3rdtermm}
\end{align}
where \label{3rdterm} follows from Lemmas \ref{lem:B1} and \ref{lem:B2} and the fact that $\|V_{\ast, \perp}\|_2 = \|u_\ast\|_F = 1$. 

 Combining \eqref{3terms1}, \eqref{2ndterm} and \eqref{3rdtermm} yields
\begin{align}
    &\text{dist}^2({v}_{t+1}, v_\ast ) \nonumber\\
    &= \frac{\|\hat{v}_t\|_2^2}{\|\hat{v}_{t+1}\|_2^2}\text{dist}^2({v}_t, v_\ast) - 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2} \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2} \text{dist}^2(v_t, v_\ast) \nonumber \\ 
    &\quad + 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2}\frac{2\sqrt{2} \delta_4 (1 + \delta_4)^2}{(1 - \delta_4)^2} \text{dist}^2(v_t,v_\ast) 
    + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_{t}\|_2^2} \frac{8 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \text{dist}^2(v_t,v_\ast)  \nonumber \\
    &\leq  \text{dist}^2({v}_t, v_\ast)\Bigg(1 - 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2} \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2}  \nonumber \\ 
    &\quad + 2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2}\frac{2\sqrt{2} \delta_4 (1 + \delta_4)^2}{(1 - \delta_4)^2}  
    + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_{t}\|_2^2} \frac{8 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \Bigg) \nonumber 
\end{align}
where we have used the fact that $\|\hat{v}_t\|_2 \leq \|\hat{v}_{t+1}\|_2$ from Lemma \ref{}. In order to ensure linear convergence we must have
\begin{align}
    &2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2} \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2} \geq  2\eta \frac{\sigma_\ast^2}{\|\hat{v}_{t+1}\|_2^2}\frac{2\sqrt{2} \delta_4 (1 + \delta_4)^2}{(1 - \delta_4)^2}  \nonumber \\
    &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad + \eta^2 \frac{\sigma_\ast^4}{\|\hat{v}_{t+1}\|_2^2 \|\hat{v}_{t}\|_2^2} \frac{8 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \nonumber \\
    &\iff \frac{\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4)}{(1+\delta_4)^2} \geq   \frac{2\sqrt{2} \delta_4 (1 + \delta_4)^2}{(1 - \delta_4)^2} + \eta \frac{\sigma_\ast^2}{ \|\hat{v}_{t}\|_2^2} \frac{4 (1+3\delta_4)^2 (1+ \sqrt{2}\delta_4)^2 (1+\delta_4)^2}{(1-\delta_4)^4} \nonumber \\
    &\iff \frac{ \|\hat{v}_{t}\|_2^2}{4\sigma_\ast^2} \left( \frac{(\langle v_t, v_\ast \rangle( \langle v_t, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4))(1-\delta_4)^4}{(1+\delta_4)^4 (1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2} - \frac{2\sqrt{2} \delta_4 (1-\delta_4)^2}{(1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2} \right) \geq  \eta  \nonumber \\
    &\Longleftarrow \frac{ \|\hat{v}_{0}\|_2^2}{4\sigma_\ast^2} \frac{(1-\delta_4)^2}{(1+3\delta_4)^2(1+ \sqrt{2}\delta_4)^2}\left( \frac{(\langle v_0, v_\ast \rangle( \langle v_0, v_\ast \rangle - \delta_4) - \delta_4 (1+\delta_4))(1-\delta_4)^4}{(1+\delta_4)^4} - {2\sqrt{2} \delta_4 } \right) \geq  \eta  
\end{align}
where in the final inequality we used the fact
% that  $\{\|\hat{v}_t\|\}_t$ is increasing (Lemma \ref{}) and 
that if $\hat{v}_t$ converges linearly to $v_\ast$, then $\langle v_t, v_\ast \rangle$ is increasing. By Assumption \ref{assump:rank1sg}, we have that the LHS is strictly greater than 0, so we can choose a sufficiently small $\eta$.

{\color{blue} $\rightarrow$ in the 1-D case, we can show convergence without normalizing and without choosing the step size proportional to $1/\|v_t\|_2^2$.}

% So, all that remains to show is that we can choose a $\delta_4$ small enough such that the above inequality holds (assume for now) (and assume $\langle v_0, v_\ast \rangle$ is large enough).


\end{proof}


==> rankkfm.tex <==
\section{Rank-$k$, Full Measurements}
We aim to solve the following problem:
\begin{align}
    \min_{\hat{U}, \hat{V}} F(\hat{U},\hat{V}) \coloneqq \frac{1}{2}\|\hat{U} \hat{V}^T - M\|_F^2 \label{rankk:objective}
\end{align}
where $M = U_\ast \Sigma_\ast V_\ast^\top$.

\begin{theorem}
For any $T \in \mathbb{N}$, our alternating minimization-descent algorithm run on \eqref{rankk:objective} for $T + 1/2$ iterations with fixed step size $\eta \leq \frac{1}{2}  \frac{ \sigma_{\min}^3(R_0)}{\sigma_{\max}(R_{0})} \frac{  \sigma_{\ast,\min}^2}{\sigma_{\ast,\max}^4}$ and initial iterate $\hat{V}_0 = V_0 R_0$ such that $V_{\ast,\perp}^\top V_0 \neq 0$ yields
\begin{align}
    \| M - \hat{U}_{T+1} \hat{V}_T^\top \|_F^2 
    &\leq \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{2 \sigma_{\max}^2(R_0)}\right)^T \|M\|_F^2 \frac{\sigma_{\max}(R_{0})}{\sigma_{\min}(R_{0})}, \label{rankk:thrm}
\end{align}
where $\sigma_{\ast,\min}$ (respectively $\sigma_{\ast,\max}$) is the minimum (respectively maximum) singular value of $M$.
Thus, if we further assume that $R_0 = I$ (very mild assumption), then we have
\begin{align}
    \| M - \hat{U}_{T+1} \hat{V}_T^\top \|_F^2 
    &\leq \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{2 }\right)^T \|M\|_F^2
\end{align}
for any $\eta \leq \frac{1}{2}\frac{  \sigma_{\ast,\min}^2}{\sigma_{\ast,\max}^4}$. Choosing $\eta = \frac{1}{2}\frac{  \sigma_{\ast,\min}^2}{\sigma_{\ast,\max}^4}$ yields
\begin{align}
    \| M - \hat{U}_{T+1} \hat{V}_T^\top \|_F^2 
    &\leq \left(1 - \frac{\sigma_{\ast,\min}^4}{4\sigma_{\ast,\max}^4 }\right)^T \|M\|_F^2.
\end{align}
\end{theorem}

\begin{proof}
The update for $\hat{U}$ is:
\begin{align}
    \hat{U}_{t+1} = U_\ast \Sigma_\ast V_\ast^\top \hat{V}_t (\hat{V}_t^\top \hat{V}_t)^{-1}
\end{align}
Let $\hat{V}_t$ have QR factorization $\hat{V}_t = V_t R_t$, where $V_t$ is orthogonal and $R_t$ is upper triangular. Also define $\Lambda_t \coloneqq V_t^\top V_\ast$. Then we have 
\begin{align}
    \hat{U}_{t+1} = U_\ast \Sigma_\ast V_\ast^\top {V}_t {R}_t ({R}_t^\top {R}_t)^{-1} = U_\ast \Sigma_\ast V_\ast^\top {V}_t {R}_t^{-\top} = U_\ast \Sigma_\ast \Lambda^\top_t {R}_t^{-\top}
\end{align}
Plugging $\hat{U}_{t+1}$ into the objective, we have
\begin{align}
    F(\hat{U}_{t+1}, \hat{V}) &= \frac{1}{2}\|U_\ast \Sigma_\ast \Lambda^\top_t {R}_t^{-\top} \hat{V}^\top - U_\ast \Sigma_\ast V_\ast^\top \|_F^2 \nonumber \\
    &= \frac{1}{2}\| \hat{V}{R}_t^{-1} \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast  \|_F^2 \label{rankk:2}
\end{align}
where \eqref{rankk:2} follows by the fact that $U_\ast$ is orthogonal. The gradient of this function with respect to $\hat{V}$ is:
\begin{align}
    \nabla_{\hat{V}} F(\hat{U}_{t+1}, \hat{V}) &=  (\hat{V}{R}_t^{-1} \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast)\Sigma_\ast \Lambda_t^\top {R}_t^{-\top},
\end{align}
thus the update for $\hat{V}_{t+1}$ is 
\begin{align}
    \hat{V}_{t+1} &= \hat{V}_t - \eta (\hat{V}_t {R}_t^{-1} \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast) \Sigma_\ast \Lambda_t^\top {R}_t^{-\top}
\end{align}
Let $S_t \coloneqq (\hat{V}_t{R}_t^{-1} \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast)\Sigma_\ast \Lambda_t^\top {R}_t^{-\top}$. Then we have
\begin{align}
    \hat{V}_{t+1}^\top \hat{V}_{t+1} &= \hat{V}_{t}^\top \hat{V}_{t} + \eta^2 S_t^\top S_t - \eta (\hat{V}_t^\top \hat{V}_t{R}_t^{-1} \Lambda_t \Sigma_\ast  - \hat{V}_t^\top V_\ast \Sigma_\ast)\Sigma_\ast \Lambda_t^\top {R}_t^{-\top} \nonumber \\
    &\quad \quad \quad \quad - \eta  {R}_t^{-1} \Lambda_t\Sigma_\ast  (\Sigma_\ast \Lambda_t^\top {R}_t^{-\top}\hat{V}_t^\top \hat{V}_t  -  \Sigma_\ast V_\ast^\top \hat{V}_t )
\end{align}
Note that
\begin{align}
    \hat{V}_t^\top \hat{V}_t{R}_t^{-1} \Lambda_t \Sigma_\ast  - \hat{V}_t^\top V_\ast \Sigma_\ast &= {R}_t^\top  V_t^\top {V}_t R_t {R}_t^{-1} \Lambda_t \Sigma_\ast  - {R}_t^\top V_t^\top V_\ast \Sigma_\ast \nonumber \\
    &= {R}_t^\top \Lambda_t \Sigma_\ast  - {R}_t^\top \Lambda_t \Sigma_\ast  \nonumber \\
    &= 0
\end{align}
A similar argument shows that the other cross term is also 0, yielding
\begin{align}
    \hat{V}_{t+1}^\top \hat{V}_{t+1} &= \hat{V}_{t}^\top \hat{V}_{t} + \eta^2 S_t^\top S_t 
\end{align}
Since $\hat{V}_{t+1}^\top \hat{V}_{t+1} = {R}_{t+1}^\top {R}_{t+1}$ and $\hat{V}_{t}^\top \hat{V}_{t} = {R}_{t}^\top {R}_{t}$, we have
\begin{align}
    {R}_{t+1}^\top {R}_{t+1} &= {R}_{t}^\top {R}_{t} + \eta^2 S_t^\top S_t  \label{rankk:r}
\end{align}
As $S_t^\top S_t$ is PSD, the singular values of ${R}_{t}$ are non-decreasing in $t$. In particular, $\|R_0\|_2 \leq \|R_t\|_2$ and $\sigma_{\min}(R_0) \leq \sigma_{\min}(R_t)$ for all $t$. 

We will later use this expression to also show that $\|R_t\|_2$ is uniformly bounded for all $t$. For now, we go back to the iterates of GD:
\begin{align}
    \hat{V}_{t+1} &= \hat{V}_t - \eta (\hat{V}_t {R}_t^{-1} \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast) \Sigma_\ast \Lambda_t^\top {R}_t^{-\top} \nonumber \\
    \Leftrightarrow  {V}_{\ast,\perp}^\top \hat{V}_{t+1} &= {V}_{\ast,\perp}^\top \hat{V}_{t} - \eta {V}_{\ast,\perp}^\top \hat{V}_t {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top} \nonumber \\
    &= {V}_{\ast,\perp}^\top \hat{V}_{t} (I_k - \eta  {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top} ) \nonumber %\\
    % \Leftrightarrow  {V}_{\ast,\perp}^\top {V}_{t+1} &=   {V}_{\ast,\perp}^\top {V}_{t} R_t (I_k - \eta  {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top} ) R_{t+1}^{-1} 
\end{align}
Thus, we have that 
\begin{align}
      \|{V}_{\ast,\perp}^\top \hat{V}_{t+1}\|_2 &\leq \|{V}_{\ast,\perp}^\top \hat{V}_{t}\|_2 \|I_k - \eta  {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top}  \|_2 \label{rankk:initcontract}   % \\
    % &=  \text{dist}(\hat{V}_{t+1}, V_\ast) \|R_t\|_2 \|(I_k - \eta  {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top} ) \|_2   
 \end{align}
% \begin{align}
%     \text{dist}(\hat{V}_{t+1}, V_\ast) = \|{V}_{\ast,\perp}^\top {V}_{t+1}\|_2 &\leq \|{V}_{\ast,\perp}^\top {V}_{t}\|_2 \|R_t\|_2 \|(I_k - \eta  {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top} ) \|_2  \|R_{t+1}^{-1}\|_2  \\
%     &=  \text{dist}(\hat{V}_{t+1}, V_\ast) \|(I_k - \eta  {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top} ) \|_2  \|R_t\|_2 \|R_{t+1}^{-1}\|_2
% \end{align}
where we have used the Cauchy Schwarz inequality. 
%By \eqref{rankk:r} and the fact that $S_t^\top S_t$ is PSD, we have that 
Next we show is that $\|(I_k - \eta  {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top} ) \|_2$ is upper bounded by a number strictly less than 1. To do so, we choose $\eta \leq \frac{\|R_0\|_2^2}{ \sigma_{\ast,\max}^2}  \leq \frac{\|R_t\|_2^2}{ \sigma_{\ast,\max}^2} =  \frac{1}{\sigma_{\max}^2(R_t^{-1}) \sigma_{\ast,\max}^2} \leq \frac{1}{\sigma_{\max}({R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top})}$, where $\sigma_{\ast, \min} = \sigma_{\min} (\Sigma_\ast)$. As ${R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top}$ is positive semi-definite, this choice of $\eta$ yields
\begin{align}
   0 \preceq \eta {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top} \preceq I
\end{align}
Therefore, we have
\begin{align}
    \|(I_k - \eta  {R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top} ) \|_2 &\leq 1 - \eta \sigma_{\min} ({R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top}) \nonumber \\
    &\leq 1 - \eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2} \nonumber% \\
    % &\leq 1 - \frac{\|R_0\|_2^2 \sigma_{\min}^2 ({R}_t^{-1}) \sigma_{\ast,\min}^2 }{\sigma_{\ast,\max}^2 }  \nonumber \\
    % &= 1 - \frac{\|R_0\|_2^2 \sigma_{\ast,\min}^2}{\|R_t\|_2^2 \sigma_{\ast,\max}^2 } 
\end{align}
Combining this with \eqref{rankk:initcontract}, we have
\begin{align}
    \|{V}_{\ast,\perp}^\top \hat{V}_{t+1}\|_2 &\leq (1 - \eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}) \|{V}_{\ast,\perp}^\top \hat{V}_{t}\|_2  \label{rankk:3contract} \\
    &\leq \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}\right)^{t} \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \label{rankk:2contract}
\end{align}
where \eqref{rankk:2contract} follows by recursively applying \eqref{rankk:3contract} and by the fact that $ \|R_j\|_2^2 \leq \|R_t\|_2^2$ for all $j <t$. 
All that remains is to show $\|R_t\|_2^2$ is uniformly upper bounded for all $t$. Recall that
\begin{align}
   {R}_{t+1}^\top {R}_{t+1} &= {R}_{t}^\top {R}_{t} + \eta^2 S_t^\top S_t \label{rankk:plusr}
\end{align}
% Since $S_t^\top S_t$ is PSD, so the singular values of ${R}_{t}$ are non-decreasing in $t$. In particular, $\|R_0\|_2 \leq \|R_t\|_2$ and $\sigma_{\min}(R_0) \leq \sigma_{\min}(R_t)$ for all $t$. 
Since the singular values of ${R}_{t}$ are non-decreasing in $t$. we have $\|R_t^{-1}\|_2 \leq \|R_0^{-1}\|_2$ for all $t$. Thus
\begin{align}
    S_t^\top S_t &=  
    %{R}_t^{-\top}\Lambda_t^\top \Sigma_\ast {R}_t^{-\top} ( \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast)\Sigma_\ast \Lambda_t^\top {R}_t^{-\top} (\hat{V}_t{R}_t^{-1} \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast)\Sigma_\ast \Lambda_t^\top {R}_t^{-\top} \nonumber \\
{R}_t^{-1} \Lambda_t \Sigma_\ast  (\Sigma_\ast \Lambda_t^\top {R}_t^{-\top} \hat{V}_t^\top    -  \Sigma_\ast V_\ast^\top )  (\hat{V}_t{R}_t^{-1} \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast)\Sigma_\ast \Lambda_t^\top {R}_t^{-\top} \nonumber \\
&= {R}_t^{-1} \Lambda_t \Sigma_\ast  (\Sigma_\ast \Lambda_t^\top {V}_t^\top    -  \Sigma_\ast V_\ast^\top )  ({V}_t \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast)\Sigma_\ast \Lambda_t^\top {R}_t^{-\top} \nonumber \\
&= {R}_t^{-1} \Lambda_t \Sigma_\ast  (\Sigma_\ast \Lambda_t^\top \Lambda_t \Sigma_\ast - \Sigma_\ast V_\ast^\top {V}_t \Lambda_t \Sigma_\ast  +  \Sigma_\ast V_\ast^\top V_\ast \Sigma_\ast - \Sigma_\ast \Lambda_t^\top V_t^\top V_\ast \Sigma_\ast)\Sigma_\ast \Lambda_t^\top {R}_t^{-\top} \nonumber \\
&= {R}_t^{-1} \Lambda_t \Sigma_\ast^2  (I_k -  \Lambda_t^\top \Lambda_t)\Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top}
% &= {R}_t^{-1} \Lambda_t \Sigma_\ast  (\Sigma_\ast \Lambda_t {R}_t^{-\top} \hat{V}_t^\top    -  \Sigma_\ast V_\ast^\top )  (\hat{V}_t{R}_t^{-1} \Lambda_t \Sigma_\ast  -  V_\ast \Sigma_\ast)\Sigma_\ast \Lambda_t^\top {R}_t^{-\top} \nonumber \\
\end{align}
Also, we have $\| I_k -  \Lambda_t^\top \Lambda_t\|_2 = \text{dist}(\hat{V}_t, V_\ast)$. Therefore, using Cauchy-Schwarz,
\begin{align}
    \| S_t^\top S_t \|_2
&\leq \sigma_{\ast,\max}^4 \|{R}_t^{-1}\|_2^2  \; \text{dist}(\hat{V}_t, V_\ast) \nonumber \\
&\leq \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^2  \; \text{dist}(\hat{V}_t, V_\ast) \nonumber \\
&= \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^2  \; \|V_{\ast,\perp}^\top V_t\|_2 \nonumber \\
&\leq  \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^2  \; \|V_{\ast,\perp}^\top R_t\|_2 \|R_t^{-1}\|_2 \nonumber \\
&=  \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3  \; \|V_{\ast,\perp}^\top V_t \hat{R}_t\|_2  \nonumber \\
&\leq \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3  \; \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}\right)^{t} \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \label{rankk:4}
\end{align}
where \eqref{rankk:4} follows from \eqref{rankk:2contract}.
Thus, recalling \eqref{rankk:plusr} we have
\begin{align}
    \|R_{t+1}\|_2^2 &\leq \|R_{t}\|_2^2 + \eta^2 \|S_t^\top S_t\|_2 \nonumber \\
    &\leq \|R_{t}\|_2^2 + \eta^2 \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3  \; \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}\right)^{t} \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \nonumber \\
    &\leq  \|R_{t}\|_2^2 + \eta^2 \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3  \; \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}\right)^{t} \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \label{rankk:eta1} \\
    &\leq  \|R_{0}\|_2^2 + \eta^2 \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3 \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2  \; \sum_{j =1}^t \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}\right)^{j}  \label{rankk:recur} \\
    &= \|R_{0}\|_2^2 + \eta^2 \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3 \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \Big(1 - \eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}\Big) \; \frac{1 - \left(\eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}\right)^t}{\eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}} \\
    &= \|R_{0}\|_2^2 + \eta^2 \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3 \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \Big( \frac{ \|{R}_t \|_2^2}{\eta\sigma_{\ast,\min}^2} - 1 \Big)
    \left(1 - \left(\eta \frac{\sigma_{\ast,\min}^2}{\|{R}_t \|_2^2}\right)^t\right) \nonumber \\
    &\leq \|R_{0}\|_2^2 + \eta^2 \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3 \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \Big( \frac{ \|{R}_t \|_2^2}{\eta\sigma_{\ast,\min}^2} - 1 \Big)
     \nonumber \\
    &= \|R_{0}\|_2^2 + \eta \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3 \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \Big( \frac{ \|{R}_t \|_2^2}{\sigma_{\ast,\min}^2} - \eta \Big) \nonumber\\
    &\leq \|R_{0}\|_2^2 + \eta \sigma_{\ast,\max}^4 \|{R}_0^{-1}\|_2^3 \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2\frac{ \|{R}_{t+1} \|_2^2}{\sigma_{\ast,\min}^2} \nonumber \\
    &=  \|R_{0}\|_2^2 + \eta \frac{ \sigma_{\max}(R_{0})}{\sigma_{\min}^3(R_0)} \frac{ \sigma_{\ast,\max}^4}{\sigma_{\ast,\min}^2}\|R_{t+1}\|_2^2 
\end{align}
where \eqref{rankk:eta1} follows from our choice of $\eta$ and \eqref{rankk:recur} follows by recursively applying \eqref{rankk:eta1} and by the fact that $\|R_j\|^2_2 < \|R_t\|_2^2$ for all $j < t$. % Next, we assume $\eta \geq $
Rearranging, we have
\begin{align}
    \left(1 - \eta \frac{ \sigma_{\max}(R_{0})}{\sigma_{\min}^3(R_0)} \frac{ \sigma_{\ast,\max}^4}{\sigma_{\ast,\min}^2}\right)\|R_{t+1}\|_2^2 &\leq \|R_0\|_2^2
\end{align}
Thus, if we further choose $\eta \leq \frac{1}{2}  \frac{ \sigma_{\min}^3(R_0)}{\sigma_{\max}(R_{0})} \frac{  \sigma_{\ast,\min}^2}{\sigma_{\ast,\max}^4}$ (note that $\frac{1}{2}  \frac{ \sigma_{\min}^3(R_0)}{\sigma_{\max}(R_{0})} \frac{  \sigma_{\ast,\min}^2}{\sigma_{\ast,\max}^4} =  \frac{1}{2} \frac{ \sigma_{\min}^3(R_0)}{\sigma_{\max}^3(R_{0})}\frac{ \sigma_{\ast,\min}^2}{\sigma^2_{\ast,\max}} \frac{\|R_0\|_2^2}{\sigma^2_{\ast,\max}} \leq \frac{\|R_0\|_2^2}{\sigma^2_{\ast,\max}}$, so this choice of $\eta$ is consistent with our previous requirement), we have
\begin{align}
\|R_{t+1}\|_2^2 &\leq 2\|R_0\|_2^2 = 2\sigma_{\max}^2(R_0)
\end{align}
for all $t \in \mathbb{N}$. Using this with \eqref{rankk:2contract} yields 
\begin{align}
    \|{V}_{\ast,\perp}^\top \hat{V}_{t+1}\|_2
    &\leq \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{2 \sigma_{\max}^2(R_0)}\right)^{t} \|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \label{rankk:6contract}
\end{align}
% Next, note that
% \begin{align}
%     \sigma_{\ast,\max}^2\sigma_{\min}^2 ({R}_0^{-1}) \geq \sigma_{\ast,\max}^2\sigma_{\min}^2 ({R}_t^{-1}) &\geq \sigma_{\min} ({R}_t^{-1} \Lambda_t \Sigma_\ast^2 \Lambda_t^\top {R}_t^{-\top}) \geq  \sigma_{\ast,\min}^2 \sigma_{\min}^2 ({R}_t^{-1})
% \end{align}
% Therefore if we choose $\eta$ such that
% $\frac{1}{2 \sigma_{\min} ({R}_0^{-1})^2 \sigma_{\ast,\min}^2} \leq \eta \leq \frac{1}{2 \sigma_{\min} ({R}_0^{-1})^2 \sigma_{\ast,\min}^2} $, %=\frac{\|R_0\|_2^2}{2 \sigma_{\ast,\min}^2} 
% then we have 
% \begin{align}
    
% \end{align}
Thus, $\|{V}_{\ast,\perp}^\top \hat{V}_{t+1}\|_2$ is linearly converging to zero with rate $1- \eta \frac{\sigma_{\ast,\min}^2}{2 \sigma_{\max}^2(R_0)}$. This implies that
\begin{align}
    \|{V}_{\ast,\perp}^\top \hat{V}_{t+1}\|_2 &\leq (1 - \sigma_{\ast, \min}^2)^t\|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \nonumber \\
    \Rightarrow \|{V}_{\ast,\perp}^\top {V}_{t+1}\|_2 \sigma_{\min}(R_{t+1}) &\leq (1 - \eta \frac{\sigma_{\ast,\min}^2}{2\sigma_{\max}^2(R_0)})^t\|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2 \nonumber \\
    \Rightarrow \text{dist}(\hat{V}_{t+1}, V_\ast) &\leq   \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{2 \sigma_{\max}^2(R_0)}\right)^t \frac{\|{V}_{\ast,\perp}^\top \hat{V}_{0}\|_2}{\sigma_{\min}(R_{0})} \leq \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{2\sigma_{\max}^2(R_0)}\right)^t \frac{\sigma_{\max}(R_{0})}{\sigma_{\min}(R_{0})} \label{rankk:contract},
\end{align}
% Namely,
% \begin{align}
% \text{dist}(\hat{V}_{t+1}, V_\ast) &\leq (1 - \sigma_{\ast, \min}^2)^t \text{dist}(\hat{V}_{0}, V_\ast)
% \end{align}
% But then with appropriate choice of $\eta$ we can obtain that the distance is zero - something is fishy

Finally we complete the proof. We have
\begin{align}
    \| M - \hat{U}_{T+1} \hat{V}_T^\top \|_F^2 &= \|M - M {V}_T R_T^{-\top} \hat{V}_T^\top \|_F^2 \label{rankk:fin1} \\
    &= \|M - M {V}_T {V}_T^\top \|_F^2 \\
    &= \|U_\ast \Sigma_\ast V_\ast^\top (I -  {V}_T {V}_T^\top) \|_F^2 \\
    &\leq \|M\|_F^2 \; \text{dist}^2(\hat{V}_T, V_\ast) \\
    &\leq \left(1 - \eta \frac{\sigma_{\ast,\min}^2}{2 \sigma_{\max}^2(R_0)}\right)^T \|M\|_F^2 \frac{\sigma_{\max}(R_{0})}{\sigma_{\min}(R_{0})} \label{rankk:finfin}
\end{align}
where \eqref{rankk:fin1} follows because $\hat{U}_{T+1} = M \hat{V}_{T} (\hat{V}_{T}^\top \hat{V}_{T})^{-1} = M {V}_{T} R_{T}^{-\top} $ is the least squares solution and \eqref{rankk:finfin} follows by 
\eqref{rankk:contract}.
\end{proof}

% \textbf{Upper Bounding} $\|R_{t}\|_2$ \textbf{for all} $t$. 

% We have:



==> submit/arxiv_version/Experiments_arxiv.tex <==
\section{Experiments} \label{sec:experiments}
We focus on three points in our experiments: (i) the effect of many local updates for the local head in FedRep (ii) the quality of the global representation learned by FedRep and (iii) the applicability of FedRep to a wide range of datasets. Full experimental details are provided in Appendix \ref{app:experiments}.

\subsection{Synthetic Data}


We start by experimenting with an instance of the multi-linear regression problem analyzed in Section \ref{sec:linear}. Consistent 
with this formulation, we generate synthetic samples $\mathbf{x}_i^j \sim \mathcal{N}(0, \mathbf{I}_d)$ and labels $y_{i}^j \sim \mathcal{N}(\mathbf{w}_i^{\ast^\top}{\mathbf{B}}^{\ast^\top}\mathbf{x}_i^j, 10^{-3})$ (here we include an additive Gaussian noise). The ground-truth heads $\mathbf{w}_i^\ast \in \mathbb{R}^k$ for clients $i \in [n]$ and the ground-truth representation ${\mathbf{B}}^\ast \in \mathbb{R}^{d \times k}$ are generated randomly by sampling and normalizing Gaussian matrices. 
% and optimal solutions as
% \begin{align}
%     \mathbf{x}_i^j &\sim \mathcal{N}(0, \mathbf{I}_d)\; \forall i \in [n], j \in [m] \\
%     \mathbf{w}_i^\ast &\sim \mathcal{N}(0, \mathbf{I}_k)\; \forall i \in [n],
% \end{align}
% and $\mathbf{B}$ is an orthogonal basis for a $k$-dimensional subspace of $\mathbb{R}^d$.
% Here we consider the noisy case:
% \begin{align}
%     \hat{F}(\mathbf{W},\mathbf{B}) = \frac{1}{2nm} \sum_{i=1}^n \sum_{j=1}^m (\langle \mathbf{x}_{i}^j, \mathbf{B}\mathbf{w}_i\rangle - y_i^j )^2
% \end{align}
% where $y_i^j \sim \mathcal{N}(\langle \mathbf{x}_{i}^j, \mathbf{B}_\ast\mathbf{w}_i^\ast \rangle, \zeta_i )$.

% Note that in this setting, the measurements are i.i.d., but the data itself is non-i.i.d. across clients because each client has a distinct ground-truth solution.


%%%%%%%HHHHHHHHHH
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.7\columnwidth]{old_synth3.eps}}
\vspace{-2mm}
\caption{Comparison of (principal angle) distances between the ground-truth and estimated representations by FedRep and alternating gradient descent algorithms for different numbers of clients $n$. In all plots, $d=10$, $k=2$, $m=5$, and $r=0.1$.}
\label{fig:synth11}
\end{center}
\vskip -0.3in
\end{figure}


\textbf{Benefit of finding the optimal head.}  We first demonstrate that the convergence of FedRep improves with larger number of clients $n$, making it highly applicable to federated settings. Further, we give evidence showing that this improvement is augmented by the minimization step in FedRep, since methods that replace the minimization step in FedRep with 1 and 10 steps of gradient descent (GD-GD and 10GD-GD, respectively) do not scale properly with $n$. 
In Figure \ref{fig:synth11}, we plot convergence trajectories for FedRep, GD-GD, and 10GD-GD for four different values of $n$ and fixed $m, d, k$ and $r$.  As we observe in Figure \ref{fig:synth11}, by increasing the number of nodes $n$, clients converge to the true representation faster. Also, running more local updates for finding the local head accelerates the convergence speed of FedRep. In particular, FedRep which exactly finds the optimal local head at each round has the fastest rate compared to GD-GD and 10GD-GD that only run 1 and 10 local updates, respectively, to learn the head.


% We plot the principal angle distance between the estimated and optimal representation. The plots for function value is similar and is included in the Appendix.


% \begin{table}[t]
% \caption{Smallest $m$ for which $F(\mathbf{W}_{500}, \mathbf{B}_{500}) \leq 10^{-6}$. Here $d=10$, $k=2$ and $\sigma = 0.1$ for all trials. We see that the  minimum $m$ required to achieve the desired accuracy actually decreases with $n$.}
% \label{table1}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Algorithm & $n=10$  &  $n=50$ & n=100 & n=500\\
% \midrule
% AltMinGD      & &  & &  \\
% AltGD-GD    &  &  & &      \\
% % LG-Fed & 85.35$\pm$ & 68/74  \\
% % FedAvg + LG-Fed & $\pm$ &   \\
% % FedAvg   & $\pm$ &   \\
% % FedSGD   & 60.67$\pm$ & 30 \\
% % Fed-MTL     & 76.59$\pm$ &   \\
% % Local     & 92.5 $\pm$ & 88.19  \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
% \caption{Function values and representation learning errors for AltMinGD and AltGD-GD. The value of $m$ is fixed in each row and $n$ is fixed in each column. We see that the relative improvement of AltMinGD over AltGD-GD increases with $n$, highlighting the advantage of AltMinGD in large-$n$ settings.}
% \label{fig:synthetic1}
% \end{center}
% \vskip -0.2in
% \end{figure}

\textbf{Generalization to new clients.} 
Next, we evaluate the effectiveness of the representation learned by FedRep in reducing the sample complexity for a new client which has not participated in training. We compare against FedSGD, which executes distributed SGD to learn a single model $(\mathbf{B},\mathbf{w})$. We first train FedRep and FedSGD on a fixed set of $n=100$ clients as in Figure~\ref{fig:fedrep1},  where $(d,k)\!=\!(20,2)$. 
The new client has access to $m_{\text{new}}$ labeled local samples. It will use the representation $\mathbf{{B}}^*\in \mathbb{R}^{d \times k}$ learned from the training clients, and learns a personalized head using this representation and its local training samples. For both FedRep and FedSGD, we solve for the optimal head given these samples and the representation learned during training. We compare the MSE of the resulting model on the new client's test data to that of a model trained by only using the $m_{\text{new}}$ labeled samples from the new client (Local Only) in Figure \ref{fig:bar_new}. The large error for FedSGD demonstrates that it does not learn the ground-truth representation. Meanwhile, the representation learned by FedRep allows an accurate model to be found for the new client as long as $m_{\text{new}}\geq k$, which drastically improves over the complexity for Local Only ($m_{\text{new}}\!=\!\Omega(d)$).

% Next, we compare against learning a single model in , learning a single overparameterized model,  MTL and AltGD-GD.

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
% \caption{Function values and representation learning errors for AltMinGD and AltGD-GD. The value of $m$ is fixed in each row and $n$ is fixed in each column. We see that the relative improvement of AltMinGD over AltGD-GD increases with $n$, highlighting the advantage of AltMinGD in large-$n$ settings.}
% \label{fig:synthetic1}
% \end{center}
% \vskip -0.2in
% \end{figure}



%%% HHHHHHHH
\begin{figure}[t]
%\vspace{-0.1in}
\begin{center}
\centerline{\includegraphics[width=0.53\columnwidth]{bar_new.eps}}
%\vskip -0.15in
\vspace{-2mm}
\caption{MSE on new clients sharing the representation after fine-tuning using various numbers of samples from the new client.}
\label{fig:bar_new}
\end{center}
\end{figure}



\subsection{Real Data}
We next investigate whether these insights apply to nonlinear models and real datasets.

\textbf{Datasets and Models.} We use four real datasets: CIFAR10 and CIFAR100 \citep{krizhevsky2009learning}, FEMNIST \citep{caldas2018leaf,cohen2017emnist} and Sent140 \citep{caldas2018leaf}. The first three are image datasets and the last is a text dataset for which the goal is to classify the sentiment of a tweet as positive or negative. 
%  each contain 50,000 training samples and 10,000 test samples from 10 and 100 classes, respectively. 
 We control the heterogeneity of CIFAR10 and CIFAR100 by assigning different numbers $S$ of classes per client, from among 10 and 100 total classes, respectively.  Each client is assigned the same number of training samples, namely $50000/n$. For FEMNIST, we restrict the dataset to 10 handwritten letters and assign samples to clients according to a log-normal distribution as in \cite{li2019feddane}. We consider a partition of $n\!=\!150$ clients with an average of 148 samples/client. For Sent140, we use the natural assignment of tweets to their author, and use $n\!=\!183$ clients with an average of 72 samples per client. We use 5-layer CNNs for the CIFAR datasets, a 2-layer MLP for FEMNIST, and an RNN for Sent$140$ \textcolor{black}{(details provided in Appendix \ref{app:experiments})}.

\textbf{Baselines.} We compare against a variety of personalized federated learning techniques as well as methods for learning a single global model and their fine-tuned analogues. Among the personalized methods, FedPer \citep{arivazhagan2019federated} is most similar to ours, as it also learns a global representation and personalized heads, but makes simultaneous local updates for both sets of parameters, therefore makes the same number of local updates for the head and the representation on each local round. Fed-MTL \citep{smith2017federated} learns local models and a regularizer to encode relationships among the clients, PerFedAvg \citep{fallah2020personalized} leverages meta-learning  to learn a single model that performs well after adaptation on each task, and LG-FedAvg \citep{liang2020think} learns local representations and a global head. APFL \citep{deng2020adaptive} interpolates between local and global models, and L2GD \citep{hanzely2020federated} and Ditto \citep{li2020ditto} learn local models that are encouraged to be close together by global regularization. For global FL methods, we consider FedAvg \citep{mcmahan2017communication}, SCAFFOLD \citep{karimireddy2020scaffold}, and FedProx \citep{li2018federated}. To obtain fine-tuning results, we first train the global model for the full training period, then each client then fine-tunes only the head on its local training data for 10 epochs of SGD before computing the final test accuracy. 
% (5) local only training with no global communication. Method (2) is the standard federated learning technique, (3) is a well-known method for achieving personalized models, and (1) and (4) are methods with similar intuitions as ours.



% We use the same five-layer CNN as in \citep{liang2020think} for CIFAR10 and an LSTM for . On each communication round, a constant fraction $r=0.1$ of all of the clients are sampled. To implement AltMinGD, each client executes $\tau \gg 1$ local minibatch SGD steps on the final layer using a batch of size $B$. Then, the base layers are updated with one minibatch SGD step with batch size $B$ and sent to the server. 



% First, we compare the output of AltMinGD to that produced by vanilla federated averaging \cite{mcmahan2017communication} with $E = 20$ local update steps.

% The parameter $E$ denotes the number of local communication rounds for FedAvg. FedSGD is FedAvg with $E=1$, i.e. distributed SGD.


% \begin{table*}[ht]
% \caption{Average local test accuracies over the final 10 rounds out of $T=200$ total rounds, with 95\% confidence intervals.
% }
% \vskip 0.15in
% \begin{center}
% \begin{small}
% % \begin{sc}
% \begin{tabular}{lcccccccc}
% \toprule\label{bigtable1}
% Dataset & FedRep & GD-GD & FedAvg &  Fed-MTL &   LG-FedAvg  & Local \\%& Post-Adapt  \\
% \midrule
% CIFAR10, $S=2$, $n=100$ & $86.08\pm .3$ & $83.52 \pm .4$ & $44.29\pm 1.9$ & $70.44 \pm .2$  & $78.12 \pm 1.1$  & $87.28 \pm .6$ \\
% CIFAR10, $S=2$, $n=1000$ &$76.41\pm .5$ & $73.07 \pm .5$ & $41.11\pm 1.6$ & $56.90 \pm .1$ &  $68.32 \pm 1.4$  &$72.17 \pm .3$\\
% CIFAR10, $S=5$, $n=100$ & $72.19 \pm .9$  &$72.26 \pm 1.0$ & $58.14 \pm 1.5$ & $54.21\pm .3$&  $57.83 \pm 1.2$  & $67.76 \pm .5$\\ %$72.66 \pm .2$
% CIFAR10, $S=5$, $n=1000$ & $53.41 \pm .7$ & $52.27 \pm .8$ & $50.40 \pm .9$ & $34.58 \pm .5$ & $41.05 \pm 1.3$ &  $47.56 \pm .4$\\ %$48.63\pm .7$
% CIFAR100, $S=20$, $n=100$ & $38.17 \pm .8$ & $37.41 \pm .5$ & $15.74 \pm .8$ & $23.38 \pm .3$ & $31.06 \pm .5$ & $32.04 \pm .7$ \\
% CIFAR100, $S=20$, $n=500$ & $21.88 \pm .6$ & $21.92 \pm .6$ & $19.43 \pm .7$  & $10.56 \pm .3$ & $14.83 \pm .4$ & $21.06 \pm .6$ \\ %24.30 \pm .6^*
% % CIFAR100, $S=50$, $n=100$ & $23.71 \pm .7$ & $23.45 \pm .6$ & $20.25\pm .8$ & $14.72 \pm .3$ & $25.07 \pm .4$ & & $17.10\pm 1.1$ \\
% % CIFAR100, $S=50$, $n=500$ & $13.33^*$ & $11.50 \pm .3$ & $18.82\pm.4$ & $6.09 \pm .2$ & $45.56$& &  $11.66 \pm 1.4$\\
% FEMNIST, $n=150$ & $65.52 \pm .8$  & $39.21 \pm .6$ & $60.71 \pm 1.8$ & $32.34 \pm .7$  & $29.78\pm .5$  &$29.12 \pm .9$ \\
% Sent$140$, $n=183$ & $72.13 \pm .2$ &$69.57 \pm .8$ & $56.82 \pm 1.4$ & $54.82 \pm .5$ & $70.84 \pm 1.4$ & $70.22 \pm .8$\\%$70.64 \pm .9$
% % FEMNIST, $n=100$ & & &  & & & & &\\
% \bottomrule
% \end{tabular}
% % \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}

\begin{table*}[ht]
\caption{Average test accuracies on various partitions of CIFAR10, CIFAR100, Sent140 and FEMNIST with participation rate $r\!=\!0.1$.
}
\vskip -1in
% \vskip 0.15in
\begin{center}
% \begin{sc}
\footnotesize
\begin{tabular}{l|ccc|cc|c|c}
\toprule\label{bigtable1}
& \multicolumn{3}{c|}{{CIFAR10}}  &  \multicolumn{2}{c|}{{CIFAR100}}       & Sent140 & FEMNIST  \\
\midrule
(\# clients $n$, \# classes per client $S$) & $(100,2)\!$ & $\!(100,5)$ & $(1000,2)$ & $(100,5)$  & $(100,20)$ & $(183,2)$ & $(150,3)$ \\%& Post-Adapt  \\
\midrule
Local Only & $\mathbf{89.79}$ & 70.68 & 78.30 & 75.29 & 41.29 & 69.88 &  60.86 \\
\midrule
FedAvg \citep{mcmahan2017communication} &  42.65 & 51.78 & 44.31 & 23.94 & 31.97 & 52.75 & 51.64 \\ %53.75 
FedAvg+FT & 87.65 & 73.68  & 82.04 & $\mathbf{79.34}$ & 55.44  &71.92  & 72.41\\ %71.54
FedProx \citep{li2018federated} & 39.92 & 50.99 & 21.93  & 20.17 & 28.52 & 52.33 &  18.89 \\
FedProx+FT & 85.81 & 72.75 & 75.41 & 78.52 & 55.09 & 71.21 & 53.54 \\
SCAFFOLD \citep{karimireddy2020scaffold} & $37.72$ & $47.33$ & $33.79$ &  20.32 & 22.52 & $51.31$ & 17.65 \\
SCAFFOLD+FT  & $86.35$ &  $68.23$ &$78.24$ & 78.88 & 44.34 & 71.49  & 52.11  \\
\midrule 
Fed-MTL \citep{smith2017federated} & 80.46 & 58.31  & 76.53  & 71.47 & 41.25 & 71.20 & 54.11 \\
PerFedAvg \citep{fallah2020personalized} & 82.27 & 67.20 & 67.36 & 72.05 &  52.49  & 68.45 & 71.51 \\
LG-Fed \citep{liang2020think} & 84.14  & 63.02 &  77.48 & 72.44 &38.76 & 70.37 & 62.08 \\
L2GD \citep{hanzely2020federated} & 81.04 & 59.98 & 71.96 & 72.13 & 42.84 & 70.67 & 66.18  \\
APFL  \citep{deng2020adaptive} & 83.77 & 72.29 & 82.39 & 78.20 & 55.44 & 69.87 & 70.74 \\
Ditto \citep{li2020ditto} & 85.39 & 70.34 & 80.36 & 78.91 &  $\mathbf{56.34}$ & 71.04 & 68.28 \\
FedPer \citep{arivazhagan2019federated} & 87.13 & 73.84 & 81.73 & 76.00 & 55.68 & 72.12 & 76.91 \\
\midrule
FedRep (Ours) & $\mathbf{87.70}$ & $\mathbf{75.68}$ & $\mathbf{83.27}$ & 79.15 & 56.10 &  $\mathbf{72.41}$ & $\mathbf{78.56}$ \\ 
\bottomrule
\end{tabular}
% \end{sc}
\end{center}
\vskip -0.1in
\end{table*}



\textbf{Implementation.}
In each experiment we sample a ratio $r\!=\!0.1$ of all the clients on every round. We initialize all models randomly and train for $T\!=\!100$ communication rounds for the CIFAR datasets, $T\!=\!50$ for Sent140, and $T\!=\!200$ for FEMNIST. In each case, for each local updates FedRep executes ten local epochs of SGD with momentum to train the local head, followed by one epoch for the representation in the case of CIFAR10 with $n\!=\!100$ and 5 epochs in all other cases. All other methods use the same number of local epochs as FedRep does for updating the representation. Accuracies are computed by taking the average local accuracies for all users over the final 10 rounds of communication, except for the fine-tuning methods. These accuracies are computed after locally training the head of the fully-trained global model for ten epochs for each client. 


%%%%%%%%%%HHHHHHH
\begin{figure}[t]
\begin{center}
%\vspace{-2mm}
\centerline{\includegraphics[width=0.56\columnwidth]{cifar.eps}}
%\vskip -0.05in
\caption{CIFAR10 local test errors for different numbers of local epochs $E$ for  FedAvg and for the heads in FedRep.}
\label{fig:cifar}
\end{center}
\vspace{-2mm}
\end{figure}



\textbf{Benefit of more local updates.} As mentioned in Section \ref{sec:intro}, a key advantage of our formulation is that it enables clients to run many local updates without causing divergence from the global optimal solution. We demonstrate an example of this in Figure \ref{fig:cifar}. Here, there are $n\!=\!100$ clients where each has $S\!=\!2$ classes of images. For FedAvg, we observe running more local updates does not necessarily improve the performance. In contrast, FedRep's performance is monotonically non-decreasing with the number of local epochs for the heads, i.e., {\em FedRep  is never hurt by more local computation on the heads.}  %, making it especially conducive to federated settings in which we want to distribute as much of the computation as possible

\textbf{Robustness to varying levels of heterogeneity, number of clients and number of samples per client.} We show the average local test errors for all of the algorithms for a variety of settings in Table \ref{bigtable1}. Recall that for the CIFAR datasets, the number of training samples per client is equal to $50000/n$, so the columns with 100 clients have 500 training samples per client, and the column with 1000 clients has only 50 training samples per client. In all cases, FedRep is either the top-performing method or is very close to the top-performing method. Surprisingly, the fine-tuning methods perform very well, especially FedAvg+FT. The superior performance of FedAvg relative SCAFFOLD is likely because all settings involve partial client participation. 
% We also observe that fine-tuning methods perform relatively well

% ideas for another plot: 1) move version of fedrep vs gdgd with comm time from rebuttal to the main body 2) show degredation of gd-gd with more local epochs... but what to compare against? fedavg with 


% Not surprisingly, the largest gain for FedRep over FedAvg comes in heterogeneous settings with many samples/client: CIFAR10 and CIFAR100 with 2 and 20 classes/client, respectively, and $n=100$. In these settings, FedRep matches, or nearly matches, the performance of local-only training.
% Meanwhile, even in homogeneous and small-data settings conducive to global-only training, i.e. $S\!=\!5$ and $n\!=\!1000$ on CIFAR10, FedRep still outperforms all the baselines, even without any regularization added to prevent over-fitting to the head. {\em This evidence supports our intuition that FedRep effectively interpolates between local and global learning.} Furthermore, FedRep outperforms all other baselines.



%% \textcolor{red}{why doe we only talk about fedrep vs fedavg? we should say we outperform all those baselines}


%%%%%%%%%%%%%%%HHHHHHHHHHHHHH
\begin{figure}[t]
\begin{center}
\vspace{-2mm}
\centerline{\includegraphics[width=0.64\columnwidth]{new_users.eps}}
\vspace{-2mm}
\caption{Test accuracy on handwritten digits from FEMNIST after fine-tuning the head of models trained on FEMNIST-letters.}
\label{fig:new_clients}
\end{center}
\vspace{-6mm}
\end{figure}

\textbf{Generalization to new clients.} 
We also evaluate the strength of the representation learned by FedRep in terms of %its ability to lead to 
adaptation for new users. To do so, we first train FedRep, FedAvg, PerFedAvg, LG-FedAvg, APFL, L2GD and FedProx
in the usual setting on the partition of FEMNIST containing images of 10 handwritten letters (FEMNIST-letters). Then, we encounter clients with data from a different partition of the FEMNIST dataset, containing images of handwritten digits. We assume we have access to a dataset of 500 samples at this new client to fine tune the head. Using these, with each of the algorithms, we fine tune the head over multiple epochs while keeping the representation fixed. 
% Over each epoch, we train the head by sweeping over these new samples, and test over a holdout validation set (again from this new partition). 
In Figure \ref{fig:new_clients}, we repeatedly sweep over the same 500 samples over multiple epochs to further refine the head, and plot the corresponding local test accuracy. As is apparent, FedRep has significantly better performance than these baselines.  


==> submit/arxiv_version/Introduction_arxiv.tex <==
\section{Introduction}
\label{sec:intro}
% keywords: heterogenous, non-iid, personalization

% Machine learning systems are increasingly transitioning away from centralized 


 
% For examples, in image classification and next-word prediction, modern models typically require millions of samples to learn accurate mappings from the high-dimensional spaces of images and phrases to labels and next words, respectively -- too many to be collected and processed on one device. 
% Fortunately, more and more devices are becoming connected and therefore able to communicate with a central server.
% In such settings, the central authority plays a crucial role in leveraging global data to provide each client with an accurate model, while  satisfying client privacy and communication constraints. 
% {\em Federated learning} \cite{mcmahan2017communication} aims to develop more effective methods that the central authority may employ in these settings. 

Many of the most heralded successes of modern machine learning have come in {\em centralized} settings, wherein a single model is trained on a large amount of centrally-stored data. The growing number of data-gathering devices, however, calls for a distributed architecture to train models. Federated learning aims at addressing this issue by providing a platform in which a group of clients collaborate to learn effective models for each client by leveraging the local computational power, memory, and data of all clients \citep{mcmahan2017communication}. The task of coordinating between the clients is fulfilled by a central server that combines the models received from the clients at each round and broadcasts the updated information to them. Importantly, the server and clients are restricted to methods that satisfy communication and privacy constraints, preventing them from directly applying centralized techniques. 

However, one of the most important challenges in federated learning is the issue of \textit{data heterogeneity}, where the underlying data distribution of client tasks could be substantially different from each other. In such settings, if the server and clients learn a single shared model (e.g., by minimizing average loss), the resulting model could perform poorly for many of the clients in the network (and also not generalize well across diverse data \citep{jiang2019improving}). 
In fact, for some clients, it might be better to simply use their own local data (even if it is small) to train a local model; see Figure~\ref{fig:fedrep1}. Finally, the (federated) trained model may not generalize well to unseen clients that have not participated in the training process. These issues raise the question: 
%%%
\begin{quote}
\vspace{-0mm}
  ``\textit{How can we exploit the data and computational power of all clients in data heterogeneous settings to learn a personalized model for each client?}''
  \vspace{-0mm}
\end{quote}
We address this question by taking  advantage of the common 
% structure/
representation among clients. Specifically, we view the data heterogeneous federated learning problem as $n$ parallel learning tasks that they possibly have some common structure, and {\em our goal is to learn and exploit this common representation to improve the quality of each client's model}. This approach draws inspiration from centralized learning, where we have  witnessed success in training multiple tasks or learning multiple classes simultaneously by leveraging a common  (low-dimensional) representation (e.g. in image classification, next-word prediction) \citep{bengio2013representation, lecun2015deep}. 
%%%% SHOULD THIS BE IN SOMEWHERE, OR SKIP? Insight suggests that statistical heterogeneity is concentrated in the labels of the data for many learning settings, so we can utilize all of the data to learn the features. 


%% In essence, these studies hypothesize that a low-dimensional data representation typically exists for common types of machine learning tasks, such as image classification and next-word prediction.


%% and (ii) neural networks are effective when trained with gradient-based methods on a large amount of data because they recover this low-dimensional representation, which makes it easy for a simple classifier to accurately map from the representation space to the label space.

% , neural networks learn a low-dimensional data representation that makes it easy for a simple classifier to accurately map from the representation space to the label space. The key takeaway from this well-supported theory is that a useful low-dimensional data representation typically exists for 

% In this work, we argue that the goal of the central authority in federated learning should also be to learn a representation.

% As it turns out, we can use these insights to address fundamental challenges in federated learning. The first is {\em statistical heterogeneity}, which describes the non-i.i.d. nature of the data across clients. This limits the effectiveness of training a single global model, since it may not generalize well across the diverse client data \cite{jiang2019improving}. Insight suggests that statistical heterogeneity is concentrated in the labels of the data for many learning settings, so we can utilize all of the data to learn the features. 

% The second challenge is {\em limited communication} between the clients and the central server, which prevents the server from accessing the data stored on each device, and instead can only access concentrated updates. As we will show, insight suggests that gradient-based updates are sufficient to learn the representation, while low-dimensionality of the representation allows the network heads to be computed locally without any communication.

\noindent \textbf{Main Contributions.} We introduce a novel federated learning framework and an associated algorithm for data heterogeneous settings. We summarize our main contributions  below.






% \begin{figure}[t]
% %\vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.6\columnwidth]{fedrep1.pdf}}
% \caption{Outline of how predictions are made in FedRep pipeline. \sanjay{\bf update figure g, h}}
% \label{fig:fedrep1}
% \end{center}
% \vskip -0.2in
% \end{figure}


%%%%%%%%%%%%%
\begin{figure}[t]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.55\columnwidth]{bar_new3.eps}}
\vspace{-2mm}
\caption{Local only training suffers in small-training data regimes, whereas training a single global model with FedSGD cannot overcome client heterogeneity even when the number of training samples is large. FedRep exploits a common representation of the clients to achieve small error in all cases.}
\label{fig:fedrep1}
\end{center}
\vskip -0.3in
\end{figure}


\begin{itemize}
    \item[(i)]  \textbf{FedRep Algorithm.} {Federated Representation Learning (FedRep)} leverages all of the data stored across clients to learn a global low-dimensional representation using gradient-based updates. Further, it enables each client to compute a personalized, low-dimensional classifier, which we term as the client's head, that accounts for the unique labeling of  each client's local data.
    %{\color{red}{In particular, given a data point $\mathbf{x}_i$, the $i$-th client predicts the label as $h_i(\phi(\mathbf{x_i}))$, where $\phi$ is the {\em global representation} mapping to a low-dimensional space, and $h_i$ is the {\em personalized} network head.}}
    
    % {\color{red}\item[(ii)] \textbf{Convergence Rate.} %FedRep achieves provably fast convergence in a linear setting. 
    % We show that FedRep converges to the optimal representation at a {\em exponentially fast rate} with near-optimal sample complexity in the case that each client aims to solve a linear regression problem with a two-layer linear neural network. 
    
    %{\color{red}{In this case, the problem is an instance of matrix sensing with sparse, rank-1 measurements. These measurements do {\em not} satisfy the restricted isometry property (RIP), so we develop new analysis to show the convergence properties of FedRep.}} 
    
    % Our analysis further implies that we only need $\mathcal{O}(\kappa^4 k^2 (k\log  (n) + \frac{ d}{n}))$ samples per client, where $n$ is the number of clients, $d$ is the dimension of the data, $k$ is the representation dimension and $\kappa$ is the condition number of the ground-truth client-heads matrix.} 
    
    %This highlights the effectiveness of FedRep in many-client, small-data-per-client regimes common in federated learning.
    
\item[(ii)] \textbf{Optimization for linear representation learning.} %FedRep achieves provably fast convergence in a linear setting. 
    We show that FedRep converges to the ground-truth representation at an {\em exponentially fast rate} in the case that each client aims to solve a linear regression problem with a two-layer linear neural network. In this special case, we reduce FedRep to alternating minimization (for the heads)-descent (for the representation). 
    %{\color{red}{In this case, the problem is an instance of matrix sensing with sparse, rank-1 measurements. These measurements do {\em not} satisfy the restricted isometry property (RIP), so we develop new analysis to show the convergence properties of FedRep.}} 
    Our analysis shows  that this simple algorithm requires only $\mathcal{O}( ( \nicefrac{d}{n}+ \log  (n))\log(\nicefrac{1}{\epsilon}))$ samples per client to reach an $\epsilon$-accurate representation, where $n$ is the number of clients and $d$ is the dimension of the data. This result is of interest beyond federated learning since it shows that alternating minimization-descent efficiently solves  the  linear multi-task representation learning problem considered in \cite{maurer2016benefit,tripuraneni2020provable,du2020fewshot}.
    % This sample complexity matches the statistical rates in \citep{tripuraneni2020provable,du2020fewshot} up to scaling with $k$ and log terms, and is  of interest beyond federated learning for showing the linear convergence of a practical algorithm to solve the linear representation learning problem.
    
    

    %% In this case, the problem is an instance of matrix sensing with rank-1, sparse measurements. These measurements do {\em not} satisfy the restricted isometry property (RIP), so we develop new analysis showing that FedRep achieves linear convergence with only $m n = \Omega(k^4 \kappa^4(n\log(n)+d))$ total samples, where $n$ is the number of clients, $m$ is the number of samples per client, $d$ is the dimension of the data, $k$ is the representation dimension and $\kappa$ is the condition number of the ground-truth client-representation matrix. This implies that we need only $m = \Omega(k^4\kappa^4(\log(n)+d/n))$ samples per client, suggesting the effectiveness of FedRep in many client, small data per client regimes common in federated learning. 
    

%  making our novel algorithm and analysis of interest beyond federated learning.  and provably faster than AltGD-GD, since the cost metric we care about is communication rounds.
    % \item \textbf{Provable improvements in local sample complexity.} To learn the representation and each client's optimal parameters, each client needs only $m = \tilde{O}(k+\frac{dk}{n})$ samples, so the local sample complexity decreases with more clients, making our algorithm particularly effective in many-client, small-data-per-client settings. Furthermore, recent work \cite{tripuraneni2020provable,du2020fewshot} shows that knowing the optimal representation reduces the sample complexity for a new client entering the system by a factor proportional to $d/\psi$, where $d$ is the ambient dimension and $\psi$ is the dimension of the representation.
    % \item \textbf{Simple case comparison with AltGD-GD?}

    \item[(iii)] \textbf{Empirical Results.} Through a combination of synthetic and real datasets (CIFAR10, CIFAR100, FEMNIST, Sent140) we show the benefits of FedRep in: (a) leveraging many local updates, (b) robustness to different levels of heterogeneity, and (c) generalization to new clients. 
    % We consider several important baselines including FedAvg \citep{mcmahan2017communication}, Fed-MTL \citep{smith2017federated}, LG-FedAvg \citep{liang2020think}, and Per-FedAvg \citep{fallah2020personalized}. 
    Our experiments indicate that FedRep outperforms several important baselines in heterogeneous settings that share a global representation.
    
    
    
    
    % \sanjay{Liam -- please update.} {\color{red} FedRep empirically improves over several competing algorithms for personalized federated learning on heterogeneous partitions of the MNIST \cite{}, CIFAR10 \cite{krizhevsky2009learning}, FEMNIST \cite{cohen2017emnist, caldas2018leaf}, and Sent140 \cite{} datasets. Even for a statistically homogeneous dataset, Shakespeare \cite{mcmahan2017communication, shakespeare2007complete}, we show that FedRep is not significantly worse than methods that learn an entire single global.}


    % and learning shallow linear neural networks. 
    % Our alternating minimization-descent algorithm for learning the representation in the federated setting is a novel algorithm for solving these types of problems, 
    % and our non-asymptotic analysis of it yields new results relevant beyond federated learning.
    % \item In a simple setting, we prove that our alternating minimization-descent approach outperforms the standard alternating gradient descent.
    %Simple case: alt-min-gd is better than alt-gd (better dependence on n and k)
    % \item Simple case: representation learning is better than no representation learning
    % \item Experiments

\end{itemize}

\noindent \textbf{Benefits of FedRep.} FedRep has numerous advantages over standard federated learning  (in which a single model is learned): 


{\em (I) Provable gains of cooperation.} From our sample complexity bounds, it follows that with FedRep, the sample complexity per client scales as $\Theta(  \nicefrac{d}{n}+ \log(n))$. On the other hand, local learning (without any collaboration) has a sample complexity that scales as $\Theta(d).$ Thus, if $1 \ll n \ll e^{\Theta(d)}$ (see Section~\ref{sec:fed-analysis} for details), we expect benefits of collaboration through federation. When $d$ is large (as is typical in practice), $e^{\Theta(d)}$ is exponentially larger, and federation helps each client. { \em To the best of our knowledge, this is the first sample-complexity-based result for personalized federated learning that demonstrates the benefit of cooperation.}



% {\color{red}{Consider for simplicity a setting where $d/n = o(\log(n))$ ($d$ is the data dimension, $n$ the number of clients). From our sample complexity bounds, it follows that with FedRep, the sample complexity is dominated by a $\log(n)$ term. On the other hand, local learning (without any collaboration) has a sample complexity that scale as $\Theta(d).$ Thus, if $\log(n) \ll \Theta(d)$ (equivalently $n \ll e^{\Theta(d)}$), we expect benefits of collaboration through federation. When $d$ is large (as is typical in practice), $e^{\Theta(d)}$ is exponentially larger, and federation helps each client. { \em To the best of our knowledge, this is the first sample-complexity-based result for federated learning that demonstrates the benefit of cooperation.}}}


% \textbf{When and whom does federation help?} {\color{red}{Observe that for a single client with no collaboration, the sample complexity scales as $\Theta(d).$ With FedRep, however, the sample complexity scales as $\Theta( \log(n) + \nicefrac{d}{n}).$ Thus, so long as $ \log(n) + \nicefrac{d}{n} \ll d,$ federation helps. This indeed holds in several settings, for instance when  $1 \ll n \ll e^{\Theta(d)}.$ In practical scenarios, $d$ (the data dimension) is large, and thus $e^{\Theta(d)}$ is exponentially larger; thus collaboration helps {\em each individual client.} Furthermore, from the point of view of a new client who enters the system later, it has a representation available for free, and this new client's sample complexity for adapting to its task is only $k \log(\nicefrac{1}{\epsilon})$. Thus, both the overall system benefits (a representation has been learned, which is useful for the new client because it now only needs to learn a head), and each individual client that did take part in the federated training also benefits.}}



{\em (II) Generalization to new clients.} For a new client, since a ready-made representation is available, the client only needs to learn a \textcolor{black}{head} with a low-dimensional representation of dimension $k$. Thus, its sample complexity scales only as $\Theta(k)$  instead of $\Theta(d)$ if no representation is learned.

{\em (III) More local updates.} By reducing the problem dimension, each client can make many local updates at each communication round, which is beneficial in learning its own individual head. This is unlike standard federated learning where multiple local updates in a heterogeneous setting moves each client {\em away} from the best averaged representation, and thus {\em hurts} performance. 


%% Further, if this single client has access to diverse data, it might 

% 1. federated setting, where complexity is as above. , the sample complexity is driven by two factors: (i) a shared cost of learning the representation (scales as $\nicefrac{\kappa^4 k^4 d}{r n}$) and (ii) simultaneous sub-exponential concentration of each sampled client's  measurements to an identity operation (scales as $\kappa^2 k^3 \log(rn)$); this is formally described in (\ref{complex}). 

%% 2. single client with no thought of the future -- d log(1/epsilon)

%% 3. Single client (even if it has diverse access to data) who want to learn a low k-dimensional representation, because for a new task tomorrow, it will give a sample complexity of k  $\log(\nicefrac{1}{\epsilon}.$ The sample complexity now is $d k \log(\nicefrac{1}{\epsilon})$

% Now when does collaboration help? 

% \begin{comment}
% \noindent \textbf{Benefits of FedRep.}


% Furthermore,  reducing the problem dimension at each client
    
%     \textbf{More Local Updates.}
    

%     Thus, our formulation leads to an algorithm that efficiently distributes computation across clients, as reducing their problem dimension allows them to make many local updates with respect to their global head.  
%     %% We call this procedure FedRep.

% \textbf{Formalizing the gain of cooperation.} Our sample complexity analysis allows us to formally quantify the gain that clients obtain by cooperating with each other. In particular, for linear neural networks, we show that to find an $\epsilon$ accurate model for a client, that client needs $\mathcal{O}(k^4(\log(n)+({d}/{n}))\log(1/\epsilon)$ samples if it participates in federated learning, while it would require $\mathcal{O}(d\log(1/\epsilon))$ samples to do this task locally without cooperating with other clients. Hence, it can be easily verified that in most realistic settings, where $k^4\ll n$ and $\log(n)\ll d $, there is a huge benefit in cooperation in terms of sample complexity. 



%     \textbf{Generalization to New Tasks.}

% \end{comment}

%First, it is strongly motivated by the success of representation learning in centralized settings, as well in similar multi-task learning settings \cite{raghu2019rapid}. Second 

% We show in Figure \ref{fig:} that FedRep attains higher accuracy than state-of-the-art methods on various partitions of the CIFAR-100 dataset. Our contributions are summarized as follows:


% The most fundamental approach to federated learning is to try to train a {\em single} model by distributing the model to a batch of selected clients and aggregating the results of the clients' local updates of the global model on each round of communication \cite{ li2018federated, karimireddy2020scaffold}. For example, the well-known FedAvg algorithm  \cite{mcmahan2017communication} averages the results of local SGD and is widely used in practice. FedAvg and similar methods are effective because they capture global information from all clients, but they often struggle as the clients' local data distributions become less similar because global information is less locally relevant in this case \cite{jiang2019improving}. Many alternative approaches have thus been developed to deal with this statistical heterogeneity in the local distributions \cite{kulkarni2020survey}.

% In this work, we propose a natural method to leverage both global information as well as the uniqueness of each clients' local data. Our framework 

% A fundamental approach to federated learning is constructing a {\em single} global model $w \in \mathbb{R}^D$ that aims to perform well on all devices \cite{mcmahan2017communication, li2018federated}. However, this approach 
% is often ineffective in {\em heterogenous} settings, with non-i.i.d. data across devices, because strong a model that performs
% \cite{jiang2019improving}. {\em Personalized federated learning} has thus emerged as an active research area wherein the goal is to balance global and local information to efficiently personalize the global model to each client's local data .

% Many real federated learning settings involve clients with heterogeneous data that nonetheless shares a common representation. For example, in autonomous driving, each car has its own unique local data which may appear varied across machines, but there typically exists a common representation of the data, e.g. one that segments roads and other cars \cite{oao}.

% To better account for the uniqueness of each client's data, 
% many recent works have proposed frameworks for {\em personalized} federated learning, in which the central authority may, for instance, facilitate the learning of unique local parameters by each client, in addition to learning a set of global parameters shared among all clients, or find a single model that is specifically designed to adapt quickly to new labels. 
% However, in these approaches the local parameters are still high-dimensional, or do not explicitly allow for parallelism

% In this work we propose a novel approach to personalized federated learning in which the central authority aims to learn a global low-dimensional {\em representation} of the data shared across all devices, or clients. On top of this representation each client learns a low-dimensional map from the representation space to the output space. The motivation for this framework is the observation that data of the same type often shares similar features while perhaps having different labels in different domains. For example, an image of a large, four-legged mammal may be labelled as a `horse' for one client and as a `zebra' for another. Learning a global low-dimensional representation critically leverages the commonality of features across clients to reduce the problem dimension for each client. We further detail our contributions as follows:
% To solve the representation learning problem, we present a novel federated learning algorithm that alternates between a stochastic gradient descent update to solve for the representation and a minimization update to solve for each client's local parameters. The minimization step is enabled by the fact that the computation is distributed across clients (each client needs to solve for only their own parameters) and that these parameters are low-dimensional by virtue of the low-dimensionality of the representation. We prove that this method achieves a linear convergence rate in a linear regression setting, and does so in a sample-efficient manner  Finally, we demonstrate empirically that it improves over state-of-the-art personalized federated learning methods on a variety of datasets.
% need to say that reducing the problem dimension enables learning with less data/per client
% However, in these approaches the local parameters learned by each client are still high-dimensional, and 
%The motivation is to utilize plentiful global data via the global parameters while customizing the model to unique local data via the local parameters.



% Ideally, personalized models 
% In this work we propose a novel method for personalized federated learning that 

% However, these existing methods for personalization . First, the local parameters for each client are often full-dimensional, raising computational concerns. Second, the global information learned often fails to capture a global representation...

% another motivation: performance in low-data, large client regimes (assuming we show sample complexity result)



% Our contributions are as follows:
%However, this representation learning strategy has yet to be applied to federated learning, where it naturally applies to realistic scenarios in which global information can aid I clients in solving their local problems.%, and non-asymptotic optimization results have yet to been shown for solving \eqref{obj}. 

